Planes in cubic fourfolds

We show that the maximal number of planes in a complex smooth cubic fourfold in ${\mathbb P}^5$ is $405$, realized by the Fermat cubic only; the maximal number of real planes in a real smooth cubic fourfold is $357$, realized by the so-called Clebsch--Segre cubic. Altogether, there are but three (up to projective equivalence) cubics with more than $350$ planes.

==> 3/3_12A2.tex <==
% -*- TeX -*-
% Niemeier lattice 12A2
% 29 classes
\newcs{max-12A2}{407}%
\newcs{count-12A2}{29}%
\newcs{counts-12A2}{\DO{1}{407}\DO{2}{315}\DO{3}{393}\DO{4}{379}\DO{5}{351}\DO{6}{345}\DO{7}{343}\DO{8}{339}\DO{9}{335}\DO{10}{327}\DO{11}{327}\DO{12}{321}\DO{13}{311}\DO{14}{308}\DO{15}{305}\DO{16}{301}\DO{17}{287}\DO{18}{287}\DO{19}{286}\DO{20}{285}\DO{21}{282}\DO{22}{273}\DO{23}{272}\DO{24}{265}\DO{25}{255}\DO{26}{250}\DO{27}{248}\DO{28}{235}\DO{29}{208}}%
\orbits
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 1
\orbit{12}{1}{407}
\h{1}&\rat(14/3){2}{\spec{1}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&&\cnt{803}&\bounds{407}{407}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{11}&\cnt{2}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{55}&\cnt{2}&\bounds{1}{1}{1}{true}&&\cr
\l{3}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{55}&\cnt{8}&\bounds{4}{4}{1}{true}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{55}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{5}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{11}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 2
\orbit{12}{2}{315}
\h{2}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1215}&\bounds{315}{405}{fail}{false}&&\cr
\l{1}&\int(2){2}{}&\int(2){2}{}&\int(0){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{15}&\cnt{81}&\bounds{21}{27}{3}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 3
\orbit{12}{3}{393}
\h{3}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&&\cnt{747}&\bounds{393}{393}{1}{false}&&\cr
\l{1}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{54}&\cnt{2}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{108}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{3}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\ln{36}&\cnt{2}&\bounds{1}{1}{1}{true}&&\cr
\l{4}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{36}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{5}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{12}&\cnt{8}&\bounds{4}{4}{1}{true}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 4
\orbit{12}{4}{379}
\h{4}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&&\cnt{743}&\bounds{379}{379}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{2}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\ln{30}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{3}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{10}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{16}&\bounds{8}{8}{1}{true}&&\cr
\l{5}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{30}&\cnt{8}&\bounds{4}{4}{1}{true}&&\cr
\l{6}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{60}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{7}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{8}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{2}&\bounds{1}{1}{1}{true}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\ln{5}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 5
\orbit{12}{5}{351}
\h{5}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&&\cnt{855}&\bounds{351}{351}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{9}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{2}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{9}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{3}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{36}&\cnt{12}&\bounds{4}{4}{1}{true}&&\cr
\l{4}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(-2/3){2}{}&\ln{9}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{5}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\rat(1/3){2}{}&\ln{36}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{6}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){2}{}&\int(0){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{6}&\cnt{9}&\bounds{3}{3}{1}{true}&&\cr
\l{7}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{9}&\cnt{16}&\bounds{8}{8}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 6
\orbit{12}{6}{345}
\h{6}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&&\cnt{743}&\bounds{345}{345}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{16}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{16}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{16}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(-1/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{16}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\ln{16}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{4}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{16}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{16}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(1){1}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{16}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){1}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 7
\orbit{12}{7}{343}
\h{7}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{991}&\bounds{343}{343}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{8}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{6}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{24}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{6}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 8
\orbit{12}{8}{339}
\h{8}&\rat(14/3){2}{\spec{1}}&\rat(14/3){2}{\spec{1}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{979}&\bounds{339}{339}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(5/3){2}{}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(5/3){2}{}&\rat(5/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{8}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(5/3){2}{}&\rat(5/3){2}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{6}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{24}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(5/3){2}{}&\rat(-1/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{6}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 9
\orbit{12}{9}{335}
\h{9}&\rat(14/3){2}{\spec{1}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&&\cnt{799}&\bounds{335}{335}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{16}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\ln{8}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{16}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{8}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{8}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{16}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{8}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(5/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{4}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(5/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{2}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{16}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\ln{4}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{8}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\ln{8}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(1/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{8}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 10
\orbit{12}{10}{327}
\h{10}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(2){\2}{}&\rat(2/3){2}{}&\int(2){\2}{}&\int(2){\2}{}&\rat(2/3){2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{743}&\bounds{327}{327}{1}{false}&&\cr
\l{1}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{24}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{24}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(1){2}{}&\rat(1/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{24}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{48}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){2}{}&\rat(1/3){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{24}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){2}{}&\rat(-2/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\rat(-1/3){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){2}{}&\int(0){2}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 11
\orbit{12}{11}{327}
\h{11}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{867}&\bounds{327}{327}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{15}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{90}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(1){2}{}&\int(1){1}{}&\int(1){2}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(-1){2}{}&\int(0){\0}{}&\ln{12}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\int(1){1}{}&\int(1){2}{}&\int(1){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{30}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 12
\orbit{12}{12}{321}
\h{12}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\rat(8/3){1}{\spec{1}}&&\cnt{867}&\bounds{321}{321}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(-2/3){2}{}&\ln{6}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{9}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{18}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{9}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{18}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\ln{9}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{9}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 13
\orbit{12}{13}{311}
\h{13}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(2){\2}{}&\rat(2/3){2}{}&\int(2){\2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{867}&\bounds{311}{311}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{4}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(-1){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{8}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{16}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\ln{4}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(4/3){1}{}&\rat(-2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{16}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){2}{}&\ln{8}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(1){1}{}&\rat(1/3){1}{}&\int(1){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 14
\orbit{12}{14}{308}
\h{14}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&&\cnt{739}&\bounds{308}{308}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(-2/3){2}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{2}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-2/3){1}{}&\rat(2/3){1}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{4}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{2}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{28}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{29}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{30}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{31}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{4}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{32}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(1/3){2}{}&\ln{4}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{33}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{34}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){2}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{35}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{36}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{37}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{38}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{39}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{40}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{41}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{42}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{43}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{44}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{45}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 15
\orbit{12}{15}{305}
\h{15}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(6){\6}{\spec{1}}&\rat(2/3){2}{}&\int(2){\2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{851}&\bounds{305}{305}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{6}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(2){2}{}&\rat(1/3){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(2){2}{}&\rat(-2/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(2/3){2}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(2){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{6}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(2/3){2}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(2){2}{}&\rat(1/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(-1/3){2}{}&\int(2){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){1}{}&\ln{12}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(2){2}{}&\rat(1/3){1}{}&\int(1){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 16
\orbit{12}{16}{301}
\h{16}&\rat(14/3){2}{\spec{1}}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&&\cnt{795}&\bounds{301}{301}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\ln{6}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{6}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){1}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(1/3){2}{}&\ln{3}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{2}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(5/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(5/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){1}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(5/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\rat(2/3){2}{}&\rat(1/3){2}{}&\ln{3}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(-2/3){2}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{6}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{3}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\rat(1/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\rat(1/3){1}{}&\rat(2/3){1}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 17
\orbit{12}{17}{287}
\h{17}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(2){\2}{}&\rat(2/3){2}{}&\int(2){\2}{}&\int(2){\2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{739}&\bounds{287}{287}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(-1/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\ln{3}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{3}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{6}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(4/3){1}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(4/3){1}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(4/3){1}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{6}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(4/3){1}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){2}{}&\int(0){\0}{}&\ln{6}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\rat(1/3){1}{}&\int(1){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\rat(-2/3){1}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{25}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(-1/3){2}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{6}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\rat(2/3){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{3}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(1){1}{}&\int(1){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{31}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){2}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{32}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{33}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{34}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{35}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 18
\orbit{12}{18}{287}
\h{18}&\rat(14/3){2}{\spec{1}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(2){\2}{}&\rat(2/3){2}{}&\int(2){\2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{795}&\bounds{287}{287}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{8}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(5/3){2}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{8}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(5/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(5/3){2}{}&\rat(-1/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(5/3){2}{}&\rat(-1/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(5/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(5/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{8}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(5/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(-1/3){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(5/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\ln{4}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(5/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){1}{}&\ln{4}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(4/3){1}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(4/3){1}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(4/3){1}{}&\rat(-2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){2}{}&\ln{4}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\rat(1/3){1}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{4}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(1){1}{}&\rat(1/3){1}{}&\int(1){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 19
\orbit{12}{19}{286}
\h{19}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(6){\6}{\spec{1}}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{847}&\bounds{286}{286}{1}{false}&&\cr
\l{1}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\rat(-1/3){2}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{10}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(-2/3){1}{}&\rat(2/3){2}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{5}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\ln{5}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{5}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(2){2}{}&\rat(1/3){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(2){2}{}&\rat(2/3){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{5}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 20
\orbit{12}{20}{285}
\h{20}&\int(6){\6}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{843}&\bounds{285}{285}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{24}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(1){1}{}&\int(1){2}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 21
\orbit{12}{21}{282}
\h{21}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&&\cnt{735}&\bounds{282}{282}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(-2/3){2}{}&\ln{3}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{6}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{3}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\rat(1/3){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{6}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){1}{}&\ln{6}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(-2/3){2}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\rat(1/3){2}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){2}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{6}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){2}{}&\rat(2/3){2}{}&\rat(2/3){1}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 22
\orbit{12}{22}{273}
\h{22}&\rat(14/3){2}{\spec{1}}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(2){\2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{791}&\bounds{273}{273}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(-2/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{4}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{4}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\rat(1/3){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(5/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{4}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(5/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(5/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(5/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{4}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{4}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\rat(1/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(1){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 23
\orbit{12}{23}{272}
\h{23}&\rat(14/3){2}{\spec{1}}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{787}&\bounds{272}{272}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(5/3){2}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{6}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(5/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{12}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{6}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){1}{}&\rat(2/3){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(1/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 24
\orbit{12}{24}{265}
\h{24}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(2){\2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(2){\2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{735}&\bounds{265}{265}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){2}{}&\ln{4}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\rat(2/3){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(1){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\rat(-1/3){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){2}{}&\int(0){\0}{}&\ln{4}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\rat(1/3){1}{}&\int(0){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(1){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){1}{}&\ln{4}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{28}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{29}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{30}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{31}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(2/3){2}{}&\int(0){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{32}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{33}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\rat(2/3){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{34}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 25
\orbit{12}{25}{255}
\h{25}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{735}&\bounds{255}{255}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{15}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{60}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{60}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 26
\orbit{12}{26}{250}
\h{26}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\int(2){\2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{731}&\bounds{250}{250}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{6}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(1){1}{}&\rat(-1/3){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){1}{}&\rat(2/3){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\ln{6}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(4/3){1}{}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){1}{}&\int(0){1}{}&\int(0){\0}{}&\ln{3}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(4/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{6}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(4/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(1){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 27
\orbit{12}{27}{248}
\h{27}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{707}&\bounds{248}{248}{1}{false}&&\cr
\l{1}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{9}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{24}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 28
\orbit{12}{28}{235}
\h{28}&\rat(26/3){2}{\spec{1}}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{639}&\bounds{235}{235}{1}{false}&&\cr
\l{1}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(7/3){1}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{30}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(7/3){1}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(5/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 12*A[2]
% Class 29
\orbit{12}{29}{208}
\h{29}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(8){\8}{\spec{1}}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{583}&\bounds{208}{208}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{20}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(2/3){2}{}&\rat(2/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(2){1}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{30}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_24A1.tex <==
% -*- TeX -*-
% Niemeier lattice 24A1
% 13 classes
\newcs{max-24A1}{759}%
\newcs{count-24A1}{13}%
\newcs{counts-24A1}{\DO{1}{759}\DO{2}{507}\DO{3}{507}\DO{4}{471}\DO{5}{451}\DO{6}{439}\DO{7}{407}\DO{8}{407}\DO{9}{393}\DO{10}{379}\DO{11}{375}\DO{12}{375}\DO{13}{311}}%
\orbits
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 1
\orbit{24}{1}{759}
\h{1}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&&\cnt{759}&\bounds{759}{759}{1}{false}&&\cr
\l{1}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{759}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 2
\orbit{24}{2}{507}
\h{2}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{999}&\bounds{507}{507}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{15}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\int(1){1}{}&\int(1){1}{}&\int(1){1}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(-1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{3}&\int(1){1}{}&\int(1){1}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{60}&\cnt{16}&\bounds{8}{8}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 3
\orbit{24}{3}{507}
\h{3}&\rat(9/2){1}{\spec{1}}&\rat(9/2){1}{\spec{1}}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{987}&\bounds{507}{507}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\rat(3/2){1}{}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{15}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{3}&\rat(3/2){1}{}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{60}&\cnt{16}&\bounds{8}{8}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 4
\orbit{24}{4}{471}
\h{4}&\rat(9/2){1}{\spec{1}}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{807}&\bounds{471}{471}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{15}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{105}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{3}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{168}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{4}&\int(0){\0}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{15}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 5
\orbit{24}{5}{451}
\h{5}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(2){\2}{}&\int(2){\2}{}&\rat(1/2){1}{}&\int(2){\2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{875}&\bounds{451}{451}{1}{false}&&\cr
\l{1}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{72}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{3}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{64}&\cnt{8}&\bounds{4}{4}{1}{true}&&\cr
\l{4}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(-1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{5}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\rat(-1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{16}&\bounds{8}{8}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 6
\orbit{24}{6}{439}
\h{6}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(2){\2}{}&\rat(1/2){1}{}&\int(2){\2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{751}&\bounds{439}{439}{1}{false}&&\cr
\l{1}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{30}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{192}&\cnt{2}&\bounds{1}{1}{1}{true}&&\cr
\l{3}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{96}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{4}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{60}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{5}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 7
\orbit{24}{7}{407}
\h{7}&\rat(9/2){1}{\spec{1}}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(2){\2}{}&\int(2){\2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{799}&\bounds{407}{407}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{7}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{7}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{3}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{56}&\cnt{8}&\bounds{4}{4}{1}{true}&&\cr
\l{4}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{21}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{5}&\rat(3/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{14}&\cnt{16}&\bounds{8}{8}{1}{true}&&\cr
\l{6}&\int(0){\0}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{7}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 8
\orbit{24}{8}{407}
\h{8}&\rat(9/2){1}{\spec{1}}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(2){\2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&&\cnt{803}&\bounds{407}{407}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{11}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{55}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{3}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{55}&\cnt{8}&\bounds{4}{4}{1}{true}&&\cr
\l{4}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{55}&\cnt{2}&\bounds{1}{1}{1}{true}&&\cr
\l{5}&\int(0){\0}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{11}&\cnt{2}&\bounds{1}{1}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 9
\orbit{24}{9}{393}
\h{9}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(2){\2}{}&\rat(1/2){1}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&&\cnt{747}&\bounds{393}{393}{1}{false}&&\cr
\l{1}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{54}&\cnt{2}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){1}{}&\int(0){\0}{}&\ln{108}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{3}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\ln{36}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{4}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\rat(-1/2){1}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{36}&\cnt{2}&\bounds{1}{1}{1}{true}&&\cr
\l{5}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{12}&\cnt{8}&\bounds{4}{4}{1}{true}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 10
\orbit{24}{10}{379}
\h{10}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{715}&\bounds{379}{379}{1}{false}&&\cr
\l{1}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{21}&\cnt{2}&\bounds{2}{2}{1}{true}&&\cr
\l{2}&\int(2){1}{}&\int(1){1}{}&\int(1){1}{}&\int(0){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{21}&\cnt{32}&\bounds{16}{16}{1}{true}&&\cr
\l{3}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 11
\orbit{24}{11}{375}
\h{11}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{735}&\bounds{375}{375}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{15}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\int(1){1}{}&\int(1){1}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{45}&\cnt{16}&\bounds{8}{8}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 12
\orbit{24}{12}{375}
\h{12}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(2){\2}{}&\int(2){\2}{}&\rat(1/2){1}{}&\int(2){\2}{}&\int(2){\2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{743}&\bounds{375}{375}{1}{false}&&\cr
\l{1}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{48}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{3}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{4}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{32}&\cnt{2}&\bounds{1}{1}{1}{true}&&\cr
\l{5}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{48}&\cnt{8}&\bounds{4}{4}{1}{true}&&\cr
\l{6}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{8}&\cnt{4}&\bounds{2}{2}{1}{true}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){1}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 24*A[1]
% Class 13
\orbit{24}{13}{311}
\h{13}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(8){\8}{\spec{1}}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{591}&\bounds{311}{311}{1}{false}&&\cr
\l{1}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{70}&\cnt{8}&\bounds{4}{4}{1}{true}&&\cr
\l{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{15}&\cnt{2}&\bounds{2}{2}{1}{true}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_2A12.tex <==
% -*- TeX -*-
% Niemeier lattice 2A12
% 98 classes
\newcs{max-2A12}{167}%
\newcs{count-2A12}{98}%
\newcs{counts-2A12}{\DO{1}{167}\DO{2}{139}\DO{3}{139}\DO{4}{138}\DO{5}{138}\DO{6}{137}\DO{7}{130}\DO{8}{129}\DO{9}{129}\DO{10}{127}\DO{11}{127}\DO{12}{127}\DO{13}{125}\DO{14}{125}\DO{15}{124}\DO{16}{122}\DO{17}{121}\DO{18}{121}\DO{19}{121}\DO{20}{119}\DO{21}{118}\DO{22}{117}\DO{23}{116}\DO{24}{116}\DO{25}{116}\DO{26}{115}\DO{27}{115}\DO{28}{115}\DO{29}{115}\DO{30}{114}\DO{31}{114}\DO{32}{114}\DO{33}{113}\DO{34}{113}\DO{35}{112}\DO{36}{111}\DO{37}{111}\DO{38}{110}\DO{39}{110}\DO{40}{110}\DO{41}{109}\DO{42}{109}\DO{43}{109}\DO{44}{108}\DO{45}{106}\DO{46}{106}\DO{47}{106}\DO{48}{105}\DO{49}{105}\DO{50}{105}\DO{51}{105}\DO{52}{105}\DO{53}{105}\DO{54}{105}\DO{55}{104}\DO{56}{104}\DO{57}{104}\DO{58}{103}\DO{59}{101}\DO{60}{101}\DO{61}{100}\DO{62}{100}\DO{63}{100}\DO{64}{100}\DO{65}{99}\DO{66}{99}\DO{67}{98}\DO{68}{98}\DO{69}{97}\DO{70}{97}\DO{71}{95}\DO{72}{95}\DO{73}{95}\DO{74}{95}\DO{75}{93}\DO{76}{92}\DO{77}{89}\DO{78}{89}\DO{79}{88}\DO{80}{87}\DO{81}{87}\DO{82}{87}\DO{83}{85}\DO{84}{84}\DO{85}{84}\DO{86}{84}\DO{87}{81}\DO{88}{79}\DO{89}{76}\DO{90}{75}\DO{91}{74}\DO{92}{73}\DO{93}{72}\DO{94}{71}\DO{95}{70}\DO{96}{70}\DO{97}{69}\DO{98}{66}}%
\orbits
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 1
\orbit{2}{1}{167}
\h{1}&\rat(114/13){9}{\spec{1}}&\rat(42/13){6}{}&&\cnt{1023}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\rat(46/13){5}{}&\rat(6/13){12}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(45/13){8}{}&\rat(7/13){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(38/13){3}{}&\rat(14/13){2}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{6}&\rat(34/13){2}{}&\rat(18/13){10}{}&\ln{1}&\cnt{210}&\bounds{35}{35}{1}{false}&&\cr
\l{7}&\rat(30/13){1}{}&\rat(22/13){5}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 2
\orbit{2}{2}{139}
\h{2}&\rat(38/13){12}{\spec{2}}&\rat(118/13){8}{\spec{4}}&&\cnt{1223}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\rat(18/13){5}{}&\rat(34/13){12}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\rat(23/13){10}{}&\rat(29/13){11}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(10/13){10}{\spec{1}}&\rat(42/13){11}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(10/13){10}{\spec{2}}&\rat(42/13){11}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(15/13){2}{}&\rat(37/13){10}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(2/13){2}{\spec{1}}&\rat(50/13){10}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(2/13){2}{\spec{2}}&\rat(50/13){10}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(12/13){12}{}&\rat(40/13){8}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 3
\orbit{2}{3}{139}
\h{3}&\rat(36/13){9}{}&\rat(120/13){6}{\spec{1}}&&\cnt{1179}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\rat(19/13){8}{}&\rat(33/13){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\rat(12/13){3}{}&\rat(40/13){2}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\l{4}&\rat(18/13){11}{}&\rat(34/13){3}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(5/13){11}{}&\rat(47/13){3}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(4/13){1}{}&\rat(48/13){5}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 4
\orbit{2}{4}{138}
\h{4}&\rat(114/13){9}{\spec{4}}&\rat(42/13){6}{}&&\cnt{1283}&\bounds{138}{138}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(40/13){10}{}&\rat(12/13){11}{}&\ln{1}&\cnt{231}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{462}&\bounds{42}{42}{1}{false}&&\cr
\l{4}&\rat(44/13){11}{}&\rat(8/13){3}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(31/13){11}{}&\rat(21/13){3}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(35/13){12}{}&\rat(17/13){8}{}&\ln{1}&\cnt{210}&\bounds{35}{35}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 5
\orbit{2}{5}{138}
\h{5}&\rat(36/13){9}{}&\rat(120/13){6}{\spec{5}}&&\cnt{1127}&\bounds{138}{138}{1}{false}&&\cr
\l{1}&\rat(20/13){5}{}&\rat(32/13){12}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(27/13){10}{}&\rat(25/13){11}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(14/13){10}{}&\rat(38/13){11}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{288}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\rat(8/13){2}{}&\rat(44/13){10}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(9/13){12}{}&\rat(43/13){8}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(-4/13){12}{}&\rat(56/13){8}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 6
\orbit{2}{6}{137}
\h{6}&\rat(116/13){12}{\spec{1}}&\rat(40/13){8}{}&&\cnt{907}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(47/13){8}{}&\rat(5/13){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(44/13){5}{}&\rat(8/13){12}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{5}&\rat(42/13){3}{}&\rat(10/13){2}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{6}&\rat(36/13){10}{}&\rat(16/13){11}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(41/13){2}{}&\rat(11/13){10}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(28/13){2}{}&\rat(24/13){10}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(27/13){1}{}&\rat(25/13){5}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(12/13){12}{}&\rat(40/13){8}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 7
\orbit{2}{7}{130}
\h{7}&\rat(48/13){11}{\spec{2}}&\rat(108/13){3}{\spec{4}}&&\cnt{959}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\rat(23/13){5}{}&\rat(29/13){12}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(33/13){10}{}&\rat(19/13){11}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(17/13){2}{}&\rat(35/13){10}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(15/13){1}{}&\rat(37/13){5}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(11/13){12}{}&\rat(41/13){8}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{11}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 8
\orbit{2}{8}{129}
\h{8}&\rat(114/13){9}{\spec{2}}&\rat(42/13){6}{}&&\cnt{799}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(58/13){8}{}&\rat(-6/13){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(46/13){5}{\spec{3}}&\rat(6/13){12}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(45/13){8}{\spec{2}}&\rat(7/13){1}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\rat(40/13){10}{}&\rat(12/13){11}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(38/13){3}{\spec{2}}&\rat(14/13){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(34/13){2}{\spec{2}}&\rat(18/13){10}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\rat(31/13){11}{}&\rat(21/13){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(22/13){12}{}&\rat(30/13){8}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(17/13){1}{\spec{2}}&\rat(35/13){5}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 9
\orbit{2}{9}{129}
\h{9}&\rat(90/13){12}{\spec{2}}&\rat(66/13){8}{\spec{2}}&&\cnt{687}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(47/13){8}{}&\rat(5/13){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(44/13){5}{}&\rat(8/13){12}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(34/13){8}{\spec{1}}&\rat(18/13){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(34/13){8}{\spec{2}}&\rat(18/13){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(42/13){3}{}&\rat(10/13){2}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(42/13){3}{}&\rat(10/13){2}{\spec{2}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(36/13){10}{}&\rat(16/13){11}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(29/13){3}{}&\rat(23/13){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(28/13){2}{}&\rat(24/13){10}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(24/13){11}{}&\rat(28/13){3}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(14/13){1}{}&\rat(38/13){5}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(12/13){12}{}&\rat(40/13){8}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 10
\orbit{2}{10}{127}
\h{10}&\rat(48/13){11}{\spec{2}}&\rat(108/13){3}{\spec{2}}&&\cnt{1323}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\rat(16/13){8}{\spec{1}}&\rat(36/13){1}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\rat(16/13){8}{\spec{2}}&\rat(36/13){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(19/13){3}{}&\rat(33/13){2}{\spec{1}}&\ln{1}&\cnt{432}&\bounds{36}{36}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(3){\2}{\spec{1}}&\ln{1}&\cnt{108}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{2}}&\int(3){\2}{\spec{1}}&\ln{1}&\cnt{324}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{1}}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 11
\orbit{2}{11}{127}
\h{11}&\rat(126/13){11}{\spec{5}}&\rat(30/13){3}{}&&\cnt{1119}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{110}&\bounds{11}{11}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{330}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\rat(35/13){11}{}&\rat(17/13){3}{}&\ln{1}&\cnt{330}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(37/13){12}{}&\rat(15/13){8}{}&\ln{1}&\cnt{252}&\bounds{42}{42}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 12
\orbit{2}{12}{127}
\h{12}&\rat(100/13){11}{\spec{1}}&\rat(56/13){3}{\spec{1}}&&\cnt{903}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(42/13){8}{\spec{1}}&\rat(10/13){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(36/13){5}{\spec{1}}&\rat(16/13){12}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(33/13){10}{\spec{1}}&\rat(19/13){11}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(32/13){3}{\spec{1}}&\rat(20/13){2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(30/13){2}{\spec{1}}&\rat(22/13){10}{}&\ln{1}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{10}&\rat(22/13){11}{\spec{1}}&\rat(30/13){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(28/13){1}{}&\rat(24/13){5}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(28/13){1}{}&\rat(24/13){5}{\spec{2}}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 13
\orbit{2}{13}{125}
\h{13}&\int(12){\12}{\spec{4}}&\int(0){\0}{}&&\cnt{1483}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){1}{}&\ln{1}&\cnt{455}&\bounds{35}{35}{1}{false}&&\cr
\l{4}&\int(4){5}{}&\int(0){12}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(4){10}{}&\int(0){11}{}&\ln{1}&\cnt{546}&\bounds{42}{42}{1}{false}&&\cr
\l{6}&\int(4){11}{}&\int(0){3}{}&\ln{1}&\cnt{286}&\bounds{26}{26}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 14
\orbit{2}{14}{125}
\h{14}&\rat(62/13){9}{\spec{2}}&\rat(94/13){6}{\spec{1}}&&\cnt{743}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\rat(45/13){8}{}&\rat(7/13){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(33/13){5}{}&\rat(19/13){12}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(32/13){8}{}&\rat(20/13){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(27/13){10}{}&\rat(25/13){11}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(25/13){3}{}&\rat(27/13){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(21/13){2}{}&\rat(31/13){10}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(18/13){11}{}&\rat(34/13){3}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(17/13){1}{}&\rat(35/13){5}{\spec{1}}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(17/13){1}{}&\rat(35/13){5}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(9/13){12}{}&\rat(43/13){8}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\rat(4/13){1}{}&\rat(48/13){5}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 15
\orbit{2}{15}{124}
\h{15}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&&\cnt{1135}&\bounds{124}{124}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(2){12}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{3}&\int(2){10}{}&\int(2){11}{}&\ln{1}&\cnt{450}&\bounds{45}{45}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(2){2}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){11}{}&\int(2){3}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(2){10}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\int(2){12}{}&\int(2){8}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 16
\orbit{2}{16}{122}
\h{16}&\rat(38/13){12}{\spec{2}}&\rat(118/13){8}{\spec{1}}&&\cnt{1067}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\rat(21/13){8}{}&\rat(31/13){1}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{2}&\rat(16/13){3}{}&\rat(36/13){2}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{70}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{140}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\rat(24/13){11}{}&\rat(28/13){3}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(11/13){11}{}&\rat(41/13){3}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(14/13){1}{}&\rat(38/13){5}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(12/13){12}{}&\rat(40/13){8}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(1/13){1}{}&\rat(51/13){5}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 17
\orbit{2}{17}{121}
\h{17}&\rat(36/13){9}{}&\rat(120/13){6}{\spec{2}}&&\cnt{1035}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\rat(32/13){8}{}&\rat(20/13){1}{\spec{1}}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(12/13){3}{}&\rat(40/13){2}{\spec{1}}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\rat(18/13){11}{}&\rat(34/13){3}{\spec{1}}&\ln{1}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\rat(-8/13){11}{}&\rat(60/13){3}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(4/13){1}{}&\rat(48/13){5}{\spec{1}}&\ln{1}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 18
\orbit{2}{18}{121}
\h{18}&\rat(48/13){11}{\spec{1}}&\rat(108/13){3}{\spec{2}}&&\cnt{1287}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\rat(16/13){8}{}&\rat(36/13){1}{}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\l{2}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{1}}&\ln{1}&\cnt{792}&\bounds{66}{66}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 19
\orbit{2}{19}{121}
\h{19}&\rat(74/13){11}{\spec{2}}&\rat(82/13){3}{\spec{2}}&&\cnt{687}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(42/13){8}{}&\rat(10/13){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(36/13){5}{}&\rat(16/13){12}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(33/13){10}{}&\rat(19/13){11}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(32/13){3}{}&\rat(20/13){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(30/13){2}{}&\rat(22/13){10}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(30/13){2}{}&\rat(22/13){10}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(17/13){2}{}&\rat(35/13){10}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(15/13){1}{}&\rat(37/13){5}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(11/13){12}{}&\rat(41/13){8}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 20
\orbit{2}{20}{119}
\h{20}&\rat(126/13){11}{\spec{4}}&\rat(30/13){3}{}&&\cnt{1011}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(42/13){8}{}&\rat(10/13){1}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{4}&\rat(46/13){10}{}&\rat(6/13){11}{}&\ln{1}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\l{5}&\rat(32/13){3}{}&\rat(20/13){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(48/13){11}{}&\rat(4/13){3}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 21
\orbit{2}{21}{118}
\h{21}&\rat(116/13){12}{\spec{3}}&\rat(40/13){8}{}&&\cnt{851}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(47/13){8}{}&\rat(5/13){1}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\rat(44/13){5}{}&\rat(8/13){12}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(49/13){10}{}&\rat(3/13){11}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(42/13){3}{}&\rat(10/13){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(36/13){10}{}&\rat(16/13){11}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(37/13){11}{}&\rat(15/13){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(28/13){2}{}&\rat(24/13){10}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(25/13){12}{}&\rat(27/13){8}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(12/13){12}{}&\rat(40/13){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 22
\orbit{2}{22}{117}
\h{22}&\int(6){\6}{}&\int(6){\6}{}&&\cnt{687}&\bounds{117}{117}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){8}{}&\int(1){1}{}&\ln{4}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(3){10}{}&\int(1){11}{}&\ln{4}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){10}{}&\int(2){11}{}&\ln{4}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{81}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 23
\orbit{2}{23}{116}
\h{23}&\rat(126/13){11}{\spec{1}}&\rat(30/13){3}{}&&\cnt{955}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(55/13){8}{}&\rat(-3/13){1}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(49/13){5}{}&\rat(3/13){12}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(42/13){8}{}&\rat(10/13){1}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(45/13){3}{}&\rat(7/13){2}{}&\ln{1}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(32/13){3}{\spec{1}}&\rat(20/13){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(32/13){3}{\spec{2}}&\rat(20/13){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{150}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(43/13){2}{}&\rat(9/13){10}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{11}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(28/13){1}{}&\rat(24/13){5}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 24
\orbit{2}{24}{116}
\h{24}&\rat(36/13){9}{}&\rat(120/13){6}{\spec{2}}&&\cnt{787}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\rat(32/13){8}{}&\rat(20/13){1}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(27/13){10}{}&\rat(25/13){11}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(12/13){3}{}&\rat(40/13){2}{\spec{2}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(18/13){11}{}&\rat(34/13){3}{\spec{2}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(18/13){11}{}&\rat(34/13){3}{\spec{3}}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(5/13){11}{}&\rat(47/13){3}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(9/13){12}{}&\rat(43/13){8}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{9}&\rat(4/13){1}{}&\rat(48/13){5}{\spec{2}}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{10}&\rat(-9/13){1}{}&\rat(61/13){5}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 25
\orbit{2}{25}{116}
\h{25}&\rat(88/13){9}{\spec{2}}&\rat(68/13){6}{\spec{1}}&&\cnt{683}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(46/13){5}{}&\rat(6/13){12}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(45/13){8}{}&\rat(7/13){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(33/13){5}{\spec{1}}&\rat(19/13){12}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(33/13){5}{\spec{2}}&\rat(19/13){12}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(38/13){3}{}&\rat(14/13){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(27/13){10}{}&\rat(25/13){11}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(34/13){2}{}&\rat(18/13){10}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(34/13){2}{}&\rat(18/13){10}{\spec{2}}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(21/13){2}{}&\rat(31/13){10}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(17/13){1}{}&\rat(35/13){5}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(9/13){12}{}&\rat(43/13){8}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 26
\orbit{2}{26}{115}
\h{26}&\rat(100/13){11}{\spec{2}}&\rat(56/13){3}{\spec{1}}&&\cnt{683}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(55/13){8}{}&\rat(-3/13){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(49/13){5}{}&\rat(3/13){12}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(42/13){8}{}&\rat(10/13){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(36/13){5}{\spec{1}}&\rat(16/13){12}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(36/13){5}{\spec{2}}&\rat(16/13){12}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(45/13){3}{}&\rat(7/13){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(33/13){10}{}&\rat(19/13){11}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(32/13){3}{}&\rat(20/13){2}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(30/13){2}{}&\rat(22/13){10}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(15/13){1}{}&\rat(37/13){5}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 27
\orbit{2}{27}{115}
\h{27}&\rat(12/13){12}{}&\rat(144/13){8}{\spec{7}}&&\cnt{1243}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\rat(-3/13){10}{}&\rat(55/13){11}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{132}&\bounds{11}{11}{1}{false}&&\cr
\l{3}&\rat(2/13){2}{}&\rat(50/13){10}{}&\ln{1}&\cnt{726}&\bounds{66}{66}{1}{false}&&\cr
\l{4}&\rat(12/13){12}{}&\rat(40/13){8}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 28
\orbit{2}{28}{115}
\h{28}&\int(8){\8}{}&\int(4){\4}{}&&\cnt{679}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){8}{}&\int(0){1}{}&\ln{2}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(3){8}{\spec{1}}&\int(1){1}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){8}{\spec{2}}&\int(1){1}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){10}{}&\int(1){11}{}&\ln{2}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){10}{}&\int(2){11}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){11}{}&\int(2){3}{}&\ln{2}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 29
\orbit{2}{29}{115}
\h{29}&\rat(116/13){12}{\spec{2}}&\rat(40/13){8}{}&&\cnt{679}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(60/13){8}{}&\rat(-8/13){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(57/13){5}{}&\rat(-5/13){12}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(47/13){8}{}&\rat(5/13){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(44/13){5}{\spec{1}}&\rat(8/13){12}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(44/13){5}{\spec{2}}&\rat(8/13){12}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\rat(42/13){3}{}&\rat(10/13){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(36/13){10}{\spec{1}}&\rat(16/13){11}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(28/13){2}{\spec{1}}&\rat(24/13){10}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(12/13){12}{\spec{1}}&\rat(40/13){8}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 30
\orbit{2}{30}{114}
\h{30}&\rat(22/13){11}{}&\rat(134/13){3}{\spec{6}}&&\cnt{1003}&\bounds{114}{114}{1}{false}&&\cr
\l{1}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(7/13){10}{}&\rat(45/13){11}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(4/13){2}{}&\rat(48/13){10}{}&\ln{1}&\cnt{275}&\bounds{25}{25}{1}{false}&&\cr
\l{6}&\rat(11/13){12}{}&\rat(41/13){8}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(11/13){12}{}&\rat(41/13){8}{\spec{2}}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(-2/13){12}{}&\rat(54/13){8}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 31
\orbit{2}{31}{114}
\h{31}&\rat(36/13){9}{}&\rat(120/13){6}{\spec{3}}&&\cnt{791}&\bounds{114}{114}{1}{false}&&\cr
\l{1}&\rat(32/13){8}{}&\rat(20/13){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(27/13){10}{}&\rat(25/13){11}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(14/13){10}{}&\rat(38/13){11}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(18/13){11}{}&\rat(34/13){3}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(8/13){2}{}&\rat(44/13){10}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(9/13){12}{}&\rat(43/13){8}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(9/13){12}{}&\rat(43/13){8}{\spec{2}}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\rat(4/13){1}{}&\rat(48/13){5}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(-4/13){12}{}&\rat(56/13){8}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 32
\orbit{2}{32}{114}
\h{32}&\rat(90/13){12}{\spec{1}}&\rat(66/13){8}{\spec{2}}&&\cnt{843}&\bounds{114}{114}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(34/13){8}{\spec{1}}&\rat(18/13){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(36/13){10}{\spec{1}}&\rat(16/13){11}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(29/13){3}{\spec{1}}&\rat(23/13){2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(28/13){2}{\spec{1}}&\rat(24/13){10}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(24/13){11}{\spec{1}}&\rat(28/13){3}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(27/13){1}{}&\rat(25/13){5}{\spec{1}}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(27/13){1}{}&\rat(25/13){5}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(12/13){12}{\spec{1}}&\rat(40/13){8}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 33
\orbit{2}{33}{113}
\h{33}&\rat(126/13){11}{\spec{3}}&\rat(30/13){3}{}&&\cnt{843}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(55/13){8}{}&\rat(-3/13){1}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(49/13){5}{}&\rat(3/13){12}{}&\ln{1}&\cnt{150}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(42/13){8}{\spec{1}}&\rat(10/13){1}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\rat(42/13){8}{\spec{2}}&\rat(10/13){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(46/13){10}{}&\rat(6/13){11}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(45/13){3}{}&\rat(7/13){2}{}&\ln{1}&\cnt{30}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(32/13){3}{}&\rat(20/13){2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{90}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(35/13){11}{}&\rat(17/13){3}{}&\ln{1}&\cnt{90}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(22/13){11}{\spec{1}}&\rat(30/13){3}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(22/13){11}{\spec{2}}&\rat(30/13){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 34
\orbit{2}{34}{113}
\h{34}&\rat(88/13){9}{\spec{1}}&\rat(68/13){6}{\spec{1}}&&\cnt{735}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(45/13){8}{}&\rat(7/13){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(33/13){5}{}&\rat(19/13){12}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(40/13){10}{}&\rat(12/13){11}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(40/13){10}{}&\rat(12/13){11}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(27/13){10}{\spec{1}}&\rat(25/13){11}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(27/13){10}{\spec{2}}&\rat(25/13){11}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\rat(31/13){11}{}&\rat(21/13){3}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{13}&\rat(21/13){2}{}&\rat(31/13){10}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(22/13){12}{}&\rat(30/13){8}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(22/13){12}{}&\rat(30/13){8}{\spec{2}}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(17/13){1}{}&\rat(35/13){5}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(9/13){12}{}&\rat(43/13){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 35
\orbit{2}{35}{112}
\h{35}&\rat(100/13){11}{\spec{1}}&\rat(56/13){3}{\spec{1}}&&\cnt{791}&\bounds{112}{112}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(42/13){8}{\spec{2}}&\rat(10/13){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(36/13){5}{\spec{2}}&\rat(16/13){12}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(46/13){10}{}&\rat(6/13){11}{\spec{1}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(46/13){10}{}&\rat(6/13){11}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(33/13){10}{\spec{2}}&\rat(19/13){11}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(32/13){3}{\spec{2}}&\rat(20/13){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(35/13){11}{}&\rat(17/13){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(30/13){2}{\spec{2}}&\rat(22/13){10}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(22/13){11}{\spec{2}}&\rat(30/13){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(22/13){11}{\spec{3}}&\rat(30/13){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(24/13){12}{}&\rat(28/13){8}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{19}&\rat(15/13){1}{}&\rat(37/13){5}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 36
\orbit{2}{36}{111}
\h{36}&\rat(90/13){12}{\spec{1}}&\rat(66/13){8}{\spec{1}}&&\cnt{831}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(31/13){5}{\spec{1}}&\rat(21/13){12}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\rat(36/13){10}{\spec{1}}&\rat(16/13){11}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(36/13){10}{\spec{1}}&\rat(16/13){11}{\spec{2}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(23/13){10}{\spec{1}}&\rat(29/13){11}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(28/13){2}{\spec{1}}&\rat(24/13){10}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(28/13){2}{\spec{1}}&\rat(24/13){10}{\spec{2}}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{11}&\rat(15/13){2}{\spec{1}}&\rat(37/13){10}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(27/13){1}{}&\rat(25/13){5}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{13}&\rat(12/13){12}{\spec{1}}&\rat(40/13){8}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 37
\orbit{2}{37}{111}
\h{37}&\rat(114/13){9}{\spec{2}}&\rat(42/13){6}{}&&\cnt{675}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(59/13){5}{}&\rat(-7/13){12}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(46/13){5}{\spec{1}}&\rat(6/13){12}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\rat(46/13){5}{\spec{2}}&\rat(6/13){12}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(45/13){8}{\spec{1}}&\rat(7/13){1}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(51/13){3}{}&\rat(1/13){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(38/13){3}{\spec{1}}&\rat(14/13){2}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{8}&\rat(34/13){2}{\spec{1}}&\rat(18/13){10}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(17/13){1}{\spec{1}}&\rat(35/13){5}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 38
\orbit{2}{38}{110}
\h{38}&\rat(48/13){11}{\spec{2}}&\rat(108/13){3}{\spec{2}}&&\cnt{791}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\rat(29/13){8}{}&\rat(23/13){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(33/13){10}{}&\rat(19/13){11}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(19/13){3}{}&\rat(33/13){2}{\spec{2}}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{\spec{2}}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{2}}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{3}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(17/13){2}{}&\rat(35/13){10}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\rat(9/13){11}{}&\rat(43/13){3}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(15/13){1}{}&\rat(37/13){5}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(15/13){1}{}&\rat(37/13){5}{\spec{2}}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(11/13){12}{}&\rat(41/13){8}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{16}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 39
\orbit{2}{39}{110}
\h{39}&\rat(88/13){9}{\spec{2}}&\rat(68/13){6}{\spec{2}}&&\cnt{679}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(46/13){5}{}&\rat(6/13){12}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(45/13){8}{}&\rat(7/13){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(32/13){8}{\spec{1}}&\rat(20/13){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(38/13){3}{}&\rat(14/13){2}{\spec{1}}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(38/13){3}{}&\rat(14/13){2}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(25/13){3}{\spec{1}}&\rat(27/13){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(25/13){3}{\spec{2}}&\rat(27/13){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(34/13){2}{}&\rat(18/13){10}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(18/13){11}{\spec{1}}&\rat(34/13){3}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{12}&\rat(17/13){1}{}&\rat(35/13){5}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(4/13){1}{\spec{1}}&\rat(48/13){5}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 40
\orbit{2}{40}{110}
\h{40}&\rat(22/13){11}{}&\rat(134/13){3}{\spec{1}}&&\cnt{1063}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\rat(16/13){8}{}&\rat(36/13){1}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\rat(6/13){3}{}&\rat(46/13){2}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{110}&\bounds{11}{11}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(9/13){11}{}&\rat(43/13){3}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 41
\orbit{2}{41}{109}
\h{41}&\int(8){\8}{\spec{2}}&\int(4){\4}{}&&\cnt{843}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){8}{\spec{3}}&\int(1){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){5}{\spec{3}}&\int(1){12}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(3){10}{\spec{2}}&\int(1){11}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(3){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){10}{\spec{2}}&\int(2){11}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){10}{\spec{3}}&\int(2){11}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){3}{\spec{3}}&\int(2){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(3){11}{}&\int(1){3}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(3){11}{}&\int(1){3}{\spec{2}}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(2){11}{\spec{2}}&\int(2){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\int(2){2}{\spec{2}}&\int(2){10}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\int(2){12}{}&\int(2){8}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 42
\orbit{2}{42}{109}
\h{42}&\rat(64/13){12}{\spec{2}}&\rat(92/13){8}{\spec{1}}&&\cnt{739}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(34/13){8}{}&\rat(18/13){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(31/13){5}{}&\rat(21/13){12}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(36/13){10}{}&\rat(16/13){11}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(36/13){10}{}&\rat(16/13){11}{\spec{2}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(29/13){3}{}&\rat(23/13){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\rat(23/13){10}{}&\rat(29/13){11}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(28/13){2}{}&\rat(24/13){10}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(28/13){2}{}&\rat(24/13){10}{\spec{2}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(24/13){11}{}&\rat(28/13){3}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(15/13){2}{}&\rat(37/13){10}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(14/13){1}{}&\rat(38/13){5}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{17}&\rat(12/13){12}{}&\rat(40/13){8}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(-1/13){12}{}&\rat(53/13){8}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 43
\orbit{2}{43}{109}
\h{43}&\rat(90/13){12}{\spec{1}}&\rat(66/13){8}{\spec{2}}&&\cnt{787}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(34/13){8}{\spec{2}}&\rat(18/13){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(36/13){10}{\spec{2}}&\rat(16/13){11}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(29/13){3}{\spec{2}}&\rat(23/13){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(37/13){11}{}&\rat(15/13){3}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(37/13){11}{}&\rat(15/13){3}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(28/13){2}{\spec{2}}&\rat(24/13){10}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(24/13){11}{\spec{2}}&\rat(28/13){3}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{14}&\rat(25/13){12}{}&\rat(27/13){8}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\rat(14/13){1}{}&\rat(38/13){5}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(12/13){12}{\spec{2}}&\rat(40/13){8}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 44
\orbit{2}{44}{108}
\h{44}&\rat(38/13){12}{\spec{2}}&\rat(118/13){8}{\spec{2}}&&\cnt{787}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\rat(23/13){10}{}&\rat(29/13){11}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(16/13){3}{}&\rat(36/13){2}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{3}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(24/13){11}{}&\rat(28/13){3}{\spec{3}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(24/13){11}{}&\rat(28/13){3}{\spec{4}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(15/13){2}{}&\rat(37/13){10}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(11/13){11}{}&\rat(41/13){3}{\spec{2}}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(14/13){1}{}&\rat(38/13){5}{\spec{3}}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(14/13){1}{}&\rat(38/13){5}{\spec{4}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{3}}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\rat(1/13){1}{}&\rat(51/13){5}{\spec{2}}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(-1/13){12}{}&\rat(53/13){8}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 45
\orbit{2}{45}{106}
\h{45}&\rat(74/13){11}{\spec{1}}&\rat(82/13){3}{\spec{1}}&&\cnt{899}&\bounds{106}{106}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(29/13){8}{}&\rat(23/13){1}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{3}&\rat(33/13){10}{}&\rat(19/13){11}{}&\ln{1}&\cnt{90}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(19/13){3}{}&\rat(33/13){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{3}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{90}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(1){\2}{\spec{3}}&\int(3){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(35/13){11}{}&\rat(17/13){3}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(35/13){11}{}&\rat(17/13){3}{\spec{2}}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(35/13){11}{}&\rat(17/13){3}{\spec{3}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\l{19}&\rat(9/13){11}{\spec{1}}&\rat(43/13){3}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(9/13){11}{\spec{2}}&\rat(43/13){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(24/13){12}{}&\rat(28/13){8}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{22}&\rat(15/13){1}{}&\rat(37/13){5}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 46
\orbit{2}{46}{106}
\h{46}&\rat(88/13){9}{\spec{2}}&\rat(68/13){6}{\spec{2}}&&\cnt{1035}&\bounds{106}{106}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(32/13){8}{\spec{2}}&\rat(20/13){1}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\rat(40/13){10}{}&\rat(12/13){11}{}&\ln{1}&\cnt{308}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{176}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(44/13){11}{}&\rat(8/13){3}{\spec{1}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(44/13){11}{}&\rat(8/13){3}{\spec{2}}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(18/13){11}{\spec{2}}&\rat(34/13){3}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(22/13){12}{}&\rat(30/13){8}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(4/13){1}{\spec{2}}&\rat(48/13){5}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 47
\orbit{2}{47}{106}
\h{47}&\rat(22/13){11}{}&\rat(134/13){3}{\spec{2}}&&\cnt{1011}&\bounds{106}{106}{1}{false}&&\cr
\l{1}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(6/13){3}{}&\rat(46/13){2}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(9/13){11}{}&\rat(43/13){3}{}&\ln{1}&\cnt{176}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(-4/13){11}{}&\rat(56/13){3}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(11/13){12}{}&\rat(41/13){8}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{308}&\bounds{28}{28}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 48
\orbit{2}{48}{105}
\h{48}&\rat(64/13){12}{\spec{2}}&\rat(92/13){8}{\spec{2}}&&\cnt{679}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(34/13){8}{}&\rat(18/13){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(36/13){10}{}&\rat(16/13){11}{\spec{1}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(29/13){3}{}&\rat(23/13){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(16/13){3}{\spec{1}}&\rat(36/13){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(16/13){3}{\spec{2}}&\rat(36/13){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(28/13){2}{}&\rat(24/13){10}{\spec{1}}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\rat(24/13){11}{}&\rat(28/13){3}{\spec{1}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(24/13){11}{}&\rat(28/13){3}{\spec{2}}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(11/13){11}{}&\rat(41/13){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(14/13){1}{}&\rat(38/13){5}{\spec{1}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(14/13){1}{}&\rat(38/13){5}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{1}}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(1/13){1}{}&\rat(51/13){5}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 49
\orbit{2}{49}{105}
\h{49}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&&\cnt{891}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){8}{\spec{2}}&\int(0){1}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(4){5}{\spec{2}}&\int(0){12}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(3){8}{\spec{4}}&\int(1){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){8}{\spec{5}}&\int(1){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){5}{\spec{4}}&\int(1){12}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){5}{\spec{5}}&\int(1){12}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(4){10}{}&\int(0){11}{\spec{1}}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\int(4){10}{}&\int(0){11}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(3){10}{\spec{2}}&\int(1){11}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(3){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(3){11}{}&\int(1){3}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 50
\orbit{2}{50}{105}
\h{50}&\rat(48/13){11}{\spec{1}}&\rat(108/13){3}{\spec{3}}&&\cnt{1035}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{216}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{240}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(4/13){2}{}&\rat(48/13){10}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(24/13){12}{}&\rat(28/13){8}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(24/13){12}{}&\rat(28/13){8}{\spec{2}}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(24/13){12}{}&\rat(28/13){8}{\spec{3}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{72}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(-2/13){12}{}&\rat(54/13){8}{}&\ln{1}&\cnt{72}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 51
\orbit{2}{51}{105}
\h{51}&\rat(48/13){11}{\spec{1}}&\rat(108/13){3}{\spec{4}}&&\cnt{923}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{462}&\bounds{42}{42}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{84}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{120}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(24/13){12}{}&\rat(28/13){8}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{5}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 52
\orbit{2}{52}{105}
\h{52}&\rat(12/13){12}{}&\rat(144/13){8}{\spec{1}}&&\cnt{1099}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(3/13){3}{}&\rat(49/13){2}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{96}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(11/13){11}{}&\rat(41/13){3}{\spec{1}}&\ln{1}&\cnt{96}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(11/13){11}{}&\rat(41/13){3}{\spec{2}}&\ln{1}&\cnt{36}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(-2/13){11}{}&\rat(54/13){3}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(12/13){12}{}&\rat(40/13){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(1/13){1}{}&\rat(51/13){5}{}&\ln{1}&\cnt{288}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(-12/13){1}{}&\rat(64/13){5}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 53
\orbit{2}{53}{105}
\h{53}&\rat(126/13){11}{\spec{2}}&\rat(30/13){3}{}&&\cnt{663}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\rat(62/13){5}{}&\rat(-10/13){12}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(55/13){8}{}&\rat(-3/13){1}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(49/13){5}{\spec{1}}&\rat(3/13){12}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(49/13){5}{\spec{2}}&\rat(3/13){12}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(42/13){8}{\spec{1}}&\rat(10/13){1}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\rat(45/13){3}{}&\rat(7/13){2}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(32/13){3}{\spec{1}}&\rat(20/13){2}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(22/13){11}{\spec{1}}&\rat(30/13){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 54
\orbit{2}{54}{105}
\h{54}&\rat(12/13){12}{}&\rat(144/13){8}{\spec{4}}&&\cnt{1011}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(10/13){10}{}&\rat(42/13){11}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{48}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(11/13){11}{}&\rat(41/13){3}{}&\ln{1}&\cnt{72}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(2/13){2}{}&\rat(50/13){10}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{3}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(1/13){1}{}&\rat(51/13){5}{}&\ln{1}&\cnt{240}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(-1/13){12}{}&\rat(53/13){8}{}&\ln{1}&\cnt{216}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{5}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 55
\orbit{2}{55}{104}
\h{55}&\rat(62/13){9}{\spec{1}}&\rat(94/13){6}{\spec{2}}&&\cnt{911}&\bounds{104}{104}{1}{false}&&\cr
\l{1}&\rat(32/13){8}{}&\rat(20/13){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(40/13){10}{}&\rat(12/13){11}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(12/13){3}{}&\rat(40/13){2}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(31/13){11}{}&\rat(21/13){3}{\spec{1}}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(18/13){11}{\spec{1}}&\rat(34/13){3}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(18/13){11}{\spec{1}}&\rat(34/13){3}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(18/13){11}{\spec{2}}&\rat(34/13){3}{\spec{1}}&\ln{1}&\cnt{90}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(18/13){11}{\spec{2}}&\rat(34/13){3}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(5/13){11}{}&\rat(47/13){3}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(22/13){12}{}&\rat(30/13){8}{\spec{1}}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{12}&\rat(4/13){1}{}&\rat(48/13){5}{}&\ln{1}&\cnt{90}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 56
\orbit{2}{56}{104}
\h{56}&\rat(48/13){11}{\spec{2}}&\rat(108/13){3}{\spec{3}}&&\cnt{675}&\bounds{104}{104}{1}{false}&&\cr
\l{1}&\rat(33/13){10}{}&\rat(19/13){11}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(17/13){2}{}&\rat(35/13){10}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(4/13){2}{\spec{1}}&\rat(48/13){10}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(4/13){2}{\spec{2}}&\rat(48/13){10}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(15/13){1}{}&\rat(37/13){5}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(11/13){12}{}&\rat(41/13){8}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(11/13){12}{}&\rat(41/13){8}{\spec{2}}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(-2/13){12}{}&\rat(54/13){8}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 57
\orbit{2}{57}{104}
\h{57}&\rat(88/13){9}{\spec{1}}&\rat(68/13){6}{\spec{2}}&&\cnt{731}&\bounds{104}{104}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(45/13){8}{}&\rat(7/13){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(32/13){8}{\spec{1}}&\rat(20/13){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(32/13){8}{\spec{2}}&\rat(20/13){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(40/13){10}{}&\rat(12/13){11}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(25/13){3}{}&\rat(27/13){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(31/13){11}{}&\rat(21/13){3}{\spec{1}}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(31/13){11}{}&\rat(21/13){3}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(18/13){11}{\spec{1}}&\rat(34/13){3}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(18/13){11}{\spec{2}}&\rat(34/13){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(22/13){12}{}&\rat(30/13){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(17/13){1}{}&\rat(35/13){5}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(4/13){1}{}&\rat(48/13){5}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 58
\orbit{2}{58}{103}
\h{58}&\rat(22/13){11}{}&\rat(134/13){3}{\spec{3}}&&\cnt{835}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(9/13){11}{}&\rat(43/13){3}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(4/13){2}{}&\rat(48/13){10}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(11/13){12}{}&\rat(41/13){8}{\spec{1}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(11/13){12}{}&\rat(41/13){8}{\spec{2}}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(-2/13){12}{}&\rat(54/13){8}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(-11/13){1}{}&\rat(63/13){5}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 59
\orbit{2}{59}{101}
\h{59}&\rat(90/13){12}{\spec{2}}&\rat(66/13){8}{\spec{1}}&&\cnt{675}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(47/13){8}{}&\rat(5/13){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(44/13){5}{}&\rat(8/13){12}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(31/13){5}{\spec{1}}&\rat(21/13){12}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(31/13){5}{\spec{2}}&\rat(21/13){12}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(42/13){3}{}&\rat(10/13){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(36/13){10}{}&\rat(16/13){11}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(36/13){10}{}&\rat(16/13){11}{\spec{2}}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(23/13){10}{}&\rat(29/13){11}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(28/13){2}{}&\rat(24/13){10}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(28/13){2}{}&\rat(24/13){10}{\spec{2}}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(15/13){2}{}&\rat(37/13){10}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(12/13){12}{}&\rat(40/13){8}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 60
\orbit{2}{60}{101}
\h{60}&\rat(38/13){12}{\spec{2}}&\rat(118/13){8}{\spec{3}}&&\cnt{775}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\rat(23/13){10}{}&\rat(29/13){11}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(10/13){10}{\spec{1}}&\rat(42/13){11}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(10/13){10}{\spec{2}}&\rat(42/13){11}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(24/13){11}{}&\rat(28/13){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(15/13){2}{}&\rat(37/13){10}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(15/13){2}{}&\rat(37/13){10}{\spec{2}}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(2/13){2}{\spec{1}}&\rat(50/13){10}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(2/13){2}{\spec{2}}&\rat(50/13){10}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(14/13){1}{}&\rat(38/13){5}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{14}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{1}}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(-1/13){12}{}&\rat(53/13){8}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 61
\orbit{2}{61}{100}
\h{61}&\rat(62/13){9}{\spec{2}}&\rat(94/13){6}{\spec{2}}&&\cnt{675}&\bounds{100}{100}{1}{false}&&\cr
\l{1}&\rat(45/13){8}{}&\rat(7/13){1}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(33/13){5}{}&\rat(19/13){12}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\rat(27/13){10}{}&\rat(25/13){11}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(14/13){10}{}&\rat(38/13){11}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(21/13){2}{}&\rat(31/13){10}{\spec{1}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(21/13){2}{}&\rat(31/13){10}{\spec{2}}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\rat(8/13){2}{\spec{1}}&\rat(44/13){10}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(8/13){2}{\spec{2}}&\rat(44/13){10}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(17/13){1}{}&\rat(35/13){5}{\spec{2}}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(9/13){12}{}&\rat(43/13){8}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(-4/13){12}{}&\rat(56/13){8}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 62
\orbit{2}{62}{100}
\h{62}&\rat(12/13){12}{}&\rat(144/13){8}{\spec{6}}&&\cnt{951}&\bounds{100}{100}{1}{false}&&\cr
\l{1}&\rat(10/13){10}{}&\rat(42/13){11}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{96}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(2/13){2}{}&\rat(50/13){10}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{1}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(-1/13){12}{}&\rat(53/13){8}{}&\ln{1}&\cnt{96}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 63
\orbit{2}{63}{100}
\h{63}&\rat(114/13){9}{\spec{3}}&\rat(42/13){6}{}&&\cnt{779}&\bounds{100}{100}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(45/13){8}{}&\rat(7/13){1}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\rat(53/13){10}{}&\rat(-1/13){11}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(40/13){10}{}&\rat(12/13){11}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(44/13){11}{}&\rat(8/13){3}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(31/13){11}{}&\rat(21/13){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(22/13){12}{}&\rat(30/13){8}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(17/13){1}{}&\rat(35/13){5}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 64
\orbit{2}{64}{100}
\h{64}&\int(6){\6}{\spec{1}}&\int(6){\6}{}&&\cnt{779}&\bounds{100}{100}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){10}{}&\int(2){11}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(2){2}{}&\ln{1}&\cnt{30}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{90}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(2){11}{}&\int(2){3}{}&\ln{1}&\cnt{210}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){10}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(1){11}{}&\int(3){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\int(3){10}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){12}{}&\int(2){8}{\spec{1}}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{12}&\int(2){12}{}&\int(2){8}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(1){1}{}&\int(3){5}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 65
\orbit{2}{65}{99}
\h{65}&\rat(22/13){11}{}&\rat(134/13){3}{\spec{4}}&&\cnt{911}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(4/13){2}{}&\rat(48/13){10}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(11/13){12}{}&\rat(41/13){8}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{231}&\bounds{21}{21}{1}{false}&&\cr
\l{6}&\rat(-2/13){12}{}&\rat(54/13){8}{\spec{1}}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(-2/13){12}{}&\rat(54/13){8}{\spec{2}}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 66
\orbit{2}{66}{99}
\h{66}&\int(10){\10}{}&\int(2){\2}{}&&\cnt{787}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(5){8}{}&\int(-1){1}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){1}{}&\ln{2}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(3){8}{\spec{1}}&\int(1){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(3){8}{\spec{3}}&\int(1){1}{}&\ln{2}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(3){10}{}&\int(1){11}{}&\ln{2}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 67
\orbit{2}{67}{98}
\h{67}&\rat(62/13){9}{\spec{1}}&\rat(94/13){6}{\spec{1}}&&\cnt{723}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\rat(32/13){8}{}&\rat(20/13){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(40/13){10}{}&\rat(12/13){11}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(40/13){10}{}&\rat(12/13){11}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(27/13){10}{}&\rat(25/13){11}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(31/13){11}{}&\rat(21/13){3}{\spec{1}}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(31/13){11}{}&\rat(21/13){3}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(18/13){11}{\spec{1}}&\rat(34/13){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(18/13){11}{\spec{2}}&\rat(34/13){3}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(22/13){12}{}&\rat(30/13){8}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(22/13){12}{}&\rat(30/13){8}{\spec{2}}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\rat(9/13){12}{}&\rat(43/13){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(4/13){1}{}&\rat(48/13){5}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 68
\orbit{2}{68}{98}
\h{68}&\rat(74/13){11}{\spec{2}}&\rat(82/13){3}{\spec{1}}&&\cnt{731}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(42/13){8}{}&\rat(10/13){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(36/13){5}{}&\rat(16/13){12}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(29/13){8}{\spec{1}}&\rat(23/13){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(29/13){8}{\spec{2}}&\rat(23/13){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(33/13){10}{}&\rat(19/13){11}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(32/13){3}{}&\rat(20/13){2}{\spec{1}}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\rat(32/13){3}{}&\rat(20/13){2}{\spec{2}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(19/13){3}{\spec{1}}&\rat(33/13){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(19/13){3}{\spec{2}}&\rat(33/13){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(30/13){2}{}&\rat(22/13){10}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(9/13){11}{}&\rat(43/13){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(15/13){1}{}&\rat(37/13){5}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 69
\orbit{2}{69}{97}
\h{69}&\rat(64/13){12}{\spec{1}}&\rat(92/13){8}{\spec{1}}&&\cnt{899}&\bounds{97}{97}{1}{false}&&\cr
\l{1}&\rat(23/13){10}{}&\rat(29/13){11}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{3}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(24/13){11}{}&\rat(28/13){3}{}&\ln{1}&\cnt{231}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(15/13){2}{}&\rat(37/13){10}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(25/13){12}{}&\rat(27/13){8}{\spec{1}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(25/13){12}{}&\rat(27/13){8}{\spec{2}}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{12}&\rat(25/13){12}{}&\rat(27/13){8}{\spec{3}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(14/13){1}{}&\rat(38/13){5}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{14}&\rat(-1/13){12}{}&\rat(53/13){8}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 70
\orbit{2}{70}{97}
\h{70}&\rat(74/13){11}{\spec{1}}&\rat(82/13){3}{\spec{2}}&&\cnt{723}&\bounds{97}{97}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(33/13){10}{}&\rat(19/13){11}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(20/13){10}{\spec{1}}&\rat(32/13){11}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(20/13){10}{\spec{2}}&\rat(32/13){11}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(35/13){11}{}&\rat(17/13){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(17/13){2}{}&\rat(35/13){10}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(24/13){12}{}&\rat(28/13){8}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(24/13){12}{}&\rat(28/13){8}{\spec{2}}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{14}&\rat(15/13){1}{}&\rat(37/13){5}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(11/13){12}{}&\rat(41/13){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 71
\orbit{2}{71}{95}
\h{71}&\rat(100/13){11}{\spec{2}}&\rat(56/13){3}{\spec{2}}&&\cnt{787}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(55/13){8}{}&\rat(-3/13){1}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(49/13){5}{}&\rat(3/13){12}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(42/13){8}{}&\rat(10/13){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(29/13){8}{\spec{1}}&\rat(23/13){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(29/13){8}{\spec{2}}&\rat(23/13){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(45/13){3}{}&\rat(7/13){2}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(32/13){3}{}&\rat(20/13){2}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(19/13){3}{\spec{1}}&\rat(33/13){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(19/13){3}{\spec{2}}&\rat(33/13){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 72
\orbit{2}{72}{95}
\h{72}&\rat(90/13){12}{\spec{1}}&\rat(66/13){8}{\spec{1}}&&\cnt{775}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(31/13){5}{\spec{2}}&\rat(21/13){12}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(36/13){10}{\spec{2}}&\rat(16/13){11}{\spec{1}}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(36/13){10}{\spec{2}}&\rat(16/13){11}{\spec{2}}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(23/13){10}{\spec{2}}&\rat(29/13){11}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(23/13){10}{\spec{3}}&\rat(29/13){11}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(37/13){11}{}&\rat(15/13){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(28/13){2}{\spec{2}}&\rat(24/13){10}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(28/13){2}{\spec{2}}&\rat(24/13){10}{\spec{2}}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(15/13){2}{\spec{2}}&\rat(37/13){10}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(25/13){12}{}&\rat(27/13){8}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(12/13){12}{\spec{2}}&\rat(40/13){8}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 73
\orbit{2}{73}{95}
\h{73}&\rat(64/13){12}{\spec{2}}&\rat(92/13){8}{\spec{2}}&&\cnt{787}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(31/13){5}{}&\rat(21/13){12}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(36/13){10}{}&\rat(16/13){11}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(23/13){10}{}&\rat(29/13){11}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(10/13){10}{\spec{1}}&\rat(42/13){11}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(10/13){10}{\spec{2}}&\rat(42/13){11}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(28/13){2}{}&\rat(24/13){10}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(15/13){2}{}&\rat(37/13){10}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(2/13){2}{\spec{1}}&\rat(50/13){10}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(2/13){2}{\spec{2}}&\rat(50/13){10}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{2}}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 74
\orbit{2}{74}{95}
\h{74}&\rat(38/13){12}{\spec{2}}&\rat(118/13){8}{\spec{2}}&&\cnt{787}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\rat(16/13){3}{}&\rat(36/13){2}{\spec{1}}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(24/13){11}{}&\rat(28/13){3}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(24/13){11}{}&\rat(28/13){3}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(11/13){11}{}&\rat(41/13){3}{\spec{1}}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(-2/13){11}{\spec{1}}&\rat(54/13){3}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(-2/13){11}{\spec{2}}&\rat(54/13){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(14/13){1}{}&\rat(38/13){5}{\spec{1}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(14/13){1}{}&\rat(38/13){5}{\spec{2}}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{1}}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(1/13){1}{}&\rat(51/13){5}{\spec{1}}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(-12/13){1}{}&\rat(64/13){5}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 75
\orbit{2}{75}{93}
\h{75}&\rat(62/13){9}{\spec{1}}&\rat(94/13){6}{\spec{2}}&&\cnt{787}&\bounds{93}{93}{1}{false}&&\cr
\l{1}&\rat(40/13){10}{}&\rat(12/13){11}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(40/13){10}{}&\rat(12/13){11}{\spec{3}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(27/13){10}{}&\rat(25/13){11}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(14/13){10}{\spec{1}}&\rat(38/13){11}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(14/13){10}{\spec{2}}&\rat(38/13){11}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(31/13){11}{}&\rat(21/13){3}{\spec{2}}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(8/13){2}{}&\rat(44/13){10}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(22/13){12}{}&\rat(30/13){8}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(22/13){12}{}&\rat(30/13){8}{\spec{3}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(9/13){12}{}&\rat(43/13){8}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(-4/13){12}{}&\rat(56/13){8}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 76
\orbit{2}{76}{92}
\h{76}&\rat(100/13){11}{\spec{1}}&\rat(56/13){3}{\spec{2}}&&\cnt{875}&\bounds{92}{92}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(42/13){8}{\spec{1}}&\rat(10/13){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(29/13){8}{\spec{1}}&\rat(23/13){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(32/13){3}{\spec{1}}&\rat(20/13){2}{}&\ln{1}&\cnt{308}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\rat(19/13){3}{\spec{1}}&\rat(33/13){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(22/13){11}{\spec{1}}&\rat(30/13){3}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(28/13){1}{}&\rat(24/13){5}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 77
\orbit{2}{77}{89}
\h{77}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&&\cnt{975}&\bounds{89}{89}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{7}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(4){8}{\spec{2}}&\int(0){1}{}&\ln{2}&\cnt{273}&\bounds{21}{21}{1}{false}&&\cr
\l{7}&\int(4){10}{}&\int(0){11}{}&\ln{2}&\cnt{78}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{156}&\bounds{13}{13}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 78
\orbit{2}{78}{89}
\h{78}&\rat(12/13){12}{}&\rat(144/13){8}{\spec{3}}&&\cnt{819}&\bounds{89}{89}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(11/13){11}{}&\rat(41/13){3}{}&\ln{1}&\cnt{108}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(-2/13){11}{}&\rat(54/13){3}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{2}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(1/13){1}{}&\rat(51/13){5}{\spec{1}}&\ln{1}&\cnt{216}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(1/13){1}{}&\rat(51/13){5}{\spec{2}}&\ln{1}&\cnt{36}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(-1/13){12}{}&\rat(53/13){8}{}&\ln{1}&\cnt{180}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(-12/13){1}{}&\rat(64/13){5}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 79
\orbit{2}{79}{88}
\h{79}&\rat(62/13){9}{\spec{2}}&\rat(94/13){6}{\spec{2}}&&\cnt{667}&\bounds{88}{88}{1}{false}&&\cr
\l{1}&\rat(45/13){8}{}&\rat(7/13){1}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(32/13){8}{}&\rat(20/13){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(25/13){3}{}&\rat(27/13){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(12/13){3}{\spec{1}}&\rat(40/13){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(12/13){3}{\spec{2}}&\rat(40/13){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(18/13){11}{}&\rat(34/13){3}{\spec{1}}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(18/13){11}{}&\rat(34/13){3}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(5/13){11}{}&\rat(47/13){3}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(17/13){1}{}&\rat(35/13){5}{\spec{1}}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(4/13){1}{}&\rat(48/13){5}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 80
\orbit{2}{80}{87}
\h{80}&\rat(22/13){11}{}&\rat(134/13){3}{\spec{5}}&&\cnt{671}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{110}&\bounds{11}{11}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(9/13){11}{}&\rat(43/13){3}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(11/13){12}{}&\rat(41/13){8}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{9}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 81
\orbit{2}{81}{87}
\h{81}&\rat(64/13){12}{\spec{1}}&\rat(92/13){8}{\spec{2}}&&\cnt{707}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\rat(16/13){3}{}&\rat(36/13){2}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{154}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\rat(24/13){11}{}&\rat(28/13){3}{\spec{1}}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\rat(24/13){11}{}&\rat(28/13){3}{\spec{2}}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(11/13){11}{}&\rat(41/13){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(25/13){12}{}&\rat(27/13){8}{\spec{1}}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{9}&\rat(14/13){1}{}&\rat(38/13){5}{\spec{1}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(14/13){1}{}&\rat(38/13){5}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(1/13){1}{}&\rat(51/13){5}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 82
\orbit{2}{82}{87}
\h{82}&\int(12){\12}{\spec{3}}&\int(0){\0}{}&&\cnt{923}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){8}{\spec{2}}&\int(0){1}{}&\ln{1}&\cnt{234}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(4){8}{\spec{3}}&\int(0){1}{}&\ln{1}&\cnt{65}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(4){5}{\spec{3}}&\int(0){12}{}&\ln{1}&\cnt{260}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(4){10}{}&\int(0){11}{}&\ln{1}&\cnt{234}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 83
\orbit{2}{83}{85}
\h{83}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&&\cnt{751}&\bounds{85}{85}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{110}&\bounds{11}{11}{1}{false}&&\cr
\l{2}&\int(2){10}{}&\int(2){11}{}&\ln{2}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{2}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){11}{}&\int(2){3}{}&\ln{2}&\cnt{99}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(2){12}{}&\int(2){8}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 84
\orbit{2}{84}{84}
\h{84}&\rat(48/13){11}{\spec{2}}&\rat(108/13){3}{\spec{1}}&&\cnt{763}&\bounds{84}{84}{1}{false}&&\cr
\l{1}&\rat(29/13){8}{}&\rat(23/13){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(33/13){10}{}&\rat(19/13){11}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(6/13){3}{\spec{1}}&\rat(46/13){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(6/13){3}{\spec{2}}&\rat(46/13){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/13){11}{}&\rat(43/13){3}{}&\ln{1}&\cnt{270}&\bounds{27}{27}{1}{false}&&\cr
\l{10}&\rat(15/13){1}{}&\rat(37/13){5}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 85
\orbit{2}{85}{84}
\h{85}&\rat(12/13){12}{}&\rat(144/13){8}{\spec{2}}&&\cnt{783}&\bounds{84}{84}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{60}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(11/13){11}{}&\rat(41/13){3}{}&\ln{1}&\cnt{180}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{3}}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(1/13){1}{}&\rat(51/13){5}{}&\ln{1}&\cnt{180}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(-1/13){12}{}&\rat(53/13){8}{}&\ln{1}&\cnt{60}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 86
\orbit{2}{86}{84}
\h{86}&\rat(100/13){11}{\spec{1}}&\rat(56/13){3}{\spec{2}}&&\cnt{763}&\bounds{84}{84}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(42/13){8}{\spec{2}}&\rat(10/13){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(29/13){8}{\spec{2}}&\rat(23/13){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(29/13){8}{\spec{3}}&\rat(23/13){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(46/13){10}{}&\rat(6/13){11}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(32/13){3}{\spec{2}}&\rat(20/13){2}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(19/13){3}{\spec{2}}&\rat(33/13){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(19/13){3}{\spec{3}}&\rat(33/13){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{22}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(35/13){11}{}&\rat(17/13){3}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(22/13){11}{\spec{2}}&\rat(30/13){3}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(22/13){11}{\spec{3}}&\rat(30/13){3}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 87
\orbit{2}{87}{81}
\h{87}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&&\cnt{739}&\bounds{81}{81}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(3){8}{}&\int(1){1}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){10}{}&\int(1){11}{}&\ln{2}&\cnt{99}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{110}&\bounds{11}{11}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\ln{2}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\ln{2}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{2}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(3){11}{}&\int(1){3}{}&\ln{2}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 88
\orbit{2}{88}{79}
\h{88}&\rat(48/13){11}{\spec{1}}&\rat(108/13){3}{\spec{2}}&&\cnt{755}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\rat(20/13){10}{}&\rat(32/13){11}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{84}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{72}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{2}}&\ln{1}&\cnt{252}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\rat(22/13){11}{}&\rat(30/13){3}{\spec{3}}&\ln{1}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(24/13){12}{}&\rat(28/13){8}{\spec{1}}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\rat(24/13){12}{}&\rat(28/13){8}{\spec{2}}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(2/13){1}{}&\rat(50/13){5}{}&\ln{1}&\cnt{84}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 89
\orbit{2}{89}{76}
\h{89}&\rat(48/13){11}{\spec{1}}&\rat(108/13){3}{\spec{1}}&&\cnt{727}&\bounds{76}{76}{1}{false}&&\cr
\l{1}&\rat(6/13){3}{}&\rat(46/13){2}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{240}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\rat(22/13){11}{}&\rat(30/13){3}{}&\ln{1}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(24/13){12}{}&\rat(28/13){8}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 90
\orbit{2}{90}{75}
\h{90}&\int(12){\12}{}&\int(0){\0}{}&&\cnt{615}&\bounds{75}{75}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{2}&\int(4){8}{}&\int(0){1}{}&\ln{2}&\cnt{195}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 91
\orbit{2}{91}{74}
\h{91}&\rat(36/13){9}{}&\rat(120/13){6}{\spec{4}}&&\cnt{651}&\bounds{74}{74}{1}{false}&&\cr
\l{1}&\rat(27/13){10}{}&\rat(25/13){11}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(14/13){10}{}&\rat(38/13){11}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\rat(8/13){2}{}&\rat(44/13){10}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(-5/13){2}{}&\rat(57/13){10}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(9/13){12}{}&\rat(43/13){8}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(-4/13){12}{}&\rat(56/13){8}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 92
\orbit{2}{92}{73}
\h{92}&\rat(126/13){11}{\spec{2}}&\rat(30/13){3}{}&&\cnt{615}&\bounds{73}{73}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(42/13){8}{\spec{2}}&\rat(10/13){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(46/13){10}{}&\rat(6/13){11}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(32/13){3}{\spec{2}}&\rat(20/13){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(35/13){11}{}&\rat(17/13){3}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(22/13){11}{\spec{2}}&\rat(30/13){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(22/13){11}{\spec{3}}&\rat(30/13){3}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(28/13){1}{}&\rat(24/13){5}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 93
\orbit{2}{93}{72}
\h{93}&\rat(88/13){9}{\spec{2}}&\rat(68/13){6}{\spec{1}}&&\cnt{643}&\bounds{72}{72}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(40/13){10}{}&\rat(12/13){11}{\spec{1}}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(40/13){10}{}&\rat(12/13){11}{\spec{2}}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{154}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\rat(44/13){11}{}&\rat(8/13){3}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(22/13){12}{}&\rat(30/13){8}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(22/13){12}{}&\rat(30/13){8}{\spec{2}}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 94
\orbit{2}{94}{71}
\h{94}&\rat(12/13){12}{}&\rat(144/13){8}{\spec{5}}&&\cnt{795}&\bounds{71}{71}{1}{false}&&\cr
\l{1}&\rat(10/13){10}{}&\rat(42/13){11}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(-11/13){2}{}&\rat(63/13){10}{}&\ln{1}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(12/13){12}{}&\rat(40/13){8}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(-1/13){12}{}&\rat(53/13){8}{}&\ln{1}&\cnt{432}&\bounds{36}{36}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 95
\orbit{2}{95}{70}
\h{95}&\rat(12/13){12}{}&\rat(144/13){8}{\spec{2}}&&\cnt{615}&\bounds{70}{70}{1}{false}&&\cr
\l{1}&\rat(-2/13){11}{}&\rat(54/13){3}{}&\ln{1}&\cnt{264}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\rat(12/13){12}{}&\rat(40/13){8}{\spec{1}}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\rat(-12/13){1}{}&\rat(64/13){5}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 96
\orbit{2}{96}{70}
\h{96}&\rat(116/13){12}{\spec{2}}&\rat(40/13){8}{}&&\cnt{559}&\bounds{70}{70}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(36/13){10}{\spec{2}}&\rat(16/13){11}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(37/13){11}{}&\rat(15/13){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(28/13){2}{\spec{2}}&\rat(24/13){10}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(27/13){1}{}&\rat(25/13){5}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(25/13){12}{}&\rat(27/13){8}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(12/13){12}{\spec{2}}&\rat(40/13){8}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 97
\orbit{2}{97}{69}
\h{97}&\int(12){\12}{\spec{5}}&\int(0){\0}{}&&\cnt{687}&\bounds{69}{69}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{216}&\bounds{27}{27}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{468}&\bounds{39}{39}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[12]
% Class 98
\orbit{2}{98}{66}
\h{98}&\rat(64/13){12}{\spec{1}}&\rat(92/13){8}{\spec{2}}&&\cnt{683}&\bounds{66}{66}{1}{false}&&\cr
\l{1}&\rat(23/13){10}{}&\rat(29/13){11}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(10/13){10}{}&\rat(42/13){11}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{3}}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{4}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(15/13){2}{}&\rat(37/13){10}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(2/13){2}{}&\rat(50/13){10}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(25/13){12}{}&\rat(27/13){8}{\spec{2}}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_2A9_D6.tex <==
% -*- TeX -*-
% Niemeier lattice 2A9_D6
% 317 classes
\newcs{max-2A9_D6}{189}%
\newcs{count-2A9_D6}{317}%
\newcs{counts-2A9_D6}{\DO{1}{189}\DO{2}{183}\DO{3}{183}\DO{4}{179}\DO{5}{179}\DO{6}{177}\DO{7}{175}\DO{8}{175}\DO{9}{173}\DO{10}{169}\DO{11}{169}\DO{12}{167}\DO{13}{167}\DO{14}{167}\DO{15}{167}\DO{16}{165}\DO{17}{165}\DO{18}{165}\DO{19}{165}\DO{20}{163}\DO{21}{163}\DO{22}{162}\DO{23}{162}\DO{24}{161}\DO{25}{161}\DO{26}{161}\DO{27}{159}\DO{28}{159}\DO{29}{159}\DO{30}{159}\DO{31}{159}\DO{32}{157}\DO{33}{157}\DO{34}{157}\DO{35}{155}\DO{36}{155}\DO{37}{155}\DO{38}{155}\DO{39}{155}\DO{40}{155}\DO{41}{155}\DO{42}{155}\DO{43}{154}\DO{44}{154}\DO{45}{153}\DO{46}{153}\DO{47}{152}\DO{48}{151}\DO{49}{151}\DO{50}{151}\DO{51}{151}\DO{52}{151}\DO{53}{151}\DO{54}{151}\DO{55}{150}\DO{56}{149}\DO{57}{149}\DO{58}{148}\DO{59}{147}\DO{60}{147}\DO{61}{147}\DO{62}{147}\DO{63}{147}\DO{64}{146}\DO{65}{146}\DO{66}{146}\DO{67}{145}\DO{68}{145}\DO{69}{145}\DO{70}{145}\DO{71}{145}\DO{72}{145}\DO{73}{145}\DO{74}{145}\DO{75}{145}\DO{76}{145}\DO{77}{145}\DO{78}{144}\DO{79}{144}\DO{80}{144}\DO{81}{143}\DO{82}{143}\DO{83}{143}\DO{84}{143}\DO{85}{143}\DO{86}{143}\DO{87}{143}\DO{88}{143}\DO{89}{143}\DO{90}{143}\DO{91}{143}\DO{92}{143}\DO{93}{143}\DO{94}{143}\DO{95}{142}\DO{96}{141}\DO{97}{141}\DO{98}{141}\DO{99}{141}\DO{100}{141}\DO{101}{140}\DO{102}{140}\DO{103}{140}\DO{104}{140}\DO{105}{139}\DO{106}{139}\DO{107}{139}\DO{108}{139}\DO{109}{139}\DO{110}{139}\DO{111}{139}\DO{112}{138}\DO{113}{138}\DO{114}{138}\DO{115}{137}\DO{116}{137}\DO{117}{137}\DO{118}{137}\DO{119}{137}\DO{120}{137}\DO{121}{137}\DO{122}{136}\DO{123}{136}\DO{124}{136}\DO{125}{135}\DO{126}{135}\DO{127}{135}\DO{128}{135}\DO{129}{135}\DO{130}{135}\DO{131}{135}\DO{132}{135}\DO{133}{135}\DO{134}{135}\DO{135}{135}\DO{136}{135}\DO{137}{135}\DO{138}{135}\DO{139}{135}\DO{140}{134}\DO{141}{134}\DO{142}{133}\DO{143}{133}\DO{144}{133}\DO{145}{133}\DO{146}{133}\DO{147}{133}\DO{148}{133}\DO{149}{133}\DO{150}{133}\DO{151}{133}\DO{152}{133}\DO{153}{133}\DO{154}{133}\DO{155}{132}\DO{156}{132}\DO{157}{132}\DO{158}{132}\DO{159}{131}\DO{160}{131}\DO{161}{131}\DO{162}{131}\DO{163}{131}\DO{164}{131}\DO{165}{131}\DO{166}{131}\DO{167}{131}\DO{168}{130}\DO{169}{130}\DO{170}{130}\DO{171}{130}\DO{172}{129}\DO{173}{129}\DO{174}{129}\DO{175}{129}\DO{176}{129}\DO{177}{129}\DO{178}{129}\DO{179}{129}\DO{180}{128}\DO{181}{127}\DO{182}{127}\DO{183}{127}\DO{184}{127}\DO{185}{127}\DO{186}{127}\DO{187}{127}\DO{188}{127}\DO{189}{127}\DO{190}{127}\DO{191}{127}\DO{192}{127}\DO{193}{127}\DO{194}{126}\DO{195}{126}\DO{196}{126}\DO{197}{126}\DO{198}{125}\DO{199}{125}\DO{200}{125}\DO{201}{125}\DO{202}{125}\DO{203}{125}\DO{204}{125}\DO{205}{124}\DO{206}{123}\DO{207}{123}\DO{208}{123}\DO{209}{123}\DO{210}{123}\DO{211}{123}\DO{212}{122}\DO{213}{122}\DO{214}{122}\DO{215}{122}\DO{216}{121}\DO{217}{121}\DO{218}{121}\DO{219}{121}\DO{220}{121}\DO{221}{121}\DO{222}{120}\DO{223}{120}\DO{224}{119}\DO{225}{119}\DO{226}{119}\DO{227}{119}\DO{228}{119}\DO{229}{119}\DO{230}{119}\DO{231}{118}\DO{232}{118}\DO{233}{118}\DO{234}{118}\DO{235}{118}\DO{236}{118}\DO{237}{117}\DO{238}{117}\DO{239}{117}\DO{240}{117}\DO{241}{117}\DO{242}{116}\DO{243}{116}\DO{244}{116}\DO{245}{116}\DO{246}{116}\DO{247}{116}\DO{248}{116}\DO{249}{115}\DO{250}{115}\DO{251}{115}\DO{252}{115}\DO{253}{115}\DO{254}{114}\DO{255}{114}\DO{256}{113}\DO{257}{113}\DO{258}{113}\DO{259}{113}\DO{260}{112}\DO{261}{111}\DO{262}{111}\DO{263}{111}\DO{264}{111}\DO{265}{111}\DO{266}{110}\DO{267}{110}\DO{268}{109}\DO{269}{109}\DO{270}{109}\DO{271}{109}\DO{272}{109}\DO{273}{109}\DO{274}{108}\DO{275}{108}\DO{276}{108}\DO{277}{107}\DO{278}{107}\DO{279}{107}\DO{280}{107}\DO{281}{106}\DO{282}{106}\DO{283}{104}\DO{284}{104}\DO{285}{104}\DO{286}{103}\DO{287}{103}\DO{288}{102}\DO{289}{101}\DO{290}{100}\DO{291}{100}\DO{292}{100}\DO{293}{99}\DO{294}{99}\DO{295}{98}\DO{296}{98}\DO{297}{98}\DO{298}{96}\DO{299}{96}\DO{300}{95}\DO{301}{95}\DO{302}{95}\DO{303}{94}\DO{304}{94}\DO{305}{93}\DO{306}{93}\DO{307}{92}\DO{308}{91}\DO{309}{91}\DO{310}{91}\DO{311}{90}\DO{312}{90}\DO{313}{87}\DO{314}{85}\DO{315}{79}\DO{316}{75}\DO{317}{67}}%
\orbits
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 1
\orbit{3}{1}{189}
\h{1}&\int(6){\6}{}&\int(6){\6}{}&\int(0){\0}{}&&\cnt{687}&\bounds{189}{189}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{4}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{4}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{4}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){7}{}&\int(1){9}{}&\int(0){2}{}&\ln{4}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 2
\orbit{3}{2}{183}
\h{2}&\rat(38/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(2){\2}{}&&\cnt{927}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(3){5}{\spec{1}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(16/5){6}{\spec{1}}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(14/5){4}{\spec{1}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(13/5){3}{\spec{1}}&\rat(2/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(12/5){7}{\spec{1}}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(12/5){2}{\spec{1}}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(12/5){2}{\spec{1}}&\rat(3/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{12}&\rat(8/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(11/5){1}{}&\rat(9/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(11/5){1}{}&\rat(4/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(11/5){1}{}&\rat(4/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 3
\orbit{3}{3}{183}
\h{3}&\rat(48/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(0){\0}{}&&\cnt{1059}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(4){5}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\rat(24/5){4}{}&\rat(-4/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(16/5){6}{\spec{1}}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{5}&\rat(14/5){4}{\spec{1}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(18/5){3}{}&\rat(2/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\l{7}&\rat(12/5){2}{\spec{1}}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(8/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 4
\orbit{3}{4}{179}
\h{4}&\rat(48/5){8}{\spec{4}}&\rat(12/5){6}{}&\int(0){\0}{}&&\cnt{1035}&\bounds{179}{179}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(16/5){6}{}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{4}&\rat(14/5){4}{}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(17/5){7}{}&\rat(3/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(18/5){8}{}&\rat(2/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(18/5){8}{}&\rat(2/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\rat(12/5){2}{}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 5
\orbit{3}{5}{179}
\h{5}&\rat(5/2){5}{}&\rat(5/2){5}{}&\int(7){2}{}&&\cnt{875}&\bounds{179}{179}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(3/2){7}{}&\rat(1/2){9}{}&\int(2){2}{}&\ln{4}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(1){8}{}&\rat(1/2){1}{}&\rat(5/2){3}{}&\ln{4}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 6
\orbit{3}{6}{177}
\h{6}&\rat(18/5){8}{\spec{1}}&\rat(42/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{1431}&\bounds{177}{177}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{315}&\bounds{35}{35}{1}{false}&&\cr
\l{4}&\rat(2/5){2}{}&\rat(18/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\rat(9/5){9}{}&\rat(11/5){3}{\spec{1}}&\int(0){2}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{6}&\rat(-1/5){9}{}&\rat(21/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 7
\orbit{3}{7}{175}
\h{7}&\int(12){\12}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1507}&\bounds{175}{175}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){5}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\int(4){4}{}&\int(0){8}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(4){7}{}&\int(0){9}{}&\int(0){2}{}&\ln{1}&\cnt{480}&\bounds{48}{48}{1}{false}&&\cr
\l{7}&\int(4){8}{}&\int(0){6}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{8}&\int(4){8}{}&\int(0){1}{}&\int(0){3}{}&\ln{1}&\cnt{320}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 8
\orbit{3}{8}{175}
\h{8}&\rat(81/10){7}{\spec{1}}&\rat(12/5){4}{}&\rat(3/2){1}{}&&\cnt{983}&\bounds{175}{175}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(16/5){4}{}&\rat(4/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(14/5){6}{}&\rat(6/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(29/10){3}{}&\rat(3/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(13/5){2}{}&\rat(7/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(13/5){2}{}&\rat(2/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(23/10){1}{}&\rat(6/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\rat(23/10){1}{}&\rat(6/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(23/10){1}{}&\rat(1/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 9
\orbit{3}{9}{173}
\h{9}&\rat(18/5){8}{\spec{2}}&\rat(42/5){6}{\spec{1}}&\int(0){\0}{}&&\cnt{1023}&\bounds{173}{173}{1}{false}&&\cr
\l{1}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(6/5){6}{\spec{1}}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{3}&\rat(6/5){6}{\spec{2}}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/5){3}{}&\rat(12/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(8/5){8}{}&\rat(12/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(2/5){2}{\spec{1}}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(2/5){2}{\spec{2}}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(6/5){1}{}&\rat(14/5){2}{}&\int(0){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(4/5){9}{}&\rat(16/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 10
\orbit{3}{10}{169}
\h{10}&\rat(21/10){7}{}&\rat(42/5){4}{\spec{4}}&\rat(3/2){1}{}&&\cnt{1035}&\bounds{169}{169}{1}{false}&&\cr
\l{1}&\rat(6/5){4}{}&\rat(14/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(12/5){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(11/10){7}{}&\rat(12/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(3/5){2}{}&\rat(12/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(2/5){8}{}&\rat(18/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(7/10){9}{}&\rat(14/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{9}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(3/10){1}{}&\rat(16/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(-3/10){9}{}&\rat(14/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 11
\orbit{3}{11}{169}
\h{11}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(9){2}{\spec{4}}&&\cnt{1371}&\bounds{169}{169}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(3/10){9}{}&\int(3){2}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\rat(3/10){3}{}&\rat(7/10){1}{}&\int(3){2}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(1/10){3}{}&\int(3){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(1/10){1}{}&\rat(9/10){7}{}&\int(3){2}{}&\ln{1}&\cnt{315}&\bounds{35}{35}{1}{false}&&\cr
\l{6}&\rat(-1/10){9}{}&\rat(11/10){3}{}&\int(3){2}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 12
\orbit{3}{12}{167}
\h{12}&\rat(38/5){8}{\spec{1}}&\rat(22/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{911}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(16/5){6}{\spec{1}}&\rat(4/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(16/5){6}{\spec{1}}&\rat(4/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(14/5){4}{\spec{1}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(11/5){6}{\spec{1}}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(13/5){3}{\spec{1}}&\rat(7/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(12/5){2}{\spec{1}}&\rat(8/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{11}&\rat(12/5){2}{\spec{1}}&\rat(8/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(8/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(7/5){2}{\spec{1}}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(11/5){1}{}&\rat(9/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\rat(11/5){1}{}&\rat(9/5){2}{}&\int(0){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 13
\orbit{3}{13}{167}
\h{13}&\rat(17/2){5}{\spec{3}}&\rat(5/2){5}{}&\int(1){2}{}&&\cnt{1087}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(7/2){7}{}&\rat(1/2){9}{}&\int(0){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(7/2){7}{}&\rat(-1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(5/2){7}{}&\rat(1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{175}&\bounds{25}{25}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(3){8}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(3){8}{}&\rat(1/2){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(5/2){9}{}&\rat(3/2){3}{}&\int(0){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(5/2){9}{}&\rat(1/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(5/2){9}{}&\int(1){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 14
\orbit{3}{14}{167}
\h{14}&\rat(48/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(0){\0}{}&&\cnt{967}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){5}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(19/5){4}{}&\rat(1/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(16/5){6}{}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(14/5){4}{\spec{1}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(14/5){4}{\spec{2}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(18/5){3}{}&\rat(2/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(17/5){2}{}&\rat(3/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(17/5){2}{}&\rat(3/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(12/5){2}{}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(11/5){1}{}&\rat(9/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 15
\orbit{3}{15}{167}
\h{15}&\rat(81/10){7}{\spec{4}}&\rat(12/5){4}{}&\rat(3/2){1}{}&&\cnt{1191}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(12/5){8}{}&\rat(8/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(12/5){8}{}&\rat(3/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\rat(27/10){9}{}&\rat(9/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(27/10){9}{}&\rat(4/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\l{7}&\rat(27/10){9}{}&\rat(4/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{8}&\rat(27/10){9}{}&\rat(-1/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 16
\orbit{3}{16}{165}
\h{16}&\rat(48/5){8}{\spec{3}}&\rat(12/5){6}{}&\int(0){\0}{}&&\cnt{855}&\bounds{165}{165}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(4){5}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(21/5){6}{}&\rat(-1/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(19/5){4}{}&\rat(1/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(16/5){6}{}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{8}&\rat(14/5){4}{\spec{1}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(14/5){4}{\spec{2}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\rat(18/5){3}{}&\rat(2/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(17/5){7}{}&\rat(3/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(13/5){8}{}&\rat(7/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(12/5){2}{}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(8/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(8/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 17
\orbit{3}{17}{165}
\h{17}&\int(6){\6}{}&\int(4){\4}{}&\int(2){\2}{}&&\cnt{703}&\bounds{165}{165}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){7}{}&\int(1){9}{}&\int(0){2}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){7}{}&\int(0){9}{}&\int(1){2}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){7}{}&\int(1){9}{}&\int(1){2}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(1){9}{}&\int(2){3}{}&\int(1){2}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(1){9}{}&\int(2){8}{}&\int(1){1}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 18
\orbit{3}{18}{165}
\h{18}&\rat(38/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(2){\2}{}&&\cnt{815}&\bounds{165}{165}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){5}{\spec{2}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(16/5){6}{\spec{2}}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(14/5){4}{\spec{2}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(17/5){7}{}&\rat(3/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(17/5){7}{}&\rat(-2/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(13/5){3}{\spec{2}}&\rat(2/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(12/5){7}{\spec{2}}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(13/5){8}{}&\rat(7/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(13/5){8}{}&\rat(2/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{17}&\rat(12/5){2}{\spec{2}}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(12/5){2}{\spec{2}}&\rat(3/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(8/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(8/5){8}{\spec{3}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(9/5){9}{}&\rat(6/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\rat(9/5){9}{}&\rat(6/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{23}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 19
\orbit{3}{19}{165}
\h{19}&\rat(28/5){8}{\spec{2}}&\rat(22/5){6}{\spec{2}}&\int(2){\2}{}&&\cnt{703}&\bounds{165}{165}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(16/5){6}{}&\rat(4/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(16/5){6}{}&\rat(4/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(14/5){4}{}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(13/5){3}{}&\rat(7/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(13/5){3}{}&\rat(2/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(8/5){3}{\spec{1}}&\rat(7/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(8/5){3}{\spec{2}}&\rat(7/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(12/5){2}{}&\rat(8/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(12/5){2}{}&\rat(8/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(12/5){2}{}&\rat(3/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\rat(6/5){1}{}&\rat(9/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{22}&\rat(4/5){9}{}&\rat(11/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 20
\orbit{3}{20}{163}
\h{20}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&&\cnt{1159}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\int(2){7}{}&\int(2){9}{}&\int(0){2}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{245}&\bounds{35}{35}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(2){4}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(2){9}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){9}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(2){9}{}&\int(2){8}{}&\int(0){1}{}&\ln{1}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 21
\orbit{3}{21}{163}
\h{21}&\rat(5/2){5}{}&\int(8){\8}{\spec{2}}&\rat(3/2){1}{}&&\cnt{871}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(2){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(1){4}{}&\int(3){8}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(3/2){7}{}&\int(2){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(1){\2}{}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\int(1){8}{}&\int(3){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(1){2}{}&\int(3){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(1){2}{}&\int(2){9}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(1/2){9}{}&\int(3){3}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(1/2){9}{}&\int(3){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(1/2){9}{}&\int(2){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(1/2){1}{}&\int(3){7}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{150}&\bounds{25}{25}{1}{false}&&\cr
\l{14}&\rat(1/2){1}{}&\int(2){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(-1/2){9}{}&\int(3){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){5}{\spec{3}}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 22
\orbit{3}{22}{162}
\h{22}&\rat(21/10){7}{}&\rat(42/5){4}{\spec{2}}&\rat(3/2){1}{}&&\cnt{1139}&\bounds{162}{162}{1}{false}&&\cr
\l{1}&\rat(9/5){6}{}&\rat(11/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(4/5){6}{}&\rat(16/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(9/10){3}{}&\rat(13/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{210}&\bounds{35}{35}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\rat(7/5){8}{}&\rat(13/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(2/5){8}{}&\rat(13/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(7/10){9}{}&\rat(14/5){3}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{144}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(3/10){1}{}&\rat(16/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(3/10){1}{}&\rat(11/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(-7/10){1}{}&\rat(16/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 23
\orbit{3}{23}{162}
\h{23}&\rat(69/10){9}{\spec{1}}&\rat(21/10){3}{}&\int(3){2}{}&&\cnt{867}&\bounds{162}{162}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(13/5){6}{\spec{1}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(27/10){7}{\spec{1}}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(23/10){3}{\spec{1}}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(11/5){2}{\spec{1}}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(11/5){2}{\spec{1}}&\rat(3/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(9/5){8}{\spec{1}}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(21/10){1}{}&\rat(9/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{13}&\rat(21/10){1}{}&\rat(7/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(21/10){1}{}&\rat(2/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(9/10){9}{\spec{1}}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 24
\orbit{3}{24}{161}
\h{24}&\rat(21/10){7}{}&\rat(12/5){4}{}&\rat(15/2){1}{\spec{2}}&&\cnt{979}&\bounds{161}{161}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(-3/5){9}{}&\rat(5/2){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(11/10){7}{}&\rat(2/5){9}{}&\rat(5/2){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\rat(9/10){3}{}&\rat(3/5){1}{}&\rat(5/2){2}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(7/10){9}{}&\rat(4/5){3}{}&\rat(5/2){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(7/10){9}{}&\rat(4/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(3/10){1}{}&\rat(6/5){7}{}&\rat(5/2){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(3/10){1}{}&\rat(6/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(-3/10){9}{}&\rat(9/5){3}{}&\rat(5/2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 25
\orbit{3}{25}{161}
\h{25}&\rat(13/2){5}{\spec{1}}&\rat(5/2){5}{}&\int(3){2}{}&&\cnt{763}&\bounds{161}{161}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(5/2){7}{}&\rat(1/2){9}{}&\int(1){2}{}&\ln{2}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(2){8}{}&\rat(1/2){1}{}&\rat(3/2){3}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(3/2){9}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 26
\orbit{3}{26}{161}
\h{26}&\rat(28/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(4){\4}{}&&\cnt{703}&\bounds{161}{161}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){5}{\spec{1}}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){5}{\spec{2}}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(16/5){6}{}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(14/5){4}{}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(13/5){3}{}&\rat(2/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(12/5){2}{}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(12/5){2}{}&\rat(3/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(12/5){2}{}&\rat(-2/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(7/5){2}{}&\rat(3/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(6/5){1}{}&\rat(4/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(4/5){9}{}&\rat(6/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 27
\orbit{3}{27}{159}
\h{27}&\rat(41/10){7}{\spec{2}}&\rat(12/5){4}{}&\rat(11/2){1}{}&&\cnt{759}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(3/2){5}{\spec{1}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(3/2){5}{\spec{2}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(14/5){6}{}&\rat(6/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(19/10){3}{}&\rat(3/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(8/5){2}{}&\rat(2/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{13}&\rat(13/10){1}{}&\rat(6/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(13/10){1}{}&\rat(6/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(13/10){1}{}&\rat(1/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(7/10){9}{}&\rat(4/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(3/10){1}{}&\rat(6/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 28
\orbit{3}{28}{159}
\h{28}&\int(0){\0}{}&\int(0){\0}{}&\int(12){\12}{\spec{1}}&&\cnt{1347}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(0){8}{}&\int(0){1}{}&\int(4){3}{}&\ln{2}&\cnt{450}&\bounds{45}{45}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(0){5}{}&\int(4){3}{}&\ln{1}&\cnt{252}&\bounds{42}{42}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 29
\orbit{3}{29}{159}
\h{29}&\rat(81/10){7}{\spec{2}}&\rat(12/5){4}{}&\rat(3/2){1}{}&&\cnt{815}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(7/2){5}{\spec{2}}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(5/2){5}{\spec{3}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(19/5){6}{}&\rat(1/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(16/5){4}{\spec{2}}&\rat(4/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(14/5){6}{\spec{2}}&\rat(6/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\rat(31/10){7}{}&\rat(2/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(29/10){3}{\spec{2}}&\rat(3/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(13/5){2}{\spec{2}}&\rat(7/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(13/5){2}{\spec{2}}&\rat(2/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(12/5){8}{}&\rat(8/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{17}&\rat(12/5){8}{}&\rat(3/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(8/5){2}{\spec{2}}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(17/10){9}{}&\rat(9/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(17/10){9}{}&\rat(4/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\rat(13/10){1}{\spec{2}}&\rat(6/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 30
\orbit{3}{30}{159}
\h{30}&\rat(8/5){8}{}&\rat(42/5){6}{\spec{4}}&\int(2){\2}{}&&\cnt{1135}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\rat(4/5){4}{}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\rat(7/5){7}{}&\rat(13/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(2/5){7}{}&\rat(13/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(2/5){2}{}&\rat(13/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{224}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\rat(4/5){9}{}&\rat(16/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(-1/5){9}{}&\rat(16/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 31
\orbit{3}{31}{159}
\h{31}&\int(8){\8}{}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{811}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){5}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(4){6}{}&\int(0){2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){6}{\spec{3}}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){7}{}&\int(1){9}{}&\int(0){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{2}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 32
\orbit{3}{32}{157}
\h{32}&\rat(29/10){9}{\spec{2}}&\rat(81/10){3}{\spec{4}}&\int(1){2}{}&&\cnt{975}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\rat(7/5){4}{}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(23/10){9}{}&\int(0){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(7/10){7}{\spec{1}}&\rat(23/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(7/10){7}{\spec{2}}&\rat(23/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(6/5){2}{}&\rat(23/10){9}{}&\rat(1/2){3}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(11/10){1}{}&\rat(29/10){7}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 33
\orbit{3}{33}{157}
\h{33}&\rat(18/5){8}{\spec{2}}&\rat(42/5){6}{\spec{4}}&\int(0){\0}{}&&\cnt{1127}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\rat(9/5){4}{}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\rat(4/5){4}{\spec{1}}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(4/5){4}{\spec{2}}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(7/5){7}{}&\rat(13/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(7/5){2}{}&\rat(13/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(4/5){9}{}&\rat(16/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 34
\orbit{3}{34}{157}
\h{34}&\int(10){\10}{}&\int(0){\0}{}&\int(2){\2}{}&&\cnt{1183}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(5){5}{}&\int(0){\0}{}&\int(-1){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{200}&\bounds{40}{40}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{2}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{5}&\int(3){7}{}&\int(0){9}{}&\int(1){2}{}&\ln{2}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 35
\orbit{3}{35}{155}
\h{35}&\rat(8/5){8}{}&\rat(52/5){6}{\spec{3}}&\int(0){\0}{}&&\cnt{1035}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(4/5){4}{}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(2/5){2}{}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\rat(-2/5){8}{}&\rat(22/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(16/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(4/5){9}{}&\rat(16/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(1/5){1}{}&\rat(19/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 36
\orbit{3}{36}{155}
\h{36}&\rat(8/5){8}{}&\rat(42/5){6}{\spec{1}}&\int(2){\2}{}&&\cnt{1031}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(3/5){3}{}&\rat(12/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(3/5){8}{}&\rat(12/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(2/5){2}{}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(4/5){9}{}&\rat(16/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(4/5){9}{}&\rat(11/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(1/5){1}{}&\rat(14/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(-1/5){9}{}&\rat(16/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 37
\orbit{3}{37}{155}
\h{37}&\rat(5/2){5}{}&\int(2){\2}{}&\rat(15/2){1}{\spec{2}}&&\cnt{975}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(3/2){7}{}&\int(0){9}{}&\rat(5/2){2}{}&\ln{2}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(1/2){7}{}&\int(1){9}{}&\rat(5/2){2}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{125}&\bounds{25}{25}{1}{false}&&\cr
\l{6}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(1/2){9}{}&\int(1){3}{}&\rat(5/2){2}{}&\ln{2}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(1/2){9}{}&\int(1){8}{}&\rat(5/2){1}{}&\ln{2}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 38
\orbit{3}{38}{155}
\h{38}&\rat(28/5){8}{\spec{2}}&\rat(32/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{811}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(16/5){6}{}&\rat(4/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(16/5){6}{}&\rat(4/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(14/5){4}{}&\rat(6/5){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(6/5){6}{\spec{1}}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(6/5){6}{\spec{2}}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(13/5){3}{}&\rat(7/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(12/5){2}{}&\rat(8/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(12/5){2}{}&\rat(8/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(2/5){2}{\spec{1}}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(2/5){2}{\spec{2}}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(6/5){1}{}&\rat(14/5){2}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(4/5){9}{}&\rat(16/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 39
\orbit{3}{39}{155}
\h{39}&\rat(8/5){8}{}&\rat(42/5){6}{\spec{2}}&\int(2){\2}{}&&\cnt{807}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(7/5){1}{\spec{2}}&\int(1){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(2/5){2}{}&\rat(18/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(4/5){9}{}&\rat(16/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(11/5){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(4/5){9}{}&\rat(11/5){3}{\spec{3}}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(1/5){1}{}&\rat(14/5){2}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(-1/5){9}{}&\rat(16/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){5}{\spec{2}}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 40
\orbit{3}{40}{155}
\h{40}&\rat(18/5){8}{\spec{2}}&\rat(42/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{799}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(9/5){4}{}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(6/5){6}{\spec{1}}&\rat(14/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(6/5){6}{\spec{2}}&\rat(14/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{12}&\rat(7/5){2}{}&\rat(13/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(7/5){2}{}&\rat(13/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(2/5){2}{\spec{1}}&\rat(18/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(2/5){2}{\spec{2}}&\rat(18/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{17}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(6/5){1}{}&\rat(14/5){2}{\spec{2}}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(4/5){9}{}&\rat(16/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 41
\orbit{3}{41}{155}
\h{41}&\rat(28/5){8}{\spec{2}}&\rat(32/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{1059}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(16/5){6}{}&\rat(4/5){2}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(14/5){4}{}&\rat(6/5){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(4/5){4}{\spec{1}}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(4/5){4}{\spec{2}}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(4/5){4}{\spec{3}}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(12/5){2}{}&\rat(8/5){4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{10}&\rat(12/5){2}{}&\rat(8/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{13}&\rat(4/5){9}{}&\rat(16/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 42
\orbit{3}{42}{155}
\h{42}&\rat(18/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(6){\6}{\spec{1}}&&\cnt{815}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(12/5){7}{}&\rat(-2/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/5){3}{}&\rat(2/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(7/5){2}{}&\rat(3/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(6/5){1}{}&\rat(4/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(6/5){1}{}&\rat(4/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(4/5){9}{}&\rat(6/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(4/5){9}{}&\rat(6/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{18}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 43
\orbit{3}{43}{154}
\h{43}&\rat(18/5){8}{\spec{2}}&\rat(32/5){6}{\spec{1}}&\int(2){\2}{}&&\cnt{759}&\bounds{154}{154}{1}{false}&&\cr
\l{1}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(9/5){4}{}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(8/5){3}{}&\rat(7/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(7/5){2}{}&\rat(8/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(6/5){1}{}&\rat(9/5){7}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(6/5){1}{}&\rat(9/5){7}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(6/5){1}{}&\rat(9/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\rat(4/5){9}{}&\rat(11/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{23}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 44
\orbit{3}{44}{154}
\h{44}&\rat(49/10){9}{\spec{2}}&\rat(41/10){3}{\spec{1}}&\int(3){2}{}&&\cnt{707}&\bounds{154}{154}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(12/5){4}{}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(27/10){7}{}&\rat(13/10){9}{}&\int(0){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(27/10){7}{}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(23/10){3}{}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{}&\rat(13/10){9}{}&\rat(1/2){3}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(11/5){2}{}&\rat(3/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(6/5){2}{}&\rat(13/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{21}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 45
\orbit{3}{45}{153}
\h{45}&\rat(89/10){9}{\spec{1}}&\rat(21/10){3}{}&\int(1){2}{}&&\cnt{919}&\bounds{153}{153}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(18/5){6}{}&\rat(2/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(17/5){4}{}&\rat(3/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(33/10){3}{}&\rat(7/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(33/10){3}{}&\rat(-3/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(27/10){7}{}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(23/10){3}{\spec{1}}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(23/10){3}{\spec{2}}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(16/5){2}{}&\rat(4/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(16/5){2}{}&\rat(3/10){9}{}&\rat(1/2){3}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{16}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(21/10){1}{}&\rat(9/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{18}&\rat(21/10){1}{}&\rat(7/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 46
\orbit{3}{46}{153}
\h{46}&\rat(69/10){9}{\spec{2}}&\rat(21/10){3}{}&\int(3){2}{}&&\cnt{699}&\bounds{153}{153}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(18/5){6}{}&\rat(2/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(17/5){4}{}&\rat(3/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(33/10){3}{}&\rat(7/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(33/10){3}{}&\rat(-3/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(27/10){7}{}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(23/10){3}{}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{81}&\bounds{27}{27}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(11/5){2}{}&\rat(3/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{17}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 47
\orbit{3}{47}{152}
\h{47}&\rat(69/10){9}{\spec{1}}&\rat(41/10){3}{\spec{1}}&\int(1){2}{}&&\cnt{863}&\bounds{152}{152}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(13/5){6}{\spec{1}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(12/5){4}{\spec{1}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(27/10){7}{\spec{1}}&\rat(13/10){9}{}&\int(0){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(27/10){7}{\spec{1}}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(23/10){3}{\spec{1}}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(17/10){7}{\spec{1}}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{\spec{1}}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\rat(11/5){2}{\spec{1}}&\rat(13/10){9}{}&\rat(1/2){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(9/5){8}{\spec{1}}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(6/5){2}{\spec{1}}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(21/10){1}{}&\rat(19/10){7}{}&\int(0){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{17}&\rat(21/10){1}{}&\rat(9/10){7}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(21/10){1}{}&\rat(9/10){7}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(21/10){1}{}&\rat(7/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{\spec{1}}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 48
\orbit{3}{48}{151}
\h{48}&\int(8){\8}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{855}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(3){4}{\spec{2}}&\int(1){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(2){6}{\spec{4}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){6}{\spec{5}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){4}{\spec{4}}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){4}{\spec{5}}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(3){7}{\spec{2}}&\int(1){9}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(3){3}{\spec{2}}&\int(1){1}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(3){8}{}&\int(1){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(3){8}{}&\int(1){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(3){8}{}&\int(1){1}{}&\int(0){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(2){8}{\spec{2}}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{19}&\int(2){2}{\spec{2}}&\int(2){4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{20}&\int(2){9}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\int(2){9}{}&\int(2){8}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 49
\orbit{3}{49}{151}
\h{49}&\rat(29/10){9}{\spec{2}}&\rat(38/5){8}{\spec{1}}&\rat(3/2){1}{}&&\cnt{923}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\rat(8/5){6}{}&\rat(12/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\rat(13/10){3}{}&\rat(11/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{2}}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(9/5){8}{}&\rat(11/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(11/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(6/5){2}{}&\rat(14/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(4/5){8}{}&\rat(16/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(4/5){8}{}&\rat(11/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(11/10){1}{}&\rat(12/5){7}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(11/10){1}{}&\rat(12/5){2}{\spec{1}}&\rat(1/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(11/10){1}{}&\rat(7/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(9/10){9}{}&\rat(13/5){3}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\rat(9/10){9}{}&\rat(8/5){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(1/10){1}{}&\rat(12/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){5}{\spec{1}}&\int(1){3}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 50
\orbit{3}{50}{151}
\h{50}&\rat(17/2){5}{\spec{3}}&\int(2){\2}{}&\rat(3/2){1}{}&&\cnt{1083}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(7/2){7}{}&\int(1){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(7/2){7}{}&\int(0){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(5/2){7}{}&\int(1){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(3){8}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(3){8}{}&\int(1){1}{}&\int(0){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(5/2){9}{}&\int(1){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{16}&\rat(5/2){9}{}&\int(1){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{17}&\rat(5/2){9}{}&\int(0){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(5/2){9}{}&\int(0){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 51
\orbit{3}{51}{151}
\h{51}&\rat(38/5){8}{\spec{1}}&\rat(22/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{799}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(16/5){6}{\spec{2}}&\rat(4/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(16/5){6}{\spec{2}}&\rat(4/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(14/5){4}{\spec{2}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(11/5){6}{\spec{2}}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(11/5){6}{\spec{3}}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(17/5){7}{}&\rat(3/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(13/5){3}{\spec{2}}&\rat(7/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(13/5){8}{}&\rat(7/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\rat(13/5){8}{}&\rat(7/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(12/5){2}{\spec{2}}&\rat(8/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(12/5){2}{\spec{2}}&\rat(8/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(8/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(8/5){8}{\spec{3}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\rat(7/5){2}{\spec{2}}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\rat(9/5){9}{}&\rat(11/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 52
\orbit{3}{52}{151}
\h{52}&\rat(28/5){8}{\spec{2}}&\rat(32/5){6}{\spec{1}}&\int(0){\0}{}&&\cnt{743}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(16/5){6}{}&\rat(4/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(16/5){6}{}&\rat(4/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(14/5){4}{}&\rat(6/5){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(14/5){4}{}&\rat(6/5){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(9/5){4}{\spec{1}}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(9/5){4}{\spec{2}}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(13/5){3}{}&\rat(7/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(12/5){2}{}&\rat(8/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(12/5){2}{}&\rat(8/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(12/5){2}{}&\rat(8/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{19}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{20}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 53
\orbit{3}{53}{151}
\h{53}&\rat(69/10){9}{\spec{1}}&\rat(18/5){8}{\spec{2}}&\rat(3/2){1}{}&&\cnt{867}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(13/5){6}{\spec{1}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(12/5){4}{\spec{1}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(27/10){7}{\spec{1}}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(23/10){3}{\spec{1}}&\rat(6/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(11/5){2}{\spec{1}}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{\spec{1}}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(9/5){8}{\spec{1}}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(9/5){8}{\spec{1}}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(21/10){1}{}&\rat(12/5){7}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(21/10){1}{}&\rat(7/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{17}&\rat(21/10){1}{}&\rat(7/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{18}&\rat(21/10){1}{}&\rat(2/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(21/10){1}{}&\rat(2/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{\spec{1}}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 54
\orbit{3}{54}{151}
\h{54}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(19/2){1}{\spec{1}}&&\cnt{1147}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(1/2){5}{}&\int(0){\0}{}&\rat(7/2){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\int(1){8}{}&\int(0){1}{}&\int(3){3}{}&\ln{2}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(1/2){9}{}&\int(0){8}{}&\rat(7/2){1}{}&\ln{2}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 55
\orbit{3}{55}{150}
\h{55}&\rat(17/2){5}{\spec{2}}&\rat(5/2){5}{}&\int(1){2}{}&&\cnt{807}&\bounds{150}{150}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(3){4}{\spec{2}}&\int(1){8}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(7/2){7}{}&\rat(1/2){9}{}&\int(0){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(7/2){7}{}&\rat(-1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(5/2){7}{\spec{1}}&\rat(1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(5/2){7}{\spec{2}}&\rat(1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\rat(5/2){3}{\spec{2}}&\rat(1/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(3){8}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\int(3){8}{}&\rat(1/2){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\int(2){2}{\spec{2}}&\int(2){4}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{19}&\rat(3/2){9}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(3/2){1}{}&\rat(3/2){7}{}&\int(1){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 56
\orbit{3}{56}{149}
\h{56}&\int(6){\6}{}&\int(0){\0}{}&\int(6){\6}{1}&&\cnt{1059}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(1){5}{\spec{1}}&\int(0){\0}{}&\int(3){1}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){5}{\spec{2}}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(3){7}{}&\int(0){9}{}&\int(1){2}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{2}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(1){9}{}&\int(0){8}{}&\int(3){1}{}&\ln{2}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 57
\orbit{3}{57}{149}
\h{57}&\rat(89/10){9}{\spec{1}}&\rat(8/5){8}{}&\rat(3/2){1}{}&&\cnt{919}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(18/5){6}{}&\rat(2/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(17/5){4}{}&\rat(3/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(12/5){4}{\spec{1}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(12/5){4}{\spec{2}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(33/10){3}{}&\rat(1/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(27/10){7}{}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(16/5){2}{}&\rat(4/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{15}&\rat(16/5){2}{}&\rat(4/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(16/5){2}{}&\rat(-1/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(11/5){2}{}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(21/10){1}{}&\rat(7/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(21/10){1}{}&\rat(2/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 58
\orbit{3}{58}{148}
\h{58}&\rat(21/10){7}{}&\rat(12/5){4}{}&\rat(15/2){1}{\spec{1}}&&\cnt{867}&\bounds{148}{148}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(7/5){8}{}&\rat(-2/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(3/5){2}{}&\rat(2/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(2/5){8}{}&\rat(3/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(7/10){9}{}&\rat(4/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{10}&\rat(3/10){1}{}&\rat(6/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(1){5}{}&\int(3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 59
\orbit{3}{59}{147}
\h{59}&\rat(5/2){5}{}&\int(4){\4}{}&\rat(11/2){1}{}&&\cnt{759}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(3/2){7}{}&\int(1){9}{}&\rat(3/2){2}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(1/2){9}{}&\int(2){3}{}&\rat(3/2){2}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(1/2){9}{}&\int(2){8}{}&\rat(3/2){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(1/2){9}{}&\int(1){8}{}&\rat(5/2){1}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(-1/2){9}{}&\int(2){8}{}&\rat(5/2){1}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 60
\orbit{3}{60}{147}
\h{60}&\rat(69/10){9}{\spec{2}}&\rat(41/10){3}{\spec{1}}&\int(1){2}{}&&\cnt{695}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(18/5){6}{}&\rat(2/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(17/5){4}{}&\rat(3/5){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(17/5){4}{}&\rat(3/5){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(12/5){4}{\spec{1}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(12/5){4}{\spec{2}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(33/10){3}{}&\rat(7/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(33/10){3}{}&\rat(-3/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(27/10){7}{}&\rat(13/10){9}{}&\int(0){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(27/10){7}{}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(23/10){3}{}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(11/5){2}{}&\rat(13/10){9}{}&\rat(1/2){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 61
\orbit{3}{61}{147}
\h{61}&\rat(38/5){8}{\spec{2}}&\rat(22/5){6}{\spec{1}}&\int(0){\0}{}&&\cnt{935}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){5}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(19/5){4}{}&\rat(1/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(16/5){6}{}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(14/5){4}{\spec{1}}&\rat(6/5){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(14/5){4}{\spec{1}}&\rat(6/5){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(14/5){4}{\spec{2}}&\rat(6/5){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(14/5){4}{\spec{2}}&\rat(6/5){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(9/5){4}{}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(18/5){3}{}&\rat(2/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(12/5){2}{}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{14}&\rat(12/5){2}{}&\rat(8/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 62
\orbit{3}{62}{147}
\h{62}&\rat(28/5){8}{\spec{1}}&\rat(32/5){6}{\spec{1}}&\int(0){\0}{}&&\cnt{923}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(9/5){4}{}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(1){\2}{\spec{3}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(13/5){8}{}&\rat(7/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(13/5){8}{}&\rat(7/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(13/5){8}{}&\rat(7/5){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(13/5){8}{}&\rat(7/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{20}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{21}&\rat(3/5){8}{\spec{1}}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(3/5){8}{\spec{2}}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\rat(9/5){9}{}&\rat(11/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{24}&\rat(9/5){9}{}&\rat(11/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{25}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 63
\orbit{3}{63}{147}
\h{63}&\rat(18/5){8}{\spec{2}}&\rat(22/5){6}{\spec{2}}&\int(4){\4}{}&&\cnt{703}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(8/5){3}{}&\rat(7/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(7/5){2}{}&\rat(3/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(3/5){8}{}&\rat(7/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(6/5){1}{}&\rat(9/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(6/5){1}{}&\rat(4/5){2}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(6/5){1}{}&\rat(4/5){2}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(4/5){9}{}&\rat(11/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{18}&\rat(4/5){9}{}&\rat(6/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(1/5){1}{}&\rat(9/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 64
\orbit{3}{64}{146}
\h{64}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&\int(6){\6}{\spec{1}}&&\cnt{1159}&\bounds{146}{146}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\int(2){7}{}&\int(0){9}{}&\int(2){2}{}&\ln{1}&\cnt{210}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(0){1}{}&\int(2){2}{}&\ln{1}&\cnt{70}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{280}&\bounds{28}{28}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\int(0){9}{}&\int(2){3}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){9}{}&\int(0){3}{}&\int(2){2}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{13}&\int(2){9}{}&\int(0){8}{}&\int(2){1}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 65
\orbit{3}{65}{146}
\h{65}&\rat(18/5){8}{\spec{1}}&\rat(32/5){6}{\spec{2}}&\int(2){\2}{}&&\cnt{1183}&\bounds{146}{146}{1}{false}&&\cr
\l{1}&\rat(4/5){4}{}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\l{6}&\rat(9/5){9}{}&\rat(6/5){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(9/5){9}{}&\rat(16/5){8}{}&\int(-1){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(9/5){9}{}&\rat(6/5){8}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(-1/5){9}{}&\rat(16/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 66
\orbit{3}{66}{146}
\h{66}&\rat(89/10){9}{\spec{3}}&\rat(21/10){3}{}&\int(1){2}{}&&\cnt{863}&\bounds{146}{146}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(18/5){6}{}&\rat(2/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(17/5){4}{}&\rat(3/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(13/5){6}{\spec{1}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(13/5){6}{\spec{2}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(37/10){7}{}&\rat(3/10){9}{}&\int(0){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(37/10){7}{}&\rat(-7/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(33/10){3}{}&\rat(7/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(33/10){3}{}&\rat(-3/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(27/10){7}{}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(23/10){3}{}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{16}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(14/5){8}{}&\rat(6/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{18}&\rat(14/5){8}{}&\rat(7/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(19/10){9}{}&\rat(11/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 67
\orbit{3}{67}{145}
\h{67}&\rat(29/10){9}{\spec{2}}&\rat(81/10){3}{\spec{2}}&\int(1){2}{}&&\cnt{1183}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\rat(8/5){6}{}&\rat(12/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(13/10){3}{}&\rat(27/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\rat(3/10){3}{\spec{1}}&\rat(27/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(3/10){3}{\spec{2}}&\rat(27/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(27/10){1}{}&\rat(-1/2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/5){8}{}&\rat(27/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{9}&\rat(11/10){1}{}&\rat(12/5){2}{\spec{1}}&\rat(1/2){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 68
\orbit{3}{68}{145}
\h{68}&\rat(38/5){8}{\spec{1}}&\rat(22/5){6}{\spec{1}}&\int(0){\0}{}&&\cnt{903}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(16/5){6}{\spec{1}}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(14/5){4}{\spec{1}}&\rat(6/5){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(14/5){4}{\spec{1}}&\rat(6/5){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(9/5){4}{\spec{1}}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(12/5){7}{\spec{1}}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(12/5){2}{\spec{1}}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{11}&\rat(12/5){2}{\spec{1}}&\rat(8/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(8/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(11/5){1}{}&\rat(9/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 69
\orbit{3}{69}{145}
\h{69}&\rat(29/10){9}{\spec{2}}&\rat(21/10){3}{}&\int(7){2}{}&&\cnt{867}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(3/10){9}{}&\int(2){2}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(13/10){3}{}&\rat(7/10){1}{}&\int(2){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(9/5){8}{}&\rat(-3/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(6/5){2}{}&\rat(3/10){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\rat(4/5){8}{}&\rat(7/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(11/10){1}{}&\rat(9/10){7}{}&\int(2){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{13}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(2/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(9/10){9}{}&\rat(11/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(3/2){5}{}&\rat(5/2){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 70
\orbit{3}{70}{145}
\h{70}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(8){\8}{\spec{1}}&&\cnt{919}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(1){5}{}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(-3/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(3/5){8}{}&\rat(2/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(2/5){2}{}&\rat(3/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(4/5){9}{}&\rat(6/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(6/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(4/5){9}{}&\rat(1/5){8}{}&\int(3){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(1/5){1}{}&\rat(4/5){2}{}&\int(3){1}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{14}&\rat(-1/5){9}{}&\rat(6/5){8}{}&\int(3){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(1){5}{}&\int(3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 71
\orbit{3}{71}{145}
\h{71}&\rat(49/10){9}{\spec{2}}&\rat(21/10){3}{}&\int(5){2}{\spec{2}}&&\cnt{751}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(27/10){7}{}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(27/10){7}{}&\rat(-7/10){9}{}&\int(2){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(23/10){3}{}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(23/10){3}{}&\rat(-3/10){1}{}&\int(2){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(17/10){7}{}&\rat(3/10){9}{}&\int(2){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(13/10){3}{\spec{1}}&\rat(7/10){1}{}&\int(2){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(13/10){3}{\spec{2}}&\rat(7/10){1}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(11/5){2}{}&\rat(3/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(9/10){7}{}&\int(2){2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{18}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(11/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{21}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 72
\orbit{3}{72}{145}
\h{72}&\rat(8/5){8}{}&\rat(52/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{1063}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(1/5){6}{}&\rat(19/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(2/5){2}{}&\rat(18/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{7}&\rat(4/5){9}{}&\rat(16/5){3}{\spec{1}}&\int(0){2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(1/5){1}{}&\rat(19/5){2}{}&\int(0){1}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\rat(-1/5){9}{}&\rat(21/5){3}{\spec{1}}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 73
\orbit{3}{73}{145}
\h{73}&\rat(13/2){5}{\spec{1}}&\rat(9/2){5}{\spec{1}}&\int(1){2}{}&&\cnt{751}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){4}{}&\int(1){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){4}{}&\int(1){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){4}{\spec{1}}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(2){4}{\spec{2}}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/2){7}{}&\rat(3/2){9}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(5/2){7}{}&\rat(1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(3/2){7}{\spec{1}}&\rat(3/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(3/2){7}{\spec{2}}&\rat(3/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\int(2){2}{}&\int(2){4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\int(2){2}{}&\rat(3/2){9}{}&\rat(1/2){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\int(1){8}{\spec{1}}&\int(3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(1){8}{\spec{2}}&\int(3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\rat(3/2){9}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\rat(3/2){9}{}&\int(2){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\rat(3/2){1}{}&\rat(5/2){7}{}&\int(0){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{26}&\rat(3/2){1}{}&\rat(3/2){7}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\rat(3/2){1}{}&\rat(3/2){7}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{28}&\rat(1/2){1}{}&\rat(5/2){7}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 74
\orbit{3}{74}{145}
\h{74}&\rat(69/10){9}{\spec{1}}&\rat(21/10){3}{}&\int(3){2}{}&&\cnt{811}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(13/5){6}{\spec{2}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(27/10){7}{\spec{2}}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(23/10){3}{\spec{2}}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(14/5){8}{}&\rat(6/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\rat(14/5){8}{}&\rat(7/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(14/5){8}{}&\rat(-3/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(11/5){2}{\spec{2}}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(11/5){2}{\spec{2}}&\rat(3/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(9/5){8}{\spec{2}}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(19/10){9}{}&\rat(11/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\rat(19/10){9}{}&\rat(3/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(9/10){9}{\spec{2}}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 75
\orbit{3}{75}{145}
\h{75}&\rat(69/10){9}{\spec{1}}&\rat(18/5){8}{\spec{2}}&\rat(3/2){1}{}&&\cnt{811}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(13/5){6}{\spec{2}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(12/5){4}{\spec{2}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(27/10){7}{\spec{2}}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(23/10){3}{\spec{2}}&\rat(6/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(14/5){8}{}&\rat(6/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(14/5){8}{}&\rat(6/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(14/5){8}{}&\rat(6/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(14/5){8}{}&\rat(1/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(11/5){2}{\spec{2}}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(11/5){2}{\spec{2}}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\rat(9/5){8}{\spec{2}}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(9/5){8}{\spec{2}}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(19/10){9}{}&\rat(8/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{22}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{23}&\rat(19/10){9}{}&\rat(3/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\rat(9/10){9}{\spec{2}}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 76
\orbit{3}{76}{145}
\h{76}&\rat(21/2){5}{\spec{3}}&\int(0){\0}{}&\rat(3/2){1}{}&&\cnt{1035}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(9/2){5}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{2}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(7/2){7}{}&\int(0){9}{}&\rat(1/2){2}{}&\ln{2}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 77
\orbit{3}{77}{145}
\h{77}&\rat(13/2){5}{\spec{1}}&\int(4){\4}{}&\rat(3/2){1}{}&&\cnt{759}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(5/2){7}{}&\int(1){9}{}&\rat(1/2){2}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(3/2){9}{}&\int(2){3}{}&\rat(1/2){2}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(3/2){9}{}&\int(2){8}{}&\rat(1/2){1}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(1/2){9}{}&\int(2){8}{}&\rat(3/2){1}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 78
\orbit{3}{78}{144}
\h{78}&\rat(18/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(6){\6}{1}&&\cnt{1059}&\bounds{144}{144}{1}{false}&&\cr
\l{1}&\int(1){5}{}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\rat(9/5){9}{}&\rat(6/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(9/5){9}{}&\rat(6/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(9/5){9}{}&\rat(-4/5){8}{}&\int(3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(1/5){1}{}&\rat(4/5){2}{}&\int(3){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(-1/5){9}{}&\rat(6/5){8}{}&\int(3){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 79
\orbit{3}{79}{144}
\h{79}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(19/2){1}{\spec{1}}&&\cnt{1147}&\bounds{144}{144}{1}{false}&&\cr
\l{1}&\rat(1/2){5}{}&\int(0){\0}{}&\rat(7/2){1}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(1/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(1/5){2}{}&\rat(4/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(-2/5){8}{}&\rat(7/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(1/10){1}{}&\rat(2/5){2}{}&\rat(7/2){1}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\l{9}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(-1/10){9}{}&\rat(3/5){8}{}&\rat(7/2){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(1){5}{}&\int(3){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 80
\orbit{3}{80}{144}
\h{80}&\int(8){\8}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{863}&\bounds{144}{144}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){5}{\spec{3}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(3){4}{\spec{2}}&\int(1){8}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(3){7}{\spec{2}}&\int(1){9}{}&\int(0){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){7}{\spec{2}}&\int(0){9}{}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(3){3}{\spec{2}}&\int(1){1}{}&\int(0){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){3}{\spec{2}}&\int(0){1}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){7}{\spec{2}}&\int(1){9}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){7}{\spec{3}}&\int(1){9}{}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){3}{\spec{3}}&\int(1){1}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(2){\2}{\spec{4}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(3){8}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\int(3){8}{}&\int(1){1}{}&\int(0){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\int(2){8}{\spec{2}}&\int(1){1}{}&\int(1){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{24}&\int(2){2}{\spec{2}}&\int(1){9}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\int(2){9}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{26}&\int(2){9}{}&\int(1){8}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{27}&\int(0){\0}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 81
\orbit{3}{81}{143}
\h{81}&\rat(48/5){8}{\spec{5}}&\rat(12/5){6}{}&\int(0){\0}{}&&\cnt{975}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(13/5){8}{}&\rat(7/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(14/5){9}{}&\rat(6/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{240}&\bounds{40}{40}{1}{false}&&\cr
\l{9}&\rat(14/5){9}{}&\rat(6/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 82
\orbit{3}{82}{143}
\h{82}&\rat(9/2){5}{\spec{1}}&\rat(5/2){5}{}&\int(5){2}{\spec{2}}&&\cnt{751}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/2){7}{}&\rat(1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(5/2){7}{}&\rat(-1/2){9}{}&\int(2){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(3/2){7}{\spec{1}}&\rat(1/2){9}{}&\int(2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(3/2){7}{\spec{2}}&\rat(1/2){9}{}&\int(2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(3/2){3}{}&\rat(1/2){1}{}&\int(2){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(2){8}{}&\rat(1/2){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{13}&\rat(3/2){9}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(3/2){9}{}&\rat(1/2){3}{}&\int(2){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\rat(1/2){9}{}&\rat(3/2){3}{}&\int(2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(1/2){1}{}&\rat(3/2){7}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 83
\orbit{3}{83}{143}
\h{83}&\int(8){\8}{}&\int(0){\0}{}&\int(4){\4}{}&&\cnt{935}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){5}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){5}{\spec{1}}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(3){7}{}&\int(0){9}{}&\int(1){2}{}&\ln{2}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 84
\orbit{3}{84}{143}
\h{84}&\rat(69/10){9}{\spec{1}}&\rat(41/10){3}{\spec{1}}&\int(1){2}{}&&\cnt{807}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(13/5){6}{\spec{2}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\rat(12/5){4}{\spec{2}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(27/10){7}{\spec{2}}&\rat(13/10){9}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(27/10){7}{\spec{2}}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(23/10){3}{\spec{2}}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(17/10){7}{\spec{2}}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(17/10){7}{\spec{3}}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(14/5){8}{}&\rat(6/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(14/5){8}{}&\rat(6/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(14/5){8}{}&\rat(7/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(11/5){2}{\spec{2}}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(11/5){2}{\spec{2}}&\rat(13/10){9}{}&\rat(1/2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\rat(9/5){8}{\spec{2}}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{21}&\rat(6/5){2}{\spec{2}}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\rat(19/10){9}{}&\rat(11/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{25}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\rat(9/10){9}{\spec{2}}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 85
\orbit{3}{85}{143}
\h{85}&\int(2){\2}{}&\int(2){\2}{}&\int(8){\8}{\spec{1}}&&\cnt{911}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(1){5}{}&\int(0){\0}{}&\int(3){1}{}&\ln{2}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(1){7}{}&\int(1){9}{}&\int(2){2}{}&\ln{4}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{3}}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{4}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{4}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(1){8}{}&\int(0){1}{}&\int(3){3}{}&\ln{4}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){8}{\spec{1}}&\int(1){1}{}&\int(3){3}{}&\ln{4}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){8}{\spec{2}}&\int(1){1}{}&\int(3){3}{}&\ln{4}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 86
\orbit{3}{86}{143}
\h{86}&\int(6){\6}{}&\int(2){\2}{}&\int(4){\4}{}&&\cnt{695}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){5}{\spec{1}}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(3){7}{}&\int(1){9}{}&\int(0){2}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){7}{}&\int(0){9}{}&\int(1){2}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){7}{}&\int(1){9}{}&\int(1){2}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(1){9}{}&\int(1){8}{}&\int(2){1}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 87
\orbit{3}{87}{143}
\h{87}&\rat(28/5){8}{\spec{2}}&\rat(22/5){6}{\spec{1}}&\int(2){\2}{}&&\cnt{695}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(16/5){6}{}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(14/5){4}{}&\rat(6/5){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(14/5){4}{}&\rat(6/5){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(9/5){4}{\spec{1}}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(9/5){4}{\spec{2}}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(13/5){3}{}&\rat(2/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(12/5){2}{}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{15}&\rat(12/5){2}{}&\rat(8/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(12/5){2}{}&\rat(3/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(7/5){2}{}&\rat(8/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{19}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{22}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 88
\orbit{3}{88}{143}
\h{88}&\int(8){\8}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{687}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){5}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){5}{\spec{1}}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){6}{}&\int(0){2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){7}{}&\int(1){9}{}&\int(0){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(3){7}{}&\int(0){9}{}&\int(1){2}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){7}{}&\int(1){9}{}&\int(1){2}{}&\ln{2}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 89
\orbit{3}{89}{143}
\h{89}&\rat(41/10){7}{\spec{2}}&\rat(32/5){4}{\spec{1}}&\rat(3/2){1}{}&&\cnt{759}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(14/5){6}{}&\rat(6/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(14/5){6}{}&\rat(6/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(11/5){4}{}&\rat(9/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(9/5){6}{}&\rat(11/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(19/10){3}{}&\rat(8/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(8/5){2}{}&\rat(7/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(3/5){2}{\spec{1}}&\rat(17/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(3/5){2}{\spec{2}}&\rat(17/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(13/10){1}{}&\rat(11/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\rat(13/10){1}{}&\rat(11/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{20}&\rat(13/10){1}{}&\rat(6/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(13/10){1}{}&\rat(6/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{23}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\rat(3/10){1}{}&\rat(11/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 90
\orbit{3}{90}{143}
\h{90}&\rat(41/10){7}{\spec{2}}&\rat(22/5){4}{\spec{1}}&\rat(7/2){1}{}&&\cnt{703}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(14/5){6}{}&\rat(6/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(11/5){4}{}&\rat(9/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(19/10){3}{}&\rat(3/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(11/10){7}{}&\rat(7/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(8/5){2}{}&\rat(7/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(8/5){2}{}&\rat(2/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(3/5){2}{\spec{1}}&\rat(7/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(3/5){2}{\spec{2}}&\rat(7/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(13/10){1}{}&\rat(11/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(13/10){1}{}&\rat(6/5){7}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(13/10){1}{}&\rat(6/5){7}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(13/10){1}{}&\rat(6/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{21}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{23}&\rat(3/10){1}{}&\rat(11/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 91
\orbit{3}{91}{143}
\h{91}&\int(4){\4}{}&\int(4){\4}{}&\int(4){\4}{}&&\cnt{703}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{4}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){7}{}&\int(1){9}{}&\int(1){2}{}&\ln{4}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{4}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{4}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{4}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 92
\orbit{3}{92}{143}
\h{92}&\rat(38/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(2){\2}{}&&\cnt{695}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){5}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(19/5){4}{}&\rat(1/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(16/5){6}{}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(14/5){4}{\spec{1}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(14/5){4}{\spec{2}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(18/5){3}{}&\rat(2/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(18/5){3}{}&\rat(-3/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(13/5){3}{}&\rat(2/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(12/5){2}{}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(12/5){2}{}&\rat(3/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{15}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 93
\orbit{3}{93}{143}
\h{93}&\rat(5/2){5}{}&\int(6){\6}{}&\rat(7/2){1}{}&&\cnt{703}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(3/2){7}{}&\int(1){9}{}&\rat(3/2){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){8}{}&\int(3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(1/2){9}{}&\int(3){3}{}&\rat(1/2){2}{}&\ln{2}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(1/2){9}{}&\int(2){3}{}&\rat(3/2){2}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(1/2){9}{}&\int(2){8}{}&\rat(3/2){1}{}&\ln{2}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(-1/2){9}{}&\int(3){3}{}&\rat(3/2){2}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){5}{\spec{1}}&\int(2){3}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 94
\orbit{3}{94}{143}
\h{94}&\rat(5/2){5}{}&\int(2){\2}{}&\rat(15/2){1}{\spec{1}}&&\cnt{863}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(3/2){7}{}&\int(1){9}{}&\rat(3/2){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){8}{}&\int(0){1}{}&\int(3){3}{}&\ln{2}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(0){8}{}&\int(1){1}{}&\int(3){3}{}&\ln{2}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(1/2){9}{}&\int(1){8}{}&\rat(5/2){1}{}&\ln{2}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(1){5}{}&\int(3){3}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 95
\orbit{3}{95}{142}
\h{95}&\rat(49/10){9}{\spec{2}}&\rat(28/5){8}{\spec{2}}&\rat(3/2){1}{}&&\cnt{703}&\bounds{142}{142}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(12/5){4}{}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(8/5){6}{\spec{1}}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(8/5){6}{\spec{2}}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(27/10){7}{}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(23/10){3}{}&\rat(6/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(11/5){2}{}&\rat(9/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(11/5){2}{}&\rat(9/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(13/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 96
\orbit{3}{96}{141}
\h{96}&\rat(89/10){9}{\spec{3}}&\rat(8/5){8}{}&\rat(3/2){1}{}&&\cnt{863}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(18/5){6}{}&\rat(2/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(17/5){4}{}&\rat(3/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(12/5){4}{\spec{1}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(12/5){4}{\spec{2}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(37/10){7}{}&\rat(4/5){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(37/10){7}{}&\rat(-1/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(33/10){3}{}&\rat(1/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(27/10){7}{}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{17}&\rat(14/5){8}{}&\rat(6/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(14/5){8}{}&\rat(1/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(11/5){2}{}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\rat(19/10){9}{}&\rat(3/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 97
\orbit{3}{97}{141}
\h{97}&\rat(9/10){9}{}&\rat(81/10){3}{\spec{2}}&\int(3){2}{}&&\cnt{803}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(17/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(1/5){2}{}&\rat(19/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{3}}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(1/10){1}{}&\rat(12/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(5/2){5}{\spec{1}}&\rat(3/2){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(5/2){5}{\spec{2}}&\rat(3/2){3}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 98
\orbit{3}{98}{141}
\h{98}&\rat(61/10){7}{\spec{1}}&\rat(12/5){4}{}&\rat(7/2){1}{}&&\cnt{755}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(14/5){6}{}&\rat(6/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(31/10){7}{}&\rat(2/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(31/10){7}{}&\rat(-3/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(19/10){3}{}&\rat(3/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(12/5){8}{}&\rat(8/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(12/5){8}{}&\rat(3/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(12/5){8}{}&\rat(-2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(8/5){2}{}&\rat(2/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(7/5){8}{\spec{1}}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(7/5){8}{\spec{2}}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(17/10){9}{}&\rat(9/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(17/10){9}{}&\rat(4/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(17/10){9}{}&\rat(4/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{23}&\rat(13/10){1}{}&\rat(6/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\rat(13/10){1}{}&\rat(6/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 99
\orbit{3}{99}{141}
\h{99}&\rat(9/10){9}{}&\rat(81/10){3}{\spec{4}}&\int(3){2}{}&&\cnt{971}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(23/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(1/5){2}{}&\rat(23/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 100
\orbit{3}{100}{141}
\h{100}&\rat(21/10){7}{}&\rat(42/5){4}{\spec{2}}&\rat(3/2){1}{}&&\cnt{811}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\rat(9/5){6}{}&\rat(11/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(6/5){4}{}&\rat(14/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(7/5){8}{}&\rat(13/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(7/5){8}{}&\rat(13/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(3/5){2}{}&\rat(17/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(2/5){8}{}&\rat(18/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(7/10){9}{}&\rat(14/5){3}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(7/10){9}{}&\rat(14/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(3/10){1}{}&\rat(16/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(3/10){1}{}&\rat(11/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(-3/10){9}{}&\rat(14/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 101
\orbit{3}{101}{140}
\h{101}&\rat(21/10){7}{}&\rat(22/5){4}{\spec{1}}&\rat(11/2){1}{}&&\cnt{755}&\bounds{140}{140}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(11/10){7}{}&\rat(7/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(3/5){2}{}&\rat(7/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(7/10){9}{}&\rat(4/5){8}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(7/10){9}{}&\rat(4/5){8}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(3/10){1}{}&\rat(11/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(3/10){1}{}&\rat(6/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(-3/10){9}{}&\rat(9/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 102
\orbit{3}{102}{140}
\h{102}&\rat(9/10){9}{}&\rat(48/5){8}{\spec{4}}&\rat(3/2){1}{}&&\cnt{1035}&\bounds{140}{140}{1}{false}&&\cr
\l{1}&\rat(2/5){4}{}&\rat(18/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(13/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(18/5){8}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(1/10){1}{}&\rat(17/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\l{8}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(-1/10){9}{}&\rat(18/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 103
\orbit{3}{103}{140}
\h{103}&\rat(28/5){8}{\spec{1}}&\rat(22/5){6}{\spec{2}}&\int(2){\2}{}&&\cnt{751}&\bounds{140}{140}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(8/5){3}{}&\rat(7/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(13/5){8}{}&\rat(7/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(13/5){8}{}&\rat(7/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(13/5){8}{}&\rat(2/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(9/5){9}{}&\rat(11/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(9/5){9}{}&\rat(6/5){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(9/5){9}{}&\rat(6/5){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(9/5){9}{}&\rat(6/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{22}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(6/5){1}{}&\rat(9/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{24}&\rat(4/5){9}{}&\rat(11/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 104
\orbit{3}{104}{140}
\h{104}&\rat(29/10){9}{\spec{2}}&\rat(38/5){8}{\spec{1}}&\rat(3/2){1}{}&&\cnt{811}&\bounds{140}{140}{1}{false}&&\cr
\l{1}&\rat(8/5){6}{}&\rat(12/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(7/5){4}{}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\rat(17/10){7}{}&\rat(9/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(11/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(9/5){8}{}&\rat(11/5){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(6/5){2}{}&\rat(14/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(6/5){2}{}&\rat(9/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(4/5){8}{}&\rat(16/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(17/5){7}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(12/5){7}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(12/5){2}{\spec{2}}&\rat(1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(7/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(9/10){9}{}&\rat(13/5){3}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(8/5){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(9/10){9}{}&\rat(8/5){8}{\spec{3}}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\rat(1/10){1}{}&\rat(17/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\rat(1/10){1}{}&\rat(12/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(3){5}{\spec{2}}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 105
\orbit{3}{105}{139}
\h{105}&\rat(9/10){9}{}&\rat(81/10){3}{\spec{2}}&\int(3){2}{}&&\cnt{1179}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\rat(3/10){3}{}&\rat(27/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(27/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(-1/5){8}{}&\rat(27/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(1/10){1}{}&\rat(12/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 106
\orbit{3}{106}{139}
\h{106}&\rat(13/2){5}{\spec{1}}&\int(0){\0}{}&\rat(11/2){1}{}&&\cnt{923}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\rat(3/2){5}{\spec{1}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(3/2){5}{\spec{2}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(5/2){7}{}&\int(0){9}{}&\rat(3/2){2}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{2}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(3/2){9}{}&\int(0){8}{}&\rat(5/2){1}{}&\ln{2}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 107
\orbit{3}{107}{139}
\h{107}&\rat(8/5){8}{}&\rat(42/5){6}{\spec{3}}&\int(2){\2}{}&&\cnt{799}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\rat(4/5){4}{}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(4/5){9}{}&\rat(11/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(4/5){9}{}&\rat(16/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(1/5){1}{}&\rat(19/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(-1/5){9}{}&\rat(16/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(-4/5){1}{}&\rat(19/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 108
\orbit{3}{108}{139}
\h{108}&\rat(29/10){9}{\spec{2}}&\rat(41/10){3}{\spec{1}}&\int(5){2}{\spec{2}}&&\cnt{751}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(3/10){9}{}&\int(2){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(13/10){3}{}&\rat(7/10){1}{}&\int(2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(7/10){7}{\spec{1}}&\rat(13/10){9}{}&\int(2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(7/10){7}{\spec{2}}&\rat(13/10){9}{}&\int(2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(6/5){2}{}&\rat(13/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(9/10){7}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(9/10){7}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(9/10){9}{}&\rat(11/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{21}&\rat(1/10){1}{}&\rat(19/10){7}{}&\int(2){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{22}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 109
\orbit{3}{109}{139}
\h{109}&\int(6){\6}{\spec{1}}&\int(4){\4}{}&\int(2){\2}{}&&\cnt{807}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){7}{}&\int(1){9}{}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(1){1}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(2){2}{}&\int(2){4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(2){2}{}&\int(1){9}{}&\int(1){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(2){9}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(2){9}{}&\int(1){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(2){9}{}&\int(1){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\int(2){9}{}&\int(2){8}{}&\int(0){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(2){9}{}&\int(1){8}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{20}&\int(1){1}{}&\int(2){7}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(1){1}{}&\int(2){2}{}&\int(1){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 110
\orbit{3}{110}{139}
\h{110}&\rat(18/5){8}{\spec{2}}&\rat(32/5){6}{\spec{2}}&\int(2){\2}{}&&\cnt{695}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(6/5){6}{\spec{1}}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(6/5){6}{\spec{2}}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(8/5){3}{}&\rat(7/5){1}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(2/5){2}{\spec{1}}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(2/5){2}{\spec{2}}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(6/5){1}{}&\rat(14/5){2}{}&\int(0){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(6/5){1}{}&\rat(9/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(4/5){9}{}&\rat(16/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(4/5){9}{}&\rat(11/5){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(4/5){9}{}&\rat(11/5){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(1/5){1}{}&\rat(14/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(-1/5){9}{}&\rat(16/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 111
\orbit{3}{111}{139}
\h{111}&\rat(5/2){5}{}&\int(6){\6}{\spec{1}}&\rat(7/2){1}{}&&\cnt{807}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(3/2){7}{}&\int(2){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\int(1){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(1/2){7}{}&\int(2){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(1){2}{}&\int(2){9}{}&\int(1){3}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(0){2}{}&\int(2){9}{}&\int(2){3}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(1/2){9}{}&\int(2){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\rat(1/2){9}{}&\int(2){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{175}&\bounds{25}{25}{1}{false}&&\cr
\l{13}&\rat(1/2){1}{}&\int(2){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{14}&\rat(1/2){1}{}&\int(2){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 112
\orbit{3}{112}{138}
\h{112}&\rat(9/2){5}{\spec{1}}&\int(6){\6}{}&\rat(3/2){1}{}&&\cnt{699}&\bounds{138}{138}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(2){4}{}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(5/2){7}{}&\int(1){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(2){8}{}&\int(2){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(2){8}{}&\int(2){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(1){8}{\spec{1}}&\int(3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(1){8}{\spec{2}}&\int(3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(1){2}{}&\int(3){4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(3/2){9}{}&\int(3){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(3/2){9}{}&\int(2){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(3/2){9}{}&\int(2){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{16}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(1/2){9}{}&\int(3){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(1/2){9}{}&\int(2){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\rat(1/2){1}{}&\int(3){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(1/2){1}{}&\int(2){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 113
\orbit{3}{113}{138}
\h{113}&\rat(9/2){5}{\spec{1}}&\rat(9/2){5}{\spec{1}}&\int(3){2}{}&&\cnt{699}&\bounds{138}{138}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(5/2){7}{}&\rat(3/2){9}{}&\int(0){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(5/2){7}{}&\rat(1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(3/2){7}{\spec{1}}&\rat(3/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(3/2){7}{\spec{2}}&\rat(3/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\rat(1/2){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(1){8}{\spec{1}}&\int(3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(1){8}{\spec{2}}&\int(3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(1){2}{}&\rat(3/2){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(3/2){9}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(3/2){9}{}&\int(2){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{17}&\rat(3/2){9}{}&\int(1){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(3/2){9}{}&\int(1){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(1/2){9}{}&\int(2){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{20}&\rat(1/2){1}{}&\rat(5/2){7}{}&\int(1){2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 114
\orbit{3}{114}{138}
\h{114}&\rat(61/10){7}{\spec{1}}&\rat(22/5){4}{\spec{1}}&\rat(3/2){1}{}&&\cnt{755}&\bounds{138}{138}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(14/5){6}{}&\rat(6/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(11/5){4}{}&\rat(9/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(31/10){7}{}&\rat(7/5){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(31/10){7}{}&\rat(2/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(12/5){8}{}&\rat(8/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(12/5){8}{}&\rat(8/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(12/5){8}{}&\rat(3/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\rat(8/5){2}{}&\rat(7/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(7/5){8}{\spec{1}}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(7/5){8}{\spec{2}}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(17/10){9}{}&\rat(9/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{21}&\rat(17/10){9}{}&\rat(9/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(17/10){9}{}&\rat(4/5){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(17/10){9}{}&\rat(4/5){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\rat(13/10){1}{}&\rat(11/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\rat(13/10){1}{}&\rat(6/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 115
\orbit{3}{115}{137}
\h{115}&\rat(29/10){9}{\spec{2}}&\rat(81/10){3}{\spec{2}}&\int(1){2}{}&&\cnt{807}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\rat(8/5){6}{}&\rat(12/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(7/5){4}{}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(13/10){3}{}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(9/5){8}{}&\rat(11/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(9/5){8}{}&\rat(11/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(9/5){8}{}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(1/5){2}{\spec{1}}&\rat(19/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(1/5){2}{\spec{2}}&\rat(19/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(29/10){7}{}&\int(0){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(19/10){7}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(11/10){1}{}&\rat(19/10){7}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(11/10){1}{}&\rat(12/5){2}{\spec{2}}&\rat(1/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{3}}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{25}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 116
\orbit{3}{116}{137}
\h{116}&\rat(18/5){8}{\spec{1}}&\rat(22/5){6}{\spec{2}}&\int(4){\4}{2}&&\cnt{1059}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\rat(3/5){3}{}&\rat(7/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(9/5){9}{}&\rat(11/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(9/5){9}{}&\rat(1/5){3}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(9/5){9}{}&\rat(1/5){3}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(9/5){9}{}&\rat(6/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(-1/5){9}{}&\rat(11/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 117
\orbit{3}{117}{137}
\h{117}&\rat(29/10){9}{\spec{2}}&\rat(18/5){8}{\spec{2}}&\rat(11/2){1}{}&&\cnt{755}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(13/10){3}{}&\rat(6/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(6/5){2}{}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(4/5){8}{}&\rat(6/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(2/5){2}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(11/10){1}{}&\rat(2/5){2}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\rat(9/10){9}{}&\rat(8/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(1/10){1}{}&\rat(12/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 118
\orbit{3}{118}{137}
\h{118}&\rat(49/10){9}{\spec{2}}&\rat(61/10){3}{\spec{1}}&\int(1){2}{}&&\cnt{751}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(13/5){6}{}&\rat(7/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(13/5){6}{}&\rat(7/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(12/5){4}{}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(8/5){6}{\spec{1}}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(8/5){6}{\spec{2}}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(27/10){7}{}&\rat(13/10){9}{}&\int(0){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(27/10){7}{}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(23/10){3}{}&\rat(17/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(23/10){3}{}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(13/10){3}{\spec{1}}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(13/10){3}{\spec{2}}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(11/5){2}{}&\rat(9/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(11/5){2}{}&\rat(9/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(11/5){2}{}&\rat(13/10){9}{}&\rat(1/2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(9/5){8}{}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{24}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{26}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{27}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{28}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 119
\orbit{3}{119}{137}
\h{119}&\int(10){\10}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&&\cnt{903}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(4){5}{\spec{2}}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){5}{\spec{3}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){5}{\spec{4}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(4){6}{\spec{2}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\int(4){4}{\spec{2}}&\int(0){8}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\int(4){7}{}&\int(0){9}{}&\int(0){2}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(3){7}{\spec{2}}&\int(0){9}{}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(3){3}{\spec{2}}&\int(0){1}{}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{4}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 120
\orbit{3}{120}{137}
\h{120}&\int(4){\4}{}&\int(2){\2}{}&\int(6){\6}{\spec{1}}&&\cnt{807}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(2){7}{}&\int(1){9}{}&\int(1){2}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){7}{}&\int(0){9}{}&\int(2){2}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){7}{\spec{1}}&\int(1){9}{}&\int(2){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(1){7}{\spec{2}}&\int(1){9}{}&\int(2){2}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(1){9}{}&\int(1){3}{}&\int(2){2}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(1){9}{}&\int(1){8}{}&\int(2){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 121
\orbit{3}{121}{137}
\h{121}&\rat(49/10){9}{\spec{2}}&\rat(18/5){8}{\spec{2}}&\rat(7/2){1}{}&&\cnt{703}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(12/5){4}{}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(27/10){7}{}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(27/10){7}{}&\rat(-1/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(23/10){3}{}&\rat(6/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(23/10){3}{}&\rat(1/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(17/10){7}{}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(13/10){3}{\spec{1}}&\rat(6/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(13/10){3}{\spec{2}}&\rat(6/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(11/5){2}{}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(11/5){2}{}&\rat(-1/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(6/5){2}{}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(4/5){8}{}&\rat(6/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{25}&\rat(9/10){9}{}&\rat(8/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{26}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{27}&\rat(1/10){1}{}&\rat(12/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 122
\orbit{3}{122}{136}
\h{122}&\rat(29/10){9}{\spec{2}}&\rat(8/5){8}{}&\rat(15/2){1}{\spec{2}}&&\cnt{971}&\bounds{136}{136}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(-1/5){9}{}&\rat(5/2){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(13/10){3}{}&\rat(1/5){1}{}&\rat(5/2){2}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\rat(7/10){7}{\spec{1}}&\rat(4/5){9}{}&\rat(5/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(7/10){7}{\spec{2}}&\rat(4/5){9}{}&\rat(5/2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(6/5){2}{}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(11/10){1}{}&\rat(2/5){7}{}&\rat(5/2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(11/10){1}{}&\rat(2/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(9/10){9}{}&\rat(3/5){3}{}&\rat(5/2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(1/10){1}{}&\rat(7/5){7}{}&\rat(5/2){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{17}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 123
\orbit{3}{123}{136}
\h{123}&\rat(61/10){7}{\spec{2}}&\rat(12/5){4}{}&\rat(7/2){1}{}&&\cnt{699}&\bounds{136}{136}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(16/5){4}{}&\rat(4/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(14/5){6}{}&\rat(6/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(29/10){3}{}&\rat(3/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(29/10){3}{}&\rat(-2/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(19/10){3}{\spec{1}}&\rat(3/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(19/10){3}{\spec{2}}&\rat(3/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(13/5){2}{}&\rat(7/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(13/5){2}{}&\rat(2/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(13/5){2}{}&\rat(-3/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(8/5){2}{}&\rat(2/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(13/10){1}{}&\rat(6/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(13/10){1}{}&\rat(6/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 124
\orbit{3}{124}{136}
\h{124}&\rat(8/5){8}{}&\rat(22/5){6}{\spec{2}}&\int(6){\6}{\spec{1}}&&\cnt{807}&\bounds{136}{136}{1}{false}&&\cr
\l{1}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(3/5){3}{}&\rat(7/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(3/5){8}{}&\rat(7/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(4/5){9}{}&\rat(11/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(4/5){9}{}&\rat(6/5){3}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(6/5){3}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(4/5){9}{}&\rat(6/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(1/5){1}{}&\rat(9/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(-1/5){9}{}&\rat(11/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 125
\orbit{3}{125}{135}
\h{125}&\rat(49/10){9}{\spec{2}}&\rat(61/10){3}{\spec{2}}&\int(1){2}{}&&\cnt{695}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(12/5){4}{}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(7/5){4}{\spec{1}}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(7/5){4}{\spec{2}}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(27/10){7}{}&\rat(13/10){9}{}&\int(0){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(27/10){7}{}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(23/10){3}{}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{}&\rat(13/10){9}{}&\rat(1/2){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(9/5){8}{}&\rat(11/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(9/5){8}{}&\rat(11/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(29/10){7}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(11/10){1}{}&\rat(19/10){7}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(11/10){1}{}&\rat(19/10){7}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 126
\orbit{3}{126}{135}
\h{126}&\rat(69/10){9}{\spec{2}}&\rat(18/5){8}{\spec{2}}&\rat(3/2){1}{}&&\cnt{699}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(18/5){6}{}&\rat(2/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(18/5){6}{}&\rat(2/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(17/5){4}{}&\rat(3/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(12/5){4}{\spec{1}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(12/5){4}{\spec{2}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\rat(33/10){3}{}&\rat(6/5){1}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(33/10){3}{}&\rat(1/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(27/10){7}{}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(23/10){3}{}&\rat(6/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{16}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(11/5){2}{}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{18}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 127
\orbit{3}{127}{135}
\h{127}&\rat(5/2){5}{}&\int(8){\8}{}&\rat(3/2){1}{}&&\cnt{695}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(1){8}{}&\int(3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(0){8}{}&\int(4){6}{}&\int(0){\0}{}&\ln{2}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(1/2){9}{}&\int(3){3}{}&\rat(1/2){2}{}&\ln{2}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(1/2){9}{}&\int(2){8}{}&\rat(3/2){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(3){5}{\spec{1}}&\int(1){3}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 128
\orbit{3}{128}{135}
\h{128}&\rat(28/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(4){\4}{2}&&\cnt{687}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(16/5){6}{}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(14/5){4}{}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(13/5){3}{}&\rat(-3/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(12/5){7}{}&\rat(-2/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(8/5){3}{\spec{1}}&\rat(2/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(8/5){3}{\spec{2}}&\rat(2/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(12/5){2}{}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(12/5){2}{}&\rat(3/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(6/5){1}{}&\rat(4/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(4/5){9}{}&\rat(6/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 129
\orbit{3}{129}{135}
\h{129}&\rat(9/10){9}{}&\rat(101/10){3}{\spec{2}}&\int(1){2}{}&&\cnt{1035}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\rat(3/5){6}{}&\rat(17/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(1/5){2}{}&\rat(19/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(41/10){3}{}&\int(-1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(1/10){1}{}&\rat(17/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(41/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 130
\orbit{3}{130}{135}
\h{130}&\rat(9/10){9}{}&\rat(28/5){8}{\spec{2}}&\rat(11/2){1}{}&&\cnt{743}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(6/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(13/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(8/5){3}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(8/5){3}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(1/10){1}{}&\rat(12/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(13/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(-9/10){1}{}&\rat(12/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){5}{\spec{1}}&\int(2){3}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){5}{\spec{2}}&\int(2){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 131
\orbit{3}{131}{135}
\h{131}&\rat(49/10){9}{\spec{1}}&\rat(21/10){3}{}&\int(5){2}{\spec{2}}&&\cnt{923}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\rat(17/10){7}{}&\rat(3/10){9}{}&\int(2){2}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\rat(13/10){3}{}&\rat(7/10){1}{}&\int(2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(19/10){9}{}&\rat(11/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(19/10){9}{}&\rat(1/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(19/10){9}{}&\rat(3/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{13}&\rat(11/10){1}{}&\rat(9/10){7}{}&\int(2){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 132
\orbit{3}{132}{135}
\h{132}&\rat(8/5){8}{}&\rat(42/5){6}{\spec{2}}&\int(2){\2}{}&&\cnt{935}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(7/5){1}{\spec{1}}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(2/5){2}{}&\rat(18/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\rat(4/5){9}{}&\rat(21/5){3}{}&\int(-1){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(4/5){9}{}&\rat(11/5){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(1/5){1}{}&\rat(14/5){2}{\spec{1}}&\int(1){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(-1/5){9}{}&\rat(21/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(3){5}{\spec{1}}&\int(1){3}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 133
\orbit{3}{133}{135}
\h{133}&\rat(18/5){8}{\spec{1}}&\rat(42/5){6}{\spec{1}}&\int(0){\0}{}&&\cnt{999}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{288}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\rat(2/5){2}{}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(9/5){9}{}&\rat(11/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 134
\orbit{3}{134}{135}
\h{134}&\rat(8/5){8}{}&\rat(52/5){6}{\spec{4}}&\int(0){\0}{}&&\cnt{863}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\rat(4/5){4}{}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\rat(7/5){7}{}&\rat(13/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(4/5){9}{}&\rat(16/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(1/5){1}{}&\rat(19/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 135
\orbit{3}{135}{135}
\h{135}&\rat(29/10){9}{\spec{2}}&\rat(61/10){3}{\spec{2}}&\int(3){2}{}&&\cnt{699}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\rat(7/5){4}{}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(9/5){8}{}&\rat(11/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(9/5){8}{}&\rat(11/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(6/5){2}{}&\rat(13/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(11/10){1}{}&\rat(29/10){7}{}&\int(0){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(11/10){1}{}&\rat(19/10){7}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(11/10){1}{}&\rat(19/10){7}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 136
\orbit{3}{136}{135}
\h{136}&\int(4){\4}{}&\int(4){\4}{}&\int(4){\4}{2}&&\cnt{687}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{4}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){7}{}&\int(0){9}{}&\int(2){2}{}&\ln{4}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){7}{\spec{1}}&\int(1){9}{}&\int(2){2}{}&\ln{4}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(1){7}{\spec{2}}&\int(1){9}{}&\int(2){2}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{4}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 137
\orbit{3}{137}{135}
\h{137}&\rat(18/5){8}{\spec{2}}&\rat(42/5){6}{\spec{3}}&\int(0){\0}{}&&\cnt{791}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(9/5){4}{}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(4/5){4}{\spec{1}}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(4/5){4}{\spec{2}}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(4/5){9}{}&\rat(16/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(1/5){1}{}&\rat(19/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 138
\orbit{3}{138}{135}
\h{138}&\rat(28/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(4){\4}{}&&\cnt{751}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(13/5){8}{}&\rat(7/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(13/5){8}{}&\rat(2/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(13/5){8}{}&\rat(-3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(7/5){2}{}&\rat(3/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(9/5){9}{}&\rat(6/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(9/5){9}{}&\rat(6/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(9/5){9}{}&\rat(1/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(6/5){1}{}&\rat(4/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(4/5){9}{}&\rat(6/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 139
\orbit{3}{139}{135}
\h{139}&\rat(21/10){7}{}&\rat(32/5){4}{\spec{1}}&\rat(7/2){1}{}&&\cnt{755}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\rat(9/5){6}{}&\rat(11/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(11/10){7}{}&\rat(7/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(9/10){3}{}&\rat(8/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(3/5){2}{}&\rat(17/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(3/5){2}{}&\rat(7/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(2/5){8}{}&\rat(8/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(7/10){9}{}&\rat(9/5){3}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(7/10){9}{}&\rat(9/5){3}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{17}&\rat(3/10){1}{}&\rat(11/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(3/10){1}{}&\rat(11/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{19}&\rat(-3/10){9}{}&\rat(14/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){5}{\spec{1}}&\int(2){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){5}{\spec{2}}&\int(2){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 140
\orbit{3}{140}{134}
\h{140}&\rat(18/5){8}{\spec{1}}&\rat(42/5){6}{\spec{4}}&\int(0){\0}{}&&\cnt{1103}&\bounds{134}{134}{1}{false}&&\cr
\l{1}&\rat(4/5){4}{}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(7/5){7}{}&\rat(13/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{432}&\bounds{48}{48}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\rat(9/5){9}{}&\rat(11/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 141
\orbit{3}{141}{134}
\h{141}&\rat(29/10){9}{\spec{2}}&\rat(61/10){3}{\spec{1}}&\int(3){2}{}&&\cnt{755}&\bounds{134}{134}{1}{false}&&\cr
\l{1}&\rat(8/5){6}{}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(13/10){3}{}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(9/5){8}{}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(6/5){2}{}&\rat(13/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(4/5){8}{}&\rat(17/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(7/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(11/10){1}{}&\rat(7/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 142
\orbit{3}{142}{133}
\h{142}&\rat(9/10){9}{}&\rat(61/10){3}{\spec{1}}&\int(5){2}{\spec{2}}&&\cnt{923}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(13/10){9}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(3/10){3}{}&\rat(17/10){1}{}&\int(2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(4/5){8}{}&\rat(17/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(11/10){3}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(11/10){3}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(9/10){9}{}&\rat(11/10){3}{\spec{3}}&\int(2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(1/10){1}{}&\rat(19/10){7}{}&\int(2){2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(1){\2}{\spec{3}}&\int(3){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 143
\orbit{3}{143}{133}
\h{143}&\int(4){\4}{}&\int(2){\2}{}&\int(6){\6}{3}&&\cnt{811}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(2){7}{}&\int(1){9}{}&\int(1){2}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){8}{}&\int(-1){1}{}&\int(3){3}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(1){8}{}&\int(0){1}{}&\int(3){3}{}&\ln{2}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(0){8}{\spec{1}}&\int(1){1}{}&\int(3){3}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(0){8}{\spec{2}}&\int(1){1}{}&\int(3){3}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(1){9}{}&\int(1){8}{}&\int(2){1}{}&\ln{2}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(1){5}{}&\int(3){3}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 144
\orbit{3}{144}{133}
\h{144}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{903}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(4){5}{\spec{2}}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(4){6}{\spec{2}}&\int(0){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(4){6}{\spec{2}}&\int(0){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(4){4}{\spec{2}}&\int(0){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(4){4}{\spec{2}}&\int(0){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(3){6}{\spec{3}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(3){4}{\spec{3}}&\int(1){8}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(4){7}{}&\int(0){9}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(3){7}{\spec{2}}&\int(1){9}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(3){3}{\spec{2}}&\int(1){1}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(3){8}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{20}&\int(3){8}{}&\int(1){1}{}&\int(0){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 145
\orbit{3}{145}{133}
\h{145}&\int(6){\6}{\spec{1}}&\int(6){\6}{}&\int(0){\0}{}&&\cnt{791}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(2){8}{}&\int(2){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(2){8}{}&\int(2){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(2){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(2){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(1){8}{}&\int(3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(1){2}{}&\int(3){4}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(2){9}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{14}&\int(2){9}{}&\int(2){8}{}&\int(0){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\int(1){1}{}&\int(3){7}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 146
\orbit{3}{146}{133}
\h{146}&\rat(9/10){9}{}&\rat(18/5){8}{\spec{2}}&\rat(15/2){1}{\spec{2}}&&\cnt{967}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(4/5){9}{}&\rat(5/2){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(3/10){3}{}&\rat(6/5){1}{}&\rat(5/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(4/5){8}{}&\rat(6/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(3/5){3}{\spec{1}}&\rat(5/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(3/5){3}{\spec{2}}&\rat(5/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(1/10){1}{}&\rat(7/5){7}{}&\rat(5/2){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(-1/10){9}{}&\rat(8/5){3}{}&\rat(5/2){2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(-9/10){1}{}&\rat(12/5){7}{}&\rat(5/2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 147
\orbit{3}{147}{133}
\h{147}&\rat(9/2){5}{\spec{1}}&\rat(5/2){5}{}&\int(5){2}{\spec{1}}&&\cnt{695}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(5/2){7}{}&\rat(1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){8}{}&\rat(1/2){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\int(2){8}{}&\rat(-1/2){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(1){8}{\spec{1}}&\rat(1/2){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(1){8}{\spec{2}}&\rat(1/2){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\int(1){2}{}&\rat(1/2){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(3/2){9}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(3/2){9}{}&\int(0){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(1/2){9}{}&\int(1){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(1/2){1}{}&\int(1){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(3/2){5}{}&\rat(5/2){3}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 148
\orbit{3}{148}{133}
\h{148}&\rat(8/5){8}{}&\rat(32/5){6}{\spec{2}}&\int(4){\4}{2}&&\cnt{935}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(3/5){3}{}&\rat(7/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(2/5){2}{}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(4/5){9}{}&\rat(16/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(4/5){9}{}&\rat(6/5){3}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(1/5){1}{}&\rat(14/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(-1/5){9}{}&\rat(11/5){3}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(-1/5){9}{}&\rat(11/5){3}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{\spec{1}}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 149
\orbit{3}{149}{133}
\h{149}&\rat(69/10){9}{\spec{1}}&\rat(8/5){8}{}&\rat(7/2){1}{}&&\cnt{859}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(12/5){4}{\spec{1}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(27/10){7}{\spec{1}}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(27/10){7}{\spec{1}}&\rat(-1/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(23/10){3}{\spec{1}}&\rat(1/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(17/10){7}{\spec{1}}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{\spec{1}}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\rat(11/5){2}{\spec{1}}&\rat(-1/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(9/5){8}{\spec{1}}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(6/5){2}{\spec{1}}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(21/10){1}{}&\rat(7/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\rat(21/10){1}{}&\rat(2/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(21/10){1}{}&\rat(2/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{19}&\rat(9/10){9}{\spec{1}}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 150
\orbit{3}{150}{133}
\h{150}&\rat(81/10){7}{\spec{3}}&\rat(12/5){4}{}&\rat(3/2){1}{}&&\cnt{799}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(14/5){6}{}&\rat(6/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\rat(31/10){7}{}&\rat(2/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(17/5){8}{}&\rat(3/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(17/5){8}{}&\rat(3/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(17/5){8}{}&\rat(-2/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(17/10){9}{}&\rat(9/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(17/10){9}{}&\rat(4/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(13/10){1}{}&\rat(6/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 151
\orbit{3}{151}{133}
\h{151}&\rat(9/10){9}{}&\rat(48/5){8}{\spec{1}}&\rat(3/2){1}{}&&\cnt{967}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\rat(3/5){6}{}&\rat(17/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(4/5){8}{}&\rat(11/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(1/5){2}{}&\rat(19/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(18/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(13/5){3}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(13/5){3}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(17/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(18/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(-9/10){1}{}&\rat(17/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 152
\orbit{3}{152}{133}
\h{152}&\rat(8/5){8}{}&\rat(32/5){6}{\spec{2}}&\int(4){\4}{}&&\cnt{935}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\rat(4/5){4}{}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(2/5){1}{\spec{2}}&\int(2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(2/5){2}{}&\rat(8/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(4/5){9}{}&\rat(16/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(4/5){9}{}&\rat(6/5){8}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\rat(-1/5){9}{}&\rat(16/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){5}{\spec{2}}&\int(2){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 153
\orbit{3}{153}{133}
\h{153}&\rat(29/10){9}{\spec{2}}&\rat(28/5){8}{\spec{2}}&\rat(7/2){1}{}&&\cnt{699}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\rat(8/5){6}{}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(13/10){3}{}&\rat(6/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(6/5){2}{}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(4/5){8}{}&\rat(6/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(9/10){9}{}&\rat(13/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(9/10){9}{}&\rat(8/5){3}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(8/5){3}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(1/10){1}{}&\rat(12/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{24}&\rat(-1/10){9}{}&\rat(13/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){5}{\spec{1}}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(2){5}{\spec{2}}&\int(2){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 154
\orbit{3}{154}{133}
\h{154}&\rat(61/10){7}{\spec{2}}&\rat(22/5){4}{\spec{1}}&\rat(3/2){1}{}&&\cnt{699}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(16/5){4}{}&\rat(4/5){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(16/5){4}{}&\rat(4/5){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(14/5){6}{}&\rat(6/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(11/5){4}{\spec{1}}&\rat(9/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(11/5){4}{\spec{2}}&\rat(9/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(29/10){3}{}&\rat(3/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(13/5){2}{}&\rat(7/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(13/5){2}{}&\rat(7/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(13/5){2}{}&\rat(2/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(8/5){2}{}&\rat(7/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(13/10){1}{}&\rat(11/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(13/10){1}{}&\rat(6/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 155
\orbit{3}{155}{132}
\h{155}&\rat(29/10){9}{\spec{2}}&\rat(8/5){8}{}&\rat(15/2){1}{\spec{1}}&&\cnt{859}&\bounds{132}{132}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(-4/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(6/5){2}{}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(6/5){2}{}&\rat(-1/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(4/5){8}{}&\rat(1/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\rat(1/5){2}{\spec{1}}&\rat(4/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(1/5){2}{\spec{2}}&\rat(4/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(2/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(1){5}{}&\int(3){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 156
\orbit{3}{156}{132}
\h{156}&\rat(8/5){8}{}&\rat(32/5){6}{\spec{1}}&\int(4){\4}{}&&\cnt{751}&\bounds{132}{132}{1}{false}&&\cr
\l{1}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(3/5){8}{}&\rat(7/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(2/5){2}{}&\rat(8/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(4/5){9}{}&\rat(11/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(4/5){9}{}&\rat(6/5){8}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(4/5){9}{}&\rat(6/5){8}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(1/5){1}{}&\rat(9/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(-1/5){9}{}&\rat(11/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){5}{\spec{1}}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){5}{\spec{2}}&\int(2){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 157
\orbit{3}{157}{132}
\h{157}&\rat(8/5){8}{}&\rat(22/5){6}{\spec{1}}&\int(6){\6}{1}&&\cnt{935}&\bounds{132}{132}{1}{false}&&\cr
\l{1}&\int(1){5}{}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(2/5){2}{}&\rat(8/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(4/5){9}{}&\rat(1/5){8}{}&\int(3){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(1/5){1}{}&\rat(4/5){2}{}&\int(3){1}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{10}&\rat(-1/5){9}{}&\rat(6/5){8}{\spec{1}}&\int(3){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(-1/5){9}{}&\rat(6/5){8}{\spec{2}}&\int(3){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 158
\orbit{3}{158}{132}
\h{158}&\rat(9/2){5}{\spec{1}}&\int(6){\6}{\spec{1}}&\rat(3/2){1}{}&&\cnt{803}&\bounds{132}{132}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){4}{}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(5/2){7}{}&\int(2){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(3/2){7}{\spec{1}}&\int(2){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(3/2){7}{\spec{2}}&\int(2){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{12}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(1){2}{}&\int(2){9}{}&\int(1){3}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{14}&\rat(3/2){9}{}&\int(2){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(3/2){9}{}&\int(2){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(1/2){9}{}&\int(2){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(1/2){1}{}&\int(2){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 159
\orbit{3}{159}{131}
\h{159}&\rat(49/10){9}{\spec{1}}&\rat(8/5){8}{}&\rat(11/2){1}{}&&\cnt{923}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\rat(6/5){2}{}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(19/10){9}{}&\rat(3/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(19/10){9}{}&\rat(3/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(19/10){9}{}&\rat(-2/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(2/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 160
\orbit{3}{160}{131}
\h{160}&\rat(9/10){9}{}&\rat(101/10){3}{\spec{5}}&\int(1){2}{}&&\cnt{1015}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(2/5){4}{}&\rat(18/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(7/10){7}{}&\rat(23/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(-1/5){8}{}&\rat(21/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(18/5){8}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(1/10){1}{}&\rat(39/10){7}{}&\int(0){2}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(29/10){7}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(1/10){1}{}&\rat(29/10){7}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(18/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(-9/10){1}{}&\rat(39/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 161
\orbit{3}{161}{131}
\h{161}&\int(6){\6}{}&\int(2){\2}{}&\int(4){\4}{2}&&\cnt{811}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){7}{}&\int(1){9}{}&\int(0){2}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){7}{}&\int(-1){9}{}&\int(2){2}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){7}{}&\int(0){9}{}&\int(2){2}{}&\ln{2}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(1){7}{\spec{1}}&\int(1){9}{}&\int(2){2}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(1){7}{\spec{2}}&\int(1){9}{}&\int(2){2}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(1){9}{}&\int(1){3}{}&\int(2){2}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 162
\orbit{3}{162}{131}
\h{162}&\rat(9/10){9}{}&\rat(38/5){8}{\spec{1}}&\rat(7/2){1}{}&&\cnt{911}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(3/10){3}{}&\rat(11/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(16/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(4/5){8}{}&\rat(11/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(-1/5){8}{}&\rat(11/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(13/5){3}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){3}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(8/5){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(1/10){1}{}&\rat(12/5){7}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(12/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{11}&\rat(-1/10){9}{}&\rat(13/5){3}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){5}{\spec{1}}&\int(1){3}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){5}{\spec{1}}&\int(2){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 163
\orbit{3}{163}{131}
\h{163}&\rat(49/10){9}{\spec{1}}&\rat(61/10){3}{\spec{1}}&\int(1){2}{}&&\cnt{923}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(8/5){6}{}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(13/10){3}{}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(9/5){8}{}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(19/10){9}{}&\rat(31/10){3}{}&\int(-1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{16}&\rat(19/10){9}{}&\rat(11/10){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(19/10){9}{}&\rat(11/10){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(19/10){9}{}&\rat(11/10){3}{\spec{3}}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 164
\orbit{3}{164}{131}
\h{164}&\rat(18/5){8}{\spec{1}}&\rat(32/5){6}{\spec{2}}&\int(2){\2}{}&&\cnt{935}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(2/5){2}{}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(9/5){9}{}&\rat(16/5){3}{}&\int(-1){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(9/5){9}{}&\rat(11/5){3}{\spec{1}}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(9/5){9}{}&\rat(11/5){3}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(9/5){9}{}&\rat(6/5){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(9/5){9}{}&\rat(6/5){8}{\spec{1}}&\int(1){1}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\rat(1/5){1}{}&\rat(14/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(-1/5){9}{}&\rat(16/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 165
\orbit{3}{165}{131}
\h{165}&\rat(38/5){8}{\spec{2}}&\rat(22/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{679}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){5}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(19/5){4}{}&\rat(1/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(16/5){6}{}&\rat(4/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(16/5){6}{}&\rat(4/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(14/5){4}{\spec{1}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(14/5){4}{\spec{2}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(18/5){3}{}&\rat(2/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(13/5){3}{}&\rat(7/5){1}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(12/5){2}{}&\rat(8/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(12/5){2}{}&\rat(8/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 166
\orbit{3}{166}{131}
\h{166}&\rat(9/2){5}{\spec{1}}&\int(4){\4}{}&\rat(7/2){1}{}&&\cnt{699}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){4}{}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(5/2){7}{}&\int(1){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(5/2){7}{}&\int(0){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(3/2){7}{\spec{1}}&\int(1){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(3/2){7}{\spec{2}}&\int(1){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\int(1){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(1){8}{\spec{1}}&\int(1){1}{}&\int(2){3}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(1){8}{\spec{2}}&\int(1){1}{}&\int(2){3}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(1){2}{}&\int(1){9}{}&\int(2){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(3/2){9}{}&\int(2){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{19}&\rat(3/2){9}{}&\int(1){3}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(3/2){9}{}&\int(1){3}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(3/2){9}{}&\int(2){8}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(3/2){9}{}&\int(2){8}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{24}&\rat(1/2){9}{}&\int(2){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\rat(1/2){9}{}&\int(2){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{26}&\rat(1/2){1}{}&\int(2){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{27}&\rat(1/2){1}{}&\int(2){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 167
\orbit{3}{167}{131}
\h{167}&\rat(49/10){9}{\spec{2}}&\rat(8/5){8}{}&\rat(11/2){1}{}&&\cnt{751}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(3/2){5}{\spec{1}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(3/2){5}{\spec{2}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(12/5){4}{}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(27/10){7}{}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(27/10){7}{}&\rat(-1/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(23/10){3}{}&\rat(1/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(17/10){7}{}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(11/5){2}{}&\rat(4/5){9}{}&\int(1){3}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(11/5){2}{}&\rat(4/5){9}{}&\int(1){3}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(11/5){2}{}&\rat(-1/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(6/5){2}{}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{18}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(11/10){1}{}&\rat(2/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 168
\orbit{3}{168}{130}
\h{168}&\rat(9/2){5}{\spec{1}}&\int(6){\6}{\spec{2}}&\rat(3/2){1}{}&&\cnt{803}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(2){4}{}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(5/2){7}{}&\int(1){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(3/2){3}{}&\int(2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(2){1}{}&\int(0){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(1){8}{\spec{1}}&\int(2){1}{}&\int(1){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(1){8}{\spec{2}}&\int(2){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(3/2){9}{}&\int(2){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{15}&\rat(3/2){9}{}&\int(2){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(1/2){9}{}&\int(2){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(1/2){1}{}&\int(2){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 169
\orbit{3}{169}{130}
\h{169}&\rat(49/10){9}{\spec{1}}&\rat(28/5){8}{\spec{1}}&\rat(3/2){1}{}&&\cnt{923}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\rat(7/5){4}{}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(9/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{11}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(6/5){2}{}&\rat(9/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(19/10){9}{}&\rat(8/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(19/10){9}{}&\rat(13/5){8}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\rat(19/10){9}{}&\rat(3/5){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(19/10){9}{}&\rat(3/5){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 170
\orbit{3}{170}{130}
\h{170}&\rat(69/10){9}{\spec{1}}&\rat(41/10){3}{\spec{2}}&\int(1){2}{}&&\cnt{847}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(13/5){6}{\spec{1}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(8/5){6}{\spec{1}}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(27/10){7}{\spec{1}}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(23/10){3}{\spec{1}}&\rat(17/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\rat(23/10){3}{\spec{1}}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(13/10){3}{\spec{1}}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{\spec{1}}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{13}&\rat(9/5){8}{\spec{1}}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(21/10){1}{}&\rat(9/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(21/10){1}{}&\rat(12/5){2}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(21/10){1}{}&\rat(7/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{17}&\rat(9/10){9}{\spec{1}}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 171
\orbit{3}{171}{130}
\h{171}&\rat(9/10){9}{}&\rat(41/10){3}{\spec{1}}&\int(7){2}{}&&\cnt{859}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(13/10){9}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(7/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(1/5){2}{}&\rat(13/10){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(11/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(3/5){8}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(3/5){8}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(19/10){7}{}&\int(2){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\rat(3/2){5}{\spec{1}}&\rat(5/2){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(3/2){5}{\spec{2}}&\rat(5/2){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 172
\orbit{3}{172}{129}
\h{172}&\rat(21/10){7}{}&\rat(42/5){4}{\spec{1}}&\rat(3/2){1}{}&&\cnt{803}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\rat(9/5){6}{}&\rat(11/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(4/5){6}{}&\rat(16/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(3/5){2}{}&\rat(17/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(7/10){9}{}&\rat(19/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(3/10){1}{}&\rat(16/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(3/10){1}{}&\rat(11/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(-3/10){9}{}&\rat(19/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(-7/10){1}{}&\rat(16/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 173
\orbit{3}{173}{129}
\h{173}&\rat(29/10){9}{\spec{2}}&\rat(81/10){3}{\spec{3}}&\int(1){2}{}&&\cnt{811}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\rat(7/5){4}{}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(-1/5){8}{\spec{1}}&\rat(21/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(-1/5){8}{\spec{2}}&\rat(21/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(11/10){1}{}&\rat(39/10){7}{}&\int(-1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(11/10){1}{}&\rat(29/10){7}{}&\int(0){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(1/10){1}{}&\rat(39/10){7}{}&\int(0){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(-9/10){1}{}&\rat(39/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 174
\orbit{3}{174}{129}
\h{174}&\rat(18/5){8}{\spec{1}}&\rat(22/5){6}{\spec{1}}&\int(4){\4}{}&&\cnt{935}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\rat(2/5){2}{}&\rat(8/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(9/5){9}{}&\rat(6/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{8}&\rat(9/5){9}{}&\rat(11/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(9/5){9}{}&\rat(6/5){8}{\spec{1}}&\int(1){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(9/5){9}{}&\rat(6/5){8}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(9/5){9}{}&\rat(1/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(-1/5){9}{}&\rat(11/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 175
\orbit{3}{175}{129}
\h{175}&\int(8){\8}{\spec{1}}&\int(0){\0}{}&\int(4){\4}{2}&&\cnt{1147}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){7}{}&\int(0){9}{}&\int(2){2}{}&\ln{2}&\cnt{280}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(2){9}{}&\int(0){3}{}&\int(2){2}{}&\ln{2}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 176
\orbit{3}{176}{129}
\h{176}&\rat(9/10){9}{}&\rat(28/5){8}{\spec{1}}&\rat(11/2){1}{}&&\cnt{923}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(9/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(4/5){8}{}&\rat(6/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(1/5){2}{}&\rat(9/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(8/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(9/10){9}{}&\rat(3/5){8}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(9/10){9}{}&\rat(3/5){8}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(1/10){1}{}&\rat(12/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{13}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{14}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(1){\2}{\spec{3}}&\int(3){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 177
\orbit{3}{177}{129}
\h{177}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{999}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{7}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(4){5}{\spec{2}}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(4){6}{\spec{2}}&\int(0){2}{}&\int(0){\0}{}&\ln{2}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(4){7}{}&\int(0){9}{}&\int(0){2}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 178
\orbit{3}{178}{129}
\h{178}&\rat(18/5){8}{\spec{2}}&\rat(22/5){6}{\spec{1}}&\int(4){\4}{2}&&\cnt{811}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\rat(9/5){4}{}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(12/5){7}{}&\rat(-2/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/5){3}{}&\rat(2/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(2/5){7}{\spec{1}}&\rat(8/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(2/5){7}{\spec{2}}&\rat(8/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(7/5){2}{}&\rat(8/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(6/5){1}{}&\rat(4/5){7}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(6/5){1}{}&\rat(4/5){7}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(4/5){9}{}&\rat(6/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{16}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(-4/5){1}{}&\rat(14/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 179
\orbit{3}{179}{129}
\h{179}&\rat(13/2){5}{\spec{1}}&\int(2){\2}{}&\rat(7/2){1}{}&&\cnt{751}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(5/2){7}{}&\int(1){9}{}&\rat(1/2){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(5/2){7}{}&\int(0){9}{}&\rat(3/2){2}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(3/2){7}{\spec{1}}&\int(1){9}{}&\rat(3/2){2}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(3/2){7}{\spec{2}}&\int(1){9}{}&\rat(3/2){2}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(1){8}{\spec{1}}&\int(1){1}{}&\int(2){3}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(1){8}{\spec{2}}&\int(1){1}{}&\int(2){3}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(3/2){9}{}&\int(1){3}{}&\rat(3/2){2}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{2}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 180
\orbit{3}{180}{128}
\h{180}&\rat(49/10){9}{\spec{1}}&\rat(41/10){3}{\spec{1}}&\int(3){2}{}&&\cnt{747}&\bounds{128}{128}{1}{false}&&\cr
\l{1}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(6/5){2}{}&\rat(13/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(19/10){9}{}&\rat(11/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(19/10){9}{}&\rat(3/5){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(19/10){9}{}&\rat(3/5){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 181
\orbit{3}{181}{127}
\h{181}&\rat(69/10){9}{\spec{2}}&\rat(41/10){3}{\spec{2}}&\int(1){2}{}&&\cnt{811}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(18/5){6}{}&\rat(2/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(17/5){4}{}&\rat(3/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(8/5){6}{\spec{1}}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(8/5){6}{\spec{2}}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(33/10){3}{}&\rat(17/10){1}{}&\int(-1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(33/10){3}{}&\rat(7/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(33/10){3}{}&\rat(-3/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(27/10){7}{}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(23/10){3}{}&\rat(17/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(23/10){3}{}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(13/10){3}{\spec{1}}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(13/10){3}{\spec{2}}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(9/5){8}{}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 182
\orbit{3}{182}{127}
\h{182}&\rat(41/10){7}{\spec{1}}&\rat(32/5){4}{\spec{2}}&\rat(3/2){1}{}&&\cnt{811}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\rat(6/5){4}{}&\rat(14/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(12/5){8}{}&\rat(8/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(12/5){8}{}&\rat(8/5){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(12/5){8}{}&\rat(3/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(2/5){8}{}&\rat(18/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(17/10){9}{}&\rat(9/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(17/10){9}{}&\rat(14/5){8}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(17/10){9}{}&\rat(9/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(17/10){9}{}&\rat(4/5){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(17/10){9}{}&\rat(4/5){8}{\spec{3}}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(7/10){9}{}&\rat(14/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(3/10){1}{}&\rat(16/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(-3/10){9}{}&\rat(14/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 183
\orbit{3}{183}{127}
\h{183}&\rat(41/10){7}{\spec{2}}&\rat(32/5){4}{\spec{2}}&\rat(3/2){1}{}&&\cnt{695}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(14/5){6}{}&\rat(6/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(11/5){4}{}&\rat(9/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(6/5){4}{\spec{1}}&\rat(14/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(6/5){4}{\spec{2}}&\rat(14/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(8/5){2}{}&\rat(12/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(8/5){2}{}&\rat(7/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(2/5){8}{}&\rat(18/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(13/10){1}{}&\rat(16/5){7}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(13/10){1}{}&\rat(11/5){7}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(13/10){1}{}&\rat(11/5){7}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(13/10){1}{}&\rat(6/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(7/10){9}{}&\rat(14/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(3/10){1}{}&\rat(16/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\rat(-3/10){9}{}&\rat(14/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 184
\orbit{3}{184}{127}
\h{184}&\rat(61/10){7}{\spec{1}}&\rat(22/5){4}{\spec{2}}&\rat(3/2){1}{}&&\cnt{747}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(14/5){6}{}&\rat(6/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(14/5){6}{}&\rat(6/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(9/5){6}{\spec{1}}&\rat(11/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(9/5){6}{\spec{2}}&\rat(11/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(31/10){7}{}&\rat(2/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(19/10){3}{}&\rat(8/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(12/5){8}{}&\rat(8/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{15}&\rat(12/5){8}{}&\rat(8/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(12/5){8}{}&\rat(3/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(7/5){8}{\spec{1}}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(7/5){8}{\spec{2}}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(17/10){9}{}&\rat(14/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(17/10){9}{}&\rat(9/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(17/10){9}{}&\rat(4/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\rat(13/10){1}{}&\rat(11/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\rat(13/10){1}{}&\rat(6/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\rat(13/10){1}{}&\rat(6/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\rat(3/10){1}{}&\rat(11/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 185
\orbit{3}{185}{127}
\h{185}&\rat(9/10){9}{}&\rat(18/5){8}{\spec{2}}&\rat(15/2){1}{\spec{1}}&&\cnt{855}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(4/5){8}{}&\rat(6/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(1/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(1/5){2}{}&\rat(4/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(-1/5){8}{}&\rat(6/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(8/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(12/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(1){5}{\spec{1}}&\int(3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(1){5}{\spec{2}}&\int(3){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 186
\orbit{3}{186}{127}
\h{186}&\rat(13/2){5}{\spec{2}}&\rat(9/2){5}{\spec{1}}&\int(1){2}{}&&\cnt{811}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(2){4}{\spec{2}}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\rat(7/2){7}{}&\rat(3/2){9}{}&\int(-1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(7/2){7}{}&\rat(1/2){9}{}&\int(0){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(7/2){7}{}&\rat(-1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(5/2){7}{}&\rat(3/2){9}{}&\int(0){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(5/2){7}{}&\rat(1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(3/2){7}{\spec{2}}&\rat(3/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(3){8}{}&\int(1){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(3){8}{}&\int(1){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\int(3){8}{}&\rat(1/2){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(1){8}{\spec{2}}&\int(3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(3/2){9}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(3/2){9}{}&\int(2){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(1/2){1}{\spec{2}}&\rat(5/2){7}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 187
\orbit{3}{187}{127}
\h{187}&\rat(9/10){9}{}&\rat(48/5){8}{\spec{3}}&\rat(3/2){1}{}&&\cnt{855}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(1/5){2}{}&\rat(19/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(-1/5){8}{}&\rat(21/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(18/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(13/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(8/5){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(8/5){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(17/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(18/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){5}{\spec{1}}&\int(1){3}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){5}{\spec{2}}&\int(1){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 188
\orbit{3}{188}{127}
\h{188}&\int(6){\6}{}&\int(0){\0}{}&\int(6){\6}{\spec{1}}&&\cnt{791}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){5}{\spec{1}}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){7}{}&\int(0){9}{}&\int(1){2}{}&\ln{2}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){7}{}&\int(0){9}{}&\int(2){2}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 189
\orbit{3}{189}{127}
\h{189}&\rat(69/10){9}{\spec{2}}&\rat(8/5){8}{}&\rat(7/2){1}{}&&\cnt{691}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(18/5){6}{}&\rat(2/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(17/5){4}{}&\rat(3/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(12/5){4}{\spec{1}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(12/5){4}{\spec{2}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(33/10){3}{}&\rat(1/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(33/10){3}{}&\rat(-4/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(27/10){7}{}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(27/10){7}{}&\rat(-1/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(23/10){3}{}&\rat(1/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(17/10){7}{}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(11/5){2}{}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(11/5){2}{}&\rat(-1/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(6/5){2}{}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 190
\orbit{3}{190}{127}
\h{190}&\rat(69/10){9}{\spec{1}}&\rat(8/5){8}{}&\rat(7/2){1}{}&&\cnt{803}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(12/5){4}{\spec{2}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(27/10){7}{\spec{2}}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(27/10){7}{\spec{2}}&\rat(-1/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(23/10){3}{\spec{2}}&\rat(1/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(17/10){7}{\spec{2}}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(17/10){7}{\spec{3}}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(14/5){8}{}&\rat(6/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(14/5){8}{}&\rat(1/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(14/5){8}{}&\rat(-4/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(11/5){2}{\spec{2}}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(11/5){2}{\spec{2}}&\rat(-1/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(9/5){8}{\spec{2}}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(6/5){2}{\spec{2}}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\rat(19/10){9}{}&\rat(3/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\rat(19/10){9}{}&\rat(3/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{26}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\rat(9/10){9}{\spec{2}}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 191
\orbit{3}{191}{127}
\h{191}&\int(4){\4}{}&\int(0){\0}{}&\int(8){\8}{\spec{1}}&&\cnt{903}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(1){5}{\spec{1}}&\int(0){\0}{}&\int(3){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(2){7}{}&\int(0){9}{}&\int(2){2}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{3}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{2}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(1){8}{}&\int(0){1}{}&\int(3){3}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(1){9}{}&\int(0){8}{}&\int(3){1}{}&\ln{2}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 192
\orbit{3}{192}{127}
\h{192}&\rat(89/10){9}{\spec{2}}&\rat(8/5){8}{}&\rat(3/2){1}{}&&\cnt{811}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(9/2){5}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(22/5){4}{}&\rat(-2/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(18/5){6}{}&\rat(2/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(17/5){4}{}&\rat(3/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(12/5){4}{\spec{1}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(33/10){3}{}&\rat(1/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\rat(27/10){7}{\spec{1}}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(11/5){2}{\spec{1}}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(9/10){9}{\spec{1}}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 193
\orbit{3}{193}{127}
\h{193}&\rat(8/5){8}{}&\rat(22/5){6}{\spec{2}}&\int(6){\6}{3}&&\cnt{811}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(-3/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(3/5){8}{}&\rat(2/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(2/5){2}{}&\rat(3/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(-2/5){8}{}&\rat(7/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(4/5){9}{}&\rat(11/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(4/5){9}{}&\rat(6/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(1/5){1}{}&\rat(9/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(1){5}{\spec{1}}&\int(3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(1){5}{\spec{2}}&\int(3){3}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 194
\orbit{3}{194}{126}
\h{194}&\rat(21/2){5}{\spec{6}}&\int(0){\0}{}&\rat(3/2){1}{}&&\cnt{1111}&\bounds{126}{126}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(7/2){7}{}&\int(0){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{480}&\bounds{48}{48}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(4){8}{}&\int(0){6}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\int(4){8}{}&\int(0){1}{}&\int(0){3}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(5/2){9}{}&\int(0){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 195
\orbit{3}{195}{126}
\h{195}&\rat(41/10){7}{\spec{2}}&\rat(22/5){4}{\spec{2}}&\rat(7/2){1}{}&&\cnt{695}&\bounds{126}{126}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(14/5){6}{}&\rat(6/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(14/5){6}{}&\rat(6/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(9/5){6}{}&\rat(11/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(19/10){3}{}&\rat(8/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(19/10){3}{}&\rat(3/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(9/10){3}{\spec{1}}&\rat(8/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(9/10){3}{\spec{2}}&\rat(8/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(8/5){2}{}&\rat(2/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(2/5){8}{}&\rat(8/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(13/10){1}{}&\rat(6/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{18}&\rat(13/10){1}{}&\rat(11/5){2}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(13/10){1}{}&\rat(11/5){2}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(13/10){1}{}&\rat(6/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\rat(13/10){1}{}&\rat(6/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{24}&\rat(3/10){1}{}&\rat(11/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{25}&\rat(-3/10){9}{}&\rat(14/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 196
\orbit{3}{196}{126}
\h{196}&\rat(17/2){5}{\spec{2}}&\int(2){\2}{}&\rat(3/2){1}{}&&\cnt{803}&\bounds{126}{126}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(5/2){5}{\spec{3}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(4){6}{}&\int(0){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(4){6}{}&\int(0){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(3){4}{\spec{2}}&\int(1){8}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(7/2){7}{}&\int(1){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(7/2){7}{}&\int(0){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(5/2){7}{\spec{1}}&\int(1){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(5/2){7}{\spec{2}}&\int(1){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(5/2){3}{\spec{2}}&\int(1){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(3){8}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\int(3){8}{}&\int(1){1}{}&\int(0){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{25}&\int(2){2}{\spec{2}}&\int(1){9}{}&\int(1){3}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{26}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\rat(3/2){1}{}&\int(1){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 197
\orbit{3}{197}{126}
\h{197}&\rat(29/10){9}{\spec{2}}&\rat(41/10){3}{\spec{1}}&\int(5){2}{\spec{1}}&&\cnt{695}&\bounds{126}{126}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(-3/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(6/5){2}{}&\rat(13/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(6/5){2}{}&\rat(3/10){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(4/5){8}{}&\rat(7/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(1/5){2}{\spec{1}}&\rat(13/10){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(1/5){2}{\spec{2}}&\rat(13/10){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(2/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\rat(9/10){9}{}&\rat(3/5){8}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(3/5){8}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\rat(3/2){5}{\spec{1}}&\rat(5/2){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\rat(3/2){5}{\spec{2}}&\rat(5/2){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 198
\orbit{3}{198}{125}
\h{198}&\int(2){\2}{}&\int(0){\0}{}&\int(10){\10}{}&&\cnt{1099}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(1){7}{}&\int(0){9}{}&\int(3){2}{}&\ln{2}&\cnt{280}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(1){9}{}&\int(0){3}{}&\int(3){2}{}&\ln{2}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 199
\orbit{3}{199}{125}
\h{199}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(9){2}{\spec{1}}&&\cnt{959}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(4/5){8}{}&\rat(-3/10){1}{}&\rat(7/2){3}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(1/5){2}{}&\rat(3/10){9}{}&\rat(7/2){3}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\rat(-1/5){8}{}&\rat(7/10){1}{}&\rat(7/2){3}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(11/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\rat(1/2){5}{}&\rat(7/2){3}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 200
\orbit{3}{200}{125}
\h{200}&\rat(49/10){9}{\spec{2}}&\rat(28/5){8}{\spec{1}}&\rat(3/2){1}{}&&\cnt{751}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(12/5){4}{}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(7/5){4}{\spec{1}}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(7/5){4}{\spec{2}}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(27/10){7}{}&\rat(9/5){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(27/10){7}{}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(23/10){3}{}&\rat(6/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(17/10){7}{}&\rat(9/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{16}&\rat(11/5){2}{}&\rat(9/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(11/5){2}{}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(6/5){2}{}&\rat(9/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{21}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{24}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 201
\orbit{3}{201}{125}
\h{201}&\rat(28/5){8}{\spec{1}}&\rat(22/5){6}{\spec{1}}&\int(2){\2}{}&&\cnt{743}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(9/5){4}{}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(7/5){7}{\spec{1}}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(7/5){7}{\spec{2}}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(13/5){8}{}&\rat(7/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(13/5){8}{}&\rat(2/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{17}&\rat(7/5){2}{}&\rat(8/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(9/5){9}{}&\rat(6/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{19}&\rat(9/5){9}{}&\rat(11/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(9/5){9}{}&\rat(6/5){8}{\spec{1}}&\int(1){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(9/5){9}{}&\rat(6/5){8}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{25}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 202
\orbit{3}{202}{125}
\h{202}&\rat(38/5){8}{\spec{1}}&\rat(22/5){6}{\spec{1}}&\int(0){\0}{}&&\cnt{791}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(16/5){6}{\spec{2}}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(14/5){4}{\spec{2}}&\rat(6/5){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(14/5){4}{\spec{2}}&\rat(6/5){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(9/5){4}{\spec{2}}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(9/5){4}{\spec{3}}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(17/5){7}{}&\rat(3/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(12/5){7}{\spec{2}}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(13/5){8}{}&\rat(7/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(12/5){2}{\spec{2}}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{17}&\rat(12/5){2}{\spec{2}}&\rat(8/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(8/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(8/5){8}{\spec{3}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{20}&\rat(9/5){9}{}&\rat(11/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 203
\orbit{3}{203}{125}
\h{203}&\rat(41/10){7}{\spec{2}}&\rat(32/5){4}{\spec{2}}&\rat(3/2){1}{}&&\cnt{811}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(14/5){6}{}&\rat(6/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(4/5){6}{\spec{1}}&\rat(16/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(4/5){6}{\spec{2}}&\rat(16/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(19/10){3}{}&\rat(8/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(8/5){2}{}&\rat(12/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(13/10){1}{}&\rat(16/5){2}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(13/10){1}{}&\rat(6/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\rat(3/10){1}{}&\rat(16/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(-7/10){1}{}&\rat(16/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 204
\orbit{3}{204}{125}
\h{204}&\rat(18/5){8}{\spec{2}}&\rat(22/5){6}{\spec{1}}&\int(4){\4}{}&&\cnt{695}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(9/5){4}{}&\rat(11/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(7/5){2}{}&\rat(8/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(7/5){2}{}&\rat(3/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(2/5){2}{\spec{1}}&\rat(8/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(2/5){2}{\spec{2}}&\rat(8/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(6/5){1}{}&\rat(4/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(4/5){9}{}&\rat(6/5){8}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(4/5){9}{}&\rat(6/5){8}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(-1/5){9}{}&\rat(11/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 205
\orbit{3}{205}{124}
\h{205}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(9){2}{\spec{2}}&&\cnt{959}&\bounds{124}{124}{1}{false}&&\cr
\l{1}&\rat(1/2){5}{}&\int(0){\0}{}&\rat(7/2){1}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(7/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(11/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(-2/5){8}{}&\rat(7/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(1/10){1}{}&\rat(2/5){2}{}&\rat(7/2){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(-1/10){9}{}&\rat(3/5){8}{}&\rat(7/2){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{10}&\rat(-9/10){1}{}&\rat(7/5){2}{}&\rat(7/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\rat(3/2){5}{}&\rat(5/2){3}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 206
\orbit{3}{206}{123}
\h{206}&\rat(18/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(6){\6}{3}&&\cnt{687}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(-3/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(7/5){2}{}&\rat(-2/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(3/5){8}{}&\rat(2/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(2/5){2}{\spec{1}}&\rat(3/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(2/5){2}{\spec{2}}&\rat(3/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(6/5){1}{}&\rat(4/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(4/5){9}{}&\rat(6/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){5}{}&\int(3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 207
\orbit{3}{207}{123}
\h{207}&\int(2){\2}{}&\int(0){\0}{}&\int(10){\10}{\spec{1}}&&\cnt{875}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(1){5}{}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(1){8}{}&\int(0){1}{}&\int(3){3}{}&\ln{2}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(1){9}{}&\int(0){8}{}&\int(3){1}{}&\ln{2}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 208
\orbit{3}{208}{123}
\h{208}&\rat(81/10){7}{\spec{2}}&\rat(12/5){4}{}&\rat(3/2){1}{}&&\cnt{687}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{\spec{1}}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(21/5){4}{}&\rat(-1/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(16/5){4}{\spec{1}}&\rat(4/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(14/5){6}{\spec{1}}&\rat(6/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(39/10){3}{}&\rat(3/5){1}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(39/10){3}{}&\rat(-2/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(29/10){3}{\spec{1}}&\rat(3/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(13/5){2}{\spec{1}}&\rat(7/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(13/5){2}{\spec{1}}&\rat(2/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{12}&\rat(8/5){2}{\spec{1}}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(13/10){1}{\spec{1}}&\rat(6/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 209
\orbit{3}{209}{123}
\h{209}&\rat(49/10){9}{\spec{2}}&\rat(21/10){3}{}&\int(5){2}{\spec{1}}&&\cnt{695}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(3/2){5}{\spec{1}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(3/2){5}{\spec{2}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(27/10){7}{}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(23/10){3}{}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(11/5){2}{}&\rat(3/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(11/5){2}{}&\rat(-7/10){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(9/5){8}{}&\rat(-3/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(6/5){2}{}&\rat(3/10){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(4/5){8}{}&\rat(7/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(2/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{20}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(3/2){5}{}&\rat(5/2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 210
\orbit{3}{210}{123}
\h{210}&\rat(8/5){8}{}&\rat(52/5){6}{\spec{1}}&\int(0){\0}{}&&\cnt{751}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(8/5){8}{}&\rat(12/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(2/5){2}{}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(16/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 211
\orbit{3}{211}{123}
\h{211}&\rat(9/2){5}{\spec{1}}&\int(2){\2}{}&\rat(11/2){1}{}&&\cnt{747}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(5/2){7}{}&\int(1){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(5/2){7}{}&\int(0){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(3/2){7}{\spec{1}}&\int(1){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(3/2){7}{\spec{2}}&\int(1){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\int(1){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\int(1){8}{\spec{1}}&\int(1){1}{}&\int(2){3}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(1){8}{\spec{2}}&\int(1){1}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\int(1){2}{}&\int(1){9}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(3/2){9}{}&\int(1){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(3/2){9}{}&\int(0){8}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\rat(3/2){9}{}&\int(0){8}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\rat(1/2){9}{}&\int(1){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\rat(1/2){1}{}&\int(1){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 212
\orbit{3}{212}{122}
\h{212}&\int(6){\6}{\spec{1}}&\int(2){\2}{}&\int(4){\4}{}&&\cnt{799}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(2){7}{}&\int(1){9}{}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(1){1}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{12}&\int(2){2}{}&\int(1){9}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){2}{}&\int(0){9}{}&\int(2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(1){2}{}&\int(1){9}{}&\int(2){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(2){9}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{17}&\int(2){9}{}&\int(1){8}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(2){9}{}&\int(0){8}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\int(2){9}{}&\int(0){8}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(1){1}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 213
\orbit{3}{213}{122}
\h{213}&\rat(49/10){9}{\spec{2}}&\rat(41/10){3}{\spec{2}}&\int(3){2}{}&&\cnt{691}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(13/5){6}{}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(8/5){6}{\spec{1}}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(8/5){6}{\spec{2}}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(27/10){7}{}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(23/10){3}{}&\rat(17/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(23/10){3}{}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(13/10){3}{\spec{1}}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(13/10){3}{\spec{2}}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(11/5){2}{}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(11/5){2}{}&\rat(3/10){9}{}&\rat(3/2){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(9/5){8}{}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{16}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(4/5){8}{}&\rat(17/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{21}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 214
\orbit{3}{214}{122}
\h{214}&\rat(17/2){5}{\spec{3}}&\int(0){\0}{}&\rat(7/2){1}{}&&\cnt{1067}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(7/2){7}{}&\int(0){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(5/2){7}{}&\int(0){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{140}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{70}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(5/2){9}{}&\int(0){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{11}&\rat(5/2){9}{}&\int(0){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 215
\orbit{3}{215}{122}
\h{215}&\rat(8/5){8}{}&\rat(22/5){6}{\spec{1}}&\int(6){\6}{\spec{1}}&&\cnt{799}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(2/5){7}{}&\rat(8/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(2/5){2}{}&\rat(8/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(4/5){9}{}&\rat(6/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{9}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(6/5){8}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(4/5){9}{}&\rat(6/5){8}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{14}&\rat(-1/5){9}{}&\rat(11/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(-4/5){1}{}&\rat(14/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 216
\orbit{3}{216}{121}
\h{216}&\rat(18/5){8}{\spec{2}}&\rat(22/5){6}{\spec{2}}&\int(4){\4}{2}&&\cnt{687}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(12/5){7}{}&\rat(-2/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(8/5){3}{}&\rat(2/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(3/5){3}{\spec{1}}&\rat(7/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(3/5){3}{\spec{2}}&\rat(7/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(6/5){1}{}&\rat(4/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(6/5){1}{}&\rat(9/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(4/5){9}{}&\rat(6/5){3}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(4/5){9}{}&\rat(6/5){3}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(-1/5){9}{}&\rat(11/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 217
\orbit{3}{217}{121}
\h{217}&\rat(9/10){9}{}&\rat(101/10){3}{\spec{1}}&\int(1){2}{}&&\cnt{919}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\rat(3/5){6}{}&\rat(17/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(3/10){3}{}&\rat(27/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(4/5){8}{}&\rat(27/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(1/10){1}{}&\rat(17/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 218
\orbit{3}{218}{121}
\h{218}&\rat(9/10){9}{}&\rat(61/10){3}{\spec{2}}&\int(5){2}{\spec{1}}&&\cnt{811}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(4/5){8}{}&\rat(7/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(1/5){2}{}&\rat(13/10){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(3/5){8}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(3/5){8}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(3/2){5}{\spec{1}}&\rat(5/2){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(3/2){5}{\spec{2}}&\rat(5/2){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 219
\orbit{3}{219}{121}
\h{219}&\rat(9/10){9}{}&\rat(38/5){8}{\spec{2}}&\rat(7/2){1}{}&&\cnt{811}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(4/5){8}{}&\rat(6/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(1/5){2}{}&\rat(19/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(18/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(13/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(8/5){3}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){3}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(1/10){1}{}&\rat(12/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(-1/10){9}{}&\rat(18/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(13/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){5}{\spec{1}}&\int(2){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){5}{\spec{2}}&\int(2){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 220
\orbit{3}{220}{121}
\h{220}&\rat(9/10){9}{}&\rat(38/5){8}{\spec{1}}&\rat(7/2){1}{}&&\cnt{799}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(9/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(16/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(4/5){8}{}&\rat(6/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(1/5){2}{}&\rat(9/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(13/5){3}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){3}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(8/5){3}{\spec{3}}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(9/10){9}{}&\rat(8/5){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(9/10){9}{}&\rat(8/5){8}{\spec{3}}&\rat(3/2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(1/10){1}{}&\rat(17/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(1/10){1}{}&\rat(12/5){7}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(1/10){1}{}&\rat(12/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\rat(-1/10){9}{}&\rat(13/5){3}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(-9/10){1}{}&\rat(17/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(3){5}{\spec{2}}&\int(1){3}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){5}{\spec{2}}&\int(2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(2){5}{\spec{3}}&\int(2){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 221
\orbit{3}{221}{121}
\h{221}&\rat(49/10){9}{\spec{2}}&\rat(18/5){8}{\spec{1}}&\rat(7/2){1}{}&&\cnt{811}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(12/5){4}{}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(27/10){7}{}&\rat(9/5){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(27/10){7}{}&\rat(-1/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(23/10){3}{}&\rat(1/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(17/10){7}{}&\rat(9/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(7/10){7}{\spec{1}}&\rat(9/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(7/10){7}{\spec{2}}&\rat(9/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{}&\rat(9/5){9}{}&\int(0){3}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(11/5){2}{}&\rat(9/5){9}{}&\int(0){3}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(11/5){2}{}&\rat(-1/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(6/5){2}{}&\rat(9/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{17}&\rat(1/5){2}{\spec{1}}&\rat(9/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(1/5){2}{\spec{2}}&\rat(9/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 222
\orbit{3}{222}{120}
\h{222}&\rat(21/10){7}{}&\rat(22/5){4}{\spec{2}}&\rat(11/2){1}{}&&\cnt{747}&\bounds{120}{120}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(9/5){6}{}&\rat(11/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(9/10){3}{}&\rat(8/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(2/5){8}{}&\rat(8/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(7/10){9}{}&\rat(4/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(3/10){1}{}&\rat(11/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(3/10){1}{}&\rat(6/5){2}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{15}&\rat(3/10){1}{}&\rat(6/5){2}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(-3/10){9}{}&\rat(14/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(-7/10){1}{}&\rat(11/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 223
\orbit{3}{223}{120}
\h{223}&\rat(13/2){5}{\spec{2}}&\rat(5/2){5}{}&\int(3){2}{}&&\cnt{691}&\bounds{120}{120}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(7/2){7}{}&\rat(1/2){9}{}&\int(0){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(7/2){7}{}&\rat(-1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(5/2){7}{}&\rat(1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(3){8}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(3){8}{}&\rat(1/2){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(3){8}{}&\rat(-1/2){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){8}{}&\rat(1/2){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(3/2){9}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\int(0){\0}{\spec{2}}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 224
\orbit{3}{224}{119}
\h{224}&\rat(18/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(6){\6}{1}&&\cnt{687}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(1){5}{\spec{1}}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(1){5}{\spec{2}}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(12/5){7}{}&\rat(3/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(7/5){2}{}&\rat(3/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(6/5){1}{}&\rat(9/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(6/5){1}{}&\rat(-1/5){2}{}&\int(3){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(1/5){8}{}&\int(3){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(1/5){1}{}&\rat(4/5){2}{}&\int(3){1}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(-1/5){9}{}&\rat(6/5){8}{}&\int(3){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 225
\orbit{3}{225}{119}
\h{225}&\rat(21/10){7}{}&\rat(32/5){4}{\spec{2}}&\rat(7/2){1}{}&&\cnt{691}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\rat(6/5){4}{}&\rat(14/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(21/10){7}{}&\rat(2/5){9}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(11/10){7}{}&\rat(7/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(3/5){2}{}&\rat(7/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(2/5){8}{}&\rat(18/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/10){9}{}&\rat(14/5){8}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(7/10){9}{}&\rat(14/5){8}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(3/10){1}{}&\rat(16/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(3/10){1}{}&\rat(11/5){7}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(3/10){1}{}&\rat(11/5){7}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(-3/10){9}{}&\rat(14/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\rat(-7/10){1}{}&\rat(16/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){5}{\spec{2}}&\int(2){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 226
\orbit{3}{226}{119}
\h{226}&\rat(48/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(0){\0}{}&&\cnt{639}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(16/5){6}{\spec{2}}&\rat(4/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(14/5){4}{\spec{2}}&\rat(6/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(17/5){7}{}&\rat(3/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(13/5){8}{}&\rat(7/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(12/5){2}{\spec{2}}&\rat(8/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(8/5){8}{\spec{2}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(8/5){8}{\spec{3}}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(11/5){1}{}&\rat(9/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 227
\orbit{3}{227}{119}
\h{227}&\int(8){\8}{\spec{1}}&\int(0){\0}{}&\int(4){\4}{}&&\cnt{899}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{\spec{3}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{2}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){9}{}&\int(0){8}{}&\int(2){1}{}&\ln{2}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 228
\orbit{3}{228}{119}
\h{228}&\int(8){\8}{\spec{2}}&\int(0){\0}{}&\int(4){\4}{}&&\cnt{847}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){5}{\spec{3}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){5}{\spec{3}}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){5}{\spec{4}}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(3){7}{\spec{2}}&\int(0){9}{}&\int(1){2}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(3){3}{\spec{2}}&\int(0){1}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{4}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){8}{\spec{2}}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\int(2){2}{\spec{2}}&\int(0){9}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(2){9}{}&\int(0){8}{}&\int(2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\int(0){\0}{\spec{2}}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 229
\orbit{3}{229}{119}
\h{229}&\rat(8/5){8}{}&\rat(32/5){6}{\spec{2}}&\int(4){\4}{}&&\cnt{687}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(2/5){1}{\spec{1}}&\int(2){3}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(3/5){8}{}&\rat(7/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(2/5){2}{}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(4/5){9}{}&\rat(16/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(4/5){9}{}&\rat(11/5){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(4/5){9}{}&\rat(11/5){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(6/5){8}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(1/5){1}{}&\rat(14/5){2}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(1/5){1}{}&\rat(9/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(-1/5){9}{}&\rat(16/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(-4/5){1}{}&\rat(14/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){5}{\spec{1}}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{\spec{1}}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 230
\orbit{3}{230}{119}
\h{230}&\int(4){\4}{}&\int(0){\0}{}&\int(8){\8}{0}&&\cnt{775}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\int(2){7}{}&\int(0){9}{}&\int(2){2}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{2}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 231
\orbit{3}{231}{118}
\h{231}&\rat(29/10){9}{\spec{2}}&\rat(81/10){3}{\spec{1}}&\int(1){2}{}&&\cnt{791}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\rat(3/5){6}{\spec{1}}&\rat(17/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\rat(3/5){6}{\spec{2}}&\rat(17/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(13/10){3}{}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\rat(9/5){8}{}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{11}&\rat(11/10){1}{}&\rat(19/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(11/10){1}{}&\rat(17/5){2}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{14}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(1/10){1}{}&\rat(17/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{16}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 232
\orbit{3}{232}{118}
\h{232}&\rat(41/10){7}{\spec{1}}&\rat(12/5){4}{}&\rat(11/2){1}{}&&\cnt{743}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(12/5){8}{}&\rat(8/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(12/5){8}{}&\rat(3/5){1}{}&\int(1){3}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(12/5){8}{}&\rat(3/5){1}{}&\int(1){3}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(12/5){8}{}&\rat(-2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(17/10){9}{}&\rat(9/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(17/10){9}{}&\rat(4/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(17/10){9}{}&\rat(4/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(17/10){9}{}&\rat(-1/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(7/10){9}{}&\rat(4/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(3/10){1}{}&\rat(6/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 233
\orbit{3}{233}{118}
\h{233}&\rat(21/2){5}{\spec{4}}&\int(0){\0}{}&\rat(3/2){1}{}&&\cnt{831}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\rat(9/2){7}{}&\int(0){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 234
\orbit{3}{234}{118}
\h{234}&\rat(9/10){9}{}&\rat(48/5){8}{\spec{5}}&\rat(3/2){1}{}&&\cnt{975}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(14/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(1/5){2}{}&\rat(14/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 235
\orbit{3}{235}{118}
\h{235}&\rat(29/10){9}{\spec{2}}&\rat(28/5){8}{\spec{1}}&\rat(7/2){1}{}&&\cnt{747}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\rat(7/5){4}{}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(9/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(17/10){7}{}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(13/10){3}{}&\rat(6/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(7/10){7}{\spec{1}}&\rat(9/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(7/10){7}{\spec{2}}&\rat(9/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(6/5){2}{}&\rat(9/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(6/5){2}{}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(4/5){8}{}&\rat(6/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(1/5){2}{\spec{1}}&\rat(9/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(1/5){2}{\spec{2}}&\rat(9/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\rat(11/10){1}{}&\rat(7/5){7}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(11/10){1}{}&\rat(7/5){7}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{24}&\rat(9/10){9}{}&\rat(8/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{27}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{28}&\rat(1/10){1}{}&\rat(12/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{29}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{31}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{32}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{33}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{34}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{35}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 236
\orbit{3}{236}{118}
\h{236}&\rat(49/10){9}{\spec{1}}&\rat(28/5){8}{\spec{2}}&\rat(3/2){1}{}&&\cnt{743}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\rat(8/5){6}{}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(19/10){9}{}&\rat(13/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(19/10){9}{}&\rat(8/5){3}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(19/10){9}{}&\rat(8/5){3}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(19/10){9}{}&\rat(3/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 237
\orbit{3}{237}{117}
\h{237}&\rat(8/5){8}{}&\rat(52/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{839}&\bounds{117}{117}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(2/5){2}{}&\rat(18/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(-3/5){2}{}&\rat(23/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/5){9}{}&\rat(16/5){3}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(-1/5){9}{}&\rat(21/5){3}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 238
\orbit{3}{238}{117}
\h{238}&\rat(49/10){9}{\spec{1}}&\rat(18/5){8}{\spec{2}}&\rat(7/2){1}{}&&\cnt{743}&\bounds{117}{117}{1}{false}&&\cr
\l{1}&\rat(17/10){7}{}&\rat(4/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(13/10){3}{}&\rat(6/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(6/5){2}{}&\rat(4/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(4/5){8}{}&\rat(6/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(19/10){9}{}&\rat(8/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\rat(19/10){9}{}&\rat(3/5){3}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(19/10){9}{}&\rat(3/5){3}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(19/10){9}{}&\rat(3/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{20}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{23}&\rat(1/10){1}{}&\rat(12/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 239
\orbit{3}{239}{117}
\h{239}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{775}&\bounds{117}{117}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{2}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\int(2){9}{}&\int(2){3}{}&\int(0){2}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){9}{}&\int(2){8}{}&\int(0){1}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 240
\orbit{3}{240}{117}
\h{240}&\rat(9/10){9}{}&\rat(61/10){3}{\spec{2}}&\int(5){2}{\spec{2}}&&\cnt{735}&\bounds{117}{117}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(13/10){9}{}&\int(2){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(11/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(1/10){1}{}&\rat(19/10){7}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(19/10){7}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(-9/10){1}{}&\rat(29/10){7}{}&\int(2){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 241
\orbit{3}{241}{117}
\h{241}&\rat(41/10){7}{\spec{1}}&\rat(32/5){4}{\spec{1}}&\rat(3/2){1}{}&&\cnt{743}&\bounds{117}{117}{1}{false}&&\cr
\l{1}&\rat(9/5){6}{}&\rat(11/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(12/5){8}{}&\rat(8/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(12/5){8}{}&\rat(8/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(12/5){8}{}&\rat(8/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(12/5){8}{}&\rat(3/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(3/5){2}{}&\rat(17/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(17/10){9}{}&\rat(14/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(17/10){9}{}&\rat(9/5){3}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\rat(17/10){9}{}&\rat(9/5){3}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(17/10){9}{}&\rat(9/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{18}&\rat(17/10){9}{}&\rat(4/5){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(17/10){9}{}&\rat(4/5){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(3/10){1}{}&\rat(11/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 242
\orbit{3}{242}{116}
\h{242}&\rat(29/10){9}{\spec{2}}&\rat(41/10){3}{\spec{2}}&\int(5){2}{\spec{1}}&&\cnt{811}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(8/5){6}{}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(13/10){3}{}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(9/5){8}{}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(-3/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(6/5){2}{}&\rat(3/10){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(4/5){8}{}&\rat(17/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(4/5){8}{}&\rat(7/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(-1/5){8}{\spec{1}}&\rat(17/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(-1/5){8}{\spec{2}}&\rat(17/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(2/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{20}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{21}&\rat(-9/10){1}{}&\rat(12/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(3/2){5}{}&\rat(5/2){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 243
\orbit{3}{243}{116}
\h{243}&\rat(13/2){5}{\spec{2}}&\int(2){\2}{}&\rat(7/2){1}{}&&\cnt{811}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(7/2){7}{}&\int(1){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(7/2){7}{}&\int(0){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(7/2){7}{}&\int(-1){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(5/2){7}{}&\int(1){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(5/2){7}{}&\int(0){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\rat(3/2){7}{\spec{2}}&\int(1){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(3/2){3}{\spec{2}}&\int(1){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\int(3){8}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(3){8}{}&\int(1){1}{}&\int(0){3}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(3){8}{}&\int(1){1}{}&\int(0){3}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\int(3){8}{}&\int(-1){1}{}&\int(2){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(1){8}{\spec{2}}&\int(1){1}{}&\int(2){3}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(1){2}{\spec{2}}&\int(1){9}{}&\int(2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(3/2){9}{}&\int(1){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{24}&\int(0){\0}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 244
\orbit{3}{244}{116}
\h{244}&\rat(9/10){9}{}&\rat(101/10){3}{\spec{3}}&\int(1){2}{}&&\cnt{847}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(4/5){8}{}&\rat(16/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(16/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(1/5){2}{}&\rat(19/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(-1/5){8}{}&\rat(21/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(39/10){7}{}&\int(0){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(-9/10){1}{}&\rat(39/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(9/2){5}{}&\rat(-1/2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 245
\orbit{3}{245}{116}
\h{245}&\rat(9/2){5}{\spec{1}}&\int(0){\0}{}&\rat(15/2){1}{\spec{2}}&&\cnt{955}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(3/2){7}{\spec{1}}&\int(0){9}{}&\rat(5/2){2}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(3/2){7}{\spec{2}}&\int(0){9}{}&\rat(5/2){2}{}&\ln{1}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\int(0){1}{}&\rat(5/2){2}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{150}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(3/2){9}{}&\int(0){3}{}&\rat(5/2){2}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{11}&\rat(3/2){9}{}&\int(0){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 246
\orbit{3}{246}{116}
\h{246}&\rat(9/10){9}{}&\rat(81/10){3}{\spec{1}}&\int(3){2}{}&&\cnt{787}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\rat(3/5){6}{}&\rat(17/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(17/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(1/10){1}{}&\rat(17/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(-9/10){1}{}&\rat(17/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 247
\orbit{3}{247}{116}
\h{247}&\rat(29/10){9}{\spec{2}}&\rat(38/5){8}{\spec{2}}&\rat(3/2){1}{}&&\cnt{691}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\rat(8/5){6}{}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(9/5){8}{}&\rat(11/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(9/5){8}{}&\rat(6/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(6/5){2}{}&\rat(14/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(6/5){2}{}&\rat(14/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(1/5){2}{\spec{1}}&\rat(19/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(1/5){2}{\spec{2}}&\rat(19/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(11/10){1}{}&\rat(12/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(9/10){9}{}&\rat(18/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(9/10){9}{}&\rat(13/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(-1/10){9}{}&\rat(18/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 248
\orbit{3}{248}{116}
\h{248}&\rat(69/10){9}{\spec{1}}&\rat(41/10){3}{\spec{2}}&\int(1){2}{}&&\cnt{791}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(13/5){6}{\spec{2}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(8/5){6}{\spec{2}}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(8/5){6}{\spec{3}}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(27/10){7}{\spec{2}}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(23/10){3}{\spec{2}}&\rat(17/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(23/10){3}{\spec{2}}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(13/10){3}{\spec{2}}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(13/10){3}{\spec{3}}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(14/5){8}{}&\rat(6/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{17}&\rat(14/5){8}{}&\rat(17/10){1}{}&\rat(-1/2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(14/5){8}{}&\rat(7/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(11/5){2}{\spec{2}}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(9/5){8}{\spec{2}}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{22}&\rat(19/10){9}{}&\rat(11/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\rat(9/10){9}{\spec{2}}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 249
\orbit{3}{249}{115}
\h{249}&\rat(13/2){5}{\spec{2}}&\int(4){\4}{}&\rat(3/2){1}{}&&\cnt{687}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){4}{\spec{2}}&\int(2){8}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\rat(7/2){7}{}&\int(1){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(7/2){7}{}&\int(0){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(5/2){7}{}&\int(1){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(3){8}{}&\int(1){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(3){8}{}&\int(1){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(3){8}{}&\int(1){1}{}&\int(0){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(3/2){9}{}&\int(2){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(3/2){9}{}&\int(2){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(3/2){9}{}&\int(1){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(1/2){9}{\spec{2}}&\int(2){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(1/2){1}{\spec{2}}&\int(2){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 250
\orbit{3}{250}{115}
\h{250}&\rat(18/5){8}{\spec{1}}&\rat(32/5){6}{\spec{1}}&\int(2){\2}{}&&\cnt{735}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(9/5){9}{}&\rat(11/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(9/5){9}{}&\rat(6/5){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(9/5){9}{}&\rat(6/5){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(9/5){9}{}&\rat(11/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(9/5){9}{}&\rat(6/5){8}{\spec{1}}&\int(1){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(9/5){9}{}&\rat(6/5){8}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 251
\orbit{3}{251}{115}
\h{251}&\rat(61/10){7}{\spec{2}}&\rat(22/5){4}{\spec{2}}&\rat(3/2){1}{}&&\cnt{691}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(16/5){4}{}&\rat(4/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(14/5){6}{}&\rat(6/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(14/5){6}{}&\rat(6/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(9/5){6}{}&\rat(11/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(29/10){3}{}&\rat(8/5){1}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(29/10){3}{}&\rat(3/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(19/10){3}{\spec{1}}&\rat(8/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(19/10){3}{\spec{2}}&\rat(8/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(13/5){2}{}&\rat(7/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(13/5){2}{}&\rat(2/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(8/5){2}{}&\rat(12/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(13/10){1}{}&\rat(11/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(13/10){1}{}&\rat(6/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(13/10){1}{}&\rat(6/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\rat(3/10){1}{}&\rat(11/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 252
\orbit{3}{252}{115}
\h{252}&\rat(18/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(6){\6}{\spec{1}}&&\cnt{791}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(9/5){9}{}&\rat(6/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(9/5){9}{}&\rat(1/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(9/5){9}{}&\rat(6/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(9/5){9}{}&\rat(1/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 253
\orbit{3}{253}{115}
\h{253}&\rat(41/10){7}{\spec{1}}&\rat(22/5){4}{\spec{1}}&\rat(7/2){1}{}&&\cnt{687}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(11/10){7}{}&\rat(7/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(12/5){8}{}&\rat(8/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(12/5){8}{}&\rat(8/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(12/5){8}{}&\rat(3/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(12/5){8}{}&\rat(-2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(7/5){8}{}&\rat(13/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\rat(3/5){2}{}&\rat(7/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(17/10){9}{}&\rat(9/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(17/10){9}{}&\rat(4/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(17/10){9}{}&\rat(9/5){8}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(17/10){9}{}&\rat(9/5){8}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(17/10){9}{}&\rat(4/5){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(17/10){9}{}&\rat(4/5){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{19}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\rat(7/10){9}{}&\rat(9/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(3/10){1}{}&\rat(11/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 254
\orbit{3}{254}{114}
\h{254}&\rat(69/10){9}{\spec{1}}&\rat(18/5){8}{\spec{1}}&\rat(3/2){1}{}&&\cnt{843}&\bounds{114}{114}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(12/5){4}{\spec{1}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(27/10){7}{\spec{1}}&\rat(9/5){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(17/10){7}{\spec{1}}&\rat(9/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(11/5){2}{\spec{1}}&\rat(9/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(6/5){2}{\spec{1}}&\rat(9/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(21/10){1}{}&\rat(7/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(21/10){1}{}&\rat(2/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(9/10){9}{\spec{1}}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 255
\orbit{3}{255}{114}
\h{255}&\rat(41/10){7}{\spec{1}}&\rat(22/5){4}{\spec{2}}&\rat(7/2){1}{}&&\cnt{811}&\bounds{114}{114}{1}{false}&&\cr
\l{1}&\rat(9/5){6}{}&\rat(11/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(2/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(9/10){3}{}&\rat(8/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(12/5){8}{}&\rat(8/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\rat(12/5){8}{}&\rat(8/5){1}{}&\int(0){3}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(12/5){8}{}&\rat(8/5){1}{}&\int(0){3}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(12/5){8}{}&\rat(3/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(12/5){8}{}&\rat(-2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(7/5){8}{}&\rat(3/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(2/5){8}{}&\rat(8/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(17/10){9}{}&\rat(14/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(17/10){9}{}&\rat(9/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(17/10){9}{}&\rat(4/5){3}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(17/10){9}{}&\rat(4/5){3}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(17/10){9}{}&\rat(4/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{19}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(7/10){9}{}&\rat(9/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(3/10){1}{}&\rat(11/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{22}&\rat(-3/10){9}{}&\rat(14/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 256
\orbit{3}{256}{113}
\h{256}&\rat(28/5){8}{\spec{1}}&\rat(32/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{727}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(11/5){6}{}&\rat(9/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(6/5){6}{\spec{1}}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(6/5){6}{\spec{2}}&\rat(14/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(13/5){8}{}&\rat(7/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(13/5){8}{}&\rat(7/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(7/5){2}{}&\rat(13/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(2/5){2}{\spec{1}}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(2/5){2}{\spec{2}}&\rat(18/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(9/5){9}{}&\rat(11/5){3}{\spec{1}}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(9/5){9}{}&\rat(11/5){3}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(6/5){1}{}&\rat(14/5){2}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(4/5){9}{}&\rat(16/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 257
\orbit{3}{257}{113}
\h{257}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{763}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(3){7}{}&\int(1){9}{}&\int(0){2}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(3){8}{}&\int(1){6}{}&\int(0){\0}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(3){8}{}&\int(1){1}{}&\int(0){3}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 258
\orbit{3}{258}{113}
\h{258}&\rat(21/2){5}{\spec{5}}&\int(0){\0}{}&\rat(3/2){1}{}&&\cnt{807}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(7/2){7}{}&\int(0){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(5/2){9}{}&\int(0){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 259
\orbit{3}{259}{113}
\h{259}&\rat(9/2){5}{\spec{1}}&\int(0){\0}{}&\rat(15/2){1}{\spec{1}}&&\cnt{843}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{\spec{1}}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{4}&\rat(5/2){7}{}&\int(0){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{90}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{90}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(1){8}{\spec{1}}&\int(0){1}{}&\int(3){3}{}&\ln{1}&\cnt{30}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(1){8}{\spec{2}}&\int(0){1}{}&\int(3){3}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(1){2}{}&\int(0){9}{}&\int(3){3}{}&\ln{1}&\cnt{150}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(3/2){9}{}&\int(0){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 260
\orbit{3}{260}{112}
\h{260}&\rat(49/10){9}{\spec{1}}&\rat(61/10){3}{\spec{2}}&\int(1){2}{}&&\cnt{735}&\bounds{112}{112}{1}{false}&&\cr
\l{1}&\rat(7/5){4}{}&\rat(13/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(13/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(11/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(11/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(6/5){2}{}&\rat(14/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(19/10){9}{}&\rat(11/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(19/10){9}{}&\rat(13/5){8}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(29/10){7}{}&\int(0){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(19/10){7}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(11/10){1}{}&\rat(19/10){7}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 261
\orbit{3}{261}{111}
\h{261}&\rat(9/10){9}{}&\rat(18/5){8}{\spec{1}}&\rat(15/2){1}{\spec{2}}&&\cnt{943}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\rat(-3/10){7}{}&\rat(9/5){9}{}&\rat(5/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(1/5){2}{}&\rat(9/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(3/5){3}{}&\rat(5/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(1/10){1}{}&\rat(7/5){7}{}&\rat(5/2){2}{}&\ln{1}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\l{7}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 262
\orbit{3}{262}{111}
\h{262}&\rat(21/10){7}{}&\rat(42/5){4}{\spec{3}}&\rat(3/2){1}{}&&\cnt{675}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\rat(6/5){4}{}&\rat(14/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(7/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(2/5){8}{}&\rat(18/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\rat(7/10){9}{}&\rat(14/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{5}&\rat(3/10){1}{}&\rat(21/5){7}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(-3/10){9}{}&\rat(14/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(-7/10){1}{}&\rat(21/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 263
\orbit{3}{263}{111}
\h{263}&\int(4){\4}{}&\int(2){\2}{}&\int(6){\6}{1}&&\cnt{679}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){5}{\spec{1}}&\int(0){\0}{}&\int(3){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){7}{}&\int(1){9}{}&\int(1){2}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(1){9}{}&\int(0){8}{\spec{1}}&\int(3){1}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(1){9}{}&\int(0){8}{\spec{2}}&\int(3){1}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){9}{}&\int(1){8}{}&\int(3){1}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 264
\orbit{3}{264}{111}
\h{264}&\int(10){\10}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&&\cnt{763}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){5}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(3){7}{}&\int(0){9}{}&\int(1){2}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{2}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 265
\orbit{3}{265}{111}
\h{265}&\rat(89/10){9}{\spec{2}}&\rat(21/10){3}{}&\int(1){2}{}&&\cnt{679}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(9/2){5}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(22/5){4}{}&\rat(-2/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(18/5){6}{}&\rat(2/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(17/5){4}{}&\rat(3/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(13/5){6}{\spec{1}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(33/10){3}{}&\rat(7/10){1}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\rat(33/10){3}{}&\rat(-3/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(27/10){7}{\spec{1}}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(23/10){3}{\spec{1}}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{\spec{1}}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(9/10){9}{\spec{1}}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 266
\orbit{3}{266}{110}
\h{266}&\rat(28/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(4){\4}{2}&&\cnt{735}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(12/5){7}{}&\rat(-2/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(8/5){3}{}&\rat(2/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\rat(7/5){7}{\spec{1}}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(7/5){7}{\spec{2}}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(13/5){8}{}&\rat(7/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(13/5){8}{}&\rat(2/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(9/5){9}{}&\rat(1/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(9/5){9}{}&\rat(6/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(6/5){1}{}&\rat(4/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(4/5){9}{}&\rat(6/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 267
\orbit{3}{267}{110}
\h{267}&\rat(13/2){5}{\spec{2}}&\rat(9/2){5}{\spec{2}}&\int(1){2}{}&&\cnt{679}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(7/2){7}{}&\rat(1/2){9}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(7/2){7}{}&\rat(-1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(5/2){7}{}&\rat(1/2){9}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{\spec{2}}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(3){8}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(3){8}{}&\rat(3/2){1}{}&\rat(-1/2){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(3){8}{}&\rat(1/2){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(2){8}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(2){8}{}&\rat(3/2){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(1){2}{\spec{2}}&\int(3){4}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(3/2){9}{}&\rat(5/2){3}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(3/2){9}{}&\rat(3/2){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(3/2){9}{}&\rat(3/2){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(1/2){9}{\spec{2}}&\rat(5/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 268
\orbit{3}{268}{109}
\h{268}&\rat(9/10){9}{}&\rat(61/10){3}{\spec{1}}&\int(5){2}{\spec{1}}&&\cnt{735}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(4/5){8}{}&\rat(17/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(7/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(1/5){2}{}&\rat(13/10){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(-1/5){8}{}&\rat(17/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(9/10){9}{}&\rat(3/5){8}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(9/10){9}{}&\rat(3/5){8}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(1/10){1}{}&\rat(7/5){2}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(1/10){1}{}&\rat(7/5){2}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(-9/10){1}{}&\rat(12/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(3/2){5}{\spec{1}}&\rat(5/2){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(3/2){5}{\spec{2}}&\rat(5/2){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 269
\orbit{3}{269}{109}
\h{269}&\rat(9/10){9}{}&\rat(41/10){3}{\spec{2}}&\int(7){2}{}&&\cnt{843}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\rat(3/10){3}{}&\rat(17/10){1}{}&\int(2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(17/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(4/5){8}{}&\rat(7/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(-1/5){8}{}&\rat(17/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(11/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(-9/10){1}{}&\rat(12/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(3/2){5}{}&\rat(5/2){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 270
\orbit{3}{270}{109}
\h{270}&\rat(18/5){8}{\spec{1}}&\rat(22/5){6}{\spec{2}}&\int(4){\4}{}&&\cnt{679}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(9/5){9}{}&\rat(11/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(9/5){9}{}&\rat(6/5){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(9/5){9}{}&\rat(6/5){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(9/5){9}{}&\rat(6/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(9/5){9}{}&\rat(1/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(1/5){1}{}&\rat(9/5){2}{}&\int(2){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 271
\orbit{3}{271}{109}
\h{271}&\rat(18/5){8}{\spec{2}}&\rat(42/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{663}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{\spec{1}}&\rat(14/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{2}&\rat(6/5){6}{\spec{2}}&\rat(14/5){2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\rat(2/5){2}{\spec{1}}&\rat(18/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(2/5){2}{\spec{2}}&\rat(18/5){4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(6/5){1}{}&\rat(14/5){2}{\spec{1}}&\int(0){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(-1/5){9}{}&\rat(21/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 272
\orbit{3}{272}{109}
\h{272}&\rat(18/5){8}{\spec{2}}&\rat(32/5){6}{\spec{2}}&\int(2){\2}{}&&\cnt{679}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\rat(4/5){4}{\spec{1}}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(4/5){4}{\spec{2}}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(7/5){2}{}&\rat(8/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(16/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(-1/5){9}{}&\rat(16/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 273
\orbit{3}{273}{109}
\h{273}&\rat(69/10){9}{\spec{1}}&\rat(18/5){8}{\spec{1}}&\rat(3/2){1}{}&&\cnt{787}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(12/5){4}{\spec{2}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(27/10){7}{\spec{2}}&\rat(9/5){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(17/10){7}{\spec{2}}&\rat(9/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(17/10){7}{\spec{3}}&\rat(9/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(14/5){8}{}&\rat(6/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(14/5){8}{}&\rat(1/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(11/5){2}{\spec{2}}&\rat(9/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(6/5){2}{\spec{2}}&\rat(9/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\rat(9/10){9}{\spec{2}}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 274
\orbit{3}{274}{108}
\h{274}&\rat(17/2){5}{\spec{2}}&\int(0){\0}{}&\rat(7/2){1}{}&&\cnt{787}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(5/2){5}{\spec{3}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(7/2){7}{}&\int(0){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(5/2){7}{\spec{1}}&\int(0){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(5/2){7}{\spec{2}}&\int(0){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\rat(5/2){3}{\spec{2}}&\int(0){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(2){2}{\spec{2}}&\int(0){9}{}&\int(2){3}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 275
\orbit{3}{275}{108}
\h{275}&\rat(29/10){9}{\spec{2}}&\rat(41/10){3}{\spec{2}}&\int(5){2}{\spec{2}}&&\cnt{735}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\rat(8/5){6}{}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(3/10){9}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(13/10){3}{}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(13/10){3}{}&\rat(7/10){1}{}&\int(2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(3/10){3}{\spec{1}}&\rat(17/10){1}{}&\int(2){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(3/10){3}{\spec{2}}&\rat(17/10){1}{}&\int(2){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(9/5){8}{}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(4/5){8}{}&\rat(17/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(9/10){7}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(9/10){9}{}&\rat(11/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 276
\orbit{3}{276}{108}
\h{276}&\rat(8/5){8}{}&\rat(32/5){6}{\spec{1}}&\int(4){\4}{2}&&\cnt{735}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(3/5){3}{}&\rat(7/5){1}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(2/5){7}{}&\rat(8/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(8/5){8}{}&\rat(7/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(3/5){8}{}&\rat(17/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/5){9}{}&\rat(6/5){3}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(4/5){9}{}&\rat(6/5){3}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(4/5){9}{}&\rat(11/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(1/5){1}{}&\rat(9/5){7}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(1/5){1}{}&\rat(9/5){7}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(-1/5){9}{}&\rat(11/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(-4/5){1}{}&\rat(14/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 277
\orbit{3}{277}{107}
\h{277}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(19/2){1}{\spec{2}}&&\cnt{751}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(3/2){7}{}&\int(0){9}{}&\rat(5/2){2}{}&\ln{2}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(1){8}{}&\int(0){1}{}&\int(3){3}{}&\ln{2}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 278
\orbit{3}{278}{107}
\h{278}&\rat(49/10){9}{\spec{1}}&\rat(21/10){3}{}&\int(5){2}{\spec{1}}&&\cnt{735}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(-3/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\rat(6/5){2}{}&\rat(3/10){9}{}&\rat(5/2){3}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\rat(4/5){8}{}&\rat(7/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(19/10){9}{}&\rat(11/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(19/10){9}{}&\rat(3/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{14}&\rat(19/10){9}{}&\rat(-2/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(11/10){1}{}&\rat(2/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(3/2){5}{}&\rat(5/2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 279
\orbit{3}{279}{107}
\h{279}&\int(10){\10}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{655}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){6}{}&\int(0){2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(3){7}{}&\int(1){9}{}&\int(0){2}{}&\ln{2}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 280
\orbit{3}{280}{107}
\h{280}&\int(12){\12}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{935}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){5}{\spec{2}}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(4){6}{\spec{2}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(4){4}{\spec{2}}&\int(0){8}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{7}&\int(4){7}{}&\int(0){9}{}&\int(0){2}{}&\ln{1}&\cnt{360}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 281
\orbit{3}{281}{106}
\h{281}&\rat(8/5){8}{}&\rat(22/5){6}{\spec{2}}&\int(6){\6}{1}&&\cnt{679}&\bounds{106}{106}{1}{false}&&\cr
\l{1}&\int(1){5}{}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(3/5){8}{}&\rat(7/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(4/5){9}{}&\rat(11/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(4/5){9}{}&\rat(1/5){8}{}&\int(3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(1/5){1}{}&\rat(4/5){2}{\spec{1}}&\int(3){1}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(1/5){1}{}&\rat(4/5){2}{\spec{2}}&\int(3){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(-1/5){9}{}&\rat(6/5){8}{}&\int(3){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(-4/5){1}{}&\rat(9/5){2}{}&\int(3){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 282
\orbit{3}{282}{106}
\h{282}&\rat(18/5){8}{\spec{1}}&\rat(42/5){6}{\spec{3}}&\int(0){\0}{}&&\cnt{767}&\bounds{106}{106}{1}{false}&&\cr
\l{1}&\rat(4/5){4}{}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(9/5){9}{}&\rat(11/5){3}{}&\int(0){2}{}&\ln{1}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\rat(9/5){9}{}&\rat(11/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(1/5){1}{}&\rat(19/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 283
\orbit{3}{283}{104}
\h{283}&\rat(9/10){9}{}&\rat(81/10){3}{\spec{3}}&\int(3){2}{}&&\cnt{675}&\bounds{104}{104}{1}{false}&&\cr
\l{1}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(-1/5){8}{}&\rat(21/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(1/10){1}{}&\rat(39/10){7}{}&\int(0){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(-9/10){1}{}&\rat(39/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\rat(5/2){5}{}&\rat(3/2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 284
\orbit{3}{284}{104}
\h{284}&\rat(49/10){9}{\spec{1}}&\rat(41/10){3}{\spec{2}}&\int(3){2}{}&&\cnt{731}&\bounds{104}{104}{1}{false}&&\cr
\l{1}&\rat(8/5){6}{}&\rat(12/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(13/10){3}{}&\rat(17/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(9/5){8}{}&\rat(17/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(9/5){8}{}&\rat(7/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(4/5){8}{}&\rat(17/10){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(19/10){9}{}&\rat(11/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(19/10){9}{}&\rat(3/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(12/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(7/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(1/10){1}{}&\rat(12/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 285
\orbit{3}{285}{104}
\h{285}&\int(6){\6}{\spec{1}}&\int(2){\2}{}&\int(4){\4}{2}&&\cnt{783}&\bounds{104}{104}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){7}{}&\int(0){9}{}&\int(2){2}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(0){1}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(1){7}{}&\int(1){9}{}&\int(2){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){3}{}&\int(1){1}{}&\int(2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\int(1){9}{}&\int(1){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){9}{}&\int(0){3}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){9}{}&\int(0){3}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(2){9}{}&\int(1){8}{}&\int(1){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\int(1){1}{}&\int(1){7}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 286
\orbit{3}{286}{103}
\h{286}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(8){\8}{0}&&\cnt{527}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(2/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(4/5){9}{}&\rat(6/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(4/5){9}{}&\rat(6/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){5}{}&\int(2){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 287
\orbit{3}{287}{103}
\h{287}&\rat(18/5){8}{\spec{1}}&\rat(42/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{775}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\rat(6/5){6}{}&\rat(14/5){2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(2/5){2}{}&\rat(18/5){4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(9/5){9}{}&\rat(11/5){3}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(9/5){9}{}&\rat(11/5){3}{\spec{3}}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(9/5){9}{}&\rat(11/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 288
\orbit{3}{288}{102}
\h{288}&\rat(9/10){9}{}&\rat(18/5){8}{\spec{1}}&\rat(15/2){1}{\spec{1}}&&\cnt{831}&\bounds{102}{102}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(9/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(1/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(1/5){2}{}&\rat(9/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(-4/5){2}{}&\rat(9/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{\spec{1}}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{\spec{2}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(1){5}{}&\int(3){3}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 289
\orbit{3}{289}{101}
\h{289}&\rat(69/10){9}{\spec{2}}&\rat(18/5){8}{\spec{1}}&\rat(3/2){1}{}&&\cnt{675}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(7/2){5}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(5/2){5}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(18/5){6}{}&\rat(2/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(12/5){4}{\spec{1}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(12/5){4}{\spec{2}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(33/10){3}{}&\rat(1/5){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(27/10){7}{}&\rat(9/5){9}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(17/10){7}{}&\rat(9/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{}&\rat(9/5){9}{}&\int(0){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(6/5){2}{}&\rat(9/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 290
\orbit{3}{290}{100}
\h{290}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&\int(6){\6}{3}&&\cnt{767}&\bounds{100}{100}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{210}&\bounds{35}{35}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(1){8}{}&\int(0){1}{}&\int(3){3}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\int(0){9}{}&\int(3){3}{}&\ln{1}&\cnt{140}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\int(2){9}{}&\int(0){8}{}&\int(2){1}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 291
\orbit{3}{291}{100}
\h{291}&\int(8){\8}{\spec{2}}&\int(0){\0}{}&\int(4){\4}{2}&&\cnt{831}&\bounds{100}{100}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){5}{\spec{3}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(2){7}{\spec{2}}&\int(0){9}{}&\int(2){2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(2){7}{\spec{3}}&\int(0){9}{}&\int(2){2}{}&\ln{1}&\cnt{30}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){3}{\spec{3}}&\int(0){1}{}&\int(2){2}{}&\ln{1}&\cnt{150}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{4}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){9}{}&\int(0){3}{}&\int(2){2}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{11}&\int(0){\0}{\spec{2}}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 292
\orbit{3}{292}{100}
\h{292}&\rat(21/10){7}{}&\rat(32/5){4}{\spec{2}}&\rat(7/2){1}{}&&\cnt{675}&\bounds{100}{100}{1}{false}&&\cr
\l{1}&\rat(4/5){6}{}&\rat(16/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(21/10){7}{}&\rat(2/5){9}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(9/10){3}{}&\rat(8/5){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(2/5){8}{}&\rat(8/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(3/10){1}{}&\rat(16/5){2}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(3/10){1}{}&\rat(16/5){2}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(-3/10){9}{}&\rat(14/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(-7/10){1}{}&\rat(16/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){5}{\spec{1}}&\int(2){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 293
\orbit{3}{293}{99}
\h{293}&\rat(28/5){8}{\spec{1}}&\rat(32/5){6}{\spec{2}}&\int(0){\0}{}&&\cnt{711}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(4/5){4}{\spec{1}}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(4/5){4}{\spec{2}}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(12/5){7}{}&\rat(8/5){9}{}&\int(0){2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{8}&\rat(6/5){1}{}&\rat(14/5){7}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(4/5){9}{}&\rat(16/5){8}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 294
\orbit{3}{294}{99}
\h{294}&\int(2){\2}{}&\int(2){\2}{}&\int(8){\8}{0}&&\cnt{651}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(1){7}{}&\int(1){9}{}&\int(2){2}{}&\ln{4}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(1){8}{}&\int(1){1}{}&\int(2){3}{}&\ln{4}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 295
\orbit{3}{295}{98}
\h{295}&\rat(9/10){9}{}&\rat(101/10){3}{\spec{4}}&\int(1){2}{}&&\cnt{695}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(23/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(4/5){8}{}&\rat(16/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(1/5){2}{}&\rat(19/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(31/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(21/10){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(29/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(-1/10){9}{}&\rat(31/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\rat(7/2){5}{}&\rat(1/2){3}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 296
\orbit{3}{296}{98}
\h{296}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(19/2){1}{\spec{2}}&&\cnt{751}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\rat(7/10){7}{}&\rat(4/5){9}{}&\rat(5/2){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(4/5){8}{}&\rat(1/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(1/5){2}{}&\rat(4/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(3/5){3}{}&\rat(5/2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(7/5){7}{}&\rat(5/2){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(1){5}{}&\int(3){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 297
\orbit{3}{297}{98}
\h{297}&\rat(29/10){9}{\spec{2}}&\rat(18/5){8}{\spec{1}}&\rat(11/2){1}{}&&\cnt{731}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\rat(3/2){5}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(17/10){7}{}&\rat(9/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(7/10){7}{\spec{1}}&\rat(9/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(7/10){7}{\spec{2}}&\rat(9/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(6/5){2}{}&\rat(9/5){9}{}&\int(1){3}{\spec{1}}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(6/5){2}{}&\rat(9/5){9}{}&\int(1){3}{\spec{2}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(1/5){2}{\spec{1}}&\rat(9/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(1/5){2}{\spec{2}}&\rat(9/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(11/10){1}{}&\rat(2/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(9/10){9}{}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(-1/10){9}{}&\rat(8/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 298
\orbit{3}{298}{96}
\h{298}&\rat(9/10){9}{}&\rat(48/5){8}{\spec{2}}&\rat(3/2){1}{}&&\cnt{639}&\bounds{96}{96}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(16/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(4/5){8}{}&\rat(11/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(13/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(13/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(9/10){9}{}&\rat(8/5){8}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(9/10){9}{}&\rat(8/5){8}{\spec{3}}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(1/10){1}{}&\rat(17/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(1/10){1}{}&\rat(12/5){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(-1/10){9}{}&\rat(13/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(3){5}{}&\int(1){3}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 299
\orbit{3}{299}{96}
\h{299}&\rat(8/5){8}{}&\rat(22/5){6}{\spec{1}}&\int(6){\6}{3}&&\cnt{671}&\bounds{96}{96}{1}{false}&&\cr
\l{1}&\rat(7/5){7}{}&\rat(8/5){9}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(-3/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(3/5){8}{}&\rat(2/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\rat(2/5){2}{}&\rat(3/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(-3/5){2}{}&\rat(8/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(4/5){9}{}&\rat(6/5){8}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/5){9}{}&\rat(6/5){8}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(1/5){1}{}&\rat(14/5){7}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(-1/5){9}{}&\rat(11/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(1){5}{}&\int(3){3}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 300
\orbit{3}{300}{95}
\h{300}&\rat(18/5){8}{\spec{1}}&\rat(12/5){6}{}&\int(6){\6}{3}&&\cnt{663}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(-3/5){1}{}&\int(3){3}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(2/5){2}{}&\rat(3/5){9}{}&\int(3){3}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(9/5){9}{}&\rat(6/5){3}{}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(9/5){9}{}&\rat(1/5){8}{}&\int(2){1}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(1){5}{}&\int(3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 301
\orbit{3}{301}{95}
\h{301}&\int(8){\8}{}&\int(0){\0}{}&\int(4){\4}{2}&&\cnt{655}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(3){5}{\spec{1}}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(2){7}{}&\int(0){9}{}&\int(2){2}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 302
\orbit{3}{302}{95}
\h{302}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{651}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){7}{}&\int(1){9}{}&\int(1){2}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){8}{}&\int(1){1}{}&\int(1){3}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){9}{}&\int(1){3}{}&\int(1){2}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){9}{}&\int(1){8}{}&\int(1){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 303
\orbit{3}{303}{94}
\h{303}&\rat(41/10){7}{\spec{1}}&\rat(32/5){4}{\spec{2}}&\rat(3/2){1}{}&&\cnt{663}&\bounds{94}{94}{1}{false}&&\cr
\l{1}&\rat(4/5){6}{}&\rat(16/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(12/5){8}{}&\rat(8/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(12/5){8}{}&\rat(8/5){1}{}&\int(0){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(7/5){8}{}&\rat(8/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(17/10){9}{}&\rat(14/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(17/10){9}{}&\rat(4/5){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(7/10){9}{}&\rat(14/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(3/10){1}{}&\rat(16/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(-7/10){1}{}&\rat(16/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 304
\orbit{3}{304}{94}
\h{304}&\rat(89/10){9}{\spec{2}}&\rat(21/10){3}{}&\int(1){2}{}&&\cnt{583}&\bounds{94}{94}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(13/5){6}{\spec{2}}&\rat(7/5){2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(27/10){7}{\spec{2}}&\rat(3/10){9}{}&\int(1){2}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(23/10){3}{\spec{2}}&\rat(7/10){1}{}&\int(1){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(14/5){8}{}&\rat(6/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\rat(14/5){8}{}&\rat(7/10){1}{}&\rat(1/2){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{\spec{2}}&\rat(9/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{13}&\rat(21/10){1}{}&\rat(9/10){7}{}&\int(1){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{14}&\rat(21/10){1}{}&\rat(7/5){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(19/10){9}{}&\rat(21/10){3}{}&\int(0){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(19/10){9}{}&\rat(11/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(9/10){9}{\spec{2}}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 305
\orbit{3}{305}{93}
\h{305}&\rat(8/5){8}{}&\rat(32/5){6}{\spec{2}}&\int(4){\4}{2}&&\cnt{655}&\bounds{93}{93}{1}{false}&&\cr
\l{1}&\rat(4/5){4}{}&\rat(16/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\rat(2/5){7}{}&\rat(8/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(8/5){8}{}&\rat(12/5){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(4/5){9}{}&\rat(6/5){3}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(-1/5){9}{}&\rat(16/5){8}{}&\int(1){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(-4/5){1}{}&\rat(14/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{\spec{2}}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 306
\orbit{3}{306}{93}
\h{306}&\int(6){\6}{}&\int(0){\0}{}&\int(6){\6}{3}&&\cnt{663}&\bounds{93}{93}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){5}{\spec{1}}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){7}{}&\int(0){9}{}&\int(1){2}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{5}&\int(1){8}{}&\int(0){1}{}&\int(3){3}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 307
\orbit{3}{307}{92}
\h{307}&\rat(89/10){9}{\spec{2}}&\rat(8/5){8}{}&\rat(3/2){1}{}&&\cnt{583}&\bounds{92}{92}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(12/5){4}{\spec{2}}&\rat(8/5){8}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(27/10){7}{\spec{2}}&\rat(4/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(14/5){8}{}&\rat(6/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(14/5){8}{}&\rat(1/5){1}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(11/5){2}{\spec{2}}&\rat(4/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(21/10){1}{}&\rat(7/5){7}{}&\rat(1/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(21/10){1}{}&\rat(2/5){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(19/10){9}{}&\rat(3/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(9/10){9}{\spec{2}}&\rat(8/5){8}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 308
\orbit{3}{308}{91}
\h{308}&\rat(49/10){9}{\spec{1}}&\rat(18/5){8}{\spec{1}}&\rat(7/2){1}{}&&\cnt{719}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\rat(17/10){7}{}&\rat(9/5){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\rat(7/10){7}{}&\rat(9/5){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(9/5){8}{}&\rat(1/5){1}{}&\int(2){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(6/5){2}{}&\rat(9/5){9}{}&\int(1){3}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(1/5){2}{}&\rat(9/5){9}{}&\int(2){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(19/10){9}{}&\rat(3/5){3}{}&\rat(3/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(19/10){9}{}&\rat(8/5){8}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(11/10){1}{}&\rat(7/5){7}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 309
\orbit{3}{309}{91}
\h{309}&\rat(9/10){9}{}&\rat(48/5){8}{\spec{2}}&\rat(3/2){1}{}&&\cnt{663}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\rat(4/5){8}{}&\rat(16/5){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\rat(-4/5){2}{}&\rat(24/5){4}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(9/10){9}{}&\rat(18/5){3}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(8/5){8}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(1/10){1}{}&\rat(12/5){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(-1/10){9}{}&\rat(18/5){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){5}{}&\int(0){3}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 310
\orbit{3}{310}{91}
\h{310}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&\int(6){\6}{1}&&\cnt{767}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){5}{}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{420}&\bounds{42}{42}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(0){9}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(1){1}{}&\int(0){2}{}&\int(3){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 311
\orbit{3}{311}{90}
\h{311}&\rat(13/2){5}{\spec{2}}&\int(0){\0}{}&\rat(11/2){1}{}&&\cnt{719}&\bounds{90}{90}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){5}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\rat(3/2){5}{\spec{2}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(7/2){7}{}&\int(0){9}{}&\rat(1/2){2}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(5/2){7}{}&\int(0){9}{}&\rat(3/2){2}{}&\ln{1}&\cnt{140}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{3}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{4}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(3){8}{}&\int(0){1}{}&\int(1){3}{\spec{2}}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(0){1}{}&\int(2){3}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(3/2){9}{}&\int(0){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\int(0){\0}{\spec{2}}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 312
\orbit{3}{312}{90}
\h{312}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(9){2}{\spec{3}}&&\cnt{639}&\bounds{90}{90}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(4/5){8}{}&\rat(7/10){1}{}&\rat(5/2){3}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(9/10){9}{}&\rat(21/10){3}{}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(9/10){9}{}&\rat(11/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(9/10){9}{}&\rat(3/5){8}{}&\rat(5/2){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(1/10){1}{}&\rat(7/5){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(-1/10){9}{}&\rat(21/10){3}{}&\int(2){2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\rat(3/2){5}{}&\rat(5/2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 313
\orbit{3}{313}{87}
\h{313}&\int(12){\12}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{543}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{180}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 314
\orbit{3}{314}{85}
\h{314}&\rat(5/2){5}{}&\int(8){\8}{\spec{1}}&\rat(3/2){1}{}&&\cnt{527}&\bounds{85}{85}{1}{false}&&\cr
\l{1}&\rat(5/2){5}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(3/2){7}{}&\int(2){9}{}&\rat(1/2){2}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\int(1){8}{}&\int(2){1}{}&\int(1){3}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(1/2){9}{}&\int(2){8}{}&\rat(3/2){1}{}&\ln{2}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 315
\orbit{3}{315}{79}
\h{315}&\rat(18/5){8}{\spec{1}}&\rat(22/5){6}{\spec{1}}&\int(4){\4}{2}&&\cnt{655}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\rat(7/5){7}{}&\rat(3/5){9}{}&\int(2){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(8/5){8}{}&\rat(12/5){6}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(9/5){9}{}&\rat(1/5){3}{}&\int(2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(9/5){9}{}&\rat(6/5){8}{\spec{1}}&\int(1){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(9/5){9}{}&\rat(6/5){8}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\rat(1/5){1}{}&\rat(9/5){7}{}&\int(2){2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 316
\orbit{3}{316}{75}
\h{316}&\int(0){\0}{}&\int(0){\0}{}&\int(12){\12}{2}&&\cnt{579}&\bounds{75}{75}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*A[9] + D[6]
% Class 317
\orbit{3}{317}{67}
\h{317}&\int(0){\0}{}&\int(0){\0}{}&\int(12){\12}{}&&\cnt{555}&\bounds{67}{67}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_2D12.tex <==
% -*- TeX -*-
% Niemeier lattice 2D12
% 34 classes
\newcs{max-2D12}{194}%
\newcs{count-2D12}{34}%
\newcs{counts-2D12}{\DO{1}{194}\DO{2}{193}\DO{3}{187}\DO{4}{187}\DO{5}{145}\DO{6}{143}\DO{7}{131}\DO{8}{130}\DO{9}{127}\DO{10}{123}\DO{11}{121}\DO{12}{119}\DO{13}{115}\DO{14}{115}\DO{15}{115}\DO{16}{114}\DO{17}{114}\DO{18}{111}\DO{19}{103}\DO{20}{103}\DO{21}{97}\DO{22}{97}\DO{23}{97}\DO{24}{95}\DO{25}{91}\DO{26}{90}\DO{27}{87}\DO{28}{87}\DO{29}{71}\DO{30}{67}\DO{31}{66}\DO{32}{62}\DO{33}{55}\DO{34}{54}}%
\orbits
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 1
\orbit{2}{1}{194}
\h{1}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&&\cnt{1675}&\bounds{194}{194}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{800}&\bounds{80}{80}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){2}{}&\int(1){1}{}&\ln{1}&\cnt{512}&\bounds{71}{71}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 2
\orbit{2}{2}{193}
\h{2}&\int(8){\8}{0}&\int(4){\4}{2}&&\cnt{1795}&\bounds{193}{193}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(2){2}{}&\ln{1}&\cnt{512}&\bounds{71}{71}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{880}&\bounds{80}{80}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 3
\orbit{2}{3}{187}
\h{3}&\int(12){\12}{\spec{3}}&\int(0){\0}{}&&\cnt{2079}&\bounds{187}{187}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\l{2}&\int(4){1}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{1584}&\bounds{132}{132}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 4
\orbit{2}{4}{187}
\h{4}&\int(9){2}{\spec{1}}&\int(3){1}{}&&\cnt{1947}&\bounds{187}{187}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{1452}&\bounds{132}{132}{1}{false}&&\cr
\l{2}&\int(3){2}{}&\int(1){1}{}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 5
\orbit{2}{5}{145}
\h{5}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&&\cnt{1063}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(2){2}{}&\ln{2}&\cnt{256}&\bounds{39}{39}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{2}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{2}}&\ln{2}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 6
\orbit{2}{6}{143}
\h{6}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&&\cnt{847}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){1}{}&\int(1){2}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){1}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 7
\orbit{2}{7}{131}
\h{7}&\int(3){2}{}&\int(9){1}{\spec{2}}&&\cnt{1231}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(3/2){1}{}&\rat(5/2){2}{}&\ln{1}&\cnt{256}&\bounds{39}{39}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{594}&\bounds{54}{54}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(0){2}{}&\int(4){1}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 8
\orbit{2}{8}{130}
\h{8}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&&\cnt{1251}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(4){1}{}&\int(0){2}{}&\ln{1}&\cnt{768}&\bounds{64}{64}{1}{false}&&\cr
\l{7}&\int(4){\2}{\spec{2}}&\int(0){\2}{}&\ln{1}&\cnt{264}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 9
\orbit{2}{9}{127}
\h{9}&\int(10){\10}{\spec{3}}&\int(2){\2}{}&&\cnt{943}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{4}&\int(4){1}{}&\int(0){2}{}&\ln{1}&\cnt{320}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(3){1}{}&\int(1){2}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{240}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 10
\orbit{2}{10}{123}
\h{10}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&&\cnt{1131}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{336}&\bounds{48}{48}{1}{false}&&\cr
\l{3}&\int(4){\2}{\spec{1}}&\int(0){\2}{}&\ln{1}&\cnt{792}&\bounds{72}{72}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 11
\orbit{2}{11}{121}
\h{11}&\int(12){\12}{2}&\int(0){\0}{}&&\cnt{1227}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{432}&\bounds{48}{48}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{792}&\bounds{72}{72}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 12
\orbit{2}{12}{119}
\h{12}&\int(8){\8}{}&\int(4){\4}{2}&&\cnt{1087}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){1}{}&\int(0){2}{}&\ln{1}&\cnt{176}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(2){2}{}&\ln{1}&\cnt{224}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{616}&\bounds{56}{56}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 13
\orbit{2}{13}{115}
\h{13}&\int(9){3}{\spec{1}}&\int(3){3}{}&&\cnt{1243}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\rat(7/2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{132}&\bounds{11}{11}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{726}&\bounds{66}{66}{1}{false}&&\cr
\l{4}&\rat(5/2){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 14
\orbit{2}{14}{115}
\h{14}&\int(1){2}{}&\int(11){1}{\spec{2}}&&\cnt{1051}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(1){2}{}&\int(3){1}{\spec{1}}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(1){2}{}&\int(3){1}{\spec{2}}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(0){2}{}&\int(4){1}{}&\ln{1}&\cnt{616}&\bounds{56}{56}{1}{false}&&\cr
\l{5}&\int(-1){2}{}&\int(5){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 15
\orbit{2}{15}{115}
\h{15}&\int(6){\6}{}&\int(6){\6}{}&&\cnt{639}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){1}{}&\int(1){2}{}&\ln{2}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 16
\orbit{2}{16}{114}
\h{16}&\int(8){\8}{0}&\int(4){\4}{}&&\cnt{803}&\bounds{114}{114}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{240}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\int(2){1}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 17
\orbit{2}{17}{114}
\h{17}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&&\cnt{779}&\bounds{114}{114}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){1}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 18
\orbit{2}{18}{111}
\h{18}&\int(6){\6}{\spec{1}}&\int(6){\6}{}&&\cnt{719}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\int(2){1}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 19
\orbit{2}{19}{103}
\h{19}&\int(8){\8}{\spec{1}}&\int(4){\4}{2}&&\cnt{783}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\int(2){2}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{308}&\bounds{28}{28}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 20
\orbit{2}{20}{103}
\h{20}&\int(12){\12}{\spec{3}}&\int(0){\0}{}&&\cnt{1007}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(4){1}{\spec{1}}&\int(0){2}{}&\ln{1}&\cnt{768}&\bounds{64}{64}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 21
\orbit{2}{21}{97}
\h{21}&\int(1){2}{}&\int(11){1}{\spec{1}}&&\cnt{991}&\bounds{97}{97}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(1){2}{}&\int(3){1}{\spec{1}}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\int(3){1}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(0){2}{}&\int(4){1}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 22
\orbit{2}{22}{97}
\h{22}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&&\cnt{839}&\bounds{97}{97}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(5){1}{}&\int(-1){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){1}{}&\int(0){2}{}&\ln{1}&\cnt{400}&\bounds{40}{40}{1}{false}&&\cr
\l{4}&\int(3){1}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 23
\orbit{2}{23}{97}
\h{23}&\int(3){2}{}&\int(9){1}{\spec{1}}&&\cnt{783}&\bounds{97}{97}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(1){2}{}&\int(3){1}{\spec{1}}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\int(3){1}{\spec{2}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(0){2}{}&\int(4){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 24
\orbit{2}{24}{95}
\h{24}&\int(5){2}{\spec{1}}&\int(7){1}{}&&\cnt{827}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{400}&\bounds{40}{40}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(2){1}{\spec{1}}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){1}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\int(0){2}{}&\int(4){1}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 25
\orbit{2}{25}{91}
\h{25}&\int(9){2}{\spec{3}}&\int(3){1}{}&&\cnt{911}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(7/2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{384}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{330}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\int(2){1}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 26
\orbit{2}{26}{90}
\h{26}&\int(7){2}{\spec{1}}&\int(5){1}{}&&\cnt{783}&\bounds{90}{90}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/2){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{176}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){1}{\spec{1}}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(2){1}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 27
\orbit{2}{27}{87}
\h{27}&\int(8){\8}{}&\int(4){\4}{}&&\cnt{623}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){1}{}&\int(0){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(3){1}{}&\int(1){2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 28
\orbit{2}{28}{87}
\h{28}&\int(5){2}{\spec{2}}&\int(7){1}{}&&\cnt{687}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{6}&\int(0){2}{}&\int(4){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 29
\orbit{2}{29}{71}
\h{29}&\int(9){3}{\spec{2}}&\int(3){3}{}&&\cnt{795}&\bounds{71}{71}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(9/2){1}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(7/2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{432}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(3/2){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{36}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 30
\orbit{2}{30}{67}
\h{30}&\int(7){2}{\spec{2}}&\int(5){1}{}&&\cnt{631}&\bounds{67}{67}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(7/2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{176}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(5/2){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{231}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 31
\orbit{2}{31}{66}
\h{31}&\int(7){3}{}&\int(5){3}{}&&\cnt{683}&\bounds{66}{66}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(7/2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(5/2){1}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{4}&\rat(5/2){1}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(1/2){2}{}&\rat(7/2){1}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 32
\orbit{2}{32}{62}
\h{32}&\int(9){2}{\spec{4}}&\int(3){1}{}&&\cnt{615}&\bounds{62}{62}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(9/2){1}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{48}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(7/2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{432}&\bounds{36}{36}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 33
\orbit{2}{33}{55}
\h{33}&\int(12){\12}{\spec{1}}&\int(0){\0}{}&&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 2*D[12]
% Class 34
\orbit{2}{34}{54}
\h{34}&\int(9){2}{\spec{2}}&\int(3){1}{}&&\cnt{543}&\bounds{54}{54}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(2){1}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_3A8.tex <==
% -*- TeX -*-
% Niemeier lattice 3A8
% 181 classes
\newcs{max-3A8}{193}%
\newcs{count-3A8}{181}%
\newcs{counts-3A8}{\DO{1}{193}\DO{2}{193}\DO{3}{189}\DO{4}{183}\DO{5}{180}\DO{6}{177}\DO{7}{177}\DO{8}{171}\DO{9}{169}\DO{10}{169}\DO{11}{168}\DO{12}{167}\DO{13}{167}\DO{14}{166}\DO{15}{165}\DO{16}{165}\DO{17}{165}\DO{18}{163}\DO{19}{162}\DO{20}{160}\DO{21}{159}\DO{22}{159}\DO{23}{159}\DO{24}{159}\DO{25}{159}\DO{26}{158}\DO{27}{158}\DO{28}{157}\DO{29}{157}\DO{30}{157}\DO{31}{155}\DO{32}{155}\DO{33}{155}\DO{34}{155}\DO{35}{154}\DO{36}{154}\DO{37}{152}\DO{38}{151}\DO{39}{151}\DO{40}{151}\DO{41}{151}\DO{42}{151}\DO{43}{151}\DO{44}{151}\DO{45}{151}\DO{46}{150}\DO{47}{150}\DO{48}{150}\DO{49}{150}\DO{50}{149}\DO{51}{149}\DO{52}{147}\DO{53}{147}\DO{54}{147}\DO{55}{147}\DO{56}{147}\DO{57}{146}\DO{58}{145}\DO{59}{145}\DO{60}{145}\DO{61}{145}\DO{62}{144}\DO{63}{144}\DO{64}{144}\DO{65}{143}\DO{66}{143}\DO{67}{143}\DO{68}{143}\DO{69}{143}\DO{70}{143}\DO{71}{143}\DO{72}{143}\DO{73}{143}\DO{74}{143}\DO{75}{141}\DO{76}{141}\DO{77}{141}\DO{78}{141}\DO{79}{141}\DO{80}{141}\DO{81}{141}\DO{82}{141}\DO{83}{139}\DO{84}{139}\DO{85}{139}\DO{86}{139}\DO{87}{138}\DO{88}{138}\DO{89}{138}\DO{90}{137}\DO{91}{137}\DO{92}{137}\DO{93}{137}\DO{94}{137}\DO{95}{136}\DO{96}{136}\DO{97}{136}\DO{98}{136}\DO{99}{135}\DO{100}{135}\DO{101}{134}\DO{102}{134}\DO{103}{133}\DO{104}{133}\DO{105}{133}\DO{106}{133}\DO{107}{133}\DO{108}{133}\DO{109}{133}\DO{110}{133}\DO{111}{133}\DO{112}{132}\DO{113}{132}\DO{114}{132}\DO{115}{131}\DO{116}{131}\DO{117}{131}\DO{118}{131}\DO{119}{130}\DO{120}{130}\DO{121}{130}\DO{122}{130}\DO{123}{129}\DO{124}{129}\DO{125}{129}\DO{126}{129}\DO{127}{129}\DO{128}{129}\DO{129}{128}\DO{130}{127}\DO{131}{127}\DO{132}{127}\DO{133}{127}\DO{134}{126}\DO{135}{123}\DO{136}{123}\DO{137}{123}\DO{138}{123}\DO{139}{122}\DO{140}{122}\DO{141}{121}\DO{142}{120}\DO{143}{120}\DO{144}{120}\DO{145}{119}\DO{146}{118}\DO{147}{116}\DO{148}{116}\DO{149}{116}\DO{150}{115}\DO{151}{115}\DO{152}{115}\DO{153}{114}\DO{154}{113}\DO{155}{113}\DO{156}{113}\DO{157}{113}\DO{158}{113}\DO{159}{112}\DO{160}{111}\DO{161}{110}\DO{162}{110}\DO{163}{110}\DO{164}{110}\DO{165}{108}\DO{166}{106}\DO{167}{105}\DO{168}{105}\DO{169}{105}\DO{170}{103}\DO{171}{102}\DO{172}{101}\DO{173}{101}\DO{174}{101}\DO{175}{100}\DO{176}{98}\DO{177}{97}\DO{178}{96}\DO{179}{90}\DO{180}{89}\DO{181}{72}}%
\orbits
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 1
\orbit{3}{1}{193}
\h{1}&\int(12){\12}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1515}&\bounds{193}{193}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){5}{}&\int(0){8}{}&\int(0){8}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{4}&\int(4){4}{}&\int(0){1}{}&\int(0){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(4){6}{}&\int(0){3}{}&\int(0){\0}{}&\ln{2}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{6}&\int(4){7}{}&\int(0){7}{}&\int(0){1}{}&\ln{2}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 2
\orbit{3}{2}{193}
\h{2}&\rat(68/9){7}{\spec{1}}&\rat(20/9){4}{}&\rat(20/9){4}{}&&\cnt{935}&\bounds{193}{193}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(28/9){5}{\spec{1}}&\rat(4/9){8}{}&\rat(4/9){8}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(26/9){4}{\spec{1}}&\rat(5/9){1}{}&\rat(5/9){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(8/3){3}{\spec{1}}&\rat(4/3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(7/3){6}{\spec{1}}&\rat(5/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(22/9){2}{\spec{1}}&\rat(10/9){2}{}&\rat(4/9){8}{}&\ln{2}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(20/9){1}{}&\rat(20/9){4}{}&\rat(-4/9){1}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(20/9){1}{}&\rat(11/9){4}{}&\rat(5/9){1}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(20/9){1}{}&\rat(8/9){7}{}&\rat(8/9){7}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 3
\orbit{3}{3}{189}
\h{3}&\int(4){6}{\spec{2}}&\int(4){6}{\spec{2}}&\int(4){6}{\spec{2}}&&\cnt{711}&\bounds{189}{189}{1}{false}&&\cr
\l{1}&\rat(8/3){5}{}&\rat(2/3){8}{}&\rat(2/3){8}{}&\ln{3}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/3){4}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\ln{6}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(4/3){4}{\spec{1}}&\rat(4/3){1}{}&\rat(4/3){1}{}&\ln{3}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(4/3){4}{\spec{2}}&\rat(4/3){1}{}&\rat(4/3){1}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{6}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(5/3){2}{}&\rat(5/3){2}{}&\rat(2/3){8}{}&\ln{3}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(4/3){7}{}&\rat(4/3){7}{}&\rat(4/3){1}{}&\ln{3}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 4
\orbit{3}{4}{183}
\h{4}&\int(8){6}{\spec{4}}&\int(2){6}{}&\int(2){6}{}&&\cnt{1143}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{144}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\rat(7/3){7}{}&\rat(4/3){7}{}&\rat(1/3){1}{}&\ln{2}&\cnt{144}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\rat(8/3){8}{}&\rat(5/3){5}{}&\rat(-1/3){8}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(8/3){8}{}&\rat(2/3){5}{}&\rat(2/3){8}{}&\ln{2}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{}&\rat(2/3){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 5
\orbit{3}{5}{180}
\h{5}&\rat(68/9){7}{\spec{1}}&\rat(20/9){4}{}&\rat(20/9){4}{}&&\cnt{823}&\bounds{180}{180}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(28/9){5}{\spec{2}}&\rat(4/9){8}{}&\rat(4/9){8}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(26/9){4}{\spec{2}}&\rat(5/9){1}{}&\rat(5/9){1}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(10/3){6}{}&\rat(2/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(8/3){3}{\spec{2}}&\rat(4/3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(7/3){6}{\spec{2}}&\rat(5/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(23/9){7}{}&\rat(8/9){7}{}&\rat(5/9){1}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(22/9){2}{\spec{2}}&\rat(10/9){2}{}&\rat(4/9){8}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(16/9){8}{}&\rat(16/9){5}{}&\rat(4/9){8}{}&\ln{2}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(16/9){8}{}&\rat(10/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(11/9){1}{}&\rat(20/9){4}{}&\rat(5/9){1}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 6
\orbit{3}{6}{177}
\h{6}&\rat(44/9){8}{\spec{2}}&\rat(44/9){8}{\spec{2}}&\rat(20/9){5}{}&&\cnt{711}&\bounds{177}{177}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(22/9){4}{}&\rat(10/9){1}{}&\rat(4/9){1}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(8/3){6}{}&\rat(4/3){3}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/3){6}{}&\rat(4/3){3}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(7/3){3}{}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(7/3){3}{}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(20/9){2}{}&\rat(20/9){2}{}&\rat(-4/9){8}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(20/9){2}{}&\rat(11/9){2}{}&\rat(5/9){8}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(16/9){7}{}&\rat(16/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{}&\ln{2}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 7
\orbit{3}{7}{177}
\h{7}&\int(8){6}{\spec{1}}&\int(2){6}{}&\int(2){6}{}&&\cnt{987}&\bounds{177}{177}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(8/3){5}{}&\rat(2/3){8}{}&\rat(2/3){8}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{2}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(8/3){2}{}&\rat(2/3){2}{}&\rat(2/3){8}{}&\ln{2}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{8}&\rat(7/3){1}{}&\rat(4/3){4}{}&\rat(1/3){1}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(7/3){1}{}&\rat(4/3){7}{}&\rat(1/3){7}{}&\ln{2}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 8
\orbit{3}{8}{171}
\h{8}&\rat(32/9){7}{\spec{2}}&\rat(56/9){4}{\spec{1}}&\rat(20/9){4}{}&&\cnt{767}&\bounds{171}{171}{1}{false}&&\cr
\l{1}&\rat(19/9){5}{}&\rat(13/9){8}{}&\rat(4/9){8}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(17/9){4}{}&\rat(14/9){1}{}&\rat(5/9){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(7/3){6}{}&\rat(5/3){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(7/3){6}{}&\rat(5/3){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(7/3){6}{}&\int(0){\0}{}&\rat(5/3){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(5/3){3}{}&\rat(7/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(13/9){2}{}&\rat(19/9){2}{}&\rat(4/9){8}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\rat(13/9){2}{}&\rat(13/9){8}{}&\rat(10/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(11/9){1}{}&\rat(29/9){4}{}&\rat(-4/9){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(11/9){1}{}&\rat(20/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(11/9){1}{}&\rat(17/9){7}{}&\rat(8/9){7}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(11/9){1}{}&\rat(14/9){1}{}&\rat(11/9){4}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(11/9){1}{}&\rat(5/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(7/9){8}{}&\rat(19/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{23}&\rat(7/9){8}{}&\rat(13/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\rat(2/9){1}{}&\rat(29/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{25}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 9
\orbit{3}{9}{169}
\h{9}&\int(4){6}{\spec{2}}&\int(4){3}{\spec{1}}&\int(4){\4}{}&&\cnt{711}&\bounds{169}{169}{1}{false}&&\cr
\l{1}&\rat(8/3){5}{}&\rat(4/3){8}{}&\int(0){8}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(8/3){5}{}&\rat(1/3){8}{}&\int(1){8}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(7/3){4}{}&\rat(2/3){1}{}&\int(1){1}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(5/3){5}{}&\rat(4/3){8}{}&\int(1){8}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\int(0){\0}{}&\int(2){6}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(5/3){2}{}&\rat(4/3){8}{}&\int(1){2}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(5/3){2}{}&\rat(1/3){8}{}&\int(2){2}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(2/3){2}{\spec{1}}&\rat(4/3){8}{}&\int(2){2}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(2/3){2}{\spec{2}}&\rat(4/3){8}{}&\int(2){2}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\rat(2/3){1}{}&\int(2){4}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 10
\orbit{3}{10}{169}
\h{10}&\int(4){6}{\spec{2}}&\int(2){3}{}&\int(6){\6}{}&&\cnt{707}&\bounds{169}{169}{1}{false}&&\cr
\l{1}&\rat(8/3){5}{}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(7/3){4}{}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(1){6}{}&\int(0){\0}{}&\int(3){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\int(3){6}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\int(3){6}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\rat(5/3){2}{}&\rat(1/3){8}{}&\int(2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(4/3){1}{}&\rat(5/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(4/3){1}{}&\rat(2/3){7}{}&\int(2){7}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{}&\rat(2/3){1}{}&\int(2){4}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(4/3){1}{}&\rat(2/3){1}{}&\int(2){4}{\spec{2}}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\rat(-1/3){1}{}&\int(3){4}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(2/3){8}{}&\rat(4/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\rat(2/3){8}{}&\rat(1/3){8}{}&\int(3){5}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(1/3){1}{}&\rat(2/3){1}{}&\int(3){4}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(1){6}{}&\int(3){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(1){3}{}&\int(3){6}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 11
\orbit{3}{11}{168}
\h{11}&\rat(14/9){7}{}&\rat(74/9){4}{\spec{2}}&\rat(20/9){4}{}&&\cnt{1091}&\bounds{168}{168}{1}{false}&&\cr
\l{1}&\rat(8/9){4}{}&\rat(23/9){1}{}&\rat(5/9){1}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\rat(4/3){6}{}&\rat(8/3){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(23/9){1}{}&\rat(-1/9){7}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(5/9){7}{}&\rat(23/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(4/9){2}{}&\rat(28/9){2}{}&\rat(4/9){8}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(7/9){8}{}&\rat(28/9){2}{}&\rat(1/9){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(7/9){8}{}&\rat(19/9){2}{\spec{1}}&\rat(10/9){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(2/9){1}{}&\rat(23/9){1}{}&\rat(11/9){4}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(-2/9){8}{}&\rat(28/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(-7/9){1}{}&\rat(23/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\rat(8/3){3}{\spec{1}}&\rat(4/3){6}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 12
\orbit{3}{12}{167}
\h{12}&\rat(62/9){8}{\spec{1}}&\rat(26/9){8}{\spec{2}}&\rat(20/9){5}{}&&\cnt{875}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{\spec{1}}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(22/9){4}{\spec{1}}&\rat(10/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(8/3){6}{\spec{1}}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{\spec{1}}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(7/3){3}{\spec{1}}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(7/3){3}{\spec{1}}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(20/9){2}{\spec{1}}&\rat(11/9){2}{}&\rat(5/9){8}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\rat(20/9){2}{\spec{1}}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{14}&\rat(16/9){7}{\spec{1}}&\rat(16/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(16/9){7}{\spec{1}}&\rat(10/9){1}{}&\rat(10/9){7}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(19/9){1}{}&\rat(13/9){4}{}&\rat(4/9){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{17}&\rat(19/9){1}{}&\rat(16/9){7}{}&\rat(1/9){7}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(19/9){1}{}&\rat(7/9){7}{}&\rat(10/9){7}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(19/9){1}{}&\rat(10/9){1}{}&\rat(7/9){4}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(19/9){1}{}&\rat(1/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\rat(8/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 13
\orbit{3}{13}{167}
\h{13}&\int(8){6}{\spec{2}}&\int(2){6}{}&\int(2){6}{}&&\cnt{819}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(11/3){5}{}&\rat(2/3){8}{}&\rat(-1/3){8}{}&\ln{2}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(10/3){4}{\spec{2}}&\rat(1/3){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(8/3){5}{\spec{2}}&\rat(2/3){8}{}&\rat(2/3){8}{}&\ln{1}&\cnt{81}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{2}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(2){3}{\spec{2}}&\int(2){6}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(2){3}{\spec{3}}&\int(2){6}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(8/3){2}{\spec{2}}&\rat(2/3){2}{}&\rat(2/3){8}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(7/3){7}{}&\rat(4/3){7}{}&\rat(1/3){1}{}&\ln{2}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(5/3){8}{}&\rat(5/3){5}{}&\rat(2/3){8}{}&\ln{2}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{\spec{2}}&\rat(4/3){7}{}&\rat(4/3){7}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 14
\orbit{3}{14}{166}
\h{14}&\rat(44/9){8}{\spec{2}}&\rat(32/9){2}{\spec{1}}&\rat(32/9){2}{\spec{1}}&&\cnt{711}&\bounds{166}{166}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{}&\rat(11/9){8}{}&\rat(2/9){8}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(22/9){4}{}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\rat(14/9){5}{\spec{1}}&\rat(11/9){8}{}&\rat(11/9){8}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(14/9){5}{\spec{2}}&\rat(11/9){8}{}&\rat(11/9){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(8/3){6}{}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(7/3){3}{}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(20/9){2}{}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(20/9){2}{}&\rat(5/9){2}{}&\rat(11/9){8}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(11/9){2}{}&\rat(14/9){2}{}&\rat(11/9){8}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(10/9){1}{}&\rat(13/9){7}{}&\rat(13/9){7}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(8/9){8}{}&\rat(17/9){5}{}&\rat(11/9){8}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 15
\orbit{3}{15}{165}
\h{15}&\rat(14/9){7}{}&\rat(74/9){4}{\spec{3}}&\rat(20/9){4}{}&&\cnt{1039}&\bounds{165}{165}{1}{false}&&\cr
\l{1}&\rat(10/9){5}{}&\rat(22/9){8}{}&\rat(4/9){8}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(2/3){3}{}&\rat(10/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(26/9){7}{}&\rat(-4/9){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(5/9){7}{}&\rat(26/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(4/9){2}{}&\rat(22/9){8}{}&\rat(10/9){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(7/9){8}{}&\rat(22/9){8}{}&\rat(7/9){5}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(2/9){1}{}&\rat(26/9){7}{}&\rat(8/9){7}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(-2/9){8}{}&\rat(22/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(10/3){6}{}&\rat(2/3){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 16
\orbit{3}{16}{165}
\h{16}&\int(2){6}{}&\int(2){3}{}&\int(8){\8}{\spec{2}}&&\cnt{875}&\bounds{165}{165}{1}{false}&&\cr
\l{1}&\rat(5/3){5}{}&\rat(1/3){8}{}&\int(2){8}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{\spec{3}}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(1){6}{}&\int(0){\0}{}&\int(3){3}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(1){3}{}&\int(0){\0}{}&\int(3){6}{\spec{2}}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{\spec{2}}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(4/3){7}{}&\rat(-1/3){1}{}&\int(3){7}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(2/3){2}{}&\rat(4/3){2}{}&\int(2){8}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(1/3){7}{}&\rat(2/3){1}{}&\int(3){7}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\rat(2/3){8}{}&\rat(4/3){5}{}&\int(2){8}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(2/3){8}{}&\rat(4/3){2}{}&\int(2){2}{\spec{2}}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(2/3){8}{}&\rat(1/3){8}{}&\int(3){5}{\spec{2}}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(1/3){1}{}&\rat(2/3){7}{}&\int(3){7}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\rat(1/3){1}{}&\rat(2/3){1}{}&\int(3){4}{\spec{2}}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{\spec{3}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(1){6}{}&\int(3){3}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(1){3}{}&\int(3){6}{\spec{2}}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{\spec{2}}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 17
\orbit{3}{17}{165}
\h{17}&\int(6){\6}{}&\int(6){\6}{}&\int(0){\0}{}&&\cnt{819}&\bounds{165}{165}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){5}{}&\int(1){8}{}&\int(0){8}{}&\ln{4}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\ln{4}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){6}{}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\ln{4}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{81}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\int(2){7}{}&\int(2){7}{}&\int(0){1}{}&\ln{2}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 18
\orbit{3}{18}{163}
\h{18}&\int(8){6}{\spec{1}}&\int(2){3}{}&\int(2){\2}{}&&\cnt{983}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(10/3){4}{}&\rat(-1/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/3){5}{}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(7/3){4}{}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(3){3}{}&\int(0){\0}{}&\int(1){6}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(8/3){2}{}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(8/3){2}{}&\rat(1/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(8/3){2}{}&\rat(1/3){8}{}&\int(1){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{16}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(7/3){1}{}&\rat(5/3){4}{}&\int(0){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(7/3){1}{}&\rat(2/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\rat(7/3){1}{}&\rat(2/3){7}{}&\int(1){7}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{20}&\rat(7/3){1}{}&\rat(2/3){1}{}&\int(1){4}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 19
\orbit{3}{19}{162}
\h{19}&\int(8){6}{\spec{4}}&\int(2){3}{}&\int(2){\2}{}&&\cnt{1139}&\bounds{162}{162}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(7/3){7}{}&\rat(2/3){7}{}&\int(1){1}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(7/3){7}{}&\rat(2/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{7}&\rat(8/3){8}{}&\rat(4/3){5}{}&\int(0){8}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(8/3){8}{}&\rat(1/3){5}{}&\int(1){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(8/3){8}{}&\rat(4/3){2}{}&\int(0){2}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(8/3){8}{}&\rat(4/3){2}{}&\int(0){2}{\spec{2}}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\rat(8/3){8}{}&\rat(1/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{12}&\rat(8/3){8}{}&\rat(1/3){8}{}&\int(1){5}{}&\ln{1}&\cnt{210}&\bounds{35}{35}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 20
\orbit{3}{20}{160}
\h{20}&\int(4){6}{\spec{2}}&\int(2){3}{}&\int(6){\6}{\spec{2}}&&\cnt{815}&\bounds{160}{160}{1}{false}&&\cr
\l{1}&\rat(8/3){5}{}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(7/3){4}{}&\rat(-1/3){1}{}&\int(2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(4/3){4}{\spec{1}}&\rat(2/3){1}{}&\int(2){1}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\rat(4/3){4}{\spec{2}}&\rat(2/3){1}{}&\int(2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(5/3){2}{}&\rat(1/3){8}{}&\int(2){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{13}&\rat(4/3){7}{}&\rat(2/3){7}{}&\int(2){1}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{}&\rat(2/3){4}{}&\int(2){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{16}&\rat(4/3){1}{}&\rat(2/3){7}{}&\int(2){7}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\rat(2/3){1}{}&\int(2){4}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(2/3){8}{}&\rat(4/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(1/3){1}{}&\rat(5/3){4}{}&\int(2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 21
\orbit{3}{21}{159}
\h{21}&\rat(62/9){8}{\spec{1}}&\rat(26/9){8}{\spec{2}}&\rat(20/9){5}{}&&\cnt{819}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(23/9){5}{\spec{2}}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(22/9){4}{\spec{2}}&\rat(10/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{\spec{2}}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(8/3){6}{\spec{2}}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(7/3){3}{\spec{2}}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(7/3){3}{\spec{2}}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(25/9){7}{}&\rat(16/9){7}{}&\rat(-5/9){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(25/9){7}{}&\rat(7/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(25/9){7}{}&\rat(10/9){1}{}&\rat(1/9){7}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(25/9){7}{}&\rat(1/9){1}{}&\rat(10/9){7}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(20/9){2}{\spec{2}}&\rat(11/9){2}{}&\rat(5/9){8}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(20/9){2}{\spec{2}}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(16/9){7}{\spec{2}}&\rat(16/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\rat(16/9){7}{\spec{2}}&\rat(10/9){1}{}&\rat(10/9){7}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(17/9){8}{}&\rat(14/9){5}{}&\rat(5/9){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{23}&\rat(17/9){8}{}&\rat(11/9){2}{}&\rat(8/9){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{24}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{25}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\rat(10/9){1}{}&\rat(16/9){7}{}&\rat(10/9){7}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{27}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{28}&\rat(8/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 22
\orbit{3}{22}{159}
\h{22}&\int(8){6}{\spec{2}}&\int(2){6}{}&\int(2){6}{}&&\cnt{819}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{\spec{1}}&\rat(1/3){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\rat(8/3){5}{\spec{1}}&\rat(2/3){8}{}&\rat(2/3){8}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{4}&\int(4){3}{}&\int(0){6}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(2){3}{\spec{1}}&\int(2){6}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(8/3){2}{\spec{1}}&\rat(2/3){2}{}&\rat(2/3){8}{}&\ln{2}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\rat(4/3){1}{\spec{1}}&\rat(4/3){7}{}&\rat(4/3){7}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 23
\orbit{3}{23}{159}
\h{23}&\int(4){\4}{}&\int(4){\4}{}&\int(4){\4}{}&&\cnt{711}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(1){8}{}&\int(1){8}{}&\ln{6}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{6}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){7}{}&\int(2){7}{}&\int(0){1}{}&\ln{6}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){7}{}&\int(1){7}{}&\int(1){1}{}&\ln{12}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 24
\orbit{3}{24}{159}
\h{24}&\rat(26/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(74/9){5}{\spec{2}}&&\cnt{1031}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\rat(13/9){4}{}&\rat(1/9){1}{}&\rat(22/9){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{\spec{1}}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{\spec{1}}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(2/3){6}{\spec{1}}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(2/3){6}{\spec{2}}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(16/9){7}{}&\rat(-2/9){7}{}&\rat(22/9){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(11/9){2}{}&\rat(-1/9){8}{}&\rat(26/9){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(7/9){7}{}&\rat(7/9){7}{}&\rat(22/9){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(2/9){2}{\spec{1}}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(2/9){2}{\spec{2}}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(10/9){1}{}&\rat(4/9){4}{}&\rat(22/9){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{15}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{\spec{1}}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(8/9){8}{}&\rat(2/9){2}{}&\rat(26/9){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{17}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{\spec{1}}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(2/3){6}{}&\rat(10/3){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 25
\orbit{3}{25}{159}
\h{25}&\rat(80/9){8}{\spec{2}}&\rat(14/9){2}{}&\rat(14/9){2}{}&&\cnt{943}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(40/9){4}{}&\rat(-2/9){1}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(32/9){5}{}&\rat(2/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{245}&\bounds{35}{35}{1}{false}&&\cr
\l{4}&\rat(22/9){4}{\spec{1}}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(10/3){3}{}&\rat(2/3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{6}&\rat(8/3){6}{\spec{1}}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(20/9){2}{\spec{1}}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{\spec{1}}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 26
\orbit{3}{26}{158}
\h{26}&\rat(26/9){8}{\spec{2}}&\rat(68/9){2}{\spec{3}}&\rat(14/9){2}{}&&\cnt{927}&\bounds{158}{158}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(20/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(4/3){3}{}&\rat(8/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(16/9){7}{}&\rat(22/9){7}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(11/9){2}{}&\rat(20/9){8}{}&\rat(5/9){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(2/9){2}{\spec{1}}&\rat(20/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(2/9){2}{\spec{2}}&\rat(20/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(10/9){1}{}&\rat(28/9){4}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(10/9){1}{}&\rat(22/9){7}{}&\rat(4/9){7}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(8/9){8}{}&\rat(20/9){8}{}&\rat(8/9){5}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{19}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 27
\orbit{3}{27}{158}
\h{27}&\rat(50/9){7}{\spec{2}}&\rat(38/9){4}{\spec{1}}&\rat(20/9){4}{}&&\cnt{707}&\bounds{158}{158}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(28/9){5}{}&\rat(13/9){8}{}&\rat(-5/9){8}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(28/9){5}{}&\rat(4/9){8}{}&\rat(4/9){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(26/9){4}{}&\rat(5/9){1}{}&\rat(5/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(19/9){5}{}&\rat(13/9){8}{}&\rat(4/9){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(8/3){3}{}&\rat(4/3){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(8/3){3}{}&\rat(4/3){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(8/3){3}{}&\int(0){\0}{}&\rat(4/3){6}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(7/3){6}{}&\rat(5/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(7/3){6}{}&\int(0){\0}{}&\rat(5/3){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(5/3){3}{\spec{1}}&\rat(7/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(5/3){3}{\spec{2}}&\rat(7/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(22/9){2}{}&\rat(10/9){2}{}&\rat(4/9){8}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(22/9){2}{}&\rat(13/9){8}{}&\rat(1/9){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(22/9){2}{}&\rat(4/9){8}{}&\rat(10/9){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{18}&\rat(13/9){2}{}&\rat(13/9){8}{}&\rat(10/9){2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(11/9){1}{}&\rat(20/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(11/9){1}{}&\rat(17/9){7}{}&\rat(8/9){7}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(11/9){1}{}&\rat(5/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(7/9){8}{}&\rat(13/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 28
\orbit{3}{28}{157}
\h{28}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{2}}&\int(0){\0}{}&&\cnt{1167}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){4}{}&\int(2){1}{}&\int(0){1}{}&\ln{2}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){7}{}&\int(2){7}{}&\int(0){1}{}&\ln{2}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){7}{}&\int(2){1}{}&\int(0){7}{}&\ln{2}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 29
\orbit{3}{29}{157}
\h{29}&\rat(80/9){8}{\spec{1}}&\rat(14/9){2}{}&\rat(14/9){2}{}&&\cnt{923}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(32/9){5}{}&\rat(2/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(31/9){4}{}&\rat(7/9){1}{}&\rat(-2/9){1}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(22/9){4}{\spec{1}}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(22/9){4}{\spec{2}}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(10/3){3}{}&\rat(2/3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(8/3){6}{}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(29/9){2}{}&\rat(14/9){2}{}&\rat(-7/9){8}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(29/9){2}{}&\rat(5/9){2}{}&\rat(2/9){8}{}&\ln{2}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{12}&\rat(20/9){2}{}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(19/9){1}{}&\rat(10/9){4}{}&\rat(7/9){1}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 30
\orbit{3}{30}{157}
\h{30}&\rat(32/9){7}{\spec{1}}&\rat(56/9){4}{\spec{2}}&\rat(20/9){4}{}&&\cnt{1067}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(4/9){2}{}&\rat(28/9){2}{}&\rat(4/9){8}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(16/9){8}{}&\rat(16/9){5}{\spec{1}}&\rat(4/9){8}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{6}&\rat(16/9){8}{}&\rat(28/9){2}{}&\rat(-8/9){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(16/9){8}{}&\rat(10/9){2}{\spec{1}}&\rat(10/9){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(16/9){8}{}&\rat(4/9){8}{\spec{1}}&\rat(16/9){5}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(-2/9){8}{}&\rat(28/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 31
\orbit{3}{31}{155}
\h{31}&\rat(8/9){8}{}&\rat(86/9){2}{\spec{2}}&\rat(14/9){2}{}&&\cnt{1043}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(2/3){6}{}&\rat(10/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(2/9){2}{}&\rat(32/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(32/9){2}{}&\rat(-4/9){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(-1/9){8}{}&\rat(32/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\rat(10/3){3}{}&\rat(2/3){6}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 32
\orbit{3}{32}{155}
\h{32}&\rat(44/9){8}{\spec{1}}&\rat(44/9){8}{\spec{1}}&\rat(20/9){5}{}&&\cnt{931}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(17/9){8}{}&\rat(5/9){8}{}&\ln{2}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(16/9){7}{}&\rat(16/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{245}&\bounds{35}{35}{1}{false}&&\cr
\l{6}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(11/9){2}{}&\rat(17/9){8}{}&\rat(8/9){2}{}&\ln{2}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(17/9){8}{}&\rat(17/9){8}{}&\rat(2/9){5}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 33
\orbit{3}{33}{155}
\h{33}&\int(6){6}{\spec{1}}&\int(4){6}{\spec{2}}&\int(2){6}{}&&\cnt{763}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(8/3){5}{}&\rat(2/3){8}{}&\rat(2/3){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(7/3){4}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(3){6}{}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(3){6}{}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){6}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){3}{}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(7/3){7}{}&\rat(4/3){7}{}&\rat(1/3){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(7/3){7}{}&\rat(4/3){1}{}&\rat(1/3){7}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(7/3){7}{}&\rat(1/3){1}{}&\rat(4/3){7}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(5/3){2}{}&\rat(5/3){2}{}&\rat(2/3){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(4/3){7}{\spec{1}}&\rat(4/3){1}{}&\rat(4/3){7}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(4/3){7}{\spec{2}}&\rat(4/3){1}{}&\rat(4/3){7}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\rat(5/3){8}{}&\rat(8/3){5}{}&\rat(-1/3){8}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(5/3){8}{}&\rat(5/3){5}{}&\rat(2/3){8}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{23}&\rat(5/3){8}{}&\rat(5/3){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{24}&\rat(5/3){8}{}&\rat(2/3){8}{}&\rat(5/3){5}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{25}&\rat(4/3){1}{}&\rat(7/3){4}{}&\rat(1/3){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\rat(4/3){1}{}&\rat(4/3){7}{}&\rat(4/3){7}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{27}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{28}&\rat(2/3){8}{}&\rat(8/3){5}{}&\rat(2/3){8}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 34
\orbit{3}{34}{155}
\h{34}&\rat(44/9){8}{\spec{2}}&\rat(50/9){2}{\spec{2}}&\rat(14/9){2}{}&&\cnt{703}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{}&\rat(11/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(22/9){4}{}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(8/3){6}{}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(7/3){3}{}&\rat(5/3){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(7/3){3}{}&\rat(5/3){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(4/3){3}{\spec{1}}&\rat(8/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(4/3){3}{\spec{2}}&\rat(8/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(20/9){2}{}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(20/9){2}{}&\rat(11/9){8}{}&\rat(5/9){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(20/9){2}{}&\rat(2/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(16/9){7}{}&\rat(22/9){7}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(10/9){1}{}&\rat(28/9){4}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(10/9){1}{}&\rat(22/9){7}{}&\rat(4/9){7}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{23}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 35
\orbit{3}{35}{154}
\h{35}&\int(4){6}{\spec{2}}&\int(2){3}{}&\int(6){\6}{\spec{1}}&&\cnt{815}&\bounds{154}{154}{1}{false}&&\cr
\l{1}&\rat(8/3){5}{}&\rat(-2/3){8}{}&\int(2){8}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(7/3){4}{}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(5/3){5}{}&\rat(1/3){8}{}&\int(2){8}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(5/3){2}{}&\rat(1/3){2}{}&\int(2){8}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(5/3){2}{}&\rat(1/3){8}{}&\int(2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(2/3){2}{\spec{1}}&\rat(4/3){2}{}&\int(2){8}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(2/3){2}{\spec{2}}&\rat(4/3){2}{}&\int(2){8}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{}&\rat(5/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(4/3){1}{}&\rat(2/3){7}{}&\int(2){7}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\rat(2/3){1}{}&\int(2){4}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{18}&\rat(2/3){8}{}&\rat(4/3){5}{}&\int(2){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(2/3){8}{}&\rat(4/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 36
\orbit{3}{36}{154}
\h{36}&\rat(80/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(20/9){5}{}&&\cnt{923}&\bounds{154}{154}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(32/9){5}{}&\rat(8/9){8}{}&\rat(-4/9){8}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(32/9){5}{}&\rat(-1/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(31/9){4}{}&\rat(1/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(23/9){5}{}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(10/3){3}{}&\rat(2/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(10/3){3}{}&\int(0){\0}{}&\rat(2/3){6}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(7/3){3}{\spec{1}}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(7/3){3}{\spec{2}}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(29/9){2}{}&\rat(2/9){2}{}&\rat(5/9){8}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(29/9){2}{}&\rat(8/9){8}{}&\rat(-1/9){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(29/9){2}{}&\rat(-1/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(19/9){1}{}&\rat(7/9){7}{}&\rat(10/9){7}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(19/9){1}{}&\rat(1/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{20}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 37
\orbit{3}{37}{152}
\h{37}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&&\cnt{1167}&\bounds{152}{152}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(2){8}{}&\int(0){8}{}&\ln{2}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){7}{}&\int(2){7}{}&\int(0){1}{}&\ln{1}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(2){2}{}&\int(0){8}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){8}{}&\int(0){2}{}&\ln{2}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){8}{}&\int(2){8}{}&\int(0){5}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 38
\orbit{3}{38}{151}
\h{38}&\rat(44/9){8}{\spec{2}}&\rat(32/9){2}{\spec{2}}&\rat(32/9){2}{\spec{2}}&&\cnt{1067}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(22/9){4}{}&\rat(16/9){1}{}&\rat(-2/9){1}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(4/9){4}{\spec{1}}&\rat(16/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(4/9){4}{\spec{2}}&\rat(16/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(4/9){4}{\spec{3}}&\rat(16/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(8/3){6}{}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(20/9){2}{}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(16/9){7}{}&\rat(4/9){7}{}&\rat(16/9){1}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(10/9){1}{}&\rat(10/9){4}{}&\rat(16/9){1}{}&\ln{2}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 39
\orbit{3}{39}{151}
\h{39}&\int(2){6}{}&\int(2){3}{}&\int(8){\8}{}&&\cnt{695}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(1){6}{}&\int(0){\0}{}&\int(3){3}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(1){3}{}&\int(0){\0}{}&\int(3){6}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{2}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(2/3){8}{}&\rat(1/3){8}{}&\int(3){5}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(2/3){8}{}&\rat(-2/3){8}{}&\int(4){5}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(1/3){1}{}&\rat(-1/3){1}{}&\int(4){4}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 40
\orbit{3}{40}{151}
\h{40}&\rat(8/9){8}{}&\rat(50/9){2}{\spec{2}}&\rat(50/9){2}{\spec{2}}&&\cnt{695}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(8/9){8}{}&\rat(17/9){5}{\spec{1}}&\rat(11/9){8}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(8/9){8}{}&\rat(17/9){5}{\spec{2}}&\rat(11/9){8}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(1/9){1}{}&\rat(22/9){7}{}&\rat(13/9){7}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(-1/9){8}{}&\rat(26/9){5}{}&\rat(11/9){8}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(-8/9){1}{}&\rat(22/9){7}{}&\rat(22/9){7}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{2}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{\spec{1}}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{\spec{2}}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 41
\orbit{3}{41}{151}
\h{41}&\rat(8/9){8}{}&\rat(68/9){2}{\spec{3}}&\rat(32/9){2}{\spec{1}}&&\cnt{923}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\rat(5/9){5}{}&\rat(20/9){8}{}&\rat(11/9){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(2/9){2}{}&\rat(20/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(17/9){5}{}&\rat(11/9){8}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{}&\rat(20/9){8}{}&\rat(8/9){5}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(8/9){8}{}&\rat(20/9){8}{}&\rat(8/9){5}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(1/9){1}{}&\rat(22/9){7}{}&\rat(13/9){7}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(-1/9){8}{}&\rat(26/9){5}{}&\rat(11/9){8}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(-1/9){8}{}&\rat(20/9){8}{}&\rat(17/9){5}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(5/3){6}{}&\rat(7/3){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 42
\orbit{3}{42}{151}
\h{42}&\rat(26/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(74/9){5}{\spec{3}}&&\cnt{1083}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(-1/9){8}{}&\rat(23/9){8}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\rat(5/9){5}{\spec{1}}&\rat(8/9){8}{}&\rat(23/9){8}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(5/9){5}{\spec{2}}&\rat(8/9){8}{}&\rat(23/9){8}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(4/3){3}{}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(16/9){7}{}&\rat(1/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\rat(16/9){7}{}&\rat(-8/9){1}{}&\rat(28/9){7}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(11/9){2}{}&\rat(2/9){2}{}&\rat(23/9){8}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(7/9){7}{}&\rat(1/9){1}{}&\rat(28/9){7}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(10/9){1}{}&\rat(7/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{13}&\rat(10/9){1}{}&\rat(-2/9){7}{}&\rat(28/9){7}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(8/9){8}{}&\rat(5/9){5}{}&\rat(23/9){8}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(1/9){1}{}&\rat(7/9){7}{}&\rat(28/9){7}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 43
\orbit{3}{43}{151}
\h{43}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(92/9){5}{\spec{3}}&&\cnt{1043}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(2/3){6}{}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(1/3){3}{}&\int(0){\0}{}&\rat(11/3){6}{}&\ln{2}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(7/9){7}{}&\rat(1/9){1}{}&\rat(28/9){7}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(2/9){2}{}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{3}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(8/9){8}{}&\rat(-1/9){8}{}&\rat(29/9){5}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(1/9){1}{}&\rat(1/9){1}{}&\rat(34/9){4}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(-1/9){8}{}&\rat(-1/9){8}{}&\rat(38/9){5}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{5}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 44
\orbit{3}{44}{151}
\h{44}&\rat(62/9){8}{\spec{2}}&\rat(26/9){8}{\spec{2}}&\rat(20/9){5}{}&&\cnt{703}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(32/9){5}{}&\rat(8/9){8}{}&\rat(-4/9){8}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(32/9){5}{}&\rat(-1/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(31/9){4}{}&\rat(10/9){1}{}&\rat(-5/9){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(31/9){4}{}&\rat(1/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(23/9){5}{}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(22/9){4}{\spec{1}}&\rat(10/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(22/9){4}{\spec{2}}&\rat(10/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(10/3){3}{}&\rat(2/3){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(10/3){3}{}&\rat(2/3){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(10/3){3}{}&\int(0){\0}{}&\rat(2/3){6}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(8/3){6}{}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(7/3){3}{}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(7/3){3}{}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(20/9){2}{}&\rat(11/9){2}{}&\rat(5/9){8}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(16/9){7}{}&\rat(16/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(10/9){1}{}&\rat(16/9){7}{}&\rat(10/9){7}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 45
\orbit{3}{45}{151}
\h{45}&\rat(26/9){8}{\spec{2}}&\rat(50/9){2}{\spec{2}}&\rat(32/9){2}{\spec{1}}&&\cnt{707}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(11/9){8}{}&\rat(11/9){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(4/3){3}{}&\rat(8/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(16/9){7}{}&\rat(22/9){7}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(16/9){7}{}&\rat(7/9){1}{}&\rat(13/9){7}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(11/9){2}{}&\rat(14/9){2}{}&\rat(11/9){8}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(10/9){1}{}&\rat(28/9){4}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(10/9){1}{}&\rat(22/9){7}{}&\rat(4/9){7}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(10/9){1}{}&\rat(22/9){7}{}&\rat(4/9){7}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(10/9){1}{}&\rat(13/9){7}{}&\rat(13/9){7}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(10/9){1}{}&\rat(7/9){1}{}&\rat(19/9){4}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(8/9){8}{}&\rat(17/9){5}{\spec{1}}&\rat(11/9){8}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(8/9){8}{}&\rat(17/9){5}{\spec{2}}&\rat(11/9){8}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{23}&\rat(8/9){8}{}&\rat(11/9){8}{}&\rat(17/9){5}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{24}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\rat(1/9){1}{}&\rat(22/9){7}{}&\rat(13/9){7}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{26}&\rat(-1/9){8}{}&\rat(26/9){5}{}&\rat(11/9){8}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{31}&\int(0){\0}{}&\rat(5/3){6}{\spec{1}}&\rat(7/3){3}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{32}&\int(0){\0}{}&\rat(5/3){6}{\spec{2}}&\rat(7/3){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 46
\orbit{3}{46}{150}
\h{46}&\rat(44/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(56/9){5}{\spec{1}}&&\cnt{755}&\bounds{150}{150}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(23/9){5}{}&\rat(-1/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(22/9){4}{}&\rat(1/9){1}{}&\rat(13/9){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(14/9){5}{\spec{1}}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(14/9){5}{\spec{2}}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(7/3){3}{}&\int(0){\0}{}&\rat(5/3){6}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(7/3){3}{}&\int(0){\0}{}&\rat(5/3){6}{\spec{2}}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(4/3){3}{\spec{1}}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(4/3){3}{\spec{2}}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(20/9){2}{}&\rat(2/9){2}{}&\rat(14/9){8}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(20/9){2}{}&\rat(-1/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\rat(16/9){7}{}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\rat(16/9){7}{}&\rat(1/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{24}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{25}&\rat(10/9){1}{}&\rat(7/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{26}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{27}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{28}&\rat(8/9){8}{}&\rat(-1/9){8}{}&\rat(29/9){5}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{29}&\rat(-1/9){8}{}&\rat(8/9){8}{}&\rat(29/9){5}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{31}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 47
\orbit{3}{47}{150}
\h{47}&\rat(14/9){7}{}&\rat(74/9){4}{\spec{2}}&\rat(20/9){4}{}&&\cnt{815}&\bounds{150}{150}{1}{false}&&\cr
\l{1}&\rat(4/3){6}{}&\rat(8/3){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(2/3){3}{}&\rat(10/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(26/9){7}{}&\rat(-4/9){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/9){7}{}&\rat(26/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(7/9){8}{}&\rat(34/9){5}{}&\rat(-5/9){8}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(7/9){8}{}&\rat(19/9){2}{\spec{2}}&\rat(10/9){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(7/9){8}{}&\rat(13/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(2/9){1}{}&\rat(29/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(2/9){1}{}&\rat(26/9){7}{}&\rat(8/9){7}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(-2/9){8}{}&\rat(34/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(10/3){6}{}&\rat(2/3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(8/3){3}{\spec{2}}&\rat(4/3){6}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(7/3){6}{\spec{1}}&\rat(5/3){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\rat(7/3){6}{\spec{2}}&\rat(5/3){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 48
\orbit{3}{48}{150}
\h{48}&\int(6){6}{\spec{1}}&\int(2){3}{}&\int(4){\4}{}&&\cnt{763}&\bounds{150}{150}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(8/3){5}{}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(7/3){4}{}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){6}{}&\int(0){\0}{}&\int(1){3}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){6}{}&\int(0){\0}{}&\int(1){3}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(2){3}{}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(7/3){7}{}&\rat(2/3){7}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(7/3){7}{}&\rat(2/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(7/3){7}{}&\rat(-1/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(5/3){2}{}&\rat(1/3){8}{}&\int(2){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{20}&\rat(4/3){7}{\spec{1}}&\rat(2/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(4/3){7}{\spec{2}}&\rat(2/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(5/3){8}{}&\rat(4/3){5}{}&\int(1){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\rat(5/3){8}{}&\rat(4/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\rat(5/3){8}{}&\rat(1/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\rat(5/3){8}{}&\rat(1/3){8}{}&\int(2){5}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{26}&\rat(4/3){1}{}&\rat(5/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\rat(4/3){1}{}&\rat(2/3){7}{}&\int(2){7}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{28}&\rat(4/3){1}{}&\rat(2/3){1}{}&\int(2){4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{29}&\rat(2/3){8}{}&\rat(4/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{31}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 49
\orbit{3}{49}{150}
\h{49}&\rat(62/9){8}{\spec{1}}&\rat(32/9){2}{\spec{1}}&\rat(14/9){2}{}&&\cnt{871}&\bounds{150}{150}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{\spec{1}}&\rat(11/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(22/9){4}{\spec{1}}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(8/3){6}{\spec{1}}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{\spec{1}}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(7/3){3}{\spec{1}}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(5/3){6}{\spec{1}}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(20/9){2}{\spec{1}}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(20/9){2}{\spec{1}}&\rat(11/9){8}{}&\rat(5/9){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(20/9){2}{\spec{1}}&\rat(2/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(16/9){7}{\spec{1}}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(11/9){2}{\spec{1}}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(19/9){1}{}&\rat(19/9){4}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{18}&\rat(19/9){1}{}&\rat(10/9){4}{\spec{1}}&\rat(7/9){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(19/9){1}{}&\rat(10/9){4}{\spec{2}}&\rat(7/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(19/9){1}{}&\rat(13/9){7}{}&\rat(4/9){7}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{21}&\rat(19/9){1}{}&\rat(7/9){1}{}&\rat(10/9){4}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{22}&\rat(8/9){8}{\spec{1}}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 50
\orbit{3}{50}{149}
\h{50}&\int(6){6}{\spec{2}}&\int(4){6}{\spec{2}}&\int(2){6}{}&&\cnt{703}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{}&\rat(4/3){1}{}&\rat(-2/3){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(10/3){4}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(8/3){5}{}&\rat(2/3){8}{}&\rat(2/3){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(7/3){4}{}&\rat(4/3){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(3){3}{}&\int(0){\0}{}&\int(1){6}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){3}{\spec{1}}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(2){3}{\spec{1}}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(2){3}{\spec{2}}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){3}{\spec{2}}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(8/3){2}{}&\rat(5/3){2}{}&\rat(-1/3){8}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(8/3){2}{}&\rat(2/3){2}{\spec{1}}&\rat(2/3){8}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(8/3){2}{}&\rat(2/3){2}{\spec{2}}&\rat(2/3){8}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(8/3){2}{}&\rat(2/3){8}{}&\rat(2/3){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(5/3){2}{}&\rat(5/3){2}{}&\rat(2/3){8}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(4/3){7}{}&\rat(4/3){1}{}&\rat(4/3){7}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(4/3){1}{}&\rat(7/3){4}{}&\rat(1/3){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\rat(4/3){1}{}&\rat(4/3){7}{}&\rat(4/3){7}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(4/3){1}{}&\rat(4/3){1}{}&\rat(4/3){4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\rat(2/3){8}{}&\rat(8/3){5}{}&\rat(2/3){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 51
\orbit{3}{51}{149}
\h{51}&\rat(26/9){8}{\spec{2}}&\rat(26/9){8}{\spec{2}}&\rat(56/9){5}{\spec{1}}&&\cnt{763}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(13/9){4}{}&\rat(10/9){1}{}&\rat(13/9){1}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(4/3){3}{}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(16/9){7}{}&\rat(16/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(16/9){7}{}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{\spec{1}}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{\spec{2}}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(16/9){7}{}&\rat(1/9){1}{}&\rat(19/9){7}{}&\ln{2}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(11/9){2}{}&\rat(11/9){2}{}&\rat(14/9){8}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(7/9){7}{}&\rat(10/9){1}{}&\rat(19/9){7}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{\spec{1}}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(8/9){8}{}&\rat(-1/9){8}{}&\rat(29/9){5}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 52
\orbit{3}{52}{147}
\h{52}&\rat(26/9){8}{\spec{2}}&\rat(68/9){2}{\spec{1}}&\rat(14/9){2}{}&&\cnt{815}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\rat(13/9){4}{}&\rat(16/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(4/3){3}{}&\rat(8/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(2/3){6}{\spec{1}}&\rat(10/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(2/3){6}{\spec{2}}&\rat(10/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(16/9){7}{}&\rat(22/9){7}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(16/9){7}{}&\rat(16/9){1}{}&\rat(4/9){7}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(11/9){2}{}&\rat(23/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(10/9){1}{}&\rat(28/9){4}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(10/9){1}{}&\rat(19/9){4}{\spec{1}}&\rat(7/9){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(10/9){1}{}&\rat(19/9){4}{\spec{2}}&\rat(7/9){1}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(10/9){1}{}&\rat(22/9){7}{}&\rat(4/9){7}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(10/9){1}{}&\rat(16/9){1}{}&\rat(10/9){4}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(8/9){8}{}&\rat(23/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\rat(8/9){8}{}&\rat(14/9){2}{\spec{1}}&\rat(14/9){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\rat(8/9){8}{}&\rat(14/9){2}{\spec{2}}&\rat(14/9){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{26}&\rat(-1/9){8}{}&\rat(23/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\rat(10/3){3}{}&\rat(2/3){6}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{31}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{32}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 53
\orbit{3}{53}{147}
\h{53}&\int(8){6}{\spec{2}}&\int(2){3}{}&\int(2){\2}{}&&\cnt{815}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(11/3){5}{}&\rat(1/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(11/3){5}{}&\rat(-2/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(10/3){4}{\spec{2}}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(10/3){4}{\spec{2}}&\rat(-1/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(8/3){5}{\spec{2}}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(7/3){4}{\spec{1}}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(7/3){4}{\spec{2}}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\int(3){6}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(3){3}{}&\int(0){\0}{}&\int(1){6}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(2){6}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(2){6}{\spec{3}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(8/3){2}{\spec{2}}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\rat(8/3){2}{\spec{2}}&\rat(1/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\rat(8/3){2}{\spec{2}}&\rat(1/3){8}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\rat(7/3){7}{}&\rat(2/3){7}{}&\int(1){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{26}&\rat(7/3){7}{}&\rat(2/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{27}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{28}&\rat(5/3){8}{}&\rat(4/3){5}{}&\int(1){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{29}&\rat(5/3){8}{}&\rat(4/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{30}&\rat(4/3){1}{\spec{2}}&\rat(5/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 54
\orbit{3}{54}{147}
\h{54}&\rat(32/9){7}{\spec{2}}&\rat(38/9){4}{\spec{1}}&\rat(38/9){4}{\spec{1}}&&\cnt{707}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\rat(19/9){5}{}&\rat(13/9){8}{}&\rat(4/9){8}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(10/9){5}{\spec{1}}&\rat(13/9){8}{}&\rat(13/9){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(10/9){5}{\spec{2}}&\rat(13/9){8}{}&\rat(13/9){8}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(7/3){6}{}&\rat(5/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(5/3){3}{}&\rat(7/3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(13/9){2}{}&\rat(10/9){2}{}&\rat(13/9){8}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(11/9){1}{}&\rat(20/9){4}{}&\rat(5/9){1}{}&\ln{2}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(11/9){1}{}&\rat(17/9){7}{}&\rat(8/9){7}{\spec{1}}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(11/9){1}{}&\rat(17/9){7}{}&\rat(8/9){7}{\spec{2}}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(7/9){8}{}&\rat(16/9){5}{}&\rat(13/9){8}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(2/9){1}{}&\rat(17/9){7}{}&\rat(17/9){7}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(-2/9){8}{}&\rat(25/9){5}{}&\rat(13/9){8}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 55
\orbit{3}{55}{147}
\h{55}&\rat(44/9){8}{\spec{2}}&\rat(26/9){8}{\spec{2}}&\rat(38/9){5}{\spec{2}}&&\cnt{707}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(22/9){4}{}&\rat(10/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(22/9){4}{}&\rat(1/9){1}{}&\rat(13/9){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(13/9){4}{\spec{1}}&\rat(10/9){1}{}&\rat(13/9){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(13/9){4}{\spec{2}}&\rat(10/9){1}{}&\rat(13/9){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(8/3){6}{}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(7/3){3}{}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(7/3){3}{}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(20/9){2}{}&\rat(11/9){2}{}&\rat(5/9){8}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(20/9){2}{}&\rat(-1/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\rat(16/9){7}{}&\rat(16/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(16/9){7}{}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{23}&\rat(7/9){7}{}&\rat(16/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\rat(10/9){1}{}&\rat(13/9){4}{}&\rat(13/9){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{25}&\rat(10/9){1}{}&\rat(16/9){7}{}&\rat(10/9){7}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{27}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{28}&\rat(8/9){8}{}&\rat(11/9){2}{}&\rat(17/9){2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{29}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{30}&\rat(1/9){1}{}&\rat(10/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{31}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{32}&\int(0){\0}{}&\rat(5/3){6}{}&\rat(7/3){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 56
\orbit{3}{56}{147}
\h{56}&\int(8){6}{\spec{2}}&\int(4){3}{\spec{1}}&\int(0){\0}{}&&\cnt{1067}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{\spec{1}}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\rat(8/3){5}{\spec{1}}&\rat(4/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(4){3}{}&\int(0){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){3}{}&\int(0){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){3}{}&\int(0){\0}{}&\int(0){6}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(2){6}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){3}{\spec{1}}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(8/3){2}{\spec{1}}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(8/3){2}{\spec{1}}&\rat(4/3){8}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(4/3){1}{\spec{1}}&\rat(8/3){4}{}&\int(0){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 57
\orbit{3}{57}{146}
\h{57}&\rat(50/9){7}{\spec{1}}&\rat(38/9){4}{\spec{1}}&\rat(20/9){4}{}&&\cnt{759}&\bounds{146}{146}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(19/9){5}{}&\rat(13/9){8}{}&\rat(4/9){8}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(7/3){6}{}&\rat(5/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(7/3){6}{}&\int(0){\0}{}&\rat(5/3){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(5/3){3}{}&\rat(7/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\rat(23/9){7}{}&\rat(17/9){7}{}&\rat(-4/9){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(23/9){7}{}&\rat(8/9){7}{\spec{1}}&\rat(5/9){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(23/9){7}{}&\rat(8/9){7}{\spec{2}}&\rat(5/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(23/9){7}{}&\rat(5/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(13/9){2}{}&\rat(13/9){8}{}&\rat(10/9){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(16/9){8}{}&\rat(25/9){5}{}&\rat(-5/9){8}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(16/9){8}{}&\rat(16/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{19}&\rat(16/9){8}{}&\rat(10/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(16/9){8}{}&\rat(13/9){8}{}&\rat(7/9){5}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\rat(16/9){8}{}&\rat(4/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(11/9){1}{}&\rat(20/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(11/9){1}{}&\rat(17/9){7}{}&\rat(8/9){7}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\rat(11/9){1}{}&\rat(5/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\rat(7/9){8}{}&\rat(13/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 58
\orbit{3}{58}{145}
\h{58}&\rat(80/9){8}{\spec{3}}&\rat(8/9){8}{}&\rat(20/9){5}{}&&\cnt{867}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(32/9){5}{}&\rat(8/9){8}{}&\rat(-4/9){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(32/9){5}{}&\rat(-1/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(31/9){4}{}&\rat(1/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(23/9){5}{\spec{1}}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(23/9){5}{\spec{2}}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(11/3){6}{}&\rat(1/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(11/3){6}{}&\int(0){\0}{}&\rat(1/3){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(10/3){3}{}&\rat(2/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(10/3){3}{}&\int(0){\0}{}&\rat(2/3){6}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(7/3){3}{}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{17}&\rat(25/9){7}{}&\rat(7/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(25/9){7}{}&\rat(1/9){1}{}&\rat(10/9){7}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 59
\orbit{3}{59}{145}
\h{59}&\rat(50/9){7}{\spec{2}}&\rat(38/9){4}{\spec{2}}&\rat(20/9){4}{}&&\cnt{703}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(28/9){5}{}&\rat(4/9){8}{}&\rat(4/9){8}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(26/9){4}{}&\rat(14/9){1}{}&\rat(-4/9){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(26/9){4}{}&\rat(5/9){1}{}&\rat(5/9){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(17/9){4}{\spec{1}}&\rat(14/9){1}{}&\rat(5/9){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(17/9){4}{\spec{2}}&\rat(14/9){1}{}&\rat(5/9){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(8/3){3}{}&\rat(4/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(8/3){3}{}&\int(0){\0}{}&\rat(4/3){6}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(7/3){6}{}&\rat(5/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(7/3){6}{}&\int(0){\0}{}&\rat(5/3){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(22/9){2}{}&\rat(19/9){2}{}&\rat(-5/9){8}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(22/9){2}{}&\rat(10/9){2}{\spec{1}}&\rat(4/9){8}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(22/9){2}{}&\rat(10/9){2}{\spec{2}}&\rat(4/9){8}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(22/9){2}{}&\rat(4/9){8}{}&\rat(10/9){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(13/9){2}{}&\rat(19/9){2}{}&\rat(4/9){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(11/9){1}{}&\rat(20/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(11/9){1}{}&\rat(14/9){1}{}&\rat(11/9){4}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\rat(11/9){1}{}&\rat(5/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\rat(7/9){8}{}&\rat(19/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{23}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 60
\orbit{3}{60}{145}
\h{60}&\int(8){6}{\spec{3}}&\int(2){6}{}&\int(2){6}{}&&\cnt{807}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(8/3){5}{}&\rat(2/3){8}{}&\rat(2/3){8}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(10/3){7}{}&\rat(4/3){7}{}&\rat(-2/3){1}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(10/3){7}{}&\rat(1/3){7}{}&\rat(1/3){1}{}&\ln{2}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(5/3){8}{}&\rat(5/3){5}{}&\rat(2/3){8}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\rat(4/3){7}{}&\rat(4/3){7}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 61
\orbit{3}{61}{145}
\h{61}&\int(10){6}{\spec{3}}&\int(2){3}{}&\int(0){\0}{}&&\cnt{1043}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(11/3){5}{}&\rat(1/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(10/3){4}{}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(4){6}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(4){6}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(2){6}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){6}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(10/3){7}{}&\rat(2/3){7}{}&\int(0){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\rat(10/3){7}{}&\rat(2/3){1}{}&\int(0){7}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(8/3){2}{}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 62
\orbit{3}{62}{144}
\h{62}&\rat(62/9){8}{\spec{1}}&\rat(32/9){2}{\spec{1}}&\rat(14/9){2}{}&&\cnt{815}&\bounds{144}{144}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(23/9){5}{\spec{2}}&\rat(11/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(22/9){4}{\spec{2}}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{\spec{2}}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(8/3){6}{\spec{2}}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(7/3){3}{\spec{2}}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(5/3){6}{\spec{2}}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(5/3){6}{\spec{3}}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(25/9){7}{}&\rat(13/9){7}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\rat(25/9){7}{}&\rat(4/9){7}{\spec{1}}&\rat(7/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(25/9){7}{}&\rat(4/9){7}{\spec{2}}&\rat(7/9){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(25/9){7}{}&\rat(7/9){1}{}&\rat(4/9){7}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\rat(20/9){2}{\spec{2}}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(20/9){2}{\spec{2}}&\rat(11/9){8}{}&\rat(5/9){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(20/9){2}{\spec{2}}&\rat(2/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(16/9){7}{\spec{2}}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{23}&\rat(11/9){2}{\spec{2}}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\rat(17/9){8}{}&\rat(17/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{25}&\rat(17/9){8}{}&\rat(14/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{26}&\rat(17/9){8}{}&\rat(5/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{27}&\rat(17/9){8}{}&\rat(11/9){8}{}&\rat(8/9){5}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{28}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{29}&\rat(8/9){8}{\spec{2}}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 63
\orbit{3}{63}{144}
\h{63}&\rat(80/9){8}{\spec{3}}&\rat(14/9){2}{}&\rat(14/9){2}{}&&\cnt{867}&\bounds{144}{144}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(32/9){5}{}&\rat(2/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\rat(31/9){4}{}&\rat(7/9){1}{}&\rat(-2/9){1}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(22/9){4}{\spec{1}}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(22/9){4}{\spec{2}}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(11/3){6}{}&\rat(1/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(10/3){3}{}&\rat(2/3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(8/3){6}{}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(25/9){7}{}&\rat(4/9){7}{}&\rat(7/9){1}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(20/9){2}{}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(17/9){8}{}&\rat(14/9){2}{}&\rat(5/9){2}{}&\ln{2}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 64
\orbit{3}{64}{144}
\h{64}&\rat(14/9){7}{}&\rat(56/9){4}{\spec{1}}&\rat(38/9){4}{\spec{1}}&&\cnt{759}&\bounds{144}{144}{1}{false}&&\cr
\l{1}&\rat(10/9){5}{}&\rat(13/9){8}{}&\rat(13/9){8}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(14/9){7}{}&\rat(5/9){1}{}&\rat(17/9){7}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(5/9){7}{}&\rat(14/9){1}{}&\rat(17/9){7}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(4/9){2}{}&\rat(19/9){2}{}&\rat(13/9){8}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(7/9){8}{}&\rat(16/9){5}{\spec{1}}&\rat(13/9){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(7/9){8}{}&\rat(16/9){5}{\spec{2}}&\rat(13/9){8}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(7/9){8}{}&\rat(19/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(7/9){8}{}&\rat(13/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(7/9){8}{}&\rat(4/9){8}{}&\rat(25/9){5}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(2/9){1}{}&\rat(29/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\rat(2/9){1}{}&\rat(17/9){7}{}&\rat(17/9){7}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{19}&\rat(-2/9){8}{}&\rat(25/9){5}{}&\rat(13/9){8}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(-2/9){8}{}&\rat(13/9){8}{}&\rat(25/9){5}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\rat(5/3){3}{\spec{1}}&\rat(7/3){6}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\rat(5/3){3}{\spec{2}}&\rat(7/3){6}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 65
\orbit{3}{65}{143}
\h{65}&\int(4){6}{\spec{1}}&\int(4){6}{\spec{2}}&\int(4){6}{\spec{2}}&&\cnt{699}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\rat(4/3){4}{}&\rat(4/3){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(7/3){7}{}&\rat(4/3){7}{}&\rat(1/3){1}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(7/3){7}{}&\rat(1/3){7}{}&\rat(4/3){1}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(4/3){7}{}&\rat(4/3){7}{}&\rat(4/3){1}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(5/3){8}{}&\rat(8/3){5}{}&\rat(-1/3){8}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/3){8}{}&\rat(5/3){5}{}&\rat(2/3){8}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(5/3){8}{}&\rat(5/3){2}{}&\rat(2/3){2}{\spec{1}}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(5/3){8}{}&\rat(5/3){2}{}&\rat(2/3){2}{\spec{2}}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(2/3){8}{}&\rat(8/3){5}{}&\rat(2/3){8}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(2/3){8}{}&\rat(5/3){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(1/3){1}{}&\rat(7/3){4}{}&\rat(4/3){1}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){6}{}&\int(2){3}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 66
\orbit{3}{66}{143}
\h{66}&\rat(44/9){8}{\spec{1}}&\rat(50/9){2}{\spec{1}}&\rat(14/9){2}{}&&\cnt{931}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\rat(13/9){4}{}&\rat(16/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(16/9){7}{}&\rat(16/9){1}{}&\rat(4/9){7}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{12}&\rat(11/9){2}{}&\rat(23/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{13}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(17/9){8}{}&\rat(17/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\rat(17/9){8}{}&\rat(23/9){2}{}&\rat(-4/9){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(17/9){8}{}&\rat(14/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(17/9){8}{}&\rat(5/9){2}{\spec{1}}&\rat(14/9){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(17/9){8}{}&\rat(5/9){2}{\spec{2}}&\rat(14/9){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(17/9){8}{}&\rat(11/9){8}{}&\rat(8/9){5}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{20}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(10/9){1}{}&\rat(16/9){1}{}&\rat(10/9){4}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(-1/9){8}{}&\rat(23/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 67
\orbit{3}{67}{143}
\h{67}&\rat(50/9){7}{\spec{1}}&\rat(38/9){4}{\spec{2}}&\rat(20/9){4}{}&&\cnt{755}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(17/9){4}{}&\rat(14/9){1}{}&\rat(5/9){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(7/3){6}{}&\rat(5/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(7/3){6}{}&\int(0){\0}{}&\rat(5/3){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(4/3){6}{\spec{1}}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(4/3){6}{\spec{2}}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(23/9){7}{}&\rat(8/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(23/9){7}{}&\rat(14/9){1}{}&\rat(-1/9){7}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(23/9){7}{}&\rat(5/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(13/9){2}{}&\rat(19/9){2}{}&\rat(4/9){8}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(16/9){8}{}&\rat(16/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{18}&\rat(16/9){8}{}&\rat(19/9){2}{}&\rat(1/9){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(16/9){8}{}&\rat(10/9){2}{\spec{1}}&\rat(10/9){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(16/9){8}{}&\rat(10/9){2}{\spec{2}}&\rat(10/9){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(16/9){8}{}&\rat(4/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{22}&\rat(11/9){1}{}&\rat(20/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(11/9){1}{}&\rat(14/9){1}{}&\rat(11/9){4}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\rat(11/9){1}{}&\rat(5/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\rat(7/9){8}{}&\rat(19/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 68
\orbit{3}{68}{143}
\h{68}&\int(6){\6}{}&\int(4){\4}{}&\int(2){\2}{}&&\cnt{703}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){5}{}&\int(1){8}{}&\int(0){8}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){5}{}&\int(0){8}{}&\int(1){8}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){5}{\spec{1}}&\int(1){8}{}&\int(1){8}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){5}{\spec{2}}&\int(1){8}{}&\int(1){8}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){6}{}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){6}{}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){6}{}&\int(0){\0}{}&\int(1){3}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(2){7}{}&\int(2){7}{}&\int(0){1}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(2){7}{}&\int(1){7}{}&\int(1){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(2){7}{}&\int(1){1}{}&\int(1){7}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(1){7}{}&\int(2){7}{}&\int(1){1}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\int(1){8}{}&\int(2){5}{}&\int(1){8}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(1){8}{}&\int(2){2}{}&\int(1){2}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 69
\orbit{3}{69}{143}
\h{69}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(92/9){5}{\spec{2}}&&\cnt{1067}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{\spec{1}}&\ln{2}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(2/3){6}{}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{2}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\rat(7/9){7}{}&\rat(7/9){7}{}&\rat(22/9){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(2/9){2}{}&\rat(-1/9){8}{}&\rat(35/9){2}{}&\ln{2}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\rat(-7/9){2}{}&\rat(8/9){8}{}&\rat(35/9){2}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{1}}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 70
\orbit{3}{70}{143}
\h{70}&\int(6){6}{\spec{1}}&\int(4){3}{\spec{1}}&\int(2){\2}{}&&\cnt{759}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(8/3){5}{}&\rat(4/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(8/3){5}{}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(7/3){4}{}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(5/3){5}{\spec{1}}&\rat(4/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(5/3){5}{\spec{2}}&\rat(4/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(3){6}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(7/3){7}{}&\rat(5/3){7}{}&\int(0){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(7/3){7}{}&\rat(2/3){7}{\spec{1}}&\int(1){1}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(7/3){7}{}&\rat(2/3){7}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\rat(7/3){7}{}&\rat(2/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\rat(5/3){2}{}&\rat(4/3){8}{}&\int(1){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{25}&\rat(4/3){7}{\spec{1}}&\rat(5/3){7}{}&\int(1){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\rat(4/3){7}{\spec{2}}&\rat(5/3){7}{}&\int(1){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{27}&\rat(5/3){8}{}&\rat(7/3){5}{}&\int(0){8}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{28}&\rat(5/3){8}{}&\rat(4/3){5}{\spec{1}}&\int(1){8}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{29}&\rat(5/3){8}{}&\rat(4/3){5}{\spec{2}}&\int(1){8}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{30}&\rat(5/3){8}{}&\rat(4/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{31}&\rat(5/3){8}{}&\rat(4/3){8}{}&\int(1){5}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{32}&\rat(4/3){1}{}&\rat(8/3){4}{}&\int(0){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{33}&\rat(4/3){1}{}&\rat(5/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{34}&\rat(4/3){1}{}&\rat(5/3){7}{}&\int(1){7}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{35}&\rat(2/3){8}{}&\rat(7/3){5}{}&\int(1){8}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{36}&\rat(1/3){1}{}&\rat(8/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{37}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 71
\orbit{3}{71}{143}
\h{71}&\rat(8/9){8}{}&\rat(50/9){2}{\spec{1}}&\rat(50/9){2}{\spec{1}}&&\cnt{931}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\rat(4/9){4}{}&\rat(16/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/9){7}{}&\rat(13/9){7}{}&\rat(16/9){1}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(2/9){2}{}&\rat(23/9){2}{}&\rat(11/9){8}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(8/9){8}{}&\rat(17/9){5}{}&\rat(11/9){8}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(23/9){2}{}&\rat(5/9){2}{\spec{1}}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(23/9){2}{}&\rat(5/9){2}{\spec{2}}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(1/9){1}{}&\rat(19/9){4}{}&\rat(16/9){1}{}&\ln{2}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(-1/9){8}{}&\rat(23/9){2}{}&\rat(14/9){2}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{3}}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{2}}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 72
\orbit{3}{72}{143}
\h{72}&\rat(14/9){7}{}&\rat(74/9){4}{\spec{1}}&\rat(20/9){4}{}&&\cnt{811}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(1/3){6}{}&\rat(11/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(4/9){2}{}&\rat(28/9){2}{}&\rat(4/9){8}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(7/9){8}{}&\rat(28/9){2}{}&\rat(1/9){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(7/9){8}{}&\rat(19/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(7/9){8}{}&\rat(13/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(2/9){1}{}&\rat(29/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(-2/9){8}{}&\rat(28/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(11/3){3}{}&\rat(1/3){6}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 73
\orbit{3}{73}{143}
\h{73}&\rat(14/9){7}{}&\rat(56/9){4}{\spec{2}}&\rat(38/9){4}{\spec{2}}&&\cnt{943}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\rat(8/9){4}{}&\rat(14/9){1}{}&\rat(14/9){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(4/3){6}{}&\int(0){\0}{\spec{1}}&\rat(8/3){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(8/9){7}{\spec{1}}&\rat(14/9){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(4/9){2}{}&\rat(28/9){2}{}&\rat(4/9){8}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(7/9){8}{}&\rat(28/9){2}{}&\rat(1/9){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(7/9){8}{}&\rat(10/9){2}{\spec{1}}&\rat(19/9){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(2/9){1}{}&\rat(20/9){4}{\spec{1}}&\rat(14/9){1}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{10}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(-2/9){8}{}&\rat(28/9){2}{}&\rat(10/9){2}{\spec{1}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(-2/9){8}{}&\rat(28/9){2}{}&\rat(10/9){2}{\spec{2}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(4/3){6}{\spec{1}}&\rat(8/3){3}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 74
\orbit{3}{74}{143}
\h{74}&\rat(62/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(38/9){5}{\spec{2}}&&\cnt{863}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{\spec{1}}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(22/9){4}{\spec{1}}&\rat(1/9){1}{}&\rat(13/9){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(8/3){6}{\spec{1}}&\int(0){\0}{}&\rat(4/3){3}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{\spec{1}}&\int(0){\0}{}&\rat(4/3){3}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(7/3){3}{\spec{1}}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(5/3){6}{\spec{1}}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(20/9){2}{\spec{1}}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{1}}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(20/9){2}{\spec{1}}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{2}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(20/9){2}{\spec{1}}&\rat(-1/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\rat(16/9){7}{\spec{1}}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(11/9){2}{\spec{1}}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(19/9){1}{}&\rat(4/9){4}{}&\rat(13/9){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{18}&\rat(19/9){1}{}&\rat(7/9){7}{}&\rat(10/9){7}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\rat(19/9){1}{}&\rat(1/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{20}&\rat(19/9){1}{}&\rat(-8/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(8/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 75
\orbit{3}{75}{141}
\h{75}&\rat(44/9){8}{\spec{2}}&\rat(26/9){8}{\spec{2}}&\rat(38/9){5}{\spec{1}}&&\cnt{703}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(23/9){5}{}&\rat(-1/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(22/9){4}{}&\rat(10/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(14/9){5}{\spec{1}}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(14/9){5}{\spec{2}}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(8/3){6}{}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(7/3){3}{}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(7/3){3}{}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(4/3){3}{\spec{1}}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(4/3){3}{\spec{2}}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(20/9){2}{}&\rat(11/9){2}{}&\rat(5/9){8}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(20/9){2}{}&\rat(2/9){2}{\spec{1}}&\rat(14/9){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(20/9){2}{}&\rat(2/9){2}{\spec{2}}&\rat(14/9){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(16/9){7}{}&\rat(16/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(16/9){7}{}&\rat(1/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\rat(11/9){2}{}&\rat(11/9){2}{}&\rat(14/9){8}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{24}&\rat(7/9){7}{}&\rat(10/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\rat(10/9){1}{}&\rat(16/9){7}{}&\rat(10/9){7}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\rat(10/9){1}{}&\rat(16/9){7}{}&\rat(10/9){7}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\rat(10/9){1}{}&\rat(7/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{28}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{29}&\rat(8/9){8}{}&\rat(14/9){5}{}&\rat(14/9){8}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{30}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{31}&\rat(1/9){1}{}&\rat(16/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{32}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{33}&\int(0){\0}{}&\rat(4/3){3}{}&\rat(8/3){6}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 76
\orbit{3}{76}{141}
\h{76}&\rat(68/9){7}{\spec{2}}&\rat(20/9){4}{}&\rat(20/9){4}{}&&\cnt{699}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(35/9){4}{}&\rat(5/9){1}{}&\rat(-4/9){1}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(28/9){5}{}&\rat(4/9){8}{}&\rat(4/9){8}{}&\ln{1}&\cnt{125}&\bounds{25}{25}{1}{false}&&\cr
\l{4}&\rat(26/9){4}{}&\rat(5/9){1}{}&\rat(5/9){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(11/3){3}{}&\rat(1/3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(8/3){3}{}&\rat(4/3){6}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(7/3){6}{}&\rat(5/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(22/9){2}{}&\rat(10/9){2}{}&\rat(4/9){8}{}&\ln{2}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(11/9){1}{}&\rat(20/9){4}{}&\rat(5/9){1}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 77
\orbit{3}{77}{141}
\h{77}&\rat(32/9){7}{\spec{1}}&\rat(38/9){4}{\spec{2}}&\rat(38/9){4}{\spec{2}}&&\cnt{943}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\rat(8/9){4}{}&\rat(14/9){1}{}&\rat(14/9){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(8/9){7}{}&\rat(14/9){1}{}&\ln{2}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(16/9){8}{}&\rat(16/9){5}{}&\rat(4/9){8}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(16/9){8}{}&\rat(19/9){2}{}&\rat(1/9){2}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(16/9){8}{}&\rat(10/9){2}{\spec{1}}&\rat(10/9){2}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(16/9){8}{}&\rat(10/9){2}{\spec{1}}&\rat(10/9){2}{\spec{2}}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(16/9){8}{}&\rat(10/9){2}{\spec{2}}&\rat(10/9){2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(2/9){1}{}&\rat(20/9){4}{}&\rat(14/9){1}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(-2/9){8}{}&\rat(19/9){2}{}&\rat(19/9){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 78
\orbit{3}{78}{141}
\h{78}&\int(6){\6}{\spec{1}}&\int(4){\4}{}&\int(2){\2}{}&&\cnt{811}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(1){8}{}&\int(1){8}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(1){1}{}&\int(1){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(2){7}{}&\int(2){7}{}&\int(0){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(2){7}{}&\int(1){7}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\int(2){7}{}&\int(1){1}{}&\int(1){7}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\int(2){2}{}&\int(2){2}{}&\int(0){8}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(2){2}{}&\int(1){2}{}&\int(1){8}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(2){2}{}&\int(1){8}{}&\int(1){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(1){7}{}&\int(2){7}{}&\int(1){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(1){2}{}&\int(2){2}{}&\int(1){8}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(2){8}{}&\int(2){5}{}&\int(0){8}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{21}&\int(2){8}{}&\int(1){5}{\spec{1}}&\int(1){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(2){8}{}&\int(1){5}{\spec{2}}&\int(1){8}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\int(2){8}{}&\int(2){2}{}&\int(0){2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\int(2){8}{}&\int(2){2}{}&\int(0){2}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\int(2){8}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{26}&\int(2){8}{}&\int(1){8}{}&\int(1){5}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{27}&\int(1){1}{}&\int(2){4}{}&\int(1){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{28}&\int(1){1}{}&\int(2){7}{}&\int(1){7}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 79
\orbit{3}{79}{141}
\h{79}&\rat(26/9){8}{\spec{2}}&\rat(50/9){2}{\spec{1}}&\rat(32/9){2}{\spec{1}}&&\cnt{759}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(11/9){8}{}&\rat(11/9){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(13/9){4}{}&\rat(16/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(16/9){7}{}&\rat(16/9){1}{}&\rat(4/9){7}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(16/9){7}{}&\rat(16/9){1}{}&\rat(4/9){7}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(16/9){7}{}&\rat(7/9){1}{}&\rat(13/9){7}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(11/9){2}{}&\rat(23/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(11/9){2}{}&\rat(14/9){2}{}&\rat(11/9){8}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(7/9){7}{}&\rat(16/9){1}{}&\rat(13/9){7}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(2/9){2}{\spec{1}}&\rat(23/9){2}{}&\rat(11/9){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(2/9){2}{\spec{2}}&\rat(23/9){2}{}&\rat(11/9){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{21}&\rat(10/9){1}{}&\rat(13/9){7}{}&\rat(13/9){7}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{22}&\rat(10/9){1}{}&\rat(16/9){1}{}&\rat(10/9){4}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\rat(10/9){1}{}&\rat(16/9){1}{}&\rat(10/9){4}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\rat(10/9){1}{}&\rat(7/9){1}{}&\rat(19/9){4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\rat(8/9){8}{}&\rat(17/9){5}{}&\rat(11/9){8}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{26}&\rat(8/9){8}{}&\rat(23/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{27}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{28}&\rat(8/9){8}{}&\rat(11/9){8}{}&\rat(17/9){5}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{29}&\rat(1/9){1}{}&\rat(16/9){1}{}&\rat(19/9){4}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{30}&\rat(-1/9){8}{}&\rat(23/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{31}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{32}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{33}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{34}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{35}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{36}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{37}&\int(0){\0}{}&\rat(5/3){6}{}&\rat(7/3){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 80
\orbit{3}{80}{141}
\h{80}&\int(8){\8}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{867}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){5}{\spec{2}}&\int(1){8}{}&\int(0){8}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(3){4}{\spec{2}}&\int(1){1}{}&\int(0){1}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){5}{\spec{3}}&\int(1){8}{}&\int(1){8}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){5}{\spec{4}}&\int(1){8}{}&\int(1){8}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){4}{\spec{3}}&\int(1){1}{}&\int(1){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){4}{\spec{4}}&\int(1){1}{}&\int(1){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(3){6}{\spec{2}}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(3){3}{\spec{2}}&\int(1){6}{}&\int(0){\0}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(3){7}{}&\int(1){7}{}&\int(0){1}{}&\ln{2}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{16}&\int(3){7}{}&\int(0){7}{\spec{1}}&\int(1){1}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(3){7}{}&\int(0){7}{\spec{2}}&\int(1){1}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(2){7}{\spec{2}}&\int(1){7}{}&\int(1){1}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(2){2}{\spec{2}}&\int(1){2}{}&\int(1){8}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(2){8}{}&\int(1){5}{}&\int(1){8}{}&\ln{2}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{21}&\int(2){8}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{22}&\int(0){\0}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 81
\orbit{3}{81}{141}
\h{81}&\int(8){6}{\spec{1}}&\int(4){3}{\spec{1}}&\int(0){\0}{}&&\cnt{971}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(8/3){5}{}&\rat(4/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){3}{}&\int(1){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(8/3){2}{}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{12}&\rat(8/3){2}{}&\rat(4/3){8}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(7/3){1}{}&\rat(5/3){4}{}&\int(0){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(7/3){1}{}&\rat(5/3){7}{}&\int(0){7}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 82
\orbit{3}{82}{141}
\h{82}&\int(8){6}{\spec{2}}&\int(4){3}{\spec{1}}&\int(0){\0}{}&&\cnt{803}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(11/3){5}{}&\rat(1/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(10/3){4}{\spec{2}}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(8/3){5}{\spec{2}}&\rat(4/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(3){3}{}&\int(1){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(3){3}{}&\int(1){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){6}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){6}{\spec{3}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\int(2){3}{\spec{2}}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(2){3}{\spec{3}}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(8/3){2}{\spec{2}}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(8/3){2}{\spec{2}}&\rat(4/3){8}{}&\int(0){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(7/3){7}{}&\rat(5/3){7}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(5/3){8}{}&\rat(7/3){5}{}&\int(0){8}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\rat(4/3){1}{\spec{2}}&\rat(8/3){4}{}&\int(0){1}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 83
\orbit{3}{83}{139}
\h{83}&\int(6){6}{\spec{2}}&\int(2){3}{}&\int(4){\4}{}&&\cnt{703}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(10/3){4}{}&\rat(-1/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(8/3){5}{}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(7/3){4}{}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){3}{}&\int(0){\0}{}&\int(1){6}{\spec{1}}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(3){3}{}&\int(0){\0}{}&\int(1){6}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(2){3}{\spec{1}}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\int(2){3}{\spec{2}}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(8/3){2}{}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(8/3){2}{}&\rat(1/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(8/3){2}{}&\rat(1/3){8}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(8/3){2}{}&\rat(-2/3){8}{}&\int(2){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(5/3){2}{}&\rat(1/3){8}{}&\int(2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(4/3){1}{}&\rat(5/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\rat(4/3){1}{}&\rat(2/3){7}{}&\int(2){7}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\rat(4/3){1}{}&\rat(2/3){1}{}&\int(2){4}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{24}&\rat(2/3){8}{}&\rat(4/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 84
\orbit{3}{84}{139}
\h{84}&\rat(8/9){8}{}&\rat(68/9){2}{\spec{1}}&\rat(32/9){2}{\spec{1}}&&\cnt{811}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(2/3){6}{}&\rat(10/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(7/9){7}{}&\rat(16/9){1}{}&\rat(13/9){7}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(2/9){2}{}&\rat(23/9){2}{}&\rat(11/9){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(17/9){5}{\spec{1}}&\rat(11/9){8}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{}&\rat(17/9){5}{\spec{2}}&\rat(11/9){8}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(8/9){8}{}&\rat(23/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(8/9){8}{}&\rat(14/9){2}{\spec{1}}&\rat(14/9){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(8/9){8}{}&\rat(14/9){2}{\spec{2}}&\rat(14/9){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(8/9){8}{}&\rat(11/9){8}{}&\rat(17/9){5}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(1/9){1}{}&\rat(22/9){7}{}&\rat(13/9){7}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(1/9){1}{}&\rat(16/9){1}{}&\rat(19/9){4}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\rat(-1/9){8}{}&\rat(26/9){5}{}&\rat(11/9){8}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(-1/9){8}{}&\rat(23/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(10/3){3}{}&\rat(2/3){6}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(10/3){3}{}&\rat(2/3){6}{\spec{2}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\rat(5/3){6}{\spec{1}}&\rat(7/3){3}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\rat(5/3){6}{\spec{2}}&\rat(7/3){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 85
\orbit{3}{85}{139}
\h{85}&\rat(44/9){8}{\spec{1}}&\rat(44/9){8}{\spec{2}}&\rat(20/9){5}{}&&\cnt{755}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(4/3){3}{}&\rat(8/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(16/9){7}{}&\rat(16/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(11/9){2}{}&\rat(20/9){2}{}&\rat(5/9){8}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(17/9){8}{}&\rat(23/9){5}{}&\rat(-4/9){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(17/9){8}{}&\rat(14/9){5}{\spec{1}}&\rat(5/9){8}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{12}&\rat(17/9){8}{}&\rat(14/9){5}{\spec{2}}&\rat(5/9){8}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(17/9){8}{}&\rat(20/9){2}{}&\rat(-1/9){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(17/9){8}{}&\rat(11/9){2}{}&\rat(8/9){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(10/9){1}{}&\rat(22/9){4}{}&\rat(4/9){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(10/9){1}{}&\rat(16/9){7}{}&\rat(10/9){7}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 86
\orbit{3}{86}{139}
\h{86}&\rat(32/9){7}{\spec{2}}&\rat(38/9){4}{\spec{1}}&\rat(38/9){4}{\spec{2}}&&\cnt{703}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\rat(19/9){5}{}&\rat(13/9){8}{}&\rat(4/9){8}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(17/9){4}{}&\rat(5/9){1}{}&\rat(14/9){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(7/3){6}{}&\rat(5/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(7/3){6}{}&\int(0){\0}{}&\rat(5/3){3}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(5/3){3}{}&\rat(7/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(4/3){6}{}&\int(0){\0}{}&\rat(8/3){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(14/9){7}{}&\rat(8/9){7}{\spec{1}}&\rat(14/9){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(14/9){7}{}&\rat(8/9){7}{\spec{2}}&\rat(14/9){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(13/9){2}{}&\rat(13/9){8}{}&\rat(10/9){2}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(13/9){2}{}&\rat(13/9){8}{}&\rat(10/9){2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(13/9){2}{}&\rat(4/9){8}{}&\rat(19/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(5/9){7}{}&\rat(17/9){7}{}&\rat(14/9){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{16}&\rat(4/9){2}{\spec{1}}&\rat(13/9){8}{}&\rat(19/9){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(4/9){2}{\spec{2}}&\rat(13/9){8}{}&\rat(19/9){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(11/9){1}{}&\rat(20/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(11/9){1}{}&\rat(11/9){4}{}&\rat(14/9){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(11/9){1}{}&\rat(17/9){7}{}&\rat(8/9){7}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{21}&\rat(11/9){1}{}&\rat(5/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{22}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\rat(7/9){8}{}&\rat(10/9){2}{}&\rat(19/9){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{24}&\rat(7/9){8}{}&\rat(13/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{25}&\rat(2/9){1}{}&\rat(20/9){4}{}&\rat(14/9){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\rat(4/3){6}{\spec{1}}&\rat(8/3){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\rat(4/3){6}{\spec{2}}&\rat(8/3){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 87
\orbit{3}{87}{138}
\h{87}&\int(8){6}{\spec{4}}&\int(4){3}{\spec{1}}&\int(0){\0}{}&&\cnt{1127}&\bounds{138}{138}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(7/3){7}{}&\rat(5/3){7}{}&\int(0){1}{}&\ln{1}&\cnt{288}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{}&\rat(4/3){5}{\spec{1}}&\int(0){8}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(8/3){8}{}&\rat(4/3){5}{\spec{2}}&\int(0){8}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\rat(8/3){8}{}&\rat(4/3){2}{}&\int(0){2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(8/3){8}{}&\rat(4/3){8}{}&\int(0){5}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 88
\orbit{3}{88}{138}
\h{88}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1007}&\bounds{138}{138}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{7}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(4){5}{\spec{2}}&\int(0){8}{}&\int(0){8}{}&\ln{2}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\int(4){6}{}&\int(0){3}{}&\int(0){\0}{}&\ln{4}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 89
\orbit{3}{89}{138}
\h{89}&\rat(62/9){8}{\spec{2}}&\rat(32/9){2}{\spec{2}}&\rat(14/9){2}{}&&\cnt{943}&\bounds{138}{138}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(32/9){5}{}&\rat(2/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(31/9){4}{}&\rat(-2/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(22/9){4}{\spec{1}}&\rat(16/9){1}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(22/9){4}{\spec{2}}&\rat(16/9){1}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(13/9){4}{}&\rat(16/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(10/3){3}{}&\rat(2/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(10/3){3}{}&\int(0){\0}{}&\rat(2/3){6}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\rat(8/3){6}{}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(20/9){2}{}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{13}&\rat(20/9){2}{}&\rat(2/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(16/9){7}{}&\rat(16/9){1}{}&\rat(4/9){7}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{15}&\rat(10/9){1}{}&\rat(16/9){1}{}&\rat(10/9){4}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{16}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 90
\orbit{3}{90}{137}
\h{90}&\int(6){6}{\spec{2}}&\int(6){3}{\spec{2}}&\int(0){\0}{}&&\cnt{943}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{}&\rat(2/3){1}{}&\int(0){1}{}&\ln{2}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(8/3){5}{}&\rat(4/3){8}{}&\int(0){8}{}&\ln{2}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(2){3}{\spec{1}}&\int(2){6}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){3}{\spec{1}}&\int(2){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\int(2){3}{\spec{2}}&\int(2){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(8/3){2}{}&\rat(4/3){2}{}&\int(0){8}{}&\ln{2}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(8/3){2}{}&\rat(4/3){8}{}&\int(0){2}{}&\ln{2}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 91
\orbit{3}{91}{137}
\h{91}&\rat(26/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(74/9){5}{\spec{1}}&&\cnt{807}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(4/3){3}{}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(2/3){6}{\spec{1}}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(2/3){6}{\spec{2}}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(16/9){7}{}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(16/9){7}{}&\rat(1/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(11/9){2}{}&\rat(-1/9){8}{}&\rat(26/9){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(2/9){2}{\spec{1}}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(2/9){2}{\spec{2}}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(10/9){1}{}&\rat(7/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(10/9){1}{}&\rat(-8/9){1}{}&\rat(34/9){4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(8/9){8}{}&\rat(2/9){2}{}&\rat(26/9){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{21}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{2}}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\rat(8/9){8}{}&\rat(-1/9){8}{}&\rat(29/9){5}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{24}&\rat(1/9){1}{}&\rat(1/9){1}{}&\rat(34/9){4}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\rat(-1/9){8}{}&\rat(8/9){8}{}&\rat(29/9){5}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\rat(2/3){6}{}&\rat(10/3){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 92
\orbit{3}{92}{137}
\h{92}&\int(6){6}{\spec{1}}&\int(6){3}{\spec{1}}&\int(0){\0}{}&&\cnt{931}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(8/3){5}{}&\rat(4/3){8}{}&\int(0){8}{}&\ln{2}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(7/3){4}{}&\rat(5/3){1}{}&\int(0){1}{}&\ln{2}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(3){6}{}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){6}{}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){6}{}&\int(1){3}{\spec{3}}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{\spec{3}}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{2}}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(7/3){7}{}&\rat(5/3){7}{}&\int(0){1}{}&\ln{2}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(7/3){7}{}&\rat(5/3){1}{}&\int(0){7}{}&\ln{2}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 93
\orbit{3}{93}{137}
\h{93}&\rat(26/9){8}{\spec{2}}&\rat(26/9){8}{\spec{2}}&\rat(56/9){5}{\spec{2}}&&\cnt{819}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(4/3){3}{}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{2}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(16/9){7}{}&\rat(16/9){7}{}&\rat(4/9){1}{\spec{2}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{\spec{2}}&\ln{2}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(16/9){7}{}&\rat(-8/9){1}{}&\rat(28/9){7}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(11/9){2}{}&\rat(11/9){2}{}&\rat(14/9){8}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(7/9){7}{}&\rat(1/9){1}{}&\rat(28/9){7}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(-2/9){7}{\spec{1}}&\rat(10/9){1}{}&\rat(28/9){7}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(-2/9){7}{\spec{2}}&\rat(10/9){1}{}&\rat(28/9){7}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{\spec{2}}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{13}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{2}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 94
\orbit{3}{94}{137}
\h{94}&\rat(8/9){8}{}&\rat(86/9){2}{\spec{1}}&\rat(14/9){2}{}&&\cnt{927}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\rat(4/9){4}{}&\rat(25/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(7/9){7}{}&\rat(25/9){1}{}&\rat(4/9){7}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\rat(8/9){8}{}&\rat(23/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(1/9){1}{}&\rat(25/9){1}{}&\rat(10/9){4}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\rat(-1/9){8}{}&\rat(23/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 95
\orbit{3}{95}{136}
\h{95}&\rat(62/9){8}{\spec{2}}&\rat(32/9){2}{\spec{1}}&\rat(14/9){2}{}&&\cnt{699}&\bounds{136}{136}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(32/9){5}{}&\rat(11/9){8}{}&\rat(-7/9){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(32/9){5}{}&\rat(2/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(31/9){4}{}&\rat(7/9){1}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(31/9){4}{}&\rat(-2/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(23/9){5}{}&\rat(11/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(22/9){4}{\spec{1}}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(22/9){4}{\spec{2}}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(10/3){3}{}&\rat(2/3){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(10/3){3}{}&\rat(2/3){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(10/3){3}{}&\int(0){\0}{}&\rat(2/3){6}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\rat(8/3){6}{}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(7/3){3}{}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{16}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(20/9){2}{}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{18}&\rat(20/9){2}{}&\rat(11/9){8}{}&\rat(5/9){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(20/9){2}{}&\rat(2/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 96
\orbit{3}{96}{136}
\h{96}&\rat(44/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(56/9){5}{\spec{1}}&&\cnt{931}&\bounds{136}{136}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{3}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(4/3){3}{}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(16/9){7}{}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\rat(16/9){7}{}&\rat(1/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{13}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(17/9){8}{}&\rat(5/9){5}{}&\rat(14/9){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(17/9){8}{}&\rat(2/9){2}{}&\rat(17/9){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{\spec{3}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(10/9){1}{}&\rat(7/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\rat(-1/9){8}{}&\rat(8/9){8}{}&\rat(29/9){5}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 97
\orbit{3}{97}{136}
\h{97}&\int(10){6}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&&\cnt{1019}&\bounds{136}{136}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(10/3){4}{\spec{1}}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(4){3}{\spec{1}}&\int(0){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(4){3}{\spec{1}}&\int(0){\0}{}&\int(0){6}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(3){3}{\spec{1}}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(2){6}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(11/3){2}{}&\rat(1/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\rat(11/3){2}{}&\rat(1/3){8}{}&\int(0){2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(8/3){2}{\spec{1}}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(7/3){1}{}&\rat(5/3){4}{}&\int(0){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 98
\orbit{3}{98}{136}
\h{98}&\rat(8/9){8}{}&\rat(86/9){2}{\spec{5}}&\rat(14/9){2}{}&&\cnt{971}&\bounds{136}{136}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(1/3){3}{}&\rat(11/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(7/9){7}{}&\rat(31/9){7}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(2/9){2}{}&\rat(20/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(-2/9){7}{}&\rat(31/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(35/9){5}{}&\rat(-7/9){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(8/9){8}{}&\rat(20/9){8}{}&\rat(8/9){5}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(1/9){1}{}&\rat(31/9){7}{}&\rat(4/9){7}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{13}&\rat(-1/9){8}{}&\rat(35/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(11/3){6}{}&\rat(1/3){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(8/3){6}{\spec{1}}&\rat(4/3){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(8/3){6}{\spec{2}}&\rat(4/3){3}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 99
\orbit{3}{99}{135}
\h{99}&\int(8){\8}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{819}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){5}{}&\int(1){8}{}&\int(-1){8}{}&\ln{4}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){5}{}&\int(0){8}{}&\int(0){8}{}&\ln{2}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(3){5}{}&\int(1){8}{}&\int(0){8}{}&\ln{4}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){5}{}&\int(1){8}{}&\int(1){8}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{4}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){7}{}&\int(1){7}{}&\int(1){1}{}&\ln{4}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 100
\orbit{3}{100}{135}
\h{100}&\rat(14/9){7}{}&\rat(56/9){4}{\spec{2}}&\rat(38/9){4}{\spec{2}}&&\cnt{819}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\rat(4/3){6}{}&\int(0){\0}{\spec{2}}&\rat(8/3){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(2/3){3}{}&\rat(10/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(14/9){7}{}&\rat(26/9){7}{}&\rat(-4/9){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(14/9){7}{}&\rat(8/9){7}{\spec{2}}&\rat(14/9){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(5/9){7}{}&\rat(26/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(5/9){7}{}&\rat(17/9){7}{}&\rat(14/9){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(4/9){2}{}&\rat(13/9){8}{}&\rat(19/9){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(-4/9){7}{}&\rat(26/9){7}{}&\rat(14/9){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(7/9){8}{}&\rat(10/9){2}{\spec{2}}&\rat(19/9){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(7/9){8}{}&\rat(13/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(2/9){1}{}&\rat(20/9){4}{\spec{2}}&\rat(14/9){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{14}&\rat(2/9){1}{}&\rat(26/9){7}{}&\rat(8/9){7}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(10/3){6}{}&\rat(2/3){3}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(10/3){6}{}&\rat(2/3){3}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(4/3){6}{\spec{2}}&\rat(8/3){3}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 101
\orbit{3}{101}{134}
\h{101}&\rat(32/9){7}{\spec{2}}&\rat(56/9){4}{\spec{2}}&\rat(20/9){4}{}&&\cnt{699}&\bounds{134}{134}{1}{false}&&\cr
\l{1}&\rat(19/9){5}{}&\rat(13/9){8}{}&\rat(4/9){8}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(7/3){6}{}&\rat(5/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(7/3){6}{}&\int(0){\0}{\spec{2}}&\rat(5/3){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(5/3){3}{}&\rat(7/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(2/3){3}{\spec{1}}&\rat(10/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(2/3){3}{\spec{2}}&\rat(10/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(14/9){7}{}&\rat(26/9){7}{}&\rat(-4/9){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(13/9){2}{}&\rat(13/9){8}{}&\rat(10/9){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(5/9){7}{}&\rat(26/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(11/9){1}{}&\rat(20/9){4}{\spec{2}}&\rat(5/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(11/9){1}{}&\rat(26/9){7}{}&\rat(-1/9){7}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(11/9){1}{}&\rat(17/9){7}{}&\rat(8/9){7}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(11/9){1}{}&\rat(5/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{17}&\rat(7/9){8}{}&\rat(13/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(2/9){1}{}&\rat(26/9){7}{}&\rat(8/9){7}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(10/3){6}{}&\rat(2/3){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 102
\orbit{3}{102}{134}
\h{102}&\int(6){6}{\spec{2}}&\int(4){3}{\spec{1}}&\int(2){\2}{}&&\cnt{699}&\bounds{134}{134}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(10/3){4}{}&\rat(-1/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/3){5}{}&\rat(4/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(8/3){5}{}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(7/3){4}{}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(5/3){5}{}&\rat(4/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){3}{}&\int(1){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){3}{}&\int(1){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(3){3}{}&\int(0){\0}{}&\int(1){6}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){3}{\spec{1}}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(2){3}{\spec{2}}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(8/3){2}{}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(8/3){2}{}&\rat(1/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(8/3){2}{}&\rat(4/3){8}{}&\int(0){2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(8/3){2}{}&\rat(4/3){8}{}&\int(0){2}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(8/3){2}{}&\rat(1/3){8}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\rat(5/3){2}{}&\rat(4/3){8}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(4/3){7}{}&\rat(5/3){7}{}&\int(1){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{24}&\rat(4/3){1}{}&\rat(8/3){4}{}&\int(0){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\rat(4/3){1}{}&\rat(5/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{26}&\rat(4/3){1}{}&\rat(5/3){7}{}&\int(1){7}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{27}&\rat(2/3){8}{}&\rat(7/3){5}{}&\int(1){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{28}&\rat(1/3){1}{}&\rat(8/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 103
\orbit{3}{103}{133}
\h{103}&\rat(14/9){7}{}&\rat(56/9){4}{\spec{1}}&\rat(38/9){4}{\spec{2}}&&\cnt{755}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\rat(8/9){4}{}&\rat(14/9){1}{}&\rat(14/9){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(4/3){6}{}&\int(0){\0}{}&\rat(8/3){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(14/9){7}{}&\rat(8/9){7}{\spec{1}}&\rat(14/9){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(14/9){7}{}&\rat(8/9){7}{\spec{2}}&\rat(14/9){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(5/9){7}{}&\rat(17/9){7}{}&\rat(14/9){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(4/9){2}{}&\rat(13/9){8}{}&\rat(19/9){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(7/9){8}{}&\rat(19/9){2}{}&\rat(10/9){2}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(7/9){8}{}&\rat(19/9){2}{}&\rat(10/9){2}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(7/9){8}{}&\rat(10/9){2}{\spec{1}}&\rat(19/9){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(7/9){8}{}&\rat(10/9){2}{\spec{2}}&\rat(19/9){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(7/9){8}{}&\rat(13/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(2/9){1}{}&\rat(29/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(2/9){1}{}&\rat(20/9){4}{}&\rat(14/9){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(-2/9){8}{}&\rat(19/9){2}{}&\rat(19/9){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(-7/9){1}{}&\rat(29/9){4}{}&\rat(14/9){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\rat(4/3){6}{\spec{1}}&\rat(8/3){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\rat(4/3){6}{\spec{2}}&\rat(8/3){3}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 104
\orbit{3}{104}{133}
\h{104}&\rat(62/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(38/9){5}{\spec{1}}&&\cnt{859}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{\spec{1}}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(23/9){5}{\spec{1}}&\rat(-1/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(14/9){5}{\spec{1}}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{\spec{1}}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(7/3){3}{\spec{1}}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(4/3){3}{\spec{1}}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(20/9){2}{\spec{1}}&\rat(2/9){2}{}&\rat(14/9){8}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\rat(20/9){2}{\spec{1}}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{14}&\rat(16/9){7}{\spec{1}}&\rat(1/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(19/9){1}{}&\rat(7/9){7}{}&\rat(10/9){7}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(19/9){1}{}&\rat(7/9){7}{}&\rat(10/9){7}{\spec{2}}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(19/9){1}{}&\rat(-2/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(19/9){1}{}&\rat(1/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{19}&\rat(8/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 105
\orbit{3}{105}{133}
\h{105}&\rat(62/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(38/9){5}{\spec{1}}&&\cnt{819}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(32/9){5}{}&\rat(8/9){8}{}&\rat(-4/9){8}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(32/9){5}{}&\rat(-1/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(31/9){4}{}&\rat(1/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(23/9){5}{}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(23/9){5}{}&\rat(-1/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(14/9){5}{\spec{1}}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(14/9){5}{\spec{2}}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(10/3){3}{}&\rat(2/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(10/3){3}{}&\int(0){\0}{}&\rat(2/3){6}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(10/3){3}{}&\int(0){\0}{}&\rat(2/3){6}{\spec{2}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(7/3){3}{}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(4/3){3}{\spec{1}}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(4/3){3}{\spec{2}}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(20/9){2}{}&\rat(2/9){2}{}&\rat(14/9){8}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\rat(16/9){7}{}&\rat(1/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(10/9){1}{}&\rat(7/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 106
\orbit{3}{106}{133}
\h{106}&\rat(26/9){8}{\spec{2}}&\rat(26/9){8}{\spec{2}}&\rat(56/9){5}{\spec{2}}&&\cnt{695}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\rat(13/9){4}{}&\rat(10/9){1}{}&\rat(13/9){1}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(2/3){6}{\spec{1}}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(2/3){6}{\spec{2}}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(16/9){7}{}&\rat(16/9){7}{}&\rat(4/9){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(16/9){7}{}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{\spec{1}}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(11/9){2}{}&\rat(-1/9){8}{}&\rat(26/9){2}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(2/9){2}{\spec{1}}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(2/9){2}{\spec{2}}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{1}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 107
\orbit{3}{107}{133}
\h{107}&\rat(44/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(56/9){5}{\spec{2}}&&\cnt{819}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(22/9){4}{}&\rat(1/9){1}{}&\rat(13/9){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(7/3){3}{}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(2/3){6}{\spec{1}}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(2/3){6}{\spec{2}}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(20/9){2}{}&\rat(-1/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(16/9){7}{}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(11/9){2}{}&\rat(-1/9){8}{}&\rat(26/9){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(2/9){2}{\spec{1}}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(2/9){2}{\spec{2}}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(8/9){8}{}&\rat(2/9){2}{}&\rat(26/9){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{1}}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(2/3){6}{}&\rat(10/3){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 108
\orbit{3}{108}{133}
\h{108}&\rat(62/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(38/9){5}{\spec{2}}&&\cnt{807}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(23/9){5}{\spec{2}}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(22/9){4}{\spec{2}}&\rat(1/9){1}{}&\rat(13/9){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{\spec{2}}&\int(0){\0}{}&\rat(4/3){3}{\spec{1}}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(8/3){6}{\spec{2}}&\int(0){\0}{}&\rat(4/3){3}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(7/3){3}{\spec{2}}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(5/3){6}{\spec{2}}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(5/3){6}{\spec{3}}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(25/9){7}{}&\rat(7/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(25/9){7}{}&\rat(-2/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(25/9){7}{}&\rat(1/9){1}{}&\rat(10/9){7}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(20/9){2}{\spec{2}}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(20/9){2}{\spec{2}}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(20/9){2}{\spec{2}}&\rat(-1/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\rat(16/9){7}{\spec{2}}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{22}&\rat(11/9){2}{\spec{2}}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\rat(17/9){8}{}&\rat(2/9){2}{}&\rat(17/9){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{24}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{26}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\rat(8/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 109
\orbit{3}{109}{133}
\h{109}&\rat(44/9){8}{\spec{2}}&\rat(50/9){2}{\spec{1}}&\rat(14/9){2}{}&&\cnt{755}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{}&\rat(11/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(22/9){4}{}&\rat(16/9){1}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(22/9){4}{}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(13/9){4}{\spec{1}}&\rat(16/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(13/9){4}{\spec{2}}&\rat(16/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(8/3){6}{}&\rat(4/3){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{}&\rat(4/3){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(7/3){3}{}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(20/9){2}{}&\rat(23/9){2}{}&\rat(-7/9){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(20/9){2}{}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(20/9){2}{}&\rat(11/9){8}{}&\rat(5/9){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(20/9){2}{}&\rat(2/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(16/9){7}{}&\rat(16/9){1}{}&\rat(4/9){7}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{22}&\rat(11/9){2}{}&\rat(23/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{25}&\rat(10/9){1}{}&\rat(16/9){1}{}&\rat(10/9){4}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{26}&\rat(8/9){8}{}&\rat(23/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{27}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{28}&\rat(-1/9){8}{}&\rat(23/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 110
\orbit{3}{110}{133}
\h{110}&\rat(26/9){8}{\spec{2}}&\rat(50/9){2}{\spec{2}}&\rat(32/9){2}{\spec{2}}&&\cnt{819}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\rat(13/9){4}{}&\rat(7/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(4/3){3}{}&\rat(8/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(16/9){7}{}&\rat(22/9){7}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(16/9){7}{}&\rat(4/9){7}{\spec{1}}&\rat(16/9){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(16/9){7}{}&\rat(4/9){7}{\spec{2}}&\rat(16/9){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/9){7}{}&\rat(13/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(-2/9){7}{\spec{1}}&\rat(22/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(-2/9){7}{\spec{2}}&\rat(22/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(10/9){1}{}&\rat(28/9){4}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(10/9){1}{}&\rat(10/9){4}{\spec{1}}&\rat(16/9){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(10/9){1}{}&\rat(10/9){4}{\spec{2}}&\rat(16/9){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(10/9){1}{}&\rat(22/9){7}{}&\rat(4/9){7}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(1/9){1}{}&\rat(19/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(-8/9){1}{}&\rat(28/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 111
\orbit{3}{111}{133}
\h{111}&\rat(44/9){8}{\spec{1}}&\rat(32/9){2}{\spec{1}}&\rat(32/9){2}{\spec{1}}&&\cnt{755}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(11/9){8}{}&\rat(11/9){8}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{2}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(11/9){2}{}&\rat(14/9){2}{}&\rat(11/9){8}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(17/9){8}{}&\rat(17/9){5}{}&\rat(2/9){8}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(17/9){8}{}&\rat(8/9){5}{\spec{1}}&\rat(11/9){8}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(17/9){8}{}&\rat(8/9){5}{\spec{2}}&\rat(11/9){8}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(17/9){8}{}&\rat(14/9){2}{}&\rat(5/9){2}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(10/9){1}{}&\rat(13/9){7}{}&\rat(13/9){7}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 112
\orbit{3}{112}{132}
\h{112}&\rat(8/9){8}{}&\rat(86/9){2}{\spec{3}}&\rat(14/9){2}{}&&\cnt{859}&\bounds{132}{132}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(2/3){6}{}&\rat(10/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(1/3){3}{}&\rat(11/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(8/9){8}{}&\rat(35/9){5}{}&\rat(-7/9){8}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(26/9){5}{\spec{1}}&\rat(2/9){8}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(26/9){5}{\spec{2}}&\rat(2/9){8}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{}&\rat(23/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(8/9){8}{}&\rat(14/9){2}{\spec{1}}&\rat(14/9){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(8/9){8}{}&\rat(14/9){2}{\spec{2}}&\rat(14/9){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(1/9){1}{}&\rat(37/9){4}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(-1/9){8}{}&\rat(35/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{14}&\rat(-1/9){8}{}&\rat(23/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(-8/9){1}{}&\rat(37/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(11/3){6}{}&\rat(1/3){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(10/3){3}{}&\rat(2/3){6}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 113
\orbit{3}{113}{132}
\h{113}&\rat(8/9){8}{}&\rat(68/9){2}{\spec{2}}&\rat(32/9){2}{\spec{1}}&&\cnt{819}&\bounds{132}{132}{1}{false}&&\cr
\l{1}&\rat(1/3){3}{}&\rat(11/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(8/9){8}{}&\rat(35/9){5}{}&\rat(-7/9){8}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(8/9){8}{}&\rat(17/9){5}{}&\rat(11/9){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(11/9){8}{}&\rat(17/9){5}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(1/9){1}{}&\rat(22/9){7}{}&\rat(13/9){7}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(-1/9){8}{}&\rat(35/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(-1/9){8}{}&\rat(26/9){5}{}&\rat(11/9){8}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(11/3){6}{}&\rat(1/3){3}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\rat(11/3){6}{}&\rat(1/3){3}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(5/3){6}{}&\rat(7/3){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 114
\orbit{3}{114}{132}
\h{114}&\int(4){6}{\spec{1}}&\int(2){3}{}&\int(6){\6}{\spec{2}}&&\cnt{803}&\bounds{132}{132}{1}{false}&&\cr
\l{1}&\rat(4/3){4}{}&\rat(2/3){1}{}&\int(2){1}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(7/3){7}{}&\rat(-1/3){7}{}&\int(2){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(7/3){7}{}&\rat(2/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(7/3){7}{}&\rat(-1/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(4/3){7}{}&\rat(2/3){7}{}&\int(2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(5/3){8}{}&\rat(4/3){5}{}&\int(1){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(5/3){8}{}&\rat(4/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(5/3){8}{}&\rat(1/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{15}&\rat(5/3){8}{}&\rat(1/3){8}{}&\int(2){5}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\rat(2/3){8}{}&\rat(4/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(1/3){1}{}&\rat(5/3){4}{}&\int(2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 115
\orbit{3}{115}{131}
\h{115}&\int(4){6}{\spec{1}}&\int(4){3}{\spec{2}}&\int(4){\4}{}&&\cnt{819}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(4/3){4}{}&\rat(5/3){1}{}&\int(1){1}{}&\ln{2}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(7/3){7}{}&\rat(2/3){7}{}&\int(1){1}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(7/3){7}{}&\rat(5/3){1}{}&\int(0){7}{\spec{1}}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(7/3){7}{}&\rat(5/3){1}{}&\int(0){7}{\spec{2}}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(7/3){7}{}&\rat(2/3){1}{}&\int(1){7}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(7/3){7}{}&\rat(-1/3){1}{}&\int(2){7}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(4/3){7}{}&\rat(5/3){1}{}&\int(1){7}{}&\ln{2}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(1/3){7}{}&\rat(5/3){1}{}&\int(2){7}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(5/3){8}{}&\rat(1/3){8}{}&\int(2){5}{}&\ln{2}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 116
\orbit{3}{116}{131}
\h{116}&\int(4){6}{\spec{1}}&\int(4){3}{\spec{1}}&\int(4){\4}{}&&\cnt{699}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(5/3){5}{}&\rat(4/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(7/3){7}{}&\rat(5/3){7}{}&\int(0){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(7/3){7}{}&\rat(2/3){7}{\spec{1}}&\int(1){1}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(7/3){7}{}&\rat(2/3){7}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(7/3){7}{}&\rat(2/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(7/3){7}{}&\rat(-1/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(4/3){7}{}&\rat(5/3){7}{}&\int(1){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(2/3){2}{}&\rat(4/3){8}{}&\int(2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(5/3){8}{}&\rat(7/3){5}{}&\int(0){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(5/3){8}{}&\rat(4/3){5}{\spec{1}}&\int(1){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(5/3){8}{}&\rat(4/3){5}{\spec{2}}&\int(1){8}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(5/3){8}{}&\rat(4/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(5/3){8}{}&\rat(1/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(5/3){8}{}&\rat(4/3){8}{}&\int(1){5}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(5/3){8}{}&\rat(4/3){8}{}&\int(1){5}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(5/3){8}{}&\rat(1/3){8}{}&\int(2){5}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\rat(2/3){8}{}&\rat(7/3){5}{}&\int(1){8}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(2/3){8}{}&\rat(4/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\rat(2/3){8}{}&\rat(4/3){8}{}&\int(2){5}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\rat(1/3){1}{}&\rat(8/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\rat(1/3){1}{}&\rat(5/3){7}{}&\int(2){7}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){6}{}&\int(2){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{30}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 117
\orbit{3}{117}{131}
\h{117}&\int(6){6}{\spec{2}}&\int(4){3}{\spec{2}}&\int(2){\2}{}&&\cnt{819}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{}&\rat(5/3){1}{}&\int(-1){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(10/3){4}{}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(10/3){4}{}&\rat(-1/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/3){5}{}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(7/3){4}{}&\rat(5/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(7/3){4}{}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/3){4}{\spec{1}}&\rat(5/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(4/3){4}{\spec{2}}&\rat(5/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\int(3){3}{}&\int(0){\0}{}&\int(1){6}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(8/3){2}{}&\rat(7/3){2}{}&\int(-1){8}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(8/3){2}{}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{17}&\rat(8/3){2}{}&\rat(1/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(8/3){2}{}&\rat(1/3){8}{}&\int(1){2}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{19}&\rat(5/3){2}{}&\rat(7/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(4/3){7}{}&\rat(5/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{22}&\rat(2/3){2}{\spec{1}}&\rat(7/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(2/3){2}{\spec{2}}&\rat(7/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\rat(4/3){1}{}&\rat(5/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\rat(4/3){1}{}&\rat(5/3){1}{}&\int(1){4}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{26}&\rat(2/3){8}{}&\rat(7/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 118
\orbit{3}{118}{131}
\h{118}&\int(8){6}{\spec{4}}&\int(4){3}{\spec{2}}&\int(0){\0}{}&&\cnt{1115}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\rat(7/3){7}{}&\rat(5/3){1}{}&\int(0){7}{}&\ln{1}&\cnt{288}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{}&\rat(4/3){5}{}&\int(0){8}{}&\ln{1}&\cnt{315}&\bounds{35}{35}{1}{false}&&\cr
\l{6}&\rat(8/3){8}{}&\rat(4/3){2}{}&\int(0){2}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 119
\orbit{3}{119}{130}
\h{119}&\int(4){6}{\spec{1}}&\int(2){3}{}&\int(6){\6}{\spec{1}}&&\cnt{803}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\rat(5/3){5}{}&\rat(1/3){8}{}&\int(2){8}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(7/3){7}{}&\rat(2/3){7}{}&\int(1){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(7/3){7}{}&\rat(2/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(7/3){7}{}&\rat(-1/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(2/3){2}{}&\rat(4/3){2}{}&\int(2){8}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(5/3){8}{}&\rat(1/3){5}{}&\int(2){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(5/3){8}{}&\rat(4/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(5/3){8}{}&\rat(1/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(5/3){8}{}&\rat(1/3){8}{}&\int(2){5}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{16}&\rat(2/3){8}{}&\rat(4/3){5}{}&\int(2){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(2/3){8}{}&\rat(4/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 120
\orbit{3}{120}{130}
\h{120}&\int(8){\8}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{859}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){5}{\spec{2}}&\int(1){8}{}&\int(0){8}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){4}{\spec{2}}&\int(1){1}{}&\int(0){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(3){6}{\spec{2}}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){6}{\spec{2}}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(3){3}{\spec{2}}&\int(1){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){3}{\spec{2}}&\int(1){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){6}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){6}{\spec{3}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(2){3}{\spec{3}}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(3){7}{}&\int(1){7}{}&\int(0){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\int(3){7}{}&\int(1){1}{}&\int(0){7}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(2){7}{\spec{2}}&\int(2){7}{}&\int(0){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(2){2}{\spec{2}}&\int(2){2}{}&\int(0){8}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(2){8}{}&\int(2){5}{}&\int(0){8}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{21}&\int(2){8}{}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 121
\orbit{3}{121}{130}
\h{121}&\int(8){6}{\spec{1}}&\int(4){3}{\spec{2}}&\int(0){\0}{}&&\cnt{959}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/3){4}{}&\rat(5/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(8/3){2}{}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{10}&\rat(5/3){2}{}&\rat(7/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(7/3){1}{}&\rat(5/3){4}{}&\int(0){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{12}&\rat(7/3){1}{}&\rat(5/3){1}{}&\int(0){4}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 122
\orbit{3}{122}{130}
\h{122}&\rat(32/9){7}{\spec{1}}&\rat(38/9){4}{\spec{1}}&\rat(38/9){4}{\spec{1}}&&\cnt{819}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\rat(10/9){5}{}&\rat(13/9){8}{}&\rat(13/9){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{2}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(16/9){8}{}&\rat(25/9){5}{}&\rat(-5/9){8}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(16/9){8}{}&\rat(16/9){5}{}&\rat(4/9){8}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(16/9){8}{}&\rat(7/9){5}{\spec{1}}&\rat(13/9){8}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(16/9){8}{}&\rat(7/9){5}{\spec{2}}&\rat(13/9){8}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(16/9){8}{}&\rat(10/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(2/9){1}{}&\rat(17/9){7}{}&\rat(17/9){7}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(-2/9){8}{}&\rat(25/9){5}{}&\rat(13/9){8}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 123
\orbit{3}{123}{129}
\h{123}&\rat(32/9){7}{\spec{2}}&\rat(38/9){4}{\spec{2}}&\rat(38/9){4}{\spec{2}}&&\cnt{699}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\rat(17/9){4}{}&\rat(14/9){1}{}&\rat(5/9){1}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(8/9){4}{\spec{1}}&\rat(14/9){1}{}&\rat(14/9){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(8/9){4}{\spec{2}}&\rat(14/9){1}{}&\rat(14/9){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(7/3){6}{}&\rat(5/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(14/9){7}{}&\rat(8/9){7}{}&\rat(14/9){1}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(13/9){2}{}&\rat(19/9){2}{}&\rat(4/9){8}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(11/9){1}{}&\rat(20/9){4}{}&\rat(5/9){1}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(11/9){1}{}&\rat(11/9){4}{}&\rat(14/9){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(7/9){8}{}&\rat(19/9){2}{}&\rat(10/9){2}{\spec{1}}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(7/9){8}{}&\rat(19/9){2}{}&\rat(10/9){2}{\spec{2}}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(2/9){1}{}&\rat(20/9){4}{}&\rat(14/9){1}{}&\ln{2}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(-2/9){8}{}&\rat(19/9){2}{}&\rat(19/9){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 124
\orbit{3}{124}{129}
\h{124}&\int(4){6}{\spec{1}}&\int(2){3}{}&\int(6){\6}{}&&\cnt{695}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(1){6}{}&\int(0){\0}{}&\int(3){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(1){3}{}&\int(0){\0}{}&\int(3){6}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\rat(7/3){7}{}&\rat(2/3){7}{}&\int(1){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(7/3){7}{}&\rat(2/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(7/3){7}{}&\rat(-1/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(5/3){8}{}&\rat(4/3){5}{}&\int(1){8}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\rat(5/3){8}{}&\rat(4/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(5/3){8}{}&\rat(1/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(5/3){8}{}&\rat(1/3){8}{}&\int(2){5}{\spec{1}}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(5/3){8}{}&\rat(1/3){8}{}&\int(2){5}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(5/3){8}{}&\rat(-2/3){8}{}&\int(3){5}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(2/3){8}{}&\rat(4/3){2}{}&\int(2){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(2/3){8}{}&\rat(1/3){8}{}&\int(3){5}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(1/3){1}{}&\rat(2/3){1}{}&\int(3){4}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){3}{}&\int(2){6}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){6}{}&\int(3){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(1){3}{}&\int(3){6}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 125
\orbit{3}{125}{129}
\h{125}&\int(8){6}{\spec{3}}&\int(2){3}{}&\int(2){\2}{}&&\cnt{803}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(8/3){5}{}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(7/3){4}{}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(3){6}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(10/3){7}{}&\rat(2/3){7}{}&\int(0){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(10/3){7}{}&\rat(-1/3){7}{}&\int(1){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(10/3){7}{}&\rat(2/3){1}{}&\int(0){7}{\spec{1}}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(10/3){7}{}&\rat(2/3){1}{}&\int(0){7}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(10/3){7}{}&\rat(-1/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(5/3){8}{}&\rat(4/3){5}{}&\int(1){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(5/3){8}{}&\rat(4/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(4/3){1}{}&\rat(5/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 126
\orbit{3}{126}{129}
\h{126}&\int(4){6}{\spec{1}}&\int(4){6}{\spec{1}}&\int(4){6}{\spec{2}}&&\cnt{819}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\rat(5/3){5}{}&\rat(5/3){8}{}&\rat(2/3){8}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(7/3){7}{}&\rat(7/3){7}{}&\rat(-2/3){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(7/3){7}{}&\rat(4/3){7}{}&\rat(1/3){1}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(7/3){7}{}&\rat(1/3){7}{}&\rat(4/3){1}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(7/3){7}{}&\rat(1/3){1}{}&\rat(4/3){7}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(4/3){7}{}&\rat(4/3){7}{}&\rat(4/3){1}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(2/3){2}{}&\rat(5/3){8}{}&\rat(5/3){2}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(5/3){8}{}&\rat(5/3){8}{}&\rat(2/3){5}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(5/3){8}{}&\rat(5/3){8}{}&\rat(2/3){5}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(5/3){8}{}&\rat(2/3){8}{}&\rat(5/3){5}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(5/3){8}{}&\rat(-1/3){8}{}&\rat(8/3){5}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(2/3){8}{}&\rat(2/3){8}{}&\rat(8/3){5}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 127
\orbit{3}{127}{129}
\h{127}&\int(6){6}{\spec{1}}&\int(4){6}{\spec{1}}&\int(2){6}{}&&\cnt{751}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(8/3){5}{}&\rat(5/3){8}{}&\rat(-1/3){8}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(8/3){5}{}&\rat(2/3){8}{}&\rat(2/3){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(5/3){5}{\spec{1}}&\rat(5/3){8}{}&\rat(2/3){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(5/3){5}{\spec{2}}&\rat(5/3){8}{}&\rat(2/3){8}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(3){6}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(2){3}{}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(7/3){7}{}&\rat(7/3){7}{}&\rat(-2/3){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(7/3){7}{}&\rat(4/3){7}{}&\rat(1/3){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(7/3){7}{}&\rat(1/3){1}{}&\rat(4/3){7}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(5/3){2}{}&\rat(5/3){8}{}&\rat(2/3){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{19}&\rat(4/3){7}{\spec{1}}&\rat(7/3){7}{}&\rat(1/3){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(4/3){7}{\spec{2}}&\rat(7/3){7}{}&\rat(1/3){1}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\rat(5/3){8}{}&\rat(5/3){5}{}&\rat(2/3){8}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{22}&\rat(5/3){8}{}&\rat(5/3){8}{}&\rat(2/3){5}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{23}&\rat(5/3){8}{}&\rat(2/3){8}{}&\rat(5/3){5}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\rat(4/3){1}{}&\rat(7/3){7}{}&\rat(1/3){7}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\rat(4/3){1}{}&\rat(4/3){7}{}&\rat(4/3){7}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{26}&\rat(2/3){8}{}&\rat(5/3){8}{}&\rat(5/3){5}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\rat(1/3){1}{}&\rat(7/3){7}{}&\rat(4/3){7}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 128
\orbit{3}{128}{129}
\h{128}&\rat(44/9){8}{\spec{1}}&\rat(26/9){8}{\spec{2}}&\rat(38/9){5}{\spec{2}}&&\cnt{751}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\rat(13/9){4}{}&\rat(10/9){1}{}&\rat(13/9){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(16/9){7}{}&\rat(16/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(16/9){7}{}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(7/9){7}{}&\rat(16/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(17/9){8}{}&\rat(14/9){5}{}&\rat(5/9){8}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\rat(17/9){8}{}&\rat(11/9){2}{}&\rat(8/9){2}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\rat(17/9){8}{}&\rat(11/9){2}{}&\rat(8/9){2}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(17/9){8}{}&\rat(2/9){2}{\spec{1}}&\rat(17/9){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(17/9){8}{}&\rat(2/9){2}{\spec{2}}&\rat(17/9){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\rat(10/9){1}{}&\rat(13/9){4}{}&\rat(13/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\rat(10/9){1}{}&\rat(16/9){7}{}&\rat(10/9){7}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\rat(1/9){1}{}&\rat(10/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\rat(5/3){6}{}&\rat(7/3){3}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 129
\orbit{3}{129}{128}
\h{129}&\rat(32/9){7}{\spec{1}}&\rat(56/9){4}{\spec{1}}&\rat(20/9){4}{}&&\cnt{747}&\bounds{128}{128}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(16/9){8}{}&\rat(25/9){5}{}&\rat(-5/9){8}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(16/9){8}{}&\rat(16/9){5}{\spec{1}}&\rat(4/9){8}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(16/9){8}{}&\rat(16/9){5}{\spec{2}}&\rat(4/9){8}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(16/9){8}{}&\rat(19/9){2}{}&\rat(1/9){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(16/9){8}{}&\rat(10/9){2}{\spec{1}}&\rat(10/9){2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(16/9){8}{}&\rat(10/9){2}{\spec{2}}&\rat(10/9){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(16/9){8}{}&\rat(13/9){8}{}&\rat(7/9){5}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(16/9){8}{}&\rat(4/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(2/9){1}{}&\rat(29/9){4}{}&\rat(5/9){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 130
\orbit{3}{130}{127}
\h{130}&\rat(8/9){8}{}&\rat(68/9){2}{\spec{3}}&\rat(32/9){2}{\spec{2}}&&\cnt{903}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/9){7}{}&\rat(13/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(2/9){2}{}&\rat(20/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\rat(-2/9){7}{}&\rat(22/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(20/9){8}{}&\rat(8/9){5}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\rat(1/9){1}{}&\rat(19/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(-8/9){1}{}&\rat(28/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 131
\orbit{3}{131}{127}
\h{131}&\rat(62/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(38/9){5}{\spec{2}}&&\cnt{691}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(32/9){5}{}&\rat(8/9){8}{}&\rat(-4/9){8}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(32/9){5}{}&\rat(-1/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(31/9){4}{}&\rat(1/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(31/9){4}{}&\rat(-8/9){1}{}&\rat(13/9){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(23/9){5}{}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(22/9){4}{\spec{1}}&\rat(1/9){1}{}&\rat(13/9){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(22/9){4}{\spec{2}}&\rat(1/9){1}{}&\rat(13/9){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(10/3){3}{}&\rat(2/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(10/3){3}{}&\int(0){\0}{}&\rat(2/3){6}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{\spec{1}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(7/3){3}{}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{2}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(20/9){2}{}&\rat(-1/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{19}&\rat(16/9){7}{}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 132
\orbit{3}{132}{127}
\h{132}&\rat(44/9){8}{\spec{1}}&\rat(26/9){8}{\spec{2}}&\rat(38/9){5}{\spec{1}}&&\cnt{747}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(4/3){3}{}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(16/9){7}{}&\rat(16/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{\spec{1}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(16/9){7}{}&\rat(10/9){1}{}&\rat(10/9){7}{\spec{2}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(16/9){7}{}&\rat(1/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(11/9){2}{}&\rat(11/9){2}{}&\rat(14/9){8}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(7/9){7}{}&\rat(10/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(17/9){8}{}&\rat(14/9){5}{}&\rat(5/9){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(17/9){8}{}&\rat(5/9){5}{\spec{1}}&\rat(14/9){8}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(17/9){8}{}&\rat(5/9){5}{\spec{2}}&\rat(14/9){8}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(17/9){8}{}&\rat(11/9){2}{}&\rat(8/9){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{19}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(10/9){1}{}&\rat(16/9){7}{}&\rat(10/9){7}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\rat(10/9){1}{}&\rat(16/9){7}{}&\rat(10/9){7}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\rat(10/9){1}{}&\rat(7/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\rat(10/9){1}{}&\rat(10/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{25}&\rat(1/9){1}{}&\rat(16/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\rat(4/3){3}{}&\rat(8/3){6}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 133
\orbit{3}{133}{127}
\h{133}&\rat(62/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(38/9){5}{\spec{1}}&&\cnt{803}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(23/9){5}{\spec{2}}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(23/9){5}{\spec{2}}&\rat(-1/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(14/9){5}{\spec{2}}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(14/9){5}{\spec{3}}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(8/3){6}{\spec{2}}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(7/3){3}{\spec{2}}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(4/3){3}{\spec{2}}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(4/3){3}{\spec{3}}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(25/9){7}{}&\rat(7/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(25/9){7}{}&\rat(1/9){1}{}&\rat(10/9){7}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(25/9){7}{}&\rat(1/9){1}{}&\rat(10/9){7}{\spec{2}}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(25/9){7}{}&\rat(-8/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(20/9){2}{\spec{2}}&\rat(2/9){2}{}&\rat(14/9){8}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(20/9){2}{\spec{2}}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(16/9){7}{\spec{2}}&\rat(1/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{23}&\rat(17/9){8}{}&\rat(5/9){5}{}&\rat(14/9){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{24}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{26}&\rat(10/9){1}{}&\rat(7/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{27}&\rat(8/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 134
\orbit{3}{134}{126}
\h{134}&\rat(26/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(74/9){5}{\spec{2}}&&\cnt{803}&\bounds{126}{126}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{3}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{\spec{2}}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(4/3){3}{}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(1/3){3}{\spec{1}}&\int(0){\0}{}&\rat(11/3){6}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(1/3){3}{\spec{2}}&\int(0){\0}{}&\rat(11/3){6}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(16/9){7}{}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(16/9){7}{}&\rat(1/9){1}{}&\rat(19/9){7}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(16/9){7}{}&\rat(-8/9){1}{}&\rat(28/9){7}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(7/9){7}{}&\rat(1/9){1}{}&\rat(28/9){7}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(10/9){1}{}&\rat(7/9){7}{}&\rat(19/9){7}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(10/9){1}{}&\rat(-2/9){7}{}&\rat(28/9){7}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{\spec{2}}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{3}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(8/9){8}{}&\rat(-1/9){8}{}&\rat(29/9){5}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{21}&\rat(1/9){1}{}&\rat(7/9){7}{}&\rat(28/9){7}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(-1/9){8}{}&\rat(8/9){8}{}&\rat(29/9){5}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\rat(1/3){3}{}&\rat(11/3){6}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 135
\orbit{3}{135}{123}
\h{135}&\rat(8/9){8}{}&\rat(50/9){2}{\spec{2}}&\rat(50/9){2}{\spec{1}}&&\cnt{747}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/9){7}{}&\rat(13/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(2/9){2}{}&\rat(11/9){8}{}&\rat(23/9){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(-2/9){7}{}&\rat(22/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(17/9){5}{\spec{1}}&\rat(11/9){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{}&\rat(17/9){5}{\spec{2}}&\rat(11/9){8}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(8/9){8}{}&\rat(5/9){2}{}&\rat(23/9){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(8/9){8}{}&\rat(11/9){8}{}&\rat(17/9){5}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(1/9){1}{}&\rat(19/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(1/9){1}{}&\rat(22/9){7}{}&\rat(13/9){7}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(-1/9){8}{}&\rat(26/9){5}{}&\rat(11/9){8}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(-1/9){8}{}&\rat(14/9){2}{}&\rat(23/9){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(-8/9){1}{}&\rat(28/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(7/3){3}{}&\rat(5/3){6}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\rat(5/3){6}{\spec{1}}&\rat(7/3){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\rat(5/3){6}{\spec{2}}&\rat(7/3){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 136
\orbit{3}{136}{123}
\h{136}&\int(12){\12}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{939}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){4}{}&\int(0){1}{}&\int(0){1}{}&\ln{1}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\l{3}&\int(4){6}{}&\int(0){3}{}&\int(0){\0}{}&\ln{2}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 137
\orbit{3}{137}{123}
\h{137}&\rat(62/9){8}{\spec{1}}&\rat(32/9){2}{\spec{2}}&\rat(14/9){2}{}&&\cnt{851}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(22/9){4}{\spec{1}}&\rat(16/9){1}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(13/9){4}{\spec{1}}&\rat(16/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(8/3){6}{\spec{1}}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(8/3){6}{\spec{1}}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(20/9){2}{\spec{1}}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{280}&\bounds{35}{35}{1}{false}&&\cr
\l{9}&\rat(20/9){2}{\spec{1}}&\rat(2/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(16/9){7}{\spec{1}}&\rat(16/9){1}{}&\rat(4/9){7}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\rat(19/9){1}{}&\rat(10/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(19/9){1}{}&\rat(16/9){1}{}&\rat(1/9){4}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{13}&\rat(8/9){8}{\spec{1}}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 138
\orbit{3}{138}{123}
\h{138}&\int(10){6}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&&\cnt{851}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(13/3){4}{}&\rat(-1/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(11/3){5}{}&\rat(1/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(10/3){4}{\spec{2}}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(4){3}{\spec{2}}&\int(0){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(4){3}{\spec{2}}&\int(0){\0}{}&\int(0){6}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(3){3}{\spec{2}}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\int(2){6}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){6}{\spec{3}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(8/3){2}{\spec{2}}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 139
\orbit{3}{139}{122}
\h{139}&\rat(44/9){8}{\spec{2}}&\rat(32/9){2}{\spec{1}}&\rat(32/9){2}{\spec{2}}&&\cnt{691}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{}&\rat(11/9){8}{}&\rat(2/9){8}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(22/9){4}{}&\rat(-2/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(13/9){4}{\spec{1}}&\rat(7/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(13/9){4}{\spec{2}}&\rat(7/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(8/3){6}{}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(7/3){3}{}&\rat(5/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(20/9){2}{}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(20/9){2}{}&\rat(2/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(16/9){7}{}&\rat(4/9){7}{\spec{1}}&\rat(16/9){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(16/9){7}{}&\rat(4/9){7}{\spec{2}}&\rat(16/9){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(7/9){7}{}&\rat(13/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(10/9){1}{}&\rat(10/9){4}{\spec{1}}&\rat(16/9){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(10/9){1}{}&\rat(10/9){4}{\spec{2}}&\rat(16/9){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{21}&\rat(1/9){1}{}&\rat(19/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 140
\orbit{3}{140}{122}
\h{140}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{907}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){5}{\spec{2}}&\int(0){8}{}&\int(0){8}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\int(4){4}{\spec{2}}&\int(0){1}{}&\int(0){1}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(3){5}{\spec{2}}&\int(1){8}{}&\int(0){8}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){5}{\spec{3}}&\int(1){8}{}&\int(0){8}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){4}{\spec{3}}&\int(1){1}{}&\int(0){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(4){6}{}&\int(0){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(4){6}{}&\int(0){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\int(4){6}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(3){6}{\spec{2}}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(3){3}{\spec{2}}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(3){7}{}&\int(1){7}{}&\int(0){1}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{19}&\int(3){7}{}&\int(1){1}{}&\int(0){7}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 141
\orbit{3}{141}{121}
\h{141}&\int(10){6}{\spec{4}}&\int(2){3}{}&\int(0){\0}{}&&\cnt{871}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(2){6}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){6}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(10/3){7}{}&\rat(2/3){7}{}&\int(0){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(10/3){7}{}&\rat(2/3){1}{}&\int(0){7}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(8/3){8}{}&\rat(4/3){5}{}&\int(0){8}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(8/3){8}{}&\rat(4/3){2}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 142
\orbit{3}{142}{120}
\h{142}&\int(6){\6}{\spec{1}}&\int(6){\6}{}&\int(0){\0}{}&&\cnt{795}&\bounds{120}{120}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(1){6}{}&\int(3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(1){3}{}&\int(3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){7}{}&\int(2){7}{}&\int(0){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(2){2}{}&\int(0){8}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(2){8}{}&\int(2){5}{\spec{1}}&\int(0){8}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\int(2){8}{}&\int(2){5}{\spec{2}}&\int(0){8}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(2){8}{}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(1){1}{}&\int(3){4}{}&\int(0){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 143
\orbit{3}{143}{120}
\h{143}&\rat(32/9){7}{\spec{2}}&\rat(56/9){4}{\spec{2}}&\rat(20/9){4}{}&&\cnt{691}&\bounds{120}{120}{1}{false}&&\cr
\l{1}&\rat(17/9){4}{}&\rat(14/9){1}{}&\rat(5/9){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\rat(7/3){6}{}&\int(0){\0}{\spec{1}}&\rat(5/3){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(13/9){2}{}&\rat(28/9){2}{}&\rat(-5/9){8}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(4/9){2}{\spec{1}}&\rat(28/9){2}{}&\rat(4/9){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(4/9){2}{\spec{2}}&\rat(28/9){2}{}&\rat(4/9){8}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(11/9){1}{}&\rat(20/9){4}{\spec{1}}&\rat(5/9){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(11/9){1}{}&\rat(14/9){1}{}&\rat(11/9){4}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(7/9){8}{}&\rat(28/9){2}{}&\rat(1/9){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(-2/9){8}{}&\rat(28/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 144
\orbit{3}{144}{120}
\h{144}&\rat(44/9){8}{\spec{1}}&\rat(50/9){2}{\spec{2}}&\rat(14/9){2}{}&&\cnt{747}&\bounds{120}{120}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(4/3){3}{}&\rat(8/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(16/9){7}{}&\rat(22/9){7}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(17/9){8}{}&\rat(26/9){5}{}&\rat(-7/9){8}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(17/9){8}{}&\rat(17/9){5}{\spec{1}}&\rat(2/9){8}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(17/9){8}{}&\rat(17/9){5}{\spec{2}}&\rat(2/9){8}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(17/9){8}{}&\rat(14/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(17/9){8}{}&\rat(5/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(17/9){8}{}&\rat(11/9){8}{}&\rat(8/9){5}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{17}&\rat(10/9){1}{}&\rat(28/9){4}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(10/9){1}{}&\rat(22/9){7}{}&\rat(4/9){7}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 145
\orbit{3}{145}{119}
\h{145}&\rat(14/9){7}{}&\rat(56/9){4}{\spec{2}}&\rat(38/9){4}{\spec{1}}&&\cnt{691}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\rat(10/9){5}{}&\rat(13/9){8}{}&\rat(13/9){8}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(2/3){3}{}&\rat(10/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(14/9){7}{}&\rat(26/9){7}{}&\rat(-4/9){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(14/9){7}{}&\rat(5/9){1}{}&\rat(17/9){7}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(5/9){7}{}&\rat(26/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(7/9){8}{}&\rat(25/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(7/9){8}{}&\rat(16/9){5}{\spec{2}}&\rat(13/9){8}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(7/9){8}{}&\rat(13/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/9){8}{}&\rat(4/9){8}{\spec{2}}&\rat(25/9){5}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(2/9){1}{}&\rat(26/9){7}{}&\rat(8/9){7}{\spec{1}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(2/9){1}{}&\rat(26/9){7}{}&\rat(8/9){7}{\spec{2}}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(2/9){1}{}&\rat(17/9){7}{}&\rat(17/9){7}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(-2/9){8}{}&\rat(25/9){5}{}&\rat(13/9){8}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(-2/9){8}{}&\rat(13/9){8}{}&\rat(25/9){5}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(-7/9){1}{}&\rat(26/9){7}{}&\rat(17/9){7}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(10/3){6}{}&\rat(2/3){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(5/3){3}{}&\rat(7/3){6}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 146
\orbit{3}{146}{118}
\h{146}&\int(6){6}{\spec{1}}&\int(4){3}{\spec{2}}&\int(2){\2}{}&&\cnt{747}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(8/3){5}{}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(7/3){4}{}&\rat(5/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(7/3){4}{}&\rat(2/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(4/3){4}{\spec{1}}&\rat(5/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(4/3){4}{\spec{2}}&\rat(5/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(3){6}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(7/3){7}{}&\rat(2/3){7}{}&\int(1){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(7/3){7}{}&\rat(5/3){1}{}&\int(0){7}{\spec{1}}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(7/3){7}{}&\rat(5/3){1}{}&\int(0){7}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(7/3){7}{}&\rat(2/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\rat(5/3){2}{}&\rat(7/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{23}&\rat(5/3){2}{}&\rat(4/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{24}&\rat(4/3){7}{\spec{1}}&\rat(5/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\rat(4/3){7}{\spec{2}}&\rat(5/3){1}{}&\int(1){7}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{26}&\rat(2/3){2}{\spec{1}}&\rat(7/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\rat(2/3){2}{\spec{2}}&\rat(7/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{28}&\rat(5/3){8}{}&\rat(4/3){5}{}&\int(1){8}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{29}&\rat(5/3){8}{}&\rat(7/3){2}{}&\int(0){2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{30}&\rat(5/3){8}{}&\rat(7/3){2}{}&\int(0){2}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{31}&\rat(5/3){8}{}&\rat(4/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{32}&\rat(4/3){1}{}&\rat(5/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{33}&\rat(4/3){1}{}&\rat(5/3){1}{}&\int(1){4}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{34}&\rat(2/3){8}{}&\rat(7/3){2}{}&\int(1){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{35}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 147
\orbit{3}{147}{116}
\h{147}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(92/9){5}{\spec{1}}&&\cnt{759}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(2/3){6}{}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(7/9){7}{}&\rat(7/9){7}{}&\rat(22/9){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(2/9){2}{}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{}&\rat(-1/9){8}{}&\rat(29/9){5}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(1/9){1}{}&\rat(1/9){1}{}&\rat(34/9){4}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 148
\orbit{3}{148}{116}
\h{148}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(92/9){5}{\spec{4}}&&\cnt{815}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\rat(5/9){5}{}&\rat(8/9){8}{}&\rat(23/9){8}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(1/3){3}{}&\int(0){\0}{}&\rat(11/3){6}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(7/9){7}{}&\rat(1/9){1}{}&\rat(28/9){7}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{}&\rat(-1/9){8}{}&\rat(29/9){5}{}&\ln{2}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 149
\orbit{3}{149}{116}
\h{149}&\rat(26/9){8}{\spec{2}}&\rat(68/9){2}{\spec{2}}&\rat(14/9){2}{}&&\cnt{691}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(4/3){3}{}&\rat(8/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(1/3){3}{\spec{1}}&\rat(11/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(1/3){3}{\spec{2}}&\rat(11/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(16/9){7}{}&\rat(22/9){7}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(16/9){7}{}&\rat(13/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(10/9){1}{}&\rat(28/9){4}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(10/9){1}{}&\rat(19/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(10/9){1}{}&\rat(22/9){7}{}&\rat(4/9){7}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(8/9){8}{}&\rat(35/9){5}{}&\rat(-7/9){8}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(-1/9){8}{}&\rat(35/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(11/3){6}{}&\rat(1/3){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 150
\orbit{3}{150}{115}
\h{150}&\rat(80/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(20/9){5}{}&&\cnt{679}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(40/9){4}{}&\rat(1/9){1}{}&\rat(-5/9){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(40/9){4}{}&\rat(-8/9){1}{}&\rat(4/9){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(32/9){5}{}&\rat(8/9){8}{}&\rat(-4/9){8}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(32/9){5}{}&\rat(-1/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(10/3){3}{}&\rat(2/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(10/3){3}{}&\int(0){\0}{}&\rat(2/3){6}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{\spec{1}}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(20/9){2}{\spec{1}}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(8/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 151
\orbit{3}{151}{115}
\h{151}&\int(6){6}{\spec{2}}&\int(4){6}{\spec{1}}&\int(2){6}{}&&\cnt{691}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{}&\rat(1/3){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(8/3){5}{}&\rat(5/3){8}{}&\rat(-1/3){8}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(8/3){5}{}&\rat(2/3){8}{}&\rat(2/3){8}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(5/3){5}{}&\rat(5/3){8}{}&\rat(2/3){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(3){3}{}&\int(0){\0}{}&\int(1){6}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){3}{\spec{1}}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\int(2){3}{\spec{1}}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){3}{\spec{2}}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){3}{\spec{2}}&\int(0){\0}{}&\int(2){6}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(8/3){2}{}&\rat(2/3){2}{}&\rat(2/3){8}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(8/3){2}{}&\rat(5/3){8}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(8/3){2}{}&\rat(2/3){8}{}&\rat(2/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(5/3){2}{}&\rat(5/3){8}{}&\rat(2/3){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(4/3){7}{}&\rat(7/3){7}{}&\rat(1/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(4/3){1}{}&\rat(7/3){7}{}&\rat(1/3){7}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(4/3){1}{}&\rat(4/3){7}{}&\rat(4/3){7}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(2/3){8}{}&\rat(5/3){8}{}&\rat(5/3){5}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\rat(1/3){1}{}&\rat(7/3){7}{}&\rat(4/3){7}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 152
\orbit{3}{152}{115}
\h{152}&\int(8){\8}{}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{679}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){5}{}&\int(0){8}{}&\int(0){8}{}&\ln{2}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(3){5}{}&\int(1){8}{}&\int(0){8}{}&\ln{2}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){6}{}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){6}{}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){7}{}&\int(2){7}{}&\int(0){1}{}&\ln{2}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 153
\orbit{3}{153}{114}
\h{153}&\int(8){6}{\spec{3}}&\int(4){3}{\spec{1}}&\int(0){\0}{}&&\cnt{791}&\bounds{114}{114}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(8/3){5}{}&\rat(4/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(2){6}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(10/3){7}{}&\rat(2/3){7}{\spec{1}}&\int(0){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(10/3){7}{}&\rat(2/3){7}{\spec{2}}&\int(0){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(10/3){7}{}&\rat(2/3){1}{}&\int(0){7}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(5/3){8}{}&\rat(7/3){5}{}&\int(0){8}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(4/3){1}{}&\rat(8/3){4}{}&\int(0){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 154
\orbit{3}{154}{113}
\h{154}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(92/9){5}{\spec{2}}&&\cnt{843}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{\spec{2}}&\ln{2}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(-1/3){6}{}&\int(0){\0}{}&\rat(13/3){3}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(2/9){2}{}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/9){8}{}&\rat(-1/9){8}{}&\rat(29/9){5}{}&\ln{2}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(1/9){1}{}&\rat(1/9){1}{}&\rat(34/9){4}{}&\ln{1}&\cnt{320}&\bounds{40}{40}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 155
\orbit{3}{155}{113}
\h{155}&\int(6){6}{\spec{1}}&\int(6){3}{\spec{2}}&\int(0){\0}{}&&\cnt{739}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(8/3){5}{}&\rat(4/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(2){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\int(2){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(1){3}{\spec{1}}&\int(3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(1){3}{\spec{2}}&\int(3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(7/3){7}{}&\rat(5/3){7}{}&\int(0){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(4/3){7}{\spec{1}}&\rat(8/3){7}{}&\int(0){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(4/3){7}{\spec{2}}&\rat(8/3){7}{}&\int(0){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\rat(5/3){8}{}&\rat(7/3){5}{}&\int(0){8}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\rat(8/3){4}{}&\int(0){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{18}&\rat(4/3){1}{}&\rat(8/3){7}{}&\int(0){7}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(2/3){8}{}&\rat(10/3){5}{}&\int(0){8}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 156
\orbit{3}{156}{113}
\h{156}&\rat(62/9){8}{\spec{1}}&\rat(32/9){2}{\spec{2}}&\rat(14/9){2}{}&&\cnt{795}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(22/9){4}{\spec{2}}&\rat(16/9){1}{}&\rat(-2/9){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(13/9){4}{\spec{2}}&\rat(16/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(13/9){4}{\spec{3}}&\rat(16/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(8/3){6}{\spec{2}}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{\spec{2}}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(25/9){7}{}&\rat(4/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(25/9){7}{}&\rat(16/9){1}{}&\rat(-5/9){7}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(20/9){2}{\spec{2}}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{14}&\rat(20/9){2}{\spec{2}}&\rat(2/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(16/9){7}{\spec{2}}&\rat(16/9){1}{}&\rat(4/9){7}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\rat(17/9){8}{}&\rat(14/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{17}&\rat(10/9){1}{}&\rat(16/9){1}{}&\rat(10/9){4}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(8/9){8}{\spec{2}}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 157
\orbit{3}{157}{113}
\h{157}&\rat(44/9){8}{\spec{1}}&\rat(32/9){2}{\spec{1}}&\rat(32/9){2}{\spec{2}}&&\cnt{735}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\rat(13/9){4}{}&\rat(7/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(16/9){7}{}&\rat(4/9){7}{\spec{1}}&\rat(16/9){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(16/9){7}{}&\rat(4/9){7}{\spec{2}}&\rat(16/9){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(7/9){7}{}&\rat(13/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(17/9){8}{}&\rat(17/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(17/9){8}{}&\rat(5/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(17/9){8}{}&\rat(11/9){8}{}&\rat(8/9){5}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{14}&\rat(10/9){1}{}&\rat(10/9){4}{\spec{1}}&\rat(16/9){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(10/9){1}{}&\rat(10/9){4}{\spec{2}}&\rat(16/9){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(1/9){1}{}&\rat(19/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 158
\orbit{3}{158}{113}
\h{158}&\rat(26/9){8}{\spec{2}}&\rat(50/9){2}{\spec{1}}&\rat(32/9){2}{\spec{2}}&&\cnt{739}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\rat(13/9){4}{}&\rat(7/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(4/9){4}{\spec{1}}&\rat(16/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(4/9){4}{\spec{2}}&\rat(16/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/3){6}{}&\rat(7/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(16/9){7}{}&\rat(4/9){7}{\spec{1}}&\rat(16/9){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(16/9){7}{}&\rat(4/9){7}{\spec{2}}&\rat(16/9){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(16/9){7}{}&\rat(16/9){1}{}&\rat(4/9){7}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(11/9){2}{}&\rat(23/9){2}{}&\rat(2/9){8}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(11/9){2}{}&\rat(11/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(7/9){7}{}&\rat(13/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(10/9){1}{}&\rat(10/9){4}{\spec{1}}&\rat(16/9){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(10/9){1}{}&\rat(10/9){4}{\spec{2}}&\rat(16/9){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(10/9){1}{}&\rat(16/9){1}{}&\rat(10/9){4}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(1/9){1}{}&\rat(19/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{21}&\rat(-1/9){8}{}&\rat(23/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 159
\orbit{3}{159}{112}
\h{159}&\rat(8/9){8}{}&\rat(68/9){2}{\spec{1}}&\rat(32/9){2}{\spec{2}}&&\cnt{791}&\bounds{112}{112}{1}{false}&&\cr
\l{1}&\rat(4/9){4}{}&\rat(16/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(2/3){6}{}&\rat(10/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(7/9){7}{}&\rat(13/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(-2/9){7}{}&\rat(22/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(14/9){2}{\spec{1}}&\rat(14/9){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{}&\rat(14/9){2}{\spec{2}}&\rat(14/9){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(1/9){1}{}&\rat(19/9){4}{\spec{1}}&\rat(16/9){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(1/9){1}{}&\rat(19/9){4}{\spec{2}}&\rat(16/9){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(-1/9){8}{}&\rat(23/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(-8/9){1}{}&\rat(28/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(10/3){3}{}&\rat(2/3){6}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 160
\orbit{3}{160}{111}
\h{160}&\int(8){6}{\spec{2}}&\int(2){3}{}&\int(2){\2}{}&&\cnt{683}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{\spec{1}}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\rat(10/3){4}{\spec{1}}&\rat(-1/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(8/3){5}{\spec{1}}&\rat(1/3){8}{}&\int(1){8}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(4){3}{}&\int(0){6}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(4){3}{}&\int(0){\0}{}&\int(0){6}{\spec{1}}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(4){3}{}&\int(0){\0}{}&\int(0){6}{\spec{2}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){6}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(8/3){2}{\spec{1}}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\rat(8/3){2}{\spec{1}}&\rat(1/3){2}{}&\int(1){8}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(8/3){2}{\spec{1}}&\rat(1/3){8}{}&\int(1){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(4/3){1}{\spec{1}}&\rat(5/3){4}{}&\int(1){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 161
\orbit{3}{161}{110}
\h{161}&\rat(32/9){7}{\spec{1}}&\rat(56/9){4}{\spec{2}}&\rat(20/9){4}{}&&\cnt{679}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(2/3){3}{}&\rat(10/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(14/9){7}{}&\rat(26/9){7}{}&\rat(-4/9){1}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(16/9){8}{}&\rat(25/9){5}{}&\rat(-5/9){8}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(16/9){8}{}&\rat(16/9){5}{\spec{2}}&\rat(4/9){8}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(16/9){8}{}&\rat(10/9){2}{\spec{2}}&\rat(10/9){2}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(16/9){8}{}&\rat(13/9){8}{}&\rat(7/9){5}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(16/9){8}{}&\rat(4/9){8}{\spec{2}}&\rat(16/9){5}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(2/9){1}{}&\rat(26/9){7}{}&\rat(8/9){7}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\rat(10/3){6}{}&\rat(2/3){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 162
\orbit{3}{162}{110}
\h{162}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{659}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(2){5}{}&\int(1){8}{}&\int(1){8}{}&\ln{2}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{4}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){7}{}&\int(1){7}{}&\int(1){1}{}&\ln{4}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(2){8}{}&\int(1){5}{}&\int(1){8}{}&\ln{4}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(2){8}{}&\int(1){2}{}&\int(1){2}{}&\ln{2}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 163
\orbit{3}{163}{110}
\h{163}&\int(10){6}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&&\cnt{703}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(11/3){5}{}&\rat(1/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(10/3){4}{}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\int(2){6}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){6}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(8/3){2}{}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(7/3){1}{}&\rat(5/3){4}{}&\int(0){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 164
\orbit{3}{164}{110}
\h{164}&\int(8){6}{\spec{2}}&\int(4){3}{\spec{2}}&\int(0){\0}{}&&\cnt{791}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(11/3){5}{}&\rat(1/3){8}{}&\int(0){8}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(10/3){4}{\spec{2}}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(7/3){4}{\spec{1}}&\rat(5/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(7/3){4}{\spec{2}}&\rat(5/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(3){3}{}&\int(1){6}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){6}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){6}{\spec{3}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(8/3){2}{\spec{2}}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{17}&\rat(7/3){7}{}&\rat(5/3){1}{}&\int(0){7}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(5/3){2}{}&\rat(7/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(5/3){8}{}&\rat(7/3){2}{}&\int(0){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 165
\orbit{3}{165}{108}
\h{165}&\rat(32/9){7}{\spec{1}}&\rat(38/9){4}{\spec{1}}&\rat(38/9){4}{\spec{2}}&&\cnt{683}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(4/3){6}{}&\int(0){\0}{}&\rat(8/3){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(14/9){7}{}&\rat(17/9){7}{}&\rat(5/9){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(14/9){7}{}&\rat(8/9){7}{\spec{1}}&\rat(14/9){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(14/9){7}{}&\rat(8/9){7}{\spec{2}}&\rat(14/9){1}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(4/9){2}{}&\rat(13/9){8}{}&\rat(19/9){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(16/9){8}{}&\rat(25/9){5}{}&\rat(-5/9){8}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(16/9){8}{}&\rat(16/9){5}{}&\rat(4/9){8}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(16/9){8}{}&\rat(10/9){2}{}&\rat(10/9){2}{\spec{1}}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(16/9){8}{}&\rat(10/9){2}{}&\rat(10/9){2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(16/9){8}{}&\rat(1/9){2}{}&\rat(19/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(16/9){8}{}&\rat(13/9){8}{}&\rat(7/9){5}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(16/9){8}{}&\rat(4/9){8}{}&\rat(16/9){5}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(2/9){1}{}&\rat(20/9){4}{}&\rat(14/9){1}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(7/3){6}{}&\rat(5/3){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(4/3){6}{\spec{1}}&\rat(8/3){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(4/3){6}{\spec{2}}&\rat(8/3){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 166
\orbit{3}{166}{106}
\h{166}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{783}&\bounds{106}{106}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){7}{}&\int(2){7}{}&\int(0){1}{}&\ln{2}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\int(2){8}{}&\int(2){5}{}&\int(0){8}{}&\ln{2}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(2){8}{}&\int(2){2}{}&\int(0){2}{}&\ln{2}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 167
\orbit{3}{167}{105}
\h{167}&\rat(44/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(56/9){5}{\spec{2}}&&\cnt{679}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{}&\rat(-1/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(14/9){5}{\spec{1}}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(14/9){5}{\spec{2}}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(8/3){6}{}&\int(0){\0}{}&\rat(4/3){3}{\spec{2}}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(4/3){3}{\spec{1}}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(4/3){3}{\spec{2}}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(20/9){2}{}&\rat(2/9){2}{}&\rat(14/9){8}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(20/9){2}{}&\rat(8/9){8}{}&\rat(8/9){2}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(16/9){7}{}&\rat(-8/9){1}{}&\rat(28/9){7}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(7/9){7}{}&\rat(1/9){1}{}&\rat(28/9){7}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(10/9){1}{}&\rat(-2/9){7}{}&\rat(28/9){7}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(8/9){8}{}&\rat(8/9){8}{}&\rat(20/9){5}{\spec{2}}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(1/9){1}{}&\rat(7/9){7}{}&\rat(28/9){7}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 168
\orbit{3}{168}{105}
\h{168}&\rat(14/9){7}{}&\rat(56/9){4}{\spec{2}}&\rat(38/9){4}{\spec{1}}&&\cnt{683}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(4/3){6}{}&\rat(8/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(14/9){7}{}&\rat(14/9){1}{}&\rat(8/9){7}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(5/9){7}{}&\rat(14/9){1}{}&\rat(17/9){7}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(4/9){2}{}&\rat(28/9){2}{}&\rat(4/9){8}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(-5/9){2}{}&\rat(28/9){2}{}&\rat(13/9){8}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(7/9){8}{}&\rat(16/9){5}{\spec{1}}&\rat(13/9){8}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\rat(7/9){8}{}&\rat(28/9){2}{}&\rat(1/9){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(7/9){8}{}&\rat(4/9){8}{\spec{1}}&\rat(25/9){5}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(2/9){1}{}&\rat(14/9){1}{}&\rat(20/9){4}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(-2/9){8}{}&\rat(28/9){2}{}&\rat(10/9){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{\spec{1}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\rat(8/3){3}{}&\rat(4/3){6}{\spec{2}}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 169
\orbit{3}{169}{105}
\h{169}&\int(4){6}{\spec{1}}&\int(4){6}{\spec{1}}&\int(4){6}{\spec{1}}&&\cnt{675}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(5/3){5}{}&\rat(5/3){8}{}&\rat(2/3){8}{}&\ln{6}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(2/3){5}{}&\rat(5/3){8}{}&\rat(5/3){8}{}&\ln{3}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(7/3){7}{}&\rat(7/3){7}{}&\rat(-2/3){1}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(7/3){7}{}&\rat(4/3){7}{}&\rat(1/3){1}{}&\ln{6}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 170
\orbit{3}{170}{103}
\h{170}&\rat(44/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(56/9){5}{\spec{2}}&&\cnt{723}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\rat(14/9){5}{}&\rat(8/9){8}{}&\rat(14/9){8}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(4/3){3}{}&\int(0){\0}{}&\rat(8/3){6}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\rat(16/9){7}{}&\rat(-8/9){1}{}&\rat(28/9){7}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(7/9){7}{}&\rat(1/9){1}{}&\rat(28/9){7}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(17/9){8}{}&\rat(5/9){5}{}&\rat(14/9){8}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{\spec{2}}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(10/9){1}{}&\rat(-2/9){7}{}&\rat(28/9){7}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(1/9){1}{}&\rat(7/9){7}{}&\rat(28/9){7}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 171
\orbit{3}{171}{102}
\h{171}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{771}&\bounds{102}{102}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(3){5}{}&\int(1){8}{}&\int(0){8}{}&\ln{2}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(3){7}{}&\int(1){7}{}&\int(0){1}{}&\ln{2}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\int(3){7}{}&\int(1){1}{}&\int(0){7}{}&\ln{2}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 172
\orbit{3}{172}{101}
\h{172}&\rat(44/9){8}{\spec{1}}&\rat(32/9){2}{\spec{2}}&\rat(32/9){2}{\spec{2}}&&\cnt{715}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\rat(4/9){4}{}&\rat(16/9){1}{}&\rat(16/9){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(16/9){7}{}&\rat(4/9){7}{}&\rat(16/9){1}{}&\ln{2}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\rat(10/9){1}{}&\rat(10/9){4}{}&\rat(16/9){1}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 173
\orbit{3}{173}{101}
\h{173}&\rat(8/9){8}{}&\rat(86/9){2}{\spec{4}}&\rat(14/9){2}{}&&\cnt{647}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(2/3){6}{}&\rat(10/3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(7/9){7}{}&\rat(22/9){7}{}&\rat(7/9){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(2/9){2}{}&\rat(20/9){8}{}&\rat(14/9){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(8/9){8}{}&\rat(23/9){2}{}&\rat(5/9){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(8/9){8}{}&\rat(14/9){2}{\spec{1}}&\rat(14/9){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(8/9){8}{}&\rat(14/9){2}{\spec{2}}&\rat(14/9){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(8/9){8}{}&\rat(20/9){8}{}&\rat(8/9){5}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\rat(1/9){1}{}&\rat(28/9){4}{}&\rat(7/9){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(-1/9){8}{}&\rat(23/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(10/3){3}{}&\rat(2/3){6}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 174
\orbit{3}{174}{101}
\h{174}&\rat(44/9){8}{\spec{1}}&\rat(8/9){8}{}&\rat(56/9){5}{\spec{2}}&&\cnt{731}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(5/3){6}{}&\int(0){\0}{}&\rat(7/3){3}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(2/3){6}{}&\int(0){\0}{}&\rat(10/3){3}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(16/9){7}{}&\rat(7/9){7}{}&\rat(13/9){1}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\rat(11/9){2}{}&\rat(8/9){8}{}&\rat(17/9){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(11/9){2}{}&\rat(-1/9){8}{}&\rat(26/9){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(2/9){2}{}&\rat(8/9){8}{}&\rat(26/9){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(17/9){8}{}&\rat(2/9){2}{}&\rat(17/9){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(17/9){8}{}&\rat(-7/9){2}{}&\rat(26/9){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{\spec{1}}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\rat(10/9){1}{}&\rat(1/9){1}{}&\rat(25/9){4}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(2/3){6}{}&\rat(10/3){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 175
\orbit{3}{175}{100}
\h{175}&\rat(80/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(20/9){5}{}&&\cnt{591}&\bounds{100}{100}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(23/9){5}{}&\rat(8/9){8}{}&\rat(5/9){8}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(8/3){6}{\spec{2}}&\int(0){\0}{}&\rat(4/3){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(7/3){3}{}&\int(0){\0}{}&\rat(5/3){6}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(25/9){7}{}&\rat(7/9){7}{}&\rat(4/9){1}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(25/9){7}{}&\rat(1/9){1}{}&\rat(10/9){7}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(20/9){2}{\spec{2}}&\rat(8/9){8}{}&\rat(8/9){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(19/9){1}{}&\rat(7/9){7}{}&\rat(10/9){7}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(19/9){1}{}&\rat(1/9){1}{}&\rat(16/9){4}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(17/9){8}{}&\rat(8/9){8}{}&\rat(11/9){5}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(17/9){8}{}&\rat(-1/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(8/9){8}{\spec{2}}&\rat(8/9){8}{}&\rat(20/9){5}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 176
\orbit{3}{176}{98}
\h{176}&\int(2){6}{}&\int(2){3}{}&\int(8){\8}{\spec{1}}&&\cnt{535}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\rat(5/3){5}{}&\rat(1/3){8}{}&\int(2){8}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(4/3){4}{}&\rat(2/3){1}{}&\int(2){1}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){6}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(4/3){7}{}&\rat(2/3){7}{}&\int(2){1}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(4/3){7}{}&\rat(2/3){1}{}&\int(2){7}{}&\ln{2}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 177
\orbit{3}{177}{97}
\h{177}&\rat(80/9){8}{\spec{2}}&\rat(14/9){2}{}&\rat(14/9){2}{}&&\cnt{591}&\bounds{97}{97}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(22/9){4}{\spec{2}}&\rat(7/9){1}{}&\rat(7/9){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(8/3){6}{\spec{2}}&\rat(4/3){3}{}&\int(0){\0}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(25/9){7}{}&\rat(4/9){7}{}&\rat(7/9){1}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(20/9){2}{\spec{2}}&\rat(14/9){2}{}&\rat(2/9){8}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(19/9){1}{}&\rat(10/9){4}{}&\rat(7/9){1}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(17/9){8}{}&\rat(14/9){2}{}&\rat(5/9){2}{}&\ln{2}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(8/9){8}{\spec{2}}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 178
\orbit{3}{178}{96}
\h{178}&\int(8){6}{\spec{3}}&\int(4){3}{\spec{2}}&\int(0){\0}{}&&\cnt{779}&\bounds{96}{96}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(7/3){4}{}&\rat(5/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){6}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(10/3){7}{}&\rat(2/3){7}{}&\int(0){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(10/3){7}{}&\rat(2/3){1}{}&\int(0){7}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(5/3){2}{}&\rat(7/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(5/3){8}{}&\rat(7/3){2}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 179
\orbit{3}{179}{90}
\h{179}&\rat(8/9){8}{}&\rat(68/9){2}{\spec{2}}&\rat(32/9){2}{\spec{2}}&&\cnt{667}&\bounds{90}{90}{1}{false}&&\cr
\l{1}&\rat(1/3){3}{}&\rat(11/3){6}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(7/9){7}{}&\rat(13/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(-2/9){7}{}&\rat(22/9){7}{}&\rat(16/9){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(8/9){8}{}&\rat(26/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(8/9){8}{}&\rat(14/9){2}{}&\rat(14/9){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(1/9){1}{}&\rat(19/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(-1/9){8}{}&\rat(35/9){5}{}&\rat(2/9){8}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(-8/9){1}{}&\rat(28/9){4}{}&\rat(16/9){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\rat(8/3){6}{}&\rat(4/3){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 180
\orbit{3}{180}{89}
\h{180}&\int(8){6}{\spec{2}}&\int(4){3}{\spec{2}}&\int(0){\0}{}&&\cnt{659}&\bounds{89}{89}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(10/3){4}{\spec{1}}&\rat(2/3){1}{}&\int(0){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){3}{}&\int(0){6}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){3}{}&\int(0){\0}{}&\int(0){6}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){6}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(8/3){2}{\spec{1}}&\rat(4/3){2}{}&\int(0){8}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*A[8]
% Class 181
\orbit{3}{181}{72}
\h{181}&\int(12){\12}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{495}&\bounds{72}{72}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{216}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_3D8.tex <==
% -*- TeX -*-
% Niemeier lattice 3D8
% 70 classes
\newcs{max-3D8}{231}%
\newcs{count-3D8}{70}%
\newcs{counts-3D8}{\DO{1}{231}\DO{2}{222}\DO{3}{219}\DO{4}{219}\DO{5}{203}\DO{6}{203}\DO{7}{202}\DO{8}{199}\DO{9}{199}\DO{10}{195}\DO{11}{191}\DO{12}{183}\DO{13}{175}\DO{14}{171}\DO{15}{167}\DO{16}{167}\DO{17}{167}\DO{18}{162}\DO{19}{162}\DO{20}{157}\DO{21}{157}\DO{22}{155}\DO{23}{151}\DO{24}{149}\DO{25}{149}\DO{26}{147}\DO{27}{146}\DO{28}{143}\DO{29}{143}\DO{30}{143}\DO{31}{143}\DO{32}{143}\DO{33}{137}\DO{34}{137}\DO{35}{135}\DO{36}{135}\DO{37}{135}\DO{38}{131}\DO{39}{131}\DO{40}{131}\DO{41}{129}\DO{42}{127}\DO{43}{127}\DO{44}{125}\DO{45}{123}\DO{46}{123}\DO{47}{121}\DO{48}{119}\DO{49}{119}\DO{50}{119}\DO{51}{119}\DO{52}{119}\DO{53}{119}\DO{54}{115}\DO{55}{113}\DO{56}{108}\DO{57}{107}\DO{58}{105}\DO{59}{103}\DO{60}{103}\DO{61}{101}\DO{62}{101}\DO{63}{97}\DO{64}{96}\DO{65}{95}\DO{66}{87}\DO{67}{87}\DO{68}{87}\DO{69}{86}\DO{70}{78}}%
\orbits
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 1
\orbit{3}{1}{231}
\h{1}&\int(4){\4}{}&\int(4){\4}{}&\int(4){\4}{}&&\cnt{687}&\bounds{231}{231}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{3}&\cnt{64}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(1){2}{}&\int(1){2}{}&\ln{3}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 2
\orbit{3}{2}{222}
\h{2}&\int(12){\12}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1319}&\bounds{222}{222}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(4){3}{}&\int(0){3}{}&\int(0){\0}{}&\ln{2}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{8}&\int(4){1}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{512}&\bounds{64}{64}{1}{false}&&\cr
\l{9}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 3
\orbit{3}{3}{219}
\h{3}&\int(8){\8}{\spec{2}}&\int(4){\4}{2}&\int(0){\0}{}&&\cnt{1647}&\bounds{219}{219}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){1}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{512}&\bounds{64}{64}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{448}&\bounds{56}{56}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{392}&\bounds{56}{56}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 4
\orbit{3}{4}{219}
\h{4}&\int(9){2}{\spec{1}}&\int(1){2}{}&\int(2){1}{}&&\cnt{1563}&\bounds{219}{219}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{392}&\bounds{56}{56}{1}{false}&&\cr
\l{3}&\int(3){2}{}&\rat(1/2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{512}&\bounds{64}{64}{1}{false}&&\cr
\l{4}&\int(3){2}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\int(3){2}{}&\int(0){2}{}&\int(1){1}{}&\ln{1}&\cnt{392}&\bounds{56}{56}{1}{false}&&\cr
\l{6}&\int(3){2}{}&\int(-1){2}{}&\int(2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 5
\orbit{3}{5}{203}
\h{5}&\int(10){\10}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{1291}&\bounds{203}{203}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){2}{}&\int(1){1}{}&\int(0){2}{}&\ln{1}&\cnt{512}&\bounds{64}{64}{1}{false}&&\cr
\l{8}&\int(3){2}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 6
\orbit{3}{6}{203}
\h{6}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&&\cnt{1127}&\bounds{203}{203}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{64}{64}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(2){2}{}&\int(0){2}{}&\ln{2}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 7
\orbit{3}{7}{202}
\h{7}&\int(8){\8}{0}&\int(4){\4}{2}&\int(0){\0}{}&&\cnt{1363}&\bounds{202}{202}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{512}&\bounds{64}{64}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{336}&\bounds{48}{48}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 8
\orbit{3}{8}{199}
\h{8}&\int(4){\4}{2}&\int(4){\4}{2}&\int(4){\4}{}&&\cnt{1151}&\bounds{199}{199}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(1){1}{}&\int(2){2}{}&\int(1){2}{}&\ln{2}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{48}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\int(0){2}{}&\int(2){1}{}&\ln{2}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 9
\orbit{3}{9}{199}
\h{9}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{895}&\bounds{199}{199}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(3){1}{\spec{2}}&\int(1){2}{}&\int(0){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(1){1}{}&\int(1){2}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(0){\0}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 10
\orbit{3}{10}{195}
\h{10}&\int(1){2}{}&\int(1){2}{}&\int(10){1}{\spec{2}}&&\cnt{1115}&\bounds{195}{195}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(1/2){3}{}&\int(0){\0}{}&\rat(7/2){3}{}&\ln{2}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{3}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\int(0){2}{}&\int(3){1}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\int(-1){2}{}&\int(4){1}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){2}{}&\int(0){2}{}&\int(4){1}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 11
\orbit{3}{11}{191}
\h{11}&\int(6){\6}{\spec{1}}&\int(4){\4}{}&\int(2){\2}{}&&\cnt{783}&\bounds{191}{191}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\int(2){1}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(2){2}{}&\int(1){1}{}&\int(1){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{14}&\int(1){2}{}&\int(2){1}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 12
\orbit{3}{12}{183}
\h{12}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{879}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(3){1}{\spec{2}}&\int(1){2}{}&\int(0){2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(2){3}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(2){1}{}&\int(0){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 13
\orbit{3}{13}{175}
\h{13}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{1151}&\bounds{175}{175}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){3}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(4){3}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(3){1}{\spec{1}}&\int(1){2}{}&\int(0){2}{}&\ln{1}&\cnt{512}&\bounds{64}{64}{1}{false}&&\cr
\l{5}&\int(2){3}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{224}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{\spec{1}}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 14
\orbit{3}{14}{171}
\h{14}&\int(10){3}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&&\cnt{1115}&\bounds{171}{171}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){3}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(4){3}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\rat(7/2){1}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{512}&\bounds{64}{64}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(2){3}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){3}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 15
\orbit{3}{15}{167}
\h{15}&\int(4){\4}{2}&\int(4){\4}{}&\int(4){\4}{}&&\cnt{655}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){2}{}&\int(2){1}{}&\int(0){2}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){2}{}&\int(1){1}{}&\int(1){2}{}&\ln{2}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){3}{}&\int(2){3}{}&\ln{1}&\cnt{64}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 16
\orbit{3}{16}{167}
\h{16}&\int(3){2}{}&\int(1){2}{}&\int(8){1}{\spec{2}}&&\cnt{1055}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(3/2){1}{}&\int(0){2}{}&\rat(5/2){2}{}&\ln{1}&\cnt{224}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\rat(1/2){1}{}&\int(1){2}{}&\rat(5/2){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\rat(1/2){1}{}&\rat(5/2){2}{}&\ln{1}&\cnt{192}&\bounds{36}{36}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(1){2}{}&\int(0){2}{}&\int(3){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(0){2}{}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 17
\orbit{3}{17}{167}
\h{17}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{1007}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){3}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(4){3}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(4){1}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\int(3){1}{}&\int(1){2}{}&\int(0){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 18
\orbit{3}{18}{162}
\h{18}&\int(8){\8}{0}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{867}&\bounds{162}{162}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{64}{64}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){1}{}&\int(0){2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 19
\orbit{3}{19}{162}
\h{19}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{843}&\bounds{162}{162}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{64}{64}{1}{false}&&\cr
\l{9}&\int(3){1}{}&\int(1){2}{}&\int(0){2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 20
\orbit{3}{20}{157}
\h{20}&\int(3){2}{}&\int(1){2}{}&\int(8){1}{\spec{1}}&&\cnt{831}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){3}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\rat(3/2){1}{}&\int(1){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(1/2){3}{}&\int(0){\0}{}&\rat(7/2){3}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{\spec{2}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(1){2}{}&\int(0){2}{}&\int(3){1}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{9}&\int(0){2}{}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\rat(1/2){3}{}&\rat(7/2){3}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 21
\orbit{3}{21}{157}
\h{21}&\int(6){\6}{}&\int(4){\4}{2}&\int(2){\2}{}&&\cnt{903}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){1}{}&\int(2){2}{}&\int(-1){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){1}{}&\int(0){2}{}&\int(1){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(1){1}{}&\int(2){2}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\int(2){2}{}&\int(1){1}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 22
\orbit{3}{22}{155}
\h{22}&\int(5){2}{\spec{1}}&\int(1){2}{}&\int(6){1}{}&&\cnt{891}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){3}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\rat(3/2){1}{}&\int(1){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\rat(1/2){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){2}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{14}&\int(2){2}{}&\int(-1){2}{}&\int(3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\int(1){2}{}&\int(0){2}{}&\int(3){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){2}{}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 23
\orbit{3}{23}{151}
\h{23}&\int(8){3}{\spec{1}}&\int(4){3}{}&\int(0){\0}{}&&\cnt{1039}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(3){3}{}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{6}&\rat(5/2){1}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\rat(5/2){2}{}&\rat(3/2){1}{}&\int(0){2}{}&\ln{1}&\cnt{336}&\bounds{42}{42}{1}{false}&&\cr
\l{10}&\rat(5/2){2}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 24
\orbit{3}{24}{149}
\h{24}&\int(8){3}{\spec{1}}&\int(2){3}{}&\int(2){\2}{}&&\cnt{1063}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(5/2){1}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(5/2){2}{}&\rat(3/2){1}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(5/2){2}{}&\rat(1/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(5/2){2}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 25
\orbit{3}{25}{149}
\h{25}&\int(3){2}{}&\int(3){2}{}&\int(6){1}{}&&\cnt{735}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){3}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(3/2){1}{}&\int(1){2}{}&\rat(3/2){2}{}&\ln{2}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(0){2}{}&\int(3){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 26
\orbit{3}{26}{147}
\h{26}&\int(6){\6}{}&\int(6){\6}{}&\int(0){\0}{}&&\cnt{903}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){1}{}&\int(1){2}{}&\int(0){2}{}&\ln{2}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 27
\orbit{3}{27}{146}
\h{27}&\int(8){\8}{0}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{619}&\bounds{146}{146}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(1){1}{}&\int(1){2}{}&\ln{2}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 28
\orbit{3}{28}{143}
\h{28}&\int(6){\6}{\spec{1}}&\int(4){\4}{2}&\int(2){\2}{}&&\cnt{751}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(1){1}{}&\int(2){2}{}&\int(1){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(1){1}{}&\int(1){2}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(1){2}{}&\int(2){2}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 29
\orbit{3}{29}{143}
\h{29}&\int(7){2}{\spec{1}}&\int(3){2}{}&\int(2){1}{}&&\cnt{847}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(5/2){1}{}&\int(1){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\rat(3/2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(2){2}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 30
\orbit{3}{30}{143}
\h{30}&\int(8){1}{\spec{2}}&\int(2){1}{}&\int(2){1}{}&&\cnt{1067}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(3){1}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(5/2){2}{}&\int(2){1}{}&\rat(-1/2){2}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(5/2){2}{}&\int(1){1}{}&\rat(1/2){2}{}&\ln{2}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 31
\orbit{3}{31}{143}
\h{31}&\int(6){3}{}&\int(6){3}{}&\int(0){\0}{}&&\cnt{891}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){3}{}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(5/2){1}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{2}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 32
\orbit{3}{32}{143}
\h{32}&\int(8){\8}{\spec{1}}&\int(4){\4}{2}&\int(0){\0}{}&&\cnt{847}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(0){\0}{\spec{2}}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 33
\orbit{3}{33}{137}
\h{33}&\int(7){2}{\spec{1}}&\int(1){2}{}&\int(4){1}{}&&\cnt{831}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\rat(5/2){1}{}&\int(1){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(5/2){1}{}&\int(0){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){3}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(3/2){1}{}&\int(1){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(2){2}{}&\rat(1/2){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{\spec{1}}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{15}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(2){2}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{17}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 34
\orbit{3}{34}{137}
\h{34}&\int(9){2}{\spec{3}}&\int(1){2}{}&\int(2){1}{}&&\cnt{943}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(7/2){3}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(7/2){1}{}&\int(1){2}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(7/2){1}{}&\int(0){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(5/2){1}{}&\int(1){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(2){2}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 35
\orbit{3}{35}{135}
\h{35}&\int(5){2}{\spec{1}}&\int(3){2}{}&\int(4){1}{}&&\cnt{719}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){3}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(3/2){1}{}&\int(1){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\rat(3/2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\rat(1/2){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{\spec{1}}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{12}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){2}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(5/2){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 36
\orbit{3}{36}{135}
\h{36}&\int(2){3}{}&\int(2){3}{}&\int(8){\8}{\spec{1}}&&\cnt{903}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){3}{}&\int(0){\0}{}&\int(2){3}{\spec{2}}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(3/2){1}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(1){3}{}&\int(0){\0}{}&\int(3){3}{}&\ln{2}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(3){1}{\spec{2}}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 37
\orbit{3}{37}{135}
\h{37}&\int(1){2}{}&\int(1){2}{}&\int(10){1}{\spec{1}}&&\cnt{831}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(1/2){3}{}&\int(0){\0}{}&\rat(7/2){3}{}&\ln{2}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(1/2){1}{}&\int(1){2}{}&\rat(5/2){2}{}&\ln{2}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(0){2}{}&\int(3){1}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 38
\orbit{3}{38}{131}
\h{38}&\int(6){\6}{}&\int(4){\4}{}&\int(2){\2}{}&&\cnt{671}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){1}{}&\int(1){2}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){1}{}&\int(0){2}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\int(2){1}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 39
\orbit{3}{39}{131}
\h{39}&\int(8){\8}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{903}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){1}{}&\int(1){2}{}&\int(-1){2}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){1}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 40
\orbit{3}{40}{131}
\h{40}&\int(5){2}{\spec{1}}&\int(5){2}{\spec{1}}&\int(2){1}{}&&\cnt{891}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(3/2){1}{}&\int(2){2}{}&\rat(1/2){2}{}&\ln{2}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(0){2}{}&\int(2){1}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 41
\orbit{3}{41}{129}
\h{41}&\int(8){3}{\spec{2}}&\int(2){3}{}&\int(2){\2}{}&&\cnt{839}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(7/2){1}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(7/2){1}{}&\rat(-1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(5/2){1}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(2){3}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){3}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 42
\orbit{3}{42}{127}
\h{42}&\int(6){\6}{\spec{1}}&\int(6){\6}{}&\int(0){\0}{}&&\cnt{751}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\int(1){3}{}&\int(3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){1}{}&\int(0){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(1){2}{}&\int(3){1}{}&\int(0){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 43
\orbit{3}{43}{127}
\h{43}&\int(5){2}{\spec{2}}&\int(1){2}{}&\int(6){1}{}&&\cnt{719}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){3}{\spec{1}}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){3}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(5/2){1}{}&\int(1){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(5/2){1}{}&\int(0){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){3}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(3/2){1}{}&\int(1){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\int(1){2}{}&\int(0){2}{}&\int(3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(0){2}{}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 44
\orbit{3}{44}{125}
\h{44}&\int(6){3}{}&\int(4){3}{}&\int(2){\2}{}&&\cnt{727}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){3}{}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(5/2){1}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(5/2){1}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(3/2){1}{\spec{1}}&\rat(3/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(3/2){1}{\spec{2}}&\rat(3/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\rat(5/2){1}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{18}&\rat(1/2){2}{}&\rat(5/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 45
\orbit{3}{45}{123}
\h{45}&\int(8){3}{\spec{2}}&\int(4){3}{}&\int(0){\0}{}&&\cnt{815}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(7/2){1}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{5}&\int(3){3}{}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(5/2){1}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(2){3}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(2){3}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\rat(5/2){1}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 46
\orbit{3}{46}{123}
\h{46}&\int(12){\12}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{747}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{336}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 47
\orbit{3}{47}{121}
\h{47}&\int(12){\12}{2}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{795}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{336}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 48
\orbit{3}{48}{119}
\h{48}&\int(10){3}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&&\cnt{831}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(7/2){1}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(2){3}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){3}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(5/2){2}{}&\rat(3/2){1}{}&\int(0){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 49
\orbit{3}{49}{119}
\h{49}&\int(5){2}{\spec{1}}&\int(5){2}{\spec{2}}&\int(2){1}{}&&\cnt{719}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\rat(5/2){1}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\rat(3/2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\rat(5/2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(5/2){3}{}&\rat(3/2){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 50
\orbit{3}{50}{119}
\h{50}&\int(4){3}{}&\int(4){3}{}&\int(4){\4}{2}&&\cnt{779}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\rat(5/2){1}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{2}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){1}{}&\rat(-1/2){2}{}&\int(2){2}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\rat(3/2){1}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{2}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{7}&\rat(1/2){1}{\spec{1}}&\rat(3/2){2}{}&\int(2){2}{}&\ln{2}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\rat(1/2){1}{\spec{2}}&\rat(3/2){2}{}&\int(2){2}{}&\ln{2}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 51
\orbit{3}{51}{119}
\h{51}&\int(6){3}{}&\int(2){3}{}&\int(4){\4}{}&&\cnt{735}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(5/2){1}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){3}{}&\int(2){3}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 52
\orbit{3}{52}{119}
\h{52}&\int(5){2}{\spec{2}}&\int(3){2}{}&\int(4){1}{}&&\cnt{679}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(5/2){1}{}&\int(1){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(5/2){1}{}&\int(0){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(3/2){1}{}&\int(1){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(5/2){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 53
\orbit{3}{53}{119}
\h{53}&\int(7){2}{\spec{2}}&\int(1){2}{}&\int(4){1}{}&&\cnt{779}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(7/2){3}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){3}{\spec{1}}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){3}{\spec{2}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(7/2){1}{}&\int(1){2}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(7/2){1}{}&\int(0){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\rat(7/2){1}{}&\int(-1){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(5/2){1}{}&\int(1){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(5/2){1}{}&\int(0){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{12}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){3}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(3/2){1}{}&\int(1){2}{}&\rat(3/2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 54
\orbit{3}{54}{115}
\h{54}&\int(2){3}{}&\int(2){3}{}&\int(8){\8}{\spec{1}}&&\cnt{779}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){3}{}&\int(0){\0}{}&\int(2){3}{\spec{1}}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(0){3}{}&\int(0){\0}{}&\int(4){3}{}&\ln{2}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(3){1}{\spec{1}}&\ln{1}&\cnt{512}&\bounds{64}{64}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 55
\orbit{3}{55}{113}
\h{55}&\int(8){1}{\spec{1}}&\int(2){1}{}&\int(2){1}{}&&\cnt{843}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(7/2){3}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){1}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{320}&\bounds{40}{40}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\int(2){1}{}&\rat(1/2){2}{}&\ln{2}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 56
\orbit{3}{56}{108}
\h{56}&\int(4){3}{}&\int(2){3}{}&\int(6){\6}{\spec{1}}&&\cnt{783}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\rat(5/2){1}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){1}{}&\rat(-1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(3/2){1}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(1/2){2}{}&\rat(3/2){1}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){3}{}&\int(2){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 57
\orbit{3}{57}{107}
\h{57}&\int(5){2}{\spec{2}}&\int(5){2}{\spec{2}}&\int(2){1}{}&&\cnt{679}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(5/2){1}{}&\int(1){2}{}&\rat(1/2){2}{}&\ln{2}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 58
\orbit{3}{58}{105}
\h{58}&\int(4){1}{}&\int(4){1}{}&\int(4){1}{}&&\cnt{675}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{6}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){1}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\ln{6}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(1){1}{\spec{1}}&\rat(3/2){2}{}&\rat(3/2){2}{}&\ln{3}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(1){1}{\spec{2}}&\rat(3/2){2}{}&\rat(3/2){2}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 59
\orbit{3}{59}{103}
\h{59}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{639}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){3}{}&\int(0){3}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(3){1}{\spec{1}}&\int(1){2}{}&\int(0){2}{}&\ln{2}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(0){\0}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 60
\orbit{3}{60}{103}
\h{60}&\int(4){3}{}&\int(4){3}{}&\int(4){\4}{}&&\cnt{679}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\rat(5/2){1}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){1}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(3/2){1}{}&\rat(3/2){2}{}&\int(1){2}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 61
\orbit{3}{61}{101}
\h{61}&\int(6){1}{}&\int(4){1}{}&\int(2){1}{}&&\cnt{731}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){1}{}&\rat(3/2){2}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){1}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){1}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(3/2){3}{\spec{1}}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(3/2){3}{\spec{2}}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\int(2){1}{}&\rat(1/2){2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(1/2){2}{}&\rat(3/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(5/2){3}{}&\rat(3/2){3}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 62
\orbit{3}{62}{101}
\h{62}&\int(6){3}{}&\int(2){3}{}&\int(4){\4}{2}&&\cnt{703}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(5/2){1}{}&\rat(-1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(3/2){1}{\spec{1}}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(3/2){1}{\spec{2}}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(1/2){2}{}&\rat(3/2){1}{}&\int(2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 63
\orbit{3}{63}{97}
\h{63}&\int(4){3}{}&\int(2){3}{}&\int(6){\6}{}&&\cnt{671}&\bounds{97}{97}{1}{false}&&\cr
\l{1}&\rat(5/2){1}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(1){3}{\spec{1}}&\int(0){\0}{}&\int(3){3}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\int(1){3}{\spec{2}}&\int(0){\0}{}&\int(3){3}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\rat(-1/2){2}{}&\int(3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(3){1}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){3}{}&\int(2){3}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(1){3}{}&\int(3){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 64
\orbit{3}{64}{96}
\h{64}&\int(7){2}{\spec{2}}&\int(3){2}{}&\int(2){1}{}&&\cnt{663}&\bounds{96}{96}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(7/2){3}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){3}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(7/2){1}{}&\int(1){2}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(7/2){1}{}&\int(0){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\rat(5/2){1}{}&\int(1){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 65
\orbit{3}{65}{95}
\h{65}&\int(8){\8}{\spec{1}}&\int(4){\4}{2}&\int(0){\0}{}&&\cnt{591}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){3}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{392}&\bounds{56}{56}{1}{false}&&\cr
\l{4}&\int(0){\0}{\spec{1}}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 66
\orbit{3}{66}{87}
\h{66}&\int(4){\4}{2}&\int(4){\4}{2}&\int(4){\4}{2}&&\cnt{591}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 67
\orbit{3}{67}{87}
\h{67}&\int(8){\8}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{623}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){1}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 68
\orbit{3}{68}{87}
\h{68}&\int(2){3}{}&\int(2){3}{}&\int(8){\8}{\spec{2}}&&\cnt{647}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){3}{}&\int(0){\0}{}&\int(3){3}{}&\ln{2}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\rat(1/2){2}{}&\rat(-1/2){2}{}&\int(4){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 69
\orbit{3}{69}{86}
\h{69}&\int(9){2}{\spec{2}}&\int(1){2}{}&\int(2){1}{}&&\cnt{607}&\bounds{86}{86}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(5/2){1}{}&\int(1){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(1){2}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*D[8]
% Class 70
\orbit{3}{70}{78}
\h{70}&\int(2){3}{}&\int(2){3}{}&\int(8){\8}{0}&&\cnt{495}&\bounds{78}{78}{1}{false}&&\cr
\l{1}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){3}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(3/2){1}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_3E8.tex <==
% -*- TeX -*-
% Niemeier lattice 3E8
% 9 classes
\newcs{max-3E8}{135}%
\newcs{count-3E8}{9}%
\newcs{counts-3E8}{\DO{1}{135}\DO{2}{120}\DO{3}{111}\DO{4}{99}\DO{5}{99}\DO{6}{87}\DO{7}{87}\DO{8}{75}\DO{9}{51}}%
\orbits
% -*- TeX -*-
% Niemeier lattice 3*E[8]
% Class 1
\orbit{3}{1}{135}
\h{1}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{975}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{512}&\bounds{64}{64}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{392}&\bounds{56}{56}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*E[8]
% Class 2
\orbit{3}{2}{120}
\h{2}&\int(12){\12}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1563}&\bounds{120}{120}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{0}{0}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{720}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*E[8]
% Class 3
\orbit{3}{3}{111}
\h{3}&\int(6){\6}{}&\int(6){\6}{}&\int(0){\0}{}&&\cnt{999}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{729}&\bounds{81}{81}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*E[8]
% Class 4
\orbit{3}{4}{99}
\h{4}&\int(10){\10}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{1163}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{240}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{672}&\bounds{48}{48}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*E[8]
% Class 5
\orbit{3}{5}{99}
\h{5}&\int(8){\8}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{1235}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{240}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{784}&\bounds{56}{56}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*E[8]
% Class 6
\orbit{3}{6}{87}
\h{6}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{1023}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{448}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*E[8]
% Class 7
\orbit{3}{7}{87}
\h{7}&\int(4){\4}{}&\int(4){\4}{}&\int(4){\4}{}&&\cnt{591}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*E[8]
% Class 8
\orbit{3}{8}{75}
\h{8}&\int(6){\6}{}&\int(4){\4}{}&\int(2){\2}{}&&\cnt{687}&\bounds{75}{75}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{112}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{378}&\bounds{42}{42}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 3*E[8]
% Class 9
\orbit{3}{9}{51}
\h{9}&\int(8){\8}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{491}&\bounds{51}{51}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{56}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_4D6.tex <==
% -*- TeX -*-
% Niemeier lattice 4D6
% 85 classes
\newcs{max-4D6}{231}%
\newcs{count-4D6}{85}%
\newcs{counts-4D6}{\DO{1}{231}\DO{2}{231}\DO{3}{219}\DO{4}{219}\DO{5}{215}\DO{6}{199}\DO{7}{195}\DO{8}{189}\DO{9}{187}\DO{10}{187}\DO{11}{187}\DO{12}{185}\DO{13}{183}\DO{14}{183}\DO{15}{183}\DO{16}{179}\DO{17}{175}\DO{18}{173}\DO{19}{169}\DO{20}{169}\DO{21}{167}\DO{22}{167}\DO{23}{167}\DO{24}{167}\DO{25}{165}\DO{26}{165}\DO{27}{163}\DO{28}{163}\DO{29}{163}\DO{30}{163}\DO{31}{163}\DO{32}{163}\DO{33}{163}\DO{34}{159}\DO{35}{159}\DO{36}{159}\DO{37}{157}\DO{38}{155}\DO{39}{153}\DO{40}{151}\DO{41}{151}\DO{42}{151}\DO{43}{151}\DO{44}{151}\DO{45}{151}\DO{46}{151}\DO{47}{149}\DO{48}{143}\DO{49}{143}\DO{50}{141}\DO{51}{141}\DO{52}{141}\DO{53}{141}\DO{54}{141}\DO{55}{139}\DO{56}{139}\DO{57}{139}\DO{58}{137}\DO{59}{136}\DO{60}{135}\DO{61}{135}\DO{62}{135}\DO{63}{135}\DO{64}{133}\DO{65}{132}\DO{66}{131}\DO{67}{131}\DO{68}{131}\DO{69}{129}\DO{70}{127}\DO{71}{127}\DO{72}{123}\DO{73}{123}\DO{74}{123}\DO{75}{121}\DO{76}{119}\DO{77}{119}\DO{78}{119}\DO{79}{115}\DO{80}{113}\DO{81}{111}\DO{82}{103}\DO{83}{103}\DO{84}{99}\DO{85}{95}}%
\orbits
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 1
\orbit{4}{1}{231}
\h{1}&\rat(3/2){3}{}&\int(9){2}{\spec{4}}&\rat(3/2){1}{}&\int(0){\0}{}&&\cnt{1371}&\bounds{231}{231}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\int(3){2}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(1){1}{}&\int(3){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{2}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\rat(1/2){3}{}&\int(3){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{5}&\rat(1/2){2}{}&\int(3){2}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{432}&\bounds{72}{72}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 2
\orbit{4}{2}{231}
\h{2}&\int(6){\6}{3}&\int(6){\6}{1}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1431}&\bounds{231}{231}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(2){3}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{432}&\bounds{72}{72}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 3
\orbit{4}{3}{219}
\h{3}&\int(4){\4}{2}&\int(4){\4}{2}&\int(4){\4}{2}&\int(0){\0}{}&&\cnt{1431}&\bounds{219}{219}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(1){3}{}&\int(2){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{3}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(2){2}{}&\int(2){2}{}&\int(0){2}{}&\int(0){2}{}&\ln{3}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 4
\orbit{4}{4}{219}
\h{4}&\int(9){2}{\spec{4}}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&&\cnt{1371}&\bounds{219}{219}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(3){2}{}&\rat(1/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{3}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\int(3){2}{}&\int(1){2}{}&\int(1){2}{}&\int(-1){2}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){2}{}&\int(1){2}{}&\int(0){2}{}&\int(0){2}{}&\ln{3}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 5
\orbit{4}{5}{215}
\h{5}&\int(6){\6}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{815}&\bounds{215}{215}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{6}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{3}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{3}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 6
\orbit{4}{6}{199}
\h{6}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{911}&\bounds{199}{199}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(3){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(3){3}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(3){3}{}&\int(0){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(3){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(2){2}{}&\int(1){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 7
\orbit{4}{7}{195}
\h{7}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1159}&\bounds{195}{195}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\int(2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\int(2){3}{}&\int(2){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{4}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(2){2}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 8
\orbit{4}{8}{189}
\h{8}&\int(3){2}{}&\int(3){2}{}&\int(3){2}{}&\int(3){2}{}&&\cnt{711}&\bounds{189}{189}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{12}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{81}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 9
\orbit{4}{9}{187}
\h{9}&\int(12){\12}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1347}&\bounds{187}{187}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(4){3}{}&\int(0){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{3}&\cnt{384}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 10
\orbit{4}{10}{187}
\h{10}&\int(10){\10}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1099}&\bounds{187}{187}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){2}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{8}&\int(3){2}{}&\int(1){2}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 11
\orbit{4}{11}{187}
\h{11}&\int(8){\8}{0}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1147}&\bounds{187}{187}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(2){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(2){2}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 12
\orbit{4}{12}{185}
\h{12}&\int(6){\6}{3}&\int(4){\4}{2}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{1183}&\bounds{185}{185}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(3){3}{}&\int(2){2}{}&\int(-1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(0){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(3){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(2){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(1){3}{}&\int(2){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\int(1){2}{}&\int(2){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 13
\orbit{4}{13}{183}
\h{13}&\int(4){\4}{}&\int(4){\4}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{703}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{4}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{4}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\ln{4}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 14
\orbit{4}{14}{183}
\h{14}&\int(6){\6}{\spec{1}}&\int(4){\4}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{799}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){3}{}&\int(2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(2){1}{}&\int(2){3}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(1){1}{}&\int(2){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(2){2}{}&\int(2){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(2){2}{}&\int(2){1}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(2){2}{}&\int(1){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{17}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{18}&\int(1){2}{}&\int(2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 15
\orbit{4}{15}{183}
\h{15}&\int(4){\4}{}&\int(4){\4}{}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{687}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{3}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{6}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(0){2}{}&\int(2){1}{}&\int(0){\0}{}&\ln{3}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 16
\orbit{4}{16}{179}
\h{16}&\rat(19/2){3}{\spec{1}}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&&\cnt{1147}&\bounds{179}{179}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(7/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(7/2){3}{}&\int(1){2}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(7/2){3}{}&\int(0){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{8}&\rat(7/2){3}{}&\int(-1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(3){1}{}&\rat(1/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\int(3){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(3){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{13}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 17
\orbit{4}{17}{175}
\h{17}&\int(5){2}{\spec{2}}&\int(3){2}{}&\int(3){2}{}&\int(1){2}{}&&\cnt{751}&\bounds{175}{175}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\rat(3/2){1}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(1){2}{}&\int(0){2}{}&\int(1){2}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 18
\orbit{4}{18}{173}
\h{18}&\rat(15/2){3}{\spec{2}}&\rat(3/2){3}{}&\rat(3/2){3}{}&\rat(3/2){3}{}&&\cnt{979}&\bounds{173}{173}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(5/2){3}{}&\int(1){1}{}&\int(0){\0}{}&\rat(1/2){2}{}&\ln{3}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{3}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(5/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{3}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(5/2){2}{}&\int(1){1}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{3}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(5/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 19
\orbit{4}{19}{169}
\h{19}&\int(6){\6}{3}&\int(4){\4}{}&\int(0){\0}{}&\int(2){\2}{}&&\cnt{935}&\bounds{169}{169}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(2){1}{}&\int(0){\0}{}&\int(-1){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(0){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){3}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(3){3}{}&\int(0){\0}{}&\int(0){2}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){1}{}&\int(2){3}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(1){3}{}&\int(2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(1){2}{}&\int(2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 20
\orbit{4}{20}{169}
\h{20}&\rat(3/2){3}{}&\int(7){2}{}&\rat(3/2){1}{}&\int(2){\2}{}&&\cnt{871}&\bounds{169}{169}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(1){1}{}&\rat(5/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(1){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(1/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(1/2){2}{}&\rat(5/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(1/2){2}{}&\int(2){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 21
\orbit{4}{21}{167}
\h{21}&\rat(15/2){3}{\spec{2}}&\int(3){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&&\cnt{967}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(5/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(5/2){2}{}&\rat(3/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(5/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(5/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\l{14}&\rat(5/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 22
\orbit{4}{22}{167}
\h{22}&\rat(11/2){3}{}&\int(5){2}{\spec{2}}&\rat(3/2){1}{}&\int(0){\0}{}&&\cnt{923}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{}&\int(2){2}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{13}&\int(2){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{15}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(1/2){3}{\spec{1}}&\int(2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(1/2){3}{\spec{2}}&\int(2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{19}&\rat(3/2){2}{}&\int(2){2}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 23
\orbit{4}{23}{167}
\h{23}&\int(4){\4}{}&\int(4){\4}{}&\int(4){\4}{2}&\int(0){\0}{}&&\cnt{935}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(2){3}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){1}{}&\int(0){3}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(1){1}{}&\int(1){3}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\int(1){2}{}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 24
\orbit{4}{24}{167}
\h{24}&\rat(15/2){3}{\spec{2}}&\int(1){2}{}&\rat(3/2){1}{}&\int(2){\2}{}&&\cnt{975}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(5/2){2}{}&\rat(1/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(5/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(5/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(5/2){2}{}&\int(1){2}{}&\rat(-1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(5/2){2}{}&\int(0){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{18}&\rat(5/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(0){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(5/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 25
\orbit{4}{25}{165}
\h{25}&\rat(15/2){3}{\spec{1}}&\int(3){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&&\cnt{855}&\bounds{165}{165}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(3){1}{}&\rat(3/2){3}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){1}{}&\rat(1/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(3){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{12}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(3/2){3}{\spec{1}}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(3/2){3}{\spec{2}}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 26
\orbit{4}{26}{165}
\h{26}&\rat(11/2){3}{}&\int(3){2}{}&\rat(3/2){1}{}&\int(2){\2}{}&&\cnt{759}&\bounds{165}{165}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{14}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(3/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{18}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 27
\orbit{4}{27}{163}
\h{27}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{875}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(3){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{12}&\int(3){3}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 28
\orbit{4}{28}{163}
\h{28}&\int(5){2}{\spec{2}}&\int(5){2}{\spec{2}}&\int(1){2}{}&\int(1){2}{}&&\cnt{923}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{4}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{4}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){2}{}&\int(1){2}{}&\int(-1){2}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(2){2}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{4}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\int(0){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 29
\orbit{4}{29}{163}
\h{29}&\int(8){\8}{0}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{899}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 30
\orbit{4}{30}{163}
\h{30}&\int(4){\4}{2}&\int(4){\4}{2}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{935}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{4}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){3}{}&\int(2){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{4}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(2){2}{}&\int(1){2}{}&\int(-1){2}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\int(2){2}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(0){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){3}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 31
\orbit{4}{31}{163}
\h{31}&\rat(11/2){3}{}&\int(1){2}{}&\rat(11/2){1}{}&\int(0){\0}{}&&\cnt{923}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{}&\int(-1){2}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(2){1}{}&\rat(1/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(2){1}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{13}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\int(1){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 32
\orbit{4}{32}{163}
\h{32}&\int(7){2}{}&\int(3){2}{}&\int(1){2}{}&\int(1){2}{}&&\cnt{863}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\int(0){\0}{}&\int(1){2}{}&\rat(1/2){1}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(2){2}{}&\int(0){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 33
\orbit{4}{33}{163}
\h{33}&\int(8){\8}{0}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{651}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(1){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 34
\orbit{4}{34}{159}
\h{34}&\rat(3/2){3}{}&\int(9){2}{\spec{1}}&\rat(3/2){1}{}&\int(0){\0}{}&&\cnt{959}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(1){1}{}&\rat(7/2){3}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(1/2){3}{}&\int(2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(0){1}{}&\rat(7/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(1/2){2}{}&\rat(7/2){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\rat(1/2){2}{}&\rat(5/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(7/2){3}{}&\rat(1/2){1}{}&\int(0){2}{}&\ln{1}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 35
\orbit{4}{35}{159}
\h{35}&\int(4){\4}{}&\int(4){\4}{2}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{687}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(2){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(1){3}{}&\int(2){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(1){2}{}&\int(2){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){2}{}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){2}{}&\int(1){3}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 36
\orbit{4}{36}{159}
\h{36}&\rat(15/2){3}{\spec{1}}&\int(1){2}{}&\rat(3/2){1}{}&\int(2){\2}{}&&\cnt{863}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(3){1}{}&\rat(1/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(3){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(3){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(3){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(3){1}{}&\int(0){\0}{}&\int(0){3}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{16}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(3/2){3}{\spec{1}}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(3/2){3}{\spec{2}}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 37
\orbit{4}{37}{157}
\h{37}&\rat(3/2){3}{}&\int(3){2}{}&\rat(3/2){1}{}&\int(6){\6}{\spec{1}}&&\cnt{815}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(1){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(1/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(1/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(1/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 38
\orbit{4}{38}{155}
\h{38}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(8){\8}{\spec{1}}&&\cnt{919}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(-1/2){2}{}&\int(3){1}{}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(1){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(3){3}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(1){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(1/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(3){1}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\int(0){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(3){3}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(1/2){2}{}&\rat(1/2){3}{}&\int(0){\0}{}&\int(3){1}{}&\ln{2}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(1/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 39
\orbit{4}{39}{153}
\h{39}&\rat(11/2){3}{}&\int(1){2}{}&\rat(7/2){1}{}&\int(2){\2}{}&&\cnt{751}&\bounds{153}{153}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(2){1}{}&\rat(1/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(2){1}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{18}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\int(1){1}{\spec{1}}&\int(0){\0}{}&\int(2){3}{}&\int(1){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(1){1}{\spec{2}}&\int(0){\0}{}&\int(2){3}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(3/2){2}{}&\int(1){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{25}&\rat(3/2){2}{}&\int(0){2}{}&\rat(3/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{26}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{27}&\rat(1/2){2}{}&\int(1){2}{}&\rat(3/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(1){2}{}&\int(2){3}{}&\int(1){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{29}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 40
\orbit{4}{40}{151}
\h{40}&\rat(7/2){3}{}&\int(7){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&&\cnt{855}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\rat(5/2){3}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(1){1}{}&\rat(5/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(1/2){3}{\spec{1}}&\int(2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(1/2){3}{\spec{2}}&\int(2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\rat(5/2){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\rat(5/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(3/2){2}{}&\int(2){2}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(1/2){2}{}&\rat(5/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 41
\orbit{4}{41}{151}
\h{41}&\rat(15/2){3}{\spec{1}}&\rat(3/2){3}{}&\rat(3/2){3}{}&\rat(3/2){3}{}&&\cnt{867}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(3){1}{}&\rat(3/2){3}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){1}{}&\rat(1/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{3}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\int(1){1}{}&\int(0){\0}{}&\rat(1/2){2}{}&\ln{3}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{3}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{3}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 42
\orbit{4}{42}{151}
\h{42}&\rat(7/2){3}{}&\int(5){2}{\spec{1}}&\rat(7/2){1}{}&\int(0){\0}{}&&\cnt{811}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\rat(5/2){3}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\rat(1/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(3/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{125}&\bounds{25}{25}{1}{false}&&\cr
\l{9}&\int(1){1}{}&\rat(5/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(1){1}{}&\rat(3/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(0){1}{\spec{1}}&\rat(5/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){1}{\spec{2}}&\rat(5/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\rat(5/2){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\int(1){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 43
\orbit{4}{43}{151}
\h{43}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{895}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(3){3}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){3}{}&\int(2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(2){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 44
\orbit{4}{44}{151}
\h{44}&\rat(7/2){3}{}&\int(3){2}{}&\rat(7/2){1}{}&\int(2){\2}{}&&\cnt{703}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\rat(1/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(1){1}{}&\rat(3/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\int(1){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\int(0){2}{}&\rat(3/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 45
\orbit{4}{45}{151}
\h{45}&\rat(15/2){3}{\spec{2}}&\int(1){2}{}&\rat(7/2){1}{}&\int(0){\0}{}&&\cnt{959}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(2){1}{}&\rat(1/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(2){1}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(5/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{14}&\rat(5/2){2}{}&\rat(-1/2){1}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(5/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(5/2){2}{}&\int(0){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{17}&\rat(5/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(0){3}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 46
\orbit{4}{46}{151}
\h{46}&\rat(11/2){3}{}&\int(3){2}{}&\rat(7/2){1}{}&\int(0){\0}{}&&\cnt{743}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(2){1}{}&\rat(1/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(2){1}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{16}&\int(1){1}{\spec{1}}&\rat(3/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(1){1}{\spec{2}}&\rat(3/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{19}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(3/2){2}{}&\int(1){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(1/2){2}{}&\rat(3/2){1}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 47
\orbit{4}{47}{149}
\h{47}&\rat(7/2){3}{}&\int(5){2}{\spec{2}}&\rat(3/2){1}{}&\int(2){\2}{}&&\cnt{751}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(1){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(1/2){3}{\spec{1}}&\int(2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(1/2){3}{\spec{2}}&\int(2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(3/2){2}{}&\int(2){2}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(3/2){2}{}&\int(2){2}{}&\rat(-1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(1/2){2}{}&\int(2){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){2}{}&\int(1){3}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 48
\orbit{4}{48}{143}
\h{48}&\rat(3/2){3}{}&\int(5){2}{\spec{2}}&\rat(3/2){1}{}&\int(4){\4}{}&&\cnt{751}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(1){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(0){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(1/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(1/2){2}{}&\int(2){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 49
\orbit{4}{49}{143}
\h{49}&\int(6){\6}{3}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{687}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{3}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(0){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{3}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{3}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 50
\orbit{4}{50}{141}
\h{50}&\rat(7/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(6){\6}{\spec{1}}&&\cnt{807}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){1}{}&\int(0){\0}{}&\int(0){3}{}&\int(2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(1){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\rat(1/2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\int(1){2}{}&\rat(-1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(3/2){2}{}&\int(0){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\rat(1/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\rat(1/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\rat(1/2){3}{}&\rat(3/2){1}{}&\int(2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(1){2}{}&\int(1){3}{}&\int(2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 51
\orbit{4}{51}{141}
\h{51}&\rat(11/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(4){\4}{}&&\cnt{751}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(-1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\int(1){1}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(1){1}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(3/2){2}{}&\rat(1/2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(1/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(2){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(1){2}{}&\int(1){3}{}&\int(2){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 52
\orbit{4}{52}{141}
\h{52}&\rat(7/2){3}{}&\int(3){2}{}&\rat(3/2){1}{}&\int(4){\4}{}&&\cnt{703}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\rat(1/2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(2){3}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(1/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(1/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(2){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(3/2){1}{}&\rat(1/2){2}{}&\int(2){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(1){2}{}&\int(1){3}{}&\int(2){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 53
\orbit{4}{53}{141}
\h{53}&\int(5){2}{\spec{1}}&\int(3){2}{}&\int(3){2}{}&\int(1){2}{}&&\cnt{695}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(0){\0}{}&\int(1){2}{}&\rat(1/2){1}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 54
\orbit{4}{54}{141}
\h{54}&\rat(15/2){3}{\spec{1}}&\int(1){2}{}&\rat(7/2){1}{}&\int(0){\0}{}&&\cnt{847}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(3){1}{}&\rat(1/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(3){1}{}&\rat(-1/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(3){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{14}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\int(2){1}{}&\rat(1/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(2){1}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(3/2){3}{\spec{1}}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(3/2){3}{\spec{2}}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(3/2){2}{}&\int(1){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 55
\orbit{4}{55}{139}
\h{55}&\rat(3/2){3}{}&\int(5){2}{\spec{1}}&\rat(3/2){1}{}&\int(4){\4}{2}&&\cnt{811}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\rat(3/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){1}{}&\rat(5/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(1/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(-1/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(1/2){2}{}&\rat(5/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(1/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 56
\orbit{4}{56}{139}
\h{56}&\rat(7/2){3}{}&\int(5){2}{\spec{2}}&\rat(7/2){1}{}&\int(0){\0}{}&&\cnt{735}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\rat(1/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){1}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\int(1){1}{}&\rat(3/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\int(2){2}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\int(1){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 57
\orbit{4}{57}{139}
\h{57}&\rat(7/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(6){\6}{3}&&\cnt{811}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(-1){2}{}&\int(0){\0}{}&\int(3){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\int(1){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(3){3}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(0){1}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\int(3){3}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){1}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\int(3){3}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\rat(1/2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(3){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(1/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(3){3}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{15}&\rat(-1/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(3){3}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\rat(1/2){1}{}&\rat(1/2){2}{}&\int(3){3}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(1){2}{}&\int(1){3}{}&\int(2){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 58
\orbit{4}{58}{137}
\h{58}&\rat(7/2){3}{}&\int(1){2}{}&\rat(7/2){1}{}&\int(4){\4}{}&&\cnt{695}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\rat(1/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(1/2){3}{\spec{1}}&\int(0){\0}{}&\rat(3/2){2}{}&\int(2){1}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(1/2){3}{\spec{2}}&\int(0){\0}{}&\rat(3/2){2}{}&\int(2){1}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\rat(1/2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\int(1){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(3/2){2}{}&\int(0){2}{}&\rat(3/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 59
\orbit{4}{59}{136}
\h{59}&\rat(11/2){3}{}&\rat(7/2){3}{}&\rat(3/2){3}{}&\rat(3/2){3}{}&&\cnt{755}&\bounds{136}{136}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(2){1}{}&\int(0){\0}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\int(1){1}{}&\int(0){\0}{}&\rat(1/2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{}&\rat(3/2){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\rat(1/2){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\int(2){1}{}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(2){1}{}&\rat(1/2){2}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(2){1}{}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(3/2){3}{}&\int(2){1}{}&\int(0){\0}{}&\rat(1/2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(3/2){3}{}&\rat(3/2){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(1){1}{\spec{1}}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(1){1}{\spec{2}}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(3/2){2}{}&\int(2){1}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(3/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{22}&\rat(3/2){2}{}&\int(1){1}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{24}&\rat(3/2){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(3/2){3}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\rat(1/2){2}{}&\int(2){1}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(2){1}{}&\rat(1/2){2}{}&\rat(3/2){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\rat(3/2){2}{}&\rat(3/2){3}{}&\int(1){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 60
\orbit{4}{60}{135}
\h{60}&\int(9){2}{\spec{1}}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&&\cnt{959}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(7/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{3}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(7/2){3}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{3}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(5/2){1}{}&\rat(1/2){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{3}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{3}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 61
\orbit{4}{61}{135}
\h{61}&\int(6){\6}{\spec{1}}&\int(4){\4}{2}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{783}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\int(2){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(1){3}{}&\int(2){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(2){2}{}&\int(1){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(2){2}{}&\int(2){2}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\int(1){2}{}&\int(2){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 62
\orbit{4}{62}{135}
\h{62}&\int(5){2}{\spec{1}}&\int(5){2}{\spec{1}}&\int(1){2}{}&\int(1){2}{}&&\cnt{811}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\rat(5/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(-1){2}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{4}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{4}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{4}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(0){\0}{}&\int(1){2}{}&\rat(1/2){1}{}&\ln{4}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 63
\orbit{4}{63}{135}
\h{63}&\rat(7/2){3}{}&\int(1){2}{}&\rat(7/2){1}{}&\int(4){\4}{2}&&\cnt{811}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\rat(1/2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(0){\0}{}&\int(0){3}{\spec{1}}&\int(2){2}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(0){\0}{}&\int(0){3}{\spec{2}}&\int(2){2}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{2}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(1){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(2){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\int(1){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\int(1){2}{}&\rat(-1/2){2}{}&\int(2){2}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\int(0){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\int(-1){2}{}&\rat(3/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(1/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 64
\orbit{4}{64}{133}
\h{64}&\rat(7/2){3}{}&\rat(7/2){3}{}&\rat(7/2){3}{}&\rat(3/2){3}{}&&\cnt{699}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{3}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\rat(1/2){3}{\spec{1}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\rat(1/2){3}{\spec{2}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{3}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){3}{}&\ln{3}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\rat(1/2){2}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{3}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\ln{3}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\rat(3/2){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{3}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{3}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\int(1){1}{}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){3}{}&\ln{3}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\ln{3}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 65
\orbit{4}{65}{132}
\h{65}&\rat(7/2){3}{}&\int(5){2}{\spec{1}}&\rat(3/2){1}{}&\int(2){\2}{}&&\cnt{695}&\bounds{132}{132}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\rat(5/2){3}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(3/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\int(1){1}{}&\rat(5/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(1/2){3}{\spec{1}}&\rat(5/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(1/2){3}{\spec{2}}&\rat(5/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\rat(5/2){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\rat(5/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(1/2){2}{}&\rat(5/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(1/2){2}{}&\rat(5/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\rat(5/2){1}{}&\rat(1/2){2}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 66
\orbit{4}{66}{131}
\h{66}&\rat(11/2){3}{}&\int(5){2}{\spec{1}}&\rat(3/2){1}{}&\int(0){\0}{}&&\cnt{735}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\int(0){2}{\spec{1}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{}&\int(0){2}{\spec{2}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){1}{}&\rat(5/2){3}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(3/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(1){1}{\spec{1}}&\rat(5/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(1){1}{\spec{2}}&\rat(5/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\rat(5/2){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(3/2){2}{}&\rat(5/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\rat(1/2){2}{}&\rat(5/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 67
\orbit{4}{67}{131}
\h{67}&\int(5){2}{\spec{1}}&\int(5){2}{\spec{2}}&\int(1){2}{}&\int(1){2}{}&&\cnt{735}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\int(2){2}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\int(0){\0}{}&\int(1){2}{}&\rat(1/2){1}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(1){2}{}&\int(2){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){2}{\spec{1}}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 68
\orbit{4}{68}{131}
\h{68}&\rat(3/2){3}{}&\int(5){2}{\spec{2}}&\rat(3/2){1}{}&\int(4){\4}{2}&&\cnt{735}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(1){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{2}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(1){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(1/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(1/2){2}{}&\int(2){2}{}&\rat(-1/2){2}{}&\int(2){2}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(1/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 69
\orbit{4}{69}{129}
\h{69}&\rat(19/2){3}{\spec{2}}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&&\cnt{751}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(3){1}{}&\rat(1/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(3){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(3/2){3}{\spec{1}}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(3/2){3}{\spec{2}}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(5/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(5/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(5/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(0){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 70
\orbit{4}{70}{127}
\h{70}&\rat(3/2){3}{}&\int(5){2}{\spec{1}}&\rat(3/2){1}{}&\int(4){\4}{}&&\cnt{695}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\rat(3/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){1}{}&\rat(5/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(1/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(1/2){2}{}&\rat(5/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(1/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(-1/2){2}{}&\rat(5/2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 71
\orbit{4}{71}{127}
\h{71}&\int(8){\8}{\spec{1}}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{879}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(2){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){2}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 72
\orbit{4}{72}{123}
\h{72}&\int(6){\6}{3}&\int(4){\4}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{671}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){3}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(0){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){1}{}&\int(2){3}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\int(2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 73
\orbit{4}{73}{123}
\h{73}&\int(6){\6}{3}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{767}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){3}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(2){3}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 74
\orbit{4}{74}{123}
\h{74}&\int(12){\12}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{579}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{180}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 75
\orbit{4}{75}{121}
\h{75}&\rat(7/2){3}{}&\int(3){2}{}&\rat(3/2){1}{}&\int(4){\4}{2}&&\cnt{687}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\rat(3/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(0){\0}{}&\int(0){3}{}&\int(2){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(3/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(1){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(1/2){3}{\spec{1}}&\rat(3/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(1/2){3}{\spec{2}}&\rat(3/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\int(1){2}{}&\rat(-1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\int(0){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(1/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(1/2){1}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(1/2){3}{}&\rat(3/2){1}{}&\int(2){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 76
\orbit{4}{76}{119}
\h{76}&\rat(3/2){3}{}&\int(3){2}{}&\rat(3/2){1}{}&\int(6){\6}{3}&&\cnt{687}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(3){3}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(0){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(1/2){2}{}&\rat(3/2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\rat(1/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(3){3}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(-1/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(3){3}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\rat(3/2){3}{}&\rat(3/2){1}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\rat(3/2){1}{}&\rat(-1/2){2}{}&\int(3){3}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\rat(1/2){1}{}&\rat(1/2){2}{}&\int(3){3}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){2}{}&\int(1){3}{}&\int(2){1}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 77
\orbit{4}{77}{119}
\h{77}&\rat(3/2){3}{}&\int(9){2}{\spec{3}}&\rat(3/2){1}{}&\int(0){\0}{}&&\cnt{639}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\rat(5/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\int(2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(1){1}{}&\rat(5/2){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 78
\orbit{4}{78}{119}
\h{78}&\rat(11/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(4){\4}{2}&&\cnt{735}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(5/2){3}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\int(1){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\int(0){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){3}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){1}{}&\int(0){\0}{}&\int(0){3}{}&\int(2){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(3/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(1){1}{\spec{1}}&\int(0){\0}{}&\int(1){3}{}&\int(2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(1){1}{\spec{2}}&\int(0){\0}{}&\int(1){3}{}&\int(2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\int(1){2}{}&\rat(-1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\int(0){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{17}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(1/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\rat(1/2){3}{}&\rat(3/2){1}{}&\int(2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 79
\orbit{4}{79}{115}
\h{79}&\int(12){\12}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{555}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{180}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 80
\orbit{4}{80}{113}
\h{80}&\rat(7/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(6){\6}{1}&&\cnt{679}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(2){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(-1/2){2}{}&\int(3){1}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(1/2){3}{\spec{1}}&\int(0){\0}{}&\rat(1/2){2}{}&\int(3){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(1/2){3}{\spec{2}}&\int(0){\0}{}&\rat(1/2){2}{}&\int(3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\rat(-1/2){3}{}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(2){3}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(1/2){2}{}&\rat(1/2){3}{}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(1/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(2){3}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(1){2}{}&\int(0){3}{}&\int(3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){2}{}&\int(1){3}{}&\int(3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 81
\orbit{4}{81}{111}
\h{81}&\int(6){\6}{3}&\int(4){\4}{2}&\int(0){\0}{}&\int(2){\2}{}&&\cnt{655}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){3}{}&\int(0){\0}{}&\int(0){2}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){3}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(2){2}{}&\int(0){2}{}&\int(1){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 82
\orbit{4}{82}{103}
\h{82}&\int(9){2}{\spec{3}}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&&\cnt{639}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(5/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{6}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){2}{}&\ln{3}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 83
\orbit{4}{83}{103}
\h{83}&\int(4){\4}{}&\int(4){\4}{2}&\int(4){\4}{2}&\int(0){\0}{}&&\cnt{655}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(1){3}{}&\int(2){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(0){2}{}&\int(2){2}{}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 84
\orbit{4}{84}{99}
\h{84}&\int(6){\6}{3}&\int(6){\6}{3}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{639}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*D[6]
% Class 85
\orbit{4}{85}{95}
\h{85}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(8){\8}{0}&&\cnt{527}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\int(1){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(2){3}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(1){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(1/2){2}{}&\int(1){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_4E6.tex <==
% -*- TeX -*-
% Niemeier lattice 4E6
% 30 classes
\newcs{max-4E6}{243}%
\newcs{count-4E6}{30}%
\newcs{counts-4E6}{\DO{1}{243}\DO{2}{183}\DO{3}{165}\DO{4}{163}\DO{5}{159}\DO{6}{149}\DO{7}{147}\DO{8}{147}\DO{9}{145}\DO{10}{143}\DO{11}{143}\DO{12}{139}\DO{13}{137}\DO{14}{137}\DO{15}{137}\DO{16}{135}\DO{17}{135}\DO{18}{131}\DO{19}{131}\DO{20}{129}\DO{21}{129}\DO{22}{127}\DO{23}{127}\DO{24}{119}\DO{25}{118}\DO{26}{111}\DO{27}{108}\DO{28}{95}\DO{29}{91}\DO{30}{88}}%
\orbits
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 1
\orbit{4}{1}{243}
\h{1}&\int(12){\12}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{2187}&\bounds{243}{243}{1}{false}&&\cr
\l{1}&\int(4){1}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{3}&\cnt{729}&\bounds{81}{81}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 2
\orbit{4}{2}{183}
\h{2}&\int(4){\4}{}&\int(4){\4}{}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{795}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{\spec{1}}&\int(0){\0}{}&\ln{6}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{\spec{2}}&\int(0){\0}{}&\ln{6}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{6}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{6}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 3
\orbit{4}{3}{165}
\h{3}&\int(6){\6}{}&\int(6){\6}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1143}&\bounds{165}{165}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{27}{27}{1}{false}&&\cr
\l{4}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{4}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 4
\orbit{4}{4}{163}
\h{4}&\rat(16/3){2}{\spec{2}}&\rat(16/3){2}{\spec{2}}&\rat(4/3){1}{}&\int(0){\0}{}&&\cnt{1291}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\rat(8/3){1}{}&\rat(8/3){1}{}&\rat(-4/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\rat(8/3){1}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{2}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(8/3){1}{}&\int(0){\0}{}&\rat(4/3){1}{}&\int(0){2}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 5
\orbit{4}{5}{159}
\h{5}&\rat(28/3){2}{\spec{1}}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&&\cnt{1243}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(10/3){2}{}&\rat(4/3){2}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(10/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\rat(10/3){2}{}&\rat(1/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\rat(8/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(8/3){1}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 6
\orbit{4}{6}{149}
\h{6}&\int(8){\8}{\spec{3}}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{951}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\int(3){1}{}&\int(1){1}{}&\int(0){2}{}&\int(0){\0}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\l{8}&\int(2){1}{}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 7
\orbit{4}{7}{147}
\h{7}&\rat(22/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(2){\2}{}&&\cnt{911}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(8/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(8/3){1}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(8/3){1}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/3){2}{}&\rat(4/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(7/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(5/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 8
\orbit{4}{8}{147}
\h{8}&\int(6){\6}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{807}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{6}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 9
\orbit{4}{9}{145}
\h{9}&\rat(10/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(6){\6}{}&&\cnt{799}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(5/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(5/3){1}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(4/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\rat(2/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\rat(4/3){2}{}&\rat(2/3){2}{}&\int(2){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 10
\orbit{4}{10}{143}
\h{10}&\rat(16/3){2}{\spec{1}}&\rat(16/3){2}{\spec{1}}&\rat(4/3){1}{}&\int(0){\0}{}&&\cnt{907}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(7/3){2}{}&\rat(7/3){2}{}&\rat(-2/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(7/3){2}{}&\rat(5/3){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(7/3){2}{}&\rat(4/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(7/3){2}{}&\rat(1/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(5/3){1}{}&\rat(5/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{250}&\bounds{50}{50}{1}{false}&&\cr
\l{11}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 11
\orbit{4}{11}{143}
\h{11}&\rat(16/3){2}{\spec{2}}&\rat(10/3){2}{}&\rat(10/3){1}{}&\int(0){\0}{}&&\cnt{919}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(8/3){1}{}&\rat(5/3){1}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(8/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(8/3){1}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{250}&\bounds{50}{50}{1}{false}&&\cr
\l{7}&\rat(2/3){1}{}&\rat(5/3){1}{}&\rat(5/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 12
\orbit{4}{12}{139}
\h{12}&\int(6){\6}{}&\int(4){\4}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{783}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(1){2}{}&\int(2){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 13
\orbit{4}{13}{137}
\h{13}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1007}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{4}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 14
\orbit{4}{14}{137}
\h{14}&\rat(22/3){2}{}&\rat(10/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&&\cnt{895}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(8/3){1}{}&\rat(5/3){1}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(8/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(8/3){1}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(8/3){1}{}&\int(0){\0}{}&\rat(4/3){1}{}&\int(0){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(7/3){2}{}&\rat(5/3){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(7/3){2}{}&\rat(4/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\rat(7/3){2}{}&\rat(1/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(5/3){1}{}&\rat(5/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 15
\orbit{4}{15}{137}
\h{15}&\rat(16/3){2}{\spec{1}}&\rat(10/3){2}{}&\rat(10/3){1}{}&\int(0){\0}{}&&\cnt{727}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(7/3){2}{}&\rat(5/3){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(7/3){2}{}&\rat(4/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(5/3){1}{}&\rat(5/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{2}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{125}&\bounds{25}{25}{1}{false}&&\cr
\l{8}&\rat(2/3){1}{\spec{1}}&\rat(5/3){1}{}&\rat(5/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(2/3){1}{\spec{2}}&\rat(5/3){1}{}&\rat(5/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 16
\orbit{4}{16}{135}
\h{16}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(8){\8}{\spec{3}}&&\cnt{959}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{3}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{3}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(4/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(2){1}{}&\ln{3}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(4/3){2}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\int(3){1}{}&\ln{3}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(2/3){1}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(3){1}{}&\ln{3}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 17
\orbit{4}{17}{135}
\h{17}&\rat(10/3){2}{}&\rat(10/3){2}{}&\rat(4/3){1}{}&\int(4){\4}{}&&\cnt{687}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(5/3){1}{}&\rat(5/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(5/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(5/3){1}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(5/3){1}{}&\int(0){\0}{}&\rat(4/3){1}{}&\int(1){2}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(5/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(2){2}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(4/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(4/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(2){1}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(2/3){1}{}&\int(0){\0}{}&\rat(4/3){1}{}&\int(2){2}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 18
\orbit{4}{18}{131}
\h{18}&\rat(16/3){2}{\spec{2}}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(4){\4}{}&&\cnt{795}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(8/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(0){1}{\spec{1}}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(0){1}{\spec{2}}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(8/3){1}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(8/3){1}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(8/3){1}{}&\rat(-2/3){2}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(4/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(2/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\rat(4/3){2}{}&\rat(2/3){2}{}&\int(2){2}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 19
\orbit{4}{19}{131}
\h{19}&\rat(16/3){2}{\spec{1}}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(4){\4}{}&&\cnt{735}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(7/3){2}{}&\rat(4/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(7/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(7/3){2}{}&\rat(-1/3){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(5/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(5/3){1}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(4/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(2/3){1}{\spec{1}}&\rat(4/3){2}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(2/3){1}{\spec{2}}&\rat(4/3){2}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\rat(4/3){2}{}&\rat(2/3){2}{}&\int(2){2}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 20
\orbit{4}{20}{129}
\h{20}&\int(10){\10}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{971}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(3){2}{}&\int(1){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{4}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 21
\orbit{4}{21}{129}
\h{21}&\rat(16/3){2}{\spec{1}}&\rat(10/3){2}{}&\rat(4/3){1}{}&\int(2){\2}{}&&\cnt{743}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(7/3){2}{}&\rat(5/3){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(7/3){2}{}&\rat(4/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(7/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(7/3){2}{}&\rat(1/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(7/3){2}{}&\int(0){\0}{}&\rat(2/3){2}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(5/3){1}{}&\rat(5/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\rat(5/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{150}&\bounds{25}{25}{1}{false}&&\cr
\l{14}&\rat(5/3){1}{}&\int(0){\0}{}&\rat(4/3){1}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(4/3){2}{}&\rat(5/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(5/3){1}{}&\rat(4/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 22
\orbit{4}{22}{127}
\h{22}&\int(4){\4}{}&\int(4){\4}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{687}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{4}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{4}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{8}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\ln{4}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 23
\orbit{4}{23}{127}
\h{23}&\rat(10/3){2}{}&\rat(10/3){2}{}&\rat(10/3){1}{}&\int(2){\2}{}&&\cnt{695}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{3}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/3){1}{}&\rat(5/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{3}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(5/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\ln{6}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{125}&\bounds{25}{25}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 24
\orbit{4}{24}{119}
\h{24}&\int(8){\8}{\spec{3}}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{927}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\int(2){2}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\int(2){1}{}&\int(2){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 25
\orbit{4}{25}{118}
\h{25}&\rat(28/3){2}{\spec{2}}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&&\cnt{735}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(8/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(8/3){1}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{200}&\bounds{40}{40}{1}{false}&&\cr
\l{9}&\rat(7/3){2}{}&\rat(4/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(4/3){2}{\spec{1}}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(4/3){2}{\spec{2}}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 26
\orbit{4}{26}{111}
\h{26}&\rat(16/3){2}{\spec{2}}&\rat(10/3){2}{}&\rat(4/3){1}{}&\int(2){\2}{}&&\cnt{671}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(8/3){1}{}&\rat(5/3){1}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(8/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(8/3){1}{}&\rat(2/3){1}{}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(8/3){1}{}&\rat(1/3){2}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(8/3){1}{}&\int(0){\0}{}&\rat(4/3){1}{}&\int(0){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(8/3){1}{}&\int(0){\0}{}&\rat(1/3){1}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(4/3){2}{}&\rat(5/3){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\rat(5/3){1}{}&\rat(4/3){1}{}&\int(1){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 27
\orbit{4}{27}{108}
\h{27}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{635}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 28
\orbit{4}{28}{95}
\h{28}&\rat(16/3){2}{\spec{2}}&\rat(16/3){2}{\spec{1}}&\rat(4/3){1}{}&\int(0){\0}{}&&\cnt{703}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\rat(8/3){1}{}&\rat(5/3){1}{}&\rat(-1/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(8/3){1}{}&\rat(4/3){2}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(8/3){1}{}&\rat(2/3){1}{\spec{1}}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(8/3){1}{}&\rat(2/3){1}{\spec{2}}&\rat(2/3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(8/3){1}{}&\int(0){\0}{}&\rat(4/3){1}{}&\int(0){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(4/3){2}{}&\rat(7/3){2}{}&\rat(1/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 29
\orbit{4}{29}{91}
\h{29}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(8){\8}{\spec{1}}&&\cnt{511}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{3}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(4/3){2}{}&\rat(4/3){2}{}&\rat(4/3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/3){2}{}&\rat(2/3){1}{}&\int(0){\0}{}&\int(2){2}{}&\ln{6}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 4*E[6]
% Class 30
\orbit{4}{30}{88}
\h{30}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{663}&\bounds{88}{88}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{216}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_6D4.tex <==
% -*- TeX -*-
% Niemeier lattice 6D4
% 36 classes
\newcs{max-6D4}{375}%
\newcs{count-6D4}{36}%
\newcs{counts-6D4}{\DO{1}{375}\DO{2}{315}\DO{3}{315}\DO{4}{315}\DO{5}{279}\DO{6}{259}\DO{7}{259}\DO{8}{251}\DO{9}{251}\DO{10}{247}\DO{11}{247}\DO{12}{233}\DO{13}{231}\DO{14}{231}\DO{15}{231}\DO{16}{231}\DO{17}{227}\DO{18}{227}\DO{19}{217}\DO{20}{217}\DO{21}{215}\DO{22}{215}\DO{23}{209}\DO{24}{205}\DO{25}{203}\DO{26}{201}\DO{27}{199}\DO{28}{195}\DO{29}{191}\DO{30}{183}\DO{31}{183}\DO{32}{183}\DO{33}{183}\DO{34}{183}\DO{35}{151}\DO{36}{123}}%
\orbits
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 1
\orbit{6}{1}{375}
\h{1}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{735}&\bounds{375}{375}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{15}&\cnt{1}&\bounds{1}{1}{1}{true}&&\cr
\l{2}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{45}&\cnt{16}&\bounds{8}{8}{1}{true}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 2
\orbit{6}{2}{315}
\h{2}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1191}&\bounds{315}{315}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){\2}{\spec{1}}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{9}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(2){3}{}&\int(0){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{18}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 3
\orbit{6}{3}{315}
\h{3}&\int(9){3}{\spec{1}}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1179}&\bounds{315}{315}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(3){3}{}&\int(1){3}{}&\int(1){3}{}&\int(-1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){3}{}&\ln{3}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){3}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{6}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 4
\orbit{6}{4}{315}
\h{4}&\int(4){\4}{3}&\int(4){\4}{3}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1215}&\bounds{315}{315}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(2){3}{}&\int(0){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){3}{}&\ln{3}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{6}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 5
\orbit{6}{5}{279}
\h{5}&\int(6){\6}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{831}&\bounds{279}{279}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{9}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{9}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{18}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 6
\orbit{6}{6}{259}
\h{6}&\int(4){\4}{3}&\int(4){\4}{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{967}&\bounds{259}{259}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(2){3}{}&\int(1){3}{}&\int(-1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(2){3}{}&\int(0){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){3}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{8}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\int(0){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\int(0){3}{}&\int(0){\0}{}&\ln{4}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 7
\orbit{6}{7}{259}
\h{7}&\int(5){3}{}&\int(5){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{955}&\bounds{259}{259}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(2){3}{}&\int(1){3}{}&\int(-1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(2){3}{}&\int(0){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){3}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){3}{}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{8}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){3}{}&\int(0){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){\0}{}&\ln{4}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 8
\orbit{6}{8}{251}
\h{8}&\int(10){\10}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{907}&\bounds{251}{251}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 9
\orbit{6}{9}{251}
\h{9}&\int(8){\8}{0}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{931}&\bounds{251}{251}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(2){3}{}&\int(0){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 10
\orbit{6}{10}{247}
\h{10}&\int(4){\4}{3}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{719}&\bounds{247}{247}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){3}{}&\ln{6}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{8}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(1){3}{}&\int(1){1}{}&\int(1){2}{}&\int(1){3}{}&\int(0){\0}{}&\ln{3}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 11
\orbit{6}{11}{247}
\h{11}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(6){\6}{\spec{1}}&\int(2){\2}{}&&\cnt{839}&\bounds{247}{247}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){3}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\ln{6}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){3}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){1}{}&\int(0){\0}{}&\ln{12}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(1){3}{}&\ln{12}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){2}{}&\int(1){2}{}&\ln{12}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{3}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 12
\orbit{6}{12}{233}
\h{12}&\int(3){3}{}&\int(3){3}{}&\int(3){3}{}&\int(3){3}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{843}&\bounds{233}{233}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{8}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{12}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){\0}{}&\ln{24}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 13
\orbit{6}{13}{231}
\h{13}&\int(7){3}{\spec{1}}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{887}&\bounds{231}{231}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(5/2){2}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{3}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(5/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){1}{}&\int(0){\0}{}&\ln{3}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(5/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{3}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(5/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(5/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){2}{}&\ln{3}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(5/2){2}{}&\rat(1/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\ln{3}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(2){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){3}{}&\ln{3}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(2){3}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\ln{3}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(3/2){1}{}&\int(1){3}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\ln{3}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 14
\orbit{6}{14}{231}
\h{14}&\int(7){3}{\spec{1}}&\int(1){3}{}&\int(1){2}{}&\int(1){2}{}&\int(1){1}{}&\int(1){1}{}&&\cnt{891}&\bounds{231}{231}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(5/2){2}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{10}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(5/2){2}{}&\int(1){3}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\ln{5}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(5/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\ln{5}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(1){3}{}&\rat(1/2){3}{}&\rat(1/2){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){3}{}&\rat(1/2){3}{}&\ln{5}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(3/2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{5}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 15
\orbit{6}{15}{231}
\h{15}&\int(5){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{783}&\bounds{231}{231}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){3}{}&\ln{6}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\ln{6}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\ln{3}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\ln{12}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){2}{}&\ln{6}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){2}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 16
\orbit{6}{16}{231}
\h{16}&\int(7){3}{\spec{1}}&\int(3){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{879}&\bounds{231}{231}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(5/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(5/2){2}{}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\int(0){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(5/2){2}{}&\rat(3/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(5/2){2}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\rat(5/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(5/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(5/2){2}{}&\int(0){\0}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(2){3}{}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(2){3}{}&\rat(3/2){1}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(2){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(2){3}{}&\int(0){3}{\spec{1}}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(2){3}{}&\int(0){3}{\spec{2}}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(3/2){1}{}&\rat(3/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){3}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(3/2){1}{}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{20}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 17
\orbit{6}{17}{227}
\h{17}&\int(3){3}{}&\int(3){3}{}&\int(1){3}{}&\int(1){3}{}&\int(4){\4}{3}&\int(0){\0}{}&&\cnt{843}&\bounds{227}{227}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(-1){3}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{4}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){\0}{}&\ln{4}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\rat(-1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){\0}{}&\ln{4}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{4}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){3}{}&\int(0){1}{}&\ln{4}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){3}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{15}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\int(2){3}{}&\int(0){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{3}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 18
\orbit{6}{18}{227}
\h{18}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(4){\4}{3}&\int(4){\4}{3}&&\cnt{843}&\bounds{227}{227}{1}{false}&&\cr
\l{1}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){3}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(1){3}{}&\int(-1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(2){3}{}&\ln{4}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\ln{4}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(2){3}{}&\int(0){\0}{}&\ln{8}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(1/2){2}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(2){3}{}&\ln{8}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(0){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(2){3}{}&\ln{2}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{3}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 19
\orbit{6}{19}{217}
\h{19}&\int(5){3}{}&\int(3){3}{}&\int(1){3}{}&\int(1){3}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{775}&\bounds{217}{217}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\rat(3/2){2}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){3}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(2){3}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(2){3}{}&\int(0){3}{\spec{1}}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(2){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(3/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{22}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{23}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\int(1){3}{}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{25}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{26}&\rat(1/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\rat(3/2){2}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 20
\orbit{6}{20}{217}
\h{20}&\int(3){3}{}&\int(3){3}{}&\int(1){3}{}&\int(1){3}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{727}&\bounds{217}{217}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{4}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){2}{}&\ln{4}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){\0}{}&\ln{4}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\ln{8}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){2}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\ln{8}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\int(0){\0}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{8}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){3}{}&\ln{8}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 21
\orbit{6}{21}{215}
\h{21}&\int(6){\6}{\spec{1}}&\int(4){\4}{3}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{815}&\bounds{215}{215}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(2){3}{}&\int(0){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){3}{}&\ln{3}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{6}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(1){3}{}&\int(2){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 22
\orbit{6}{22}{215}
\h{22}&\int(3){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&&\cnt{831}&\bounds{215}{215}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{3}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(3/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{6}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(3/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{6}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){2}{}&\ln{6}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){\0}{}&\ln{6}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){3}{}&\ln{3}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(1){3}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){1}{}&\int(0){\0}{}&\ln{3}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(1/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{6}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(2){1}{}&\int(0){2}{}&\ln{3}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){3}{}&\rat(1/2){1}{}&\rat(1/2){2}{}&\int(2){3}{}&\int(0){\0}{}&\ln{3}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{3}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 23
\orbit{6}{23}{209}
\h{23}&\int(3){3}{}&\int(3){3}{}&\int(3){3}{}&\int(1){3}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{719}&\bounds{209}{209}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{3}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){2}{}&\ln{6}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(0){3}{\spec{1}}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\ln{6}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\ln{3}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\int(1){3}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{3}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{6}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\ln{6}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){2}{}&\int(0){\0}{}&\ln{3}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(3/2){1}{}&\int(0){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 24
\orbit{6}{24}{205}
\h{24}&\int(5){3}{}&\int(3){3}{}&\int(1){2}{}&\int(1){2}{}&\int(1){1}{}&\int(1){1}{}&&\cnt{779}&\bounds{205}{205}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{4}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\rat(3/2){2}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\ln{4}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(1){3}{}&\rat(1/2){3}{}&\rat(1/2){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){3}{}&\int(0){\0}{}&\int(1){2}{}&\rat(1/2){1}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{4}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(1){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\rat(3/2){1}{}&\rat(1/2){3}{}&\int(0){\0}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{4}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\ln{4}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\int(1){1}{}&\rat(1/2){3}{}&\ln{4}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(1){3}{}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\ln{4}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(1/2){2}{}&\rat(3/2){2}{}&\int(1){2}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\rat(3/2){2}{}&\int(1){2}{}&\int(0){\0}{}&\rat(1/2){3}{}&\int(1){1}{}&\ln{4}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 25
\orbit{6}{25}{203}
\h{25}&\int(5){3}{}&\int(3){3}{}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{767}&\bounds{203}{203}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{4}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){1}{}&\ln{4}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\int(1){3}{}&\int(0){3}{\spec{1}}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){\0}{}&\ln{4}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\ln{4}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(1){3}{}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(1/2){2}{}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 26
\orbit{6}{26}{201}
\h{26}&\int(3){3}{}&\int(3){3}{}&\int(3){2}{}&\int(1){2}{}&\int(1){1}{}&\int(1){1}{}&&\cnt{723}&\bounds{201}{201}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(1){2}{}&\int(0){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(0){2}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(0){2}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\ln{3}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(3/2){2}{}&\rat(3/2){1}{}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(-1/2){3}{}&\int(0){\0}{}&\ln{3}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\rat(3/2){1}{}&\rat(1/2){3}{}&\int(0){\0}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{6}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\rat(1/2){3}{}&\int(0){\0}{}&\rat(1/2){3}{}&\ln{6}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\ln{6}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{6}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\rat(1/2){3}{}&\int(1){1}{}&\ln{3}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(3/2){1}{}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(3/2){1}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){1}{}&\ln{6}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(3/2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{3}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{15}&\rat(3/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){\0}{}&\rat(1/2){2}{}&\ln{6}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(3/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){1}{}&\ln{6}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 27
\orbit{6}{27}{199}
\h{27}&\int(5){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(4){\4}{3}&\int(0){\0}{}&&\cnt{767}&\bounds{199}{199}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(0){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){3}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\rat(-1/2){1}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\rat(-1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){3}{}&\int(0){1}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){3}{}&\rat(1/2){1}{}&\rat(1/2){2}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\int(2){3}{}&\int(0){3}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{3}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 28
\orbit{6}{28}{195}
\h{28}&\int(8){\8}{0}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{683}&\bounds{195}{195}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{6}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{9}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 29
\orbit{6}{29}{191}
\h{29}&\int(3){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(4){\4}{3}&\int(2){\2}{}&&\cnt{719}&\bounds{191}{191}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(3/2){2}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(3/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\rat(-1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\int(0){\0}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){3}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){3}{}&\int(0){1}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(3/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(-1/2){2}{}&\int(2){3}{}&\int(1){1}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){3}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(1){3}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{19}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){3}{}&\int(1){1}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\int(0){3}{\spec{1}}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(1){3}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){1}{}&\int(1){2}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(1){3}{}&\rat(1/2){1}{}&\rat(1/2){2}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(2){3}{}&\int(1){1}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\int(2){3}{}&\int(0){3}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){3}{}&\int(2){3}{}&\int(1){3}{}&\ln{2}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{27}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{3}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{28}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 30
\orbit{6}{30}{183}
\h{30}&\int(3){3}{}&\int(3){3}{}&\int(1){3}{}&\int(1){3}{}&\int(4){\4}{2}&\int(0){\0}{}&&\cnt{711}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(3/2){2}{}&\rat(3/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(0){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(3/2){2}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){3}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(3/2){2}{}&\int(1){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){2}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(0){3}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(1){3}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(3/2){1}{}&\rat(3/2){1}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(3/2){1}{}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){1}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(3/2){1}{}&\int(1){3}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(3/2){1}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\rat(3/2){1}{}&\int(0){3}{\spec{1}}&\rat(1/2){2}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(3/2){1}{}&\int(0){3}{\spec{2}}&\rat(1/2){2}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(3/2){1}{}&\int(0){\0}{}&\int(1){3}{}&\rat(1/2){2}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(3/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(2){2}{}&\int(0){3}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(1/2){2}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{21}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(2){2}{}&\int(0){1}{}&\ln{2}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(1/2){2}{}&\int(0){\0}{}&\rat(1/2){1}{}&\int(1){3}{}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 31
\orbit{6}{31}{183}
\h{31}&\int(9){3}{\spec{2}}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{671}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(5/2){2}{}&\int(1){3}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){1}{}&\ln{12}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(5/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 32
\orbit{6}{32}{183}
\h{32}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(4){\4}{3}&\int(4){\4}{2}&&\cnt{711}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){3}{}&\rat(1/2){1}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){2}{}&\ln{8}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(1){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(1){3}{}&\ln{8}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(1){2}{}&\int(2){2}{}&\ln{4}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(1/2){1}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\int(2){3}{}&\int(2){2}{}&\ln{4}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{3}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 33
\orbit{6}{33}{183}
\h{33}&\int(4){\4}{3}&\int(4){\4}{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{703}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{4}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(2){3}{}&\int(0){3}{}&\int(0){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{4}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(1){1}{}&\int(1){2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){2}{}&\ln{4}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){2}{}&\int(0){1}{}&\ln{4}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(1){2}{}&\int(1){1}{}&\int(1){3}{}&\int(0){\0}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 34
\orbit{6}{34}{183}
\h{34}&\int(4){\4}{3}&\int(4){\4}{3}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{687}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(4){\4}{3}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{3}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){3}{}&\int(0){3}{}&\ln{3}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(1){2}{}&\int(1){1}{}&\int(0){\0}{}&\int(0){1}{}&\int(0){\0}{}&\ln{3}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 35
\orbit{6}{35}{151}
\h{35}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(8){\8}{0}&\int(0){\0}{}&&\cnt{559}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{4}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){3}{}&\int(1){3}{}&\int(0){\0}{}&\int(0){\0}{}&\int(2){3}{}&\int(0){3}{}&\ln{6}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(1){3}{}&\rat(1/2){2}{}&\rat(1/2){1}{}&\int(0){\0}{}&\int(2){1}{}&\int(0){\0}{}&\ln{12}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{3}&\int(0){\0}{}&\ln{3}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice 6*D[4]
% Class 36
\orbit{6}{36}{123}
\h{36}&\int(12){\12}{1}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{363}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{1}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{5}&\cnt{72}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_A11_D7_E6.tex <==
% -*- TeX -*-
% Niemeier lattice A11_D7_E6
% 314 classes
\newcs{max-A11_D7_E6}{207}%
\newcs{count-A11_D7_E6}{314}%
\newcs{counts-A11_D7_E6}{\DO{1}{207}\DO{2}{207}\DO{3}{203}\DO{4}{199}\DO{5}{195}\DO{6}{191}\DO{7}{191}\DO{8}{187}\DO{9}{183}\DO{10}{179}\DO{11}{177}\DO{12}{175}\DO{13}{171}\DO{14}{167}\DO{15}{167}\DO{16}{167}\DO{17}{167}\DO{18}{163}\DO{19}{163}\DO{20}{161}\DO{21}{161}\DO{22}{161}\DO{23}{159}\DO{24}{159}\DO{25}{159}\DO{26}{159}\DO{27}{159}\DO{28}{157}\DO{29}{157}\DO{30}{157}\DO{31}{157}\DO{32}{157}\DO{33}{155}\DO{34}{155}\DO{35}{153}\DO{36}{153}\DO{37}{153}\DO{38}{153}\DO{39}{153}\DO{40}{153}\DO{41}{153}\DO{42}{153}\DO{43}{152}\DO{44}{152}\DO{45}{151}\DO{46}{151}\DO{47}{151}\DO{48}{151}\DO{49}{151}\DO{50}{151}\DO{51}{151}\DO{52}{151}\DO{53}{149}\DO{54}{149}\DO{55}{149}\DO{56}{149}\DO{57}{148}\DO{58}{147}\DO{59}{147}\DO{60}{147}\DO{61}{147}\DO{62}{147}\DO{63}{147}\DO{64}{147}\DO{65}{145}\DO{66}{145}\DO{67}{145}\DO{68}{145}\DO{69}{145}\DO{70}{144}\DO{71}{143}\DO{72}{143}\DO{73}{143}\DO{74}{143}\DO{75}{143}\DO{76}{143}\DO{77}{143}\DO{78}{143}\DO{79}{142}\DO{80}{142}\DO{81}{142}\DO{82}{141}\DO{83}{141}\DO{84}{141}\DO{85}{141}\DO{86}{139}\DO{87}{139}\DO{88}{139}\DO{89}{139}\DO{90}{139}\DO{91}{139}\DO{92}{139}\DO{93}{139}\DO{94}{139}\DO{95}{139}\DO{96}{139}\DO{97}{139}\DO{98}{138}\DO{99}{137}\DO{100}{137}\DO{101}{137}\DO{102}{137}\DO{103}{137}\DO{104}{137}\DO{105}{137}\DO{106}{137}\DO{107}{137}\DO{108}{137}\DO{109}{137}\DO{110}{136}\DO{111}{136}\DO{112}{136}\DO{113}{135}\DO{114}{135}\DO{115}{135}\DO{116}{135}\DO{117}{135}\DO{118}{135}\DO{119}{135}\DO{120}{134}\DO{121}{133}\DO{122}{133}\DO{123}{133}\DO{124}{133}\DO{125}{133}\DO{126}{133}\DO{127}{132}\DO{128}{132}\DO{129}{131}\DO{130}{131}\DO{131}{131}\DO{132}{131}\DO{133}{131}\DO{134}{131}\DO{135}{131}\DO{136}{130}\DO{137}{130}\DO{138}{130}\DO{139}{130}\DO{140}{129}\DO{141}{129}\DO{142}{129}\DO{143}{129}\DO{144}{128}\DO{145}{128}\DO{146}{127}\DO{147}{127}\DO{148}{127}\DO{149}{127}\DO{150}{127}\DO{151}{127}\DO{152}{127}\DO{153}{127}\DO{154}{127}\DO{155}{127}\DO{156}{126}\DO{157}{126}\DO{158}{126}\DO{159}{125}\DO{160}{125}\DO{161}{125}\DO{162}{125}\DO{163}{125}\DO{164}{125}\DO{165}{124}\DO{166}{124}\DO{167}{123}\DO{168}{123}\DO{169}{123}\DO{170}{123}\DO{171}{123}\DO{172}{123}\DO{173}{123}\DO{174}{123}\DO{175}{123}\DO{176}{123}\DO{177}{122}\DO{178}{122}\DO{179}{122}\DO{180}{122}\DO{181}{121}\DO{182}{121}\DO{183}{121}\DO{184}{121}\DO{185}{121}\DO{186}{121}\DO{187}{121}\DO{188}{120}\DO{189}{120}\DO{190}{119}\DO{191}{119}\DO{192}{119}\DO{193}{119}\DO{194}{119}\DO{195}{119}\DO{196}{119}\DO{197}{119}\DO{198}{119}\DO{199}{118}\DO{200}{118}\DO{201}{118}\DO{202}{117}\DO{203}{117}\DO{204}{117}\DO{205}{117}\DO{206}{116}\DO{207}{116}\DO{208}{116}\DO{209}{116}\DO{210}{115}\DO{211}{115}\DO{212}{115}\DO{213}{115}\DO{214}{115}\DO{215}{115}\DO{216}{115}\DO{217}{114}\DO{218}{114}\DO{219}{113}\DO{220}{113}\DO{221}{113}\DO{222}{113}\DO{223}{113}\DO{224}{113}\DO{225}{113}\DO{226}{113}\DO{227}{112}\DO{228}{112}\DO{229}{112}\DO{230}{112}\DO{231}{111}\DO{232}{111}\DO{233}{111}\DO{234}{111}\DO{235}{111}\DO{236}{111}\DO{237}{110}\DO{238}{110}\DO{239}{109}\DO{240}{109}\DO{241}{109}\DO{242}{109}\DO{243}{108}\DO{244}{108}\DO{245}{108}\DO{246}{108}\DO{247}{107}\DO{248}{107}\DO{249}{107}\DO{250}{107}\DO{251}{107}\DO{252}{107}\DO{253}{107}\DO{254}{106}\DO{255}{106}\DO{256}{105}\DO{257}{105}\DO{258}{105}\DO{259}{105}\DO{260}{105}\DO{261}{105}\DO{262}{104}\DO{263}{103}\DO{264}{103}\DO{265}{103}\DO{266}{103}\DO{267}{103}\DO{268}{103}\DO{269}{102}\DO{270}{101}\DO{271}{101}\DO{272}{100}\DO{273}{100}\DO{274}{99}\DO{275}{99}\DO{276}{99}\DO{277}{99}\DO{278}{99}\DO{279}{98}\DO{280}{98}\DO{281}{98}\DO{282}{97}\DO{283}{97}\DO{284}{95}\DO{285}{95}\DO{286}{95}\DO{287}{94}\DO{288}{93}\DO{289}{93}\DO{290}{91}\DO{291}{91}\DO{292}{91}\DO{293}{91}\DO{294}{91}\DO{295}{90}\DO{296}{90}\DO{297}{89}\DO{298}{89}\DO{299}{88}\DO{300}{88}\DO{301}{88}\DO{302}{87}\DO{303}{87}\DO{304}{87}\DO{305}{86}\DO{306}{83}\DO{307}{83}\DO{308}{83}\DO{309}{83}\DO{310}{79}\DO{311}{78}\DO{312}{77}\DO{313}{74}\DO{314}{65}}%
\orbits
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 1
\orbit{3}{1}{207}
\h{1}&\int(3){6}{}&\int(9){2}{\spec{1}}&\int(0){\0}{}&&\cnt{1467}&\bounds{207}{207}{1}{false}&&\cr
\l{1}&\int(1){6}{}&\int(3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{432}&\bounds{72}{72}{1}{false}&&\cr
\l{3}&\int(1){10}{}&\int(3){2}{}&\int(0){1}{}&\ln{2}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 2
\orbit{3}{2}{207}
\h{2}&\int(12){\12}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1539}&\bounds{207}{207}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{504}&\bounds{72}{72}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 3
\orbit{3}{3}{203}
\h{3}&\int(0){\0}{}&\int(0){\0}{}&\int(12){\12}{\spec{3}}&&\cnt{2187}&\bounds{203}{203}{1}{false}&&\cr
\l{1}&\int(0){4}{}&\int(0){\0}{}&\int(4){1}{}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\l{2}&\int(0){10}{}&\int(0){2}{}&\int(4){1}{}&\ln{1}&\cnt{924}&\bounds{84}{84}{1}{false}&&\cr
\l{3}&\int(0){1}{}&\int(0){1}{}&\int(4){1}{}&\ln{1}&\cnt{768}&\bounds{64}{64}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 4
\orbit{3}{4}{199}
\h{4}&\int(12){\12}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1491}&\bounds{199}{199}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{4}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\l{5}&\int(4){4}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(4){9}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{384}&\bounds{64}{64}{1}{false}&&\cr
\l{7}&\int(4){10}{}&\int(0){2}{}&\int(0){1}{}&\ln{1}&\cnt{378}&\bounds{42}{42}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 5
\orbit{3}{5}{195}
\h{5}&\rat(32/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&&\cnt{1291}&\bounds{195}{195}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(4){6}{\spec{1}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{392}&\bounds{56}{56}{1}{false}&&\cr
\l{3}&\rat(16/3){4}{}&\int(0){\0}{}&\rat(-4/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(10/3){4}{\spec{1}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{320}&\bounds{40}{40}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\int(4){3}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{7}&\rat(8/3){2}{\spec{1}}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 6
\orbit{3}{6}{191}
\h{6}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(28/3){2}{\spec{1}}&&\cnt{1243}&\bounds{191}{191}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(4/3){4}{}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\rat(2/3){8}{}&\int(0){\0}{}&\rat(10/3){2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\rat(4/3){10}{}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(2/3){2}{}&\int(0){2}{}&\rat(10/3){2}{}&\ln{1}&\cnt{392}&\bounds{56}{56}{1}{false}&&\cr
\l{7}&\rat(2/3){11}{}&\int(0){3}{}&\rat(10/3){2}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 7
\orbit{3}{7}{191}
\h{7}&\int(8){\8}{}&\int(4){\4}{2}&\int(0){\0}{}&&\cnt{1043}&\bounds{191}{191}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){6}{\spec{3}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{8}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{2}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 8
\orbit{3}{8}{187}
\h{8}&\int(11){6}{\spec{3}}&\int(1){2}{}&\int(0){\0}{}&&\cnt{1019}&\bounds{187}{187}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(5){6}{}&\int(-1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 9
\orbit{3}{9}{183}
\h{9}&\int(8){\8}{}&\int(0){\0}{}&\int(4){\4}{}&&\cnt{795}&\bounds{183}{183}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{\spec{1}}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{\spec{2}}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(2){8}{\spec{1}}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(2){8}{\spec{3}}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 10
\orbit{3}{10}{179}
\h{10}&\rat(26/3){8}{\spec{1}}&\int(2){\2}{}&\rat(4/3){2}{}&&\cnt{1023}&\bounds{179}{179}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(8/3){2}{}&\int(1){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(8/3){2}{}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(5/3){2}{}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(7/3){1}{}&\int(1){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 11
\orbit{3}{11}{177}
\h{11}&\int(9){6}{\spec{5}}&\int(1){2}{}&\int(2){\2}{}&&\cnt{1127}&\bounds{177}{177}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{144}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(3){10}{}&\int(0){2}{}&\int(1){1}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\l{11}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(5/2){11}{}&\rat(1/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 12
\orbit{3}{12}{175}
\h{12}&\rat(20/3){8}{\spec{2}}&\int(0){\0}{}&\rat(16/3){2}{\spec{2}}&&\cnt{1539}&\bounds{175}{175}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{450}&\bounds{50}{50}{1}{false}&&\cr
\l{3}&\rat(4/3){4}{\spec{4}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{320}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{6}&\rat(4/3){10}{\spec{2}}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{280}&\bounds{28}{28}{1}{false}&&\cr
\l{7}&\int(0){\0}{\spec{2}}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 13
\orbit{3}{13}{171}
\h{13}&\rat(26/3){8}{\spec{1}}&\int(0){\0}{}&\rat(10/3){2}{}&&\cnt{1007}&\bounds{171}{171}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(7/3){4}{}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(8/3){2}{}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{350}&\bounds{50}{50}{1}{false}&&\cr
\l{9}&\rat(7/3){1}{}&\int(0){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 14
\orbit{3}{14}{167}
\h{14}&\int(3){6}{}&\int(1){2}{}&\int(8){\8}{\spec{3}}&&\cnt{959}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(1){4}{}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(1){10}{}&\int(0){2}{}&\int(3){1}{}&\ln{1}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\l{8}&\int(1){2}{}&\int(1){2}{}&\int(2){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\int(0){10}{}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(1/2){1}{}&\rat(1/2){1}{}&\int(3){1}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 15
\orbit{3}{15}{167}
\h{15}&\int(8){\8}{}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{671}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 16
\orbit{3}{16}{167}
\h{16}&\rat(29/3){10}{\spec{1}}&\int(1){2}{}&\rat(4/3){1}{}&&\cnt{959}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(11/3){4}{}&\int(0){\0}{}&\rat(1/3){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(8/3){4}{\spec{1}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(8/3){4}{\spec{2}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(7/2){3}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(10/3){2}{}&\int(1){2}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(10/3){2}{}&\int(0){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\rat(7/3){2}{}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(13/6){1}{}&\rat(1/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 17
\orbit{3}{17}{167}
\h{17}&\rat(5/3){10}{}&\int(9){2}{\spec{1}}&\rat(4/3){1}{}&&\cnt{1467}&\bounds{167}{167}{1}{false}&&\cr
\l{1}&\int(1){6}{}&\int(3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{240}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\rat(5/3){10}{}&\int(3){2}{}&\rat(-2/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(2/3){10}{}&\int(3){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{320}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\rat(1/3){2}{}&\int(3){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{450}&\bounds{50}{50}{1}{false}&&\cr
\l{6}&\rat(-1/3){10}{}&\int(3){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 18
\orbit{3}{18}{163}
\h{18}&\rat(32/3){8}{\spec{4}}&\int(0){\0}{}&\rat(4/3){2}{}&&\cnt{1019}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\rat(14/3){8}{}&\int(0){\0}{}&\rat(-2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{10}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(8/3){8}{\spec{3}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(4){9}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{14}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{16}&\rat(8/3){2}{}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 19
\orbit{3}{19}{163}
\h{19}&\rat(20/3){8}{\spec{2}}&\int(0){\0}{}&\rat(16/3){2}{\spec{2}}&&\cnt{1043}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\rat(4/3){4}{\spec{1}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(4/3){4}{\spec{2}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(4/3){4}{\spec{3}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\rat(8/3){2}{}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(4/3){10}{\spec{1}}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{11}&\rat(4/3){1}{}&\int(0){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(0){\0}{\spec{1}}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 20
\orbit{3}{20}{161}
\h{20}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&\int(6){\6}{}&&\cnt{1143}&\bounds{161}{161}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{378}&\bounds{42}{42}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(0){2}{}&\int(2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){11}{}&\int(0){3}{}&\int(2){2}{}&\ln{1}&\cnt{192}&\bounds{36}{36}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 21
\orbit{3}{21}{161}
\h{21}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{895}&\bounds{161}{161}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){6}{\spec{3}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(3){6}{\spec{3}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){6}{\spec{4}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\int(4){4}{\spec{2}}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(4){9}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(3){9}{\spec{2}}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(3){3}{\spec{2}}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 22
\orbit{3}{22}{161}
\h{22}&\int(10){\10}{}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{919}&\bounds{161}{161}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(5){6}{}&\int(-1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){6}{\spec{1}}&\int(0){2}{}&\int(0){\0}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 23
\orbit{3}{23}{159}
\h{23}&\rat(8/3){8}{}&\int(2){\2}{}&\rat(22/3){2}{}&&\cnt{911}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(4/3){4}{}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(4/3){10}{}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(4/3){10}{}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(2/3){2}{}&\int(1){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(1/3){10}{}&\int(1){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(2/3){11}{}&\int(1){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{10}&\rat(1/3){1}{}&\int(1){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 24
\orbit{3}{24}{159}
\h{24}&\rat(26/3){8}{\spec{4}}&\int(0){\0}{}&\rat(10/3){2}{}&&\cnt{1215}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(7/3){10}{}&\int(0){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{280}&\bounds{28}{28}{1}{false}&&\cr
\l{7}&\rat(8/3){11}{}&\int(0){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{320}&\bounds{60}{60}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 25
\orbit{3}{25}{159}
\h{25}&\rat(26/3){8}{\spec{2}}&\int(2){\2}{}&\rat(4/3){2}{}&&\cnt{799}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){6}{\spec{2}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(3){6}{\spec{3}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(10/3){4}{\spec{3}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(8/3){8}{\spec{3}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(3){3}{\spec{2}}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(8/3){2}{\spec{2}}&\int(1){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(8/3){2}{\spec{2}}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(7/3){10}{}&\int(1){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{20}&\rat(5/3){2}{\spec{2}}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 26
\orbit{3}{26}{159}
\h{26}&\rat(20/3){8}{\spec{2}}&\int(4){\4}{2}&\rat(4/3){2}{}&&\cnt{1291}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(2){6}{\spec{3}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{320}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{240}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(10/3){10}{}&\int(2){2}{}&\rat(-4/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(4/3){10}{\spec{2}}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(2/3){2}{\spec{3}}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(0){\0}{\spec{2}}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 27
\orbit{3}{27}{159}
\h{27}&\int(7){6}{\spec{1}}&\int(5){2}{\spec{1}}&\int(0){\0}{}&&\cnt{907}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{2}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 28
\orbit{3}{28}{157}
\h{28}&\int(3){6}{}&\int(3){2}{}&\int(6){\6}{}&&\cnt{807}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{5}&\rat(1/2){11}{}&\rat(3/2){3}{}&\int(2){2}{}&\ln{2}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{27}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 29
\orbit{3}{29}{157}
\h{29}&\rat(23/3){10}{\spec{1}}&\int(1){2}{}&\rat(10/3){1}{}&&\cnt{903}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(10/3){8}{\spec{1}}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(8/3){4}{\spec{1}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{5}&\rat(7/3){8}{\spec{1}}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(7/3){2}{\spec{1}}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(7/3){2}{\spec{1}}&\int(0){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(5/3){10}{\spec{1}}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(4/3){2}{\spec{1}}&\int(1){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(13/6){1}{}&\rat(1/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 30
\orbit{3}{30}{157}
\h{30}&\int(3){6}{}&\int(7){2}{\spec{2}}&\int(2){\2}{}&&\cnt{863}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(1){10}{}&\int(2){2}{}&\int(1){1}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(1/2){11}{}&\rat(5/2){3}{}&\int(1){2}{}&\ln{2}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 31
\orbit{3}{31}{157}
\h{31}&\int(9){6}{\spec{3}}&\int(3){2}{}&\int(0){\0}{}&&\cnt{783}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\rat(5/2){9}{\spec{1}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(5/2){9}{\spec{2}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 32
\orbit{3}{32}{157}
\h{32}&\rat(29/3){10}{\spec{3}}&\int(1){2}{}&\rat(4/3){1}{}&&\cnt{847}&\bounds{157}{157}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(13/3){8}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(11/3){4}{}&\int(0){\0}{}&\rat(1/3){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{10}&\rat(8/3){4}{\spec{1}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(8/3){4}{\spec{2}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{13}&\rat(7/2){3}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(8/3){10}{}&\int(1){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(8/3){10}{}&\int(0){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(7/3){2}{}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(5/3){10}{\spec{1}}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(5/3){10}{\spec{2}}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 33
\orbit{3}{33}{155}
\h{33}&\rat(5/3){10}{}&\int(1){2}{}&\rat(28/3){1}{\spec{2}}&&\cnt{1243}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\rat(4/3){8}{}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(2/3){4}{}&\int(0){\0}{}&\rat(10/3){1}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(5/3){10}{}&\int(-1){2}{}&\rat(10/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(2/3){10}{}&\int(0){2}{}&\rat(10/3){1}{}&\ln{1}&\cnt{240}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\rat(1/3){2}{}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(-1/3){10}{}&\int(1){2}{}&\rat(10/3){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(5/6){11}{}&\rat(1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(1/6){1}{}&\rat(1/2){1}{}&\rat(10/3){1}{}&\ln{1}&\cnt{320}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 34
\orbit{3}{34}{155}
\h{34}&\rat(32/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&&\cnt{1055}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(13/3){4}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(10/3){4}{\spec{1}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\rat(10/3){4}{\spec{2}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\int(4){3}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{36}{36}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{10}&\rat(11/3){2}{}&\int(0){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{11}&\rat(8/3){2}{}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 35
\orbit{3}{35}{153}
\h{35}&\int(9){6}{\spec{5}}&\int(3){2}{}&\int(0){\0}{}&&\cnt{1119}&\bounds{153}{153}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{9}&\rat(5/2){11}{}&\rat(3/2){3}{}&\int(0){2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 36
\orbit{3}{36}{153}
\h{36}&\rat(14/3){8}{\spec{2}}&\int(0){\0}{}&\rat(22/3){2}{}&&\cnt{895}&\bounds{153}{153}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(7/3){4}{}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(4/3){4}{\spec{1}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(4/3){4}{\spec{2}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(5/3){2}{}&\int(0){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(4/3){10}{}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(4/3){1}{}&\int(0){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 37
\orbit{3}{37}{153}
\h{37}&\int(4){\4}{}&\int(2){\2}{}&\int(6){\6}{}&&\cnt{799}&\bounds{153}{153}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(1){11}{}&\int(1){3}{}&\int(2){2}{}&\ln{2}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 38
\orbit{3}{38}{153}
\h{38}&\rat(11/3){10}{\spec{2}}&\int(1){2}{}&\rat(22/3){1}{}&&\cnt{903}&\bounds{153}{153}{1}{false}&&\cr
\l{1}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(5/3){4}{}&\int(0){\0}{}&\rat(7/3){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(4/3){8}{\spec{1}}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(4/3){8}{\spec{2}}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(5/3){10}{}&\int(0){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(4/3){2}{}&\int(1){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(4/3){2}{}&\int(0){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(2/3){10}{}&\int(1){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(1/3){2}{\spec{1}}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(1/3){2}{\spec{2}}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(7/6){1}{}&\rat(1/2){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{17}&\rat(5/6){11}{}&\rat(1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 39
\orbit{3}{39}{153}
\h{39}&\int(10){\10}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&&\cnt{895}&\bounds{153}{153}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){6}{\spec{3}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(4){4}{\spec{2}}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(3){8}{\spec{2}}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(3){8}{\spec{3}}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(3){4}{\spec{3}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(4){9}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{4}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(3){10}{}&\int(0){2}{}&\int(1){1}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 40
\orbit{3}{40}{153}
\h{40}&\rat(33/4){9}{\spec{1}}&\rat(15/4){1}{}&\int(0){\0}{}&&\cnt{951}&\bounds{153}{153}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(11/4){3}{}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{5}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(7/4){3}{}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(5/2){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(9/4){1}{}&\rat(7/4){1}{}&\int(0){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 41
\orbit{3}{41}{153}
\h{41}&\int(3){6}{}&\int(9){2}{\spec{3}}&\int(0){\0}{}&&\cnt{971}&\bounds{153}{153}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(1/2){9}{}&\rat(7/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\rat(1/2){11}{}&\rat(7/2){3}{}&\int(0){2}{}&\ln{2}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 42
\orbit{3}{42}{153}
\h{42}&\int(6){\6}{}&\int(0){\0}{}&\int(6){\6}{}&&\cnt{783}&\bounds{153}{153}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){8}{\spec{1}}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{4}&\int(2){8}{\spec{2}}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{81}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{2}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 43
\orbit{3}{43}{152}
\h{43}&\int(8){\8}{\spec{1}}&\int(4){\4}{2}&\int(0){\0}{}&&\cnt{1255}&\bounds{152}{152}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{42}{42}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{2}&\cnt{270}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 44
\orbit{3}{44}{152}
\h{44}&\int(11){6}{\spec{5}}&\int(1){2}{}&\int(0){\0}{}&&\cnt{847}&\bounds{152}{152}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{48}{48}{1}{false}&&\cr
\l{9}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 45
\orbit{3}{45}{151}
\h{45}&\rat(20/3){8}{\spec{2}}&\int(4){\4}{2}&\rat(4/3){2}{}&&\cnt{795}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\rat(8/3){2}{}&\int(2){2}{}&\rat(-2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(8/3){2}{}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(5/3){2}{}&\int(2){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(4/3){10}{\spec{1}}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{13}&\rat(2/3){2}{\spec{1}}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(2/3){2}{\spec{2}}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{\spec{1}}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 46
\orbit{3}{46}{151}
\h{46}&\rat(107/12){7}{\spec{1}}&\rat(7/4){3}{}&\rat(4/3){1}{}&&\cnt{1079}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(11/3){4}{}&\int(0){\0}{}&\rat(1/3){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(13/4){3}{}&\rat(3/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{9}&\rat(17/6){2}{}&\rat(1/2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{280}&\bounds{40}{40}{1}{false}&&\cr
\l{10}&\rat(29/12){1}{}&\rat(5/4){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\rat(29/12){1}{}&\rat(1/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 47
\orbit{3}{47}{151}
\h{47}&\rat(33/4){9}{\spec{1}}&\rat(7/4){1}{}&\int(2){\2}{}&&\cnt{971}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(3){4}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(11/4){3}{}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(5/2){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{11}&\rat(9/4){1}{}&\rat(7/4){1}{}&\int(0){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(9/4){1}{}&\rat(3/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 48
\orbit{3}{48}{151}
\h{48}&\rat(17/3){10}{\spec{2}}&\int(1){2}{}&\rat(16/3){1}{\spec{1}}&&\cnt{795}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\rat(4/3){8}{\spec{1}}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(4/3){8}{\spec{2}}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(7/3){2}{}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(7/3){2}{}&\int(-1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(4/3){2}{}&\int(0){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\rat(1/3){2}{\spec{1}}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(1/3){2}{\spec{2}}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(5/6){11}{}&\rat(1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 49
\orbit{3}{49}{151}
\h{49}&\rat(29/3){10}{\spec{5}}&\int(1){2}{}&\rat(4/3){1}{}&&\cnt{1071}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(8/3){10}{}&\int(1){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(8/3){10}{}&\int(0){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(17/6){11}{}&\rat(1/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{320}&\bounds{64}{64}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 50
\orbit{3}{50}{151}
\h{50}&\int(6){\6}{}&\int(2){\2}{}&\int(4){\4}{}&&\cnt{687}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){8}{\spec{1}}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(2){8}{\spec{2}}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(1){11}{}&\int(1){3}{}&\int(2){2}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 51
\orbit{3}{51}{151}
\h{51}&\rat(23/3){10}{\spec{1}}&\int(3){2}{}&\rat(4/3){1}{}&&\cnt{911}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(10/3){8}{\spec{1}}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(8/3){4}{\spec{1}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(5/2){9}{\spec{1}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{\spec{1}}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(7/3){2}{\spec{1}}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{11}&\rat(5/3){10}{\spec{1}}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(13/6){1}{}&\rat(3/2){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(13/6){1}{}&\rat(1/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 52
\orbit{3}{52}{151}
\h{52}&\rat(29/3){10}{\spec{2}}&\int(1){2}{}&\rat(4/3){1}{}&&\cnt{795}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(5){6}{}&\int(-1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(14/3){4}{}&\int(0){\0}{}&\rat(-2/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(11/3){4}{}&\int(0){\0}{}&\rat(1/3){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(10/3){8}{\spec{1}}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{9}&\rat(8/3){4}{\spec{1}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(8/3){4}{\spec{2}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(7/2){3}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{12}&\rat(7/3){2}{\spec{1}}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(5/3){10}{\spec{1}}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 53
\orbit{3}{53}{149}
\h{53}&\rat(23/3){10}{\spec{2}}&\int(3){2}{}&\rat(4/3){1}{}&&\cnt{687}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(11/3){4}{}&\int(0){\0}{}&\rat(1/3){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(8/3){4}{\spec{1}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(8/3){4}{\spec{2}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(7/2){3}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(7/3){2}{}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 54
\orbit{3}{54}{149}
\h{54}&\int(5){6}{\spec{1}}&\int(3){2}{}&\int(4){\4}{}&&\cnt{687}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){8}{\spec{1}}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){8}{\spec{2}}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){4}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(1){10}{\spec{1}}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(1){10}{\spec{2}}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(1){2}{}&\int(1){2}{}&\int(2){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(3/2){11}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(3/2){11}{}&\rat(1/2){3}{}&\int(2){2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(1/2){11}{}&\rat(3/2){3}{}&\int(2){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(1/2){1}{}&\rat(3/2){1}{}&\int(2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 55
\orbit{3}{55}{149}
\h{55}&\rat(14/3){8}{\spec{2}}&\int(6){\6}{\spec{1}}&\rat(4/3){2}{}&&\cnt{799}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(5/3){2}{}&\int(2){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(5/3){2}{}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(4/3){10}{}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{14}&\rat(2/3){2}{\spec{1}}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(2/3){2}{\spec{2}}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(4/3){1}{}&\int(2){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{17}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 56
\orbit{3}{56}{149}
\h{56}&\rat(35/12){7}{}&\rat(31/4){3}{\spec{1}}&\rat(4/3){1}{}&&\cnt{1023}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\rat(3/2){6}{}&\rat(5/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(5/4){3}{}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\rat(7/6){10}{}&\rat(5/2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(5/6){2}{}&\rat(5/2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\rat(1/6){10}{}&\rat(5/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(7/12){11}{}&\rat(11/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(5/12){1}{}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 57
\orbit{3}{57}{148}
\h{57}&\rat(35/12){7}{}&\rat(31/4){3}{\spec{2}}&\rat(4/3){1}{}&&\cnt{855}&\bounds{148}{148}{1}{false}&&\cr
\l{1}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(5/4){3}{}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\rat(3/4){9}{}&\rat(13/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(7/6){10}{}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(7/12){11}{}&\rat(11/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{200}&\bounds{40}{40}{1}{false}&&\cr
\l{8}&\rat(5/12){1}{}&\rat(13/4){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{9}&\rat(5/12){1}{}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(-7/12){1}{}&\rat(13/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 58
\orbit{3}{58}{147}
\h{58}&\int(6){\6}{}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&&\cnt{783}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{2}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 59
\orbit{3}{59}{147}
\h{59}&\rat(8/3){8}{}&\int(4){\4}{2}&\rat(16/3){2}{\spec{2}}&&\cnt{1043}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(4/3){4}{}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(4/3){10}{}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(4/3){10}{}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(2/3){2}{}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{280}&\bounds{40}{40}{1}{false}&&\cr
\l{7}&\rat(-2/3){10}{}&\int(2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(1/3){1}{}&\int(1){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 60
\orbit{3}{60}{147}
\h{60}&\rat(26/3){8}{\spec{2}}&\int(0){\0}{}&\rat(10/3){2}{}&&\cnt{919}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\int(4){6}{\spec{1}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\rat(13/3){4}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(10/3){4}{\spec{1}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(10/3){4}{\spec{2}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{7}&\rat(7/3){4}{\spec{1}}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(4){3}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(8/3){2}{\spec{1}}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 61
\orbit{3}{61}{147}
\h{61}&\int(9){6}{\spec{3}}&\int(1){2}{}&\int(2){\2}{}&&\cnt{791}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(3){8}{\spec{1}}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){8}{\spec{2}}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(3){4}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(3){10}{}&\int(0){2}{}&\int(1){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 62
\orbit{3}{62}{147}
\h{62}&\rat(20/3){8}{\spec{1}}&\int(0){\0}{}&\rat(16/3){2}{\spec{1}}&&\cnt{907}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(7/3){4}{}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{5}&\rat(5/3){8}{\spec{1}}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(5/3){8}{\spec{2}}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(5/3){8}{\spec{3}}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(1){\2}{\spec{3}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(7/3){10}{}&\int(0){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{16}&\rat(5/3){2}{}&\int(0){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{17}&\rat(5/3){11}{}&\int(0){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 63
\orbit{3}{63}{147}
\h{63}&\int(7){6}{\spec{1}}&\int(1){2}{}&\int(4){\4}{}&&\cnt{735}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){8}{\spec{1}}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){8}{\spec{2}}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(1){10}{\spec{1}}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(1){10}{\spec{2}}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(3/2){11}{}&\rat(1/2){3}{}&\int(2){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 64
\orbit{3}{64}{147}
\h{64}&\rat(26/3){8}{\spec{4}}&\int(2){\2}{}&\rat(4/3){2}{}&&\cnt{1231}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(10/3){10}{}&\int(1){2}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(7/3){10}{}&\int(1){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(8/3){11}{}&\int(1){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\rat(8/3){11}{}&\int(0){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 65
\orbit{3}{65}{145}
\h{65}&\rat(23/3){10}{\spec{1}}&\int(3){2}{}&\rat(4/3){1}{}&&\cnt{799}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\rat(10/3){8}{\spec{2}}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(8/3){4}{\spec{2}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(5/2){9}{\spec{2}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(5/2){3}{\spec{2}}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(8/3){10}{}&\int(1){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(8/3){10}{}&\int(0){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(7/3){2}{\spec{2}}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(5/3){10}{\spec{2}}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(5/3){10}{\spec{3}}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\rat(11/6){11}{}&\rat(3/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{20}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 66
\orbit{3}{66}{145}
\h{66}&\rat(41/4){9}{\spec{1}}&\rat(7/4){1}{}&\int(0){\0}{}&&\cnt{1007}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(9/2){6}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(4){4}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(15/4){3}{}&\rat(1/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{7}&\rat(11/4){3}{\spec{1}}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(11/4){3}{\spec{2}}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(7/2){2}{}&\rat(1/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{12}&\rat(9/4){1}{}&\rat(7/4){1}{}&\int(0){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 67
\orbit{3}{67}{145}
\h{67}&\rat(107/12){7}{\spec{4}}&\rat(7/4){3}{}&\rat(4/3){1}{}&&\cnt{1183}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(15/4){9}{}&\rat(1/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(19/6){10}{}&\rat(1/2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{8}&\rat(19/6){10}{}&\rat(-1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(13/6){10}{}&\rat(1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(31/12){11}{}&\rat(7/4){3}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(31/12){11}{}&\rat(3/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 68
\orbit{3}{68}{145}
\h{68}&\rat(17/4){9}{\spec{2}}&\rat(31/4){1}{\spec{2}}&\int(0){\0}{}&&\cnt{1007}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\rat(3/2){6}{\spec{1}}&\rat(5/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\rat(3/2){6}{\spec{2}}&\rat(5/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(7/4){3}{}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\rat(3/2){10}{}&\rat(5/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\rat(5/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{11}&\rat(5/4){1}{}&\rat(11/4){1}{}&\int(0){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 69
\orbit{3}{69}{145}
\h{69}&\int(5){6}{\spec{1}}&\int(1){2}{}&\int(6){\6}{}&&\cnt{791}&\bounds{145}{145}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){8}{\spec{1}}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){8}{\spec{2}}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(2){4}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\int(1){10}{\spec{1}}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(1){10}{\spec{2}}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(1){2}{}&\int(1){2}{}&\int(2){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\rat(3/2){11}{}&\rat(1/2){3}{}&\int(2){2}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 70
\orbit{3}{70}{144}
\h{70}&\int(2){\2}{}&\int(10){\10}{}&\int(0){\0}{}&&\cnt{1195}&\bounds{144}{144}{1}{false}&&\cr
\l{1}&\int(1){6}{}&\int(3){2}{}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{42}{42}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(1){10}{}&\int(3){2}{}&\int(0){1}{}&\ln{2}&\cnt{270}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 71
\orbit{3}{71}{143}
\h{71}&\int(9){6}{\spec{4}}&\int(3){2}{}&\int(0){\0}{}&&\cnt{1167}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{4}&\rat(9/2){9}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 72
\orbit{3}{72}{143}
\h{72}&\int(4){\4}{}&\int(4){\4}{2}&\int(4){\4}{}&&\cnt{795}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{\spec{1}}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{\spec{2}}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(1){10}{}&\int(2){2}{}&\int(1){1}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(0){10}{\spec{1}}&\int(2){2}{}&\int(2){1}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){10}{\spec{2}}&\int(2){2}{}&\int(2){1}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(1){11}{}&\int(1){3}{}&\int(2){2}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 73
\orbit{3}{73}{143}
\h{73}&\rat(32/3){8}{\spec{5}}&\int(0){\0}{}&\rat(4/3){2}{}&&\cnt{959}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(4){9}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{280}&\bounds{40}{40}{1}{false}&&\cr
\l{12}&\rat(8/3){11}{}&\int(0){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 74
\orbit{3}{74}{143}
\h{74}&\rat(29/3){10}{\spec{4}}&\int(1){2}{}&\rat(4/3){1}{}&&\cnt{1019}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{280}&\bounds{40}{40}{1}{false}&&\cr
\l{5}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(11/3){10}{}&\int(1){2}{}&\rat(-2/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(11/3){10}{}&\int(0){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(11/3){10}{}&\int(-1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(7/3){2}{}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 75
\orbit{3}{75}{143}
\h{75}&\int(0){\0}{}&\int(4){\4}{2}&\int(8){\8}{\spec{1}}&&\cnt{1255}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(0){10}{}&\int(2){2}{}&\int(2){1}{}&\ln{2}&\cnt{396}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{240}&\bounds{40}{40}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 76
\orbit{3}{76}{143}
\h{76}&\int(8){\8}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{687}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 77
\orbit{3}{77}{143}
\h{77}&\int(8){\8}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{855}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){6}{\spec{3}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(3){8}{\spec{2}}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(3){4}{\spec{2}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(3){9}{\spec{2}}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(3){3}{\spec{2}}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{4}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(3){10}{}&\int(0){2}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\int(2){10}{\spec{2}}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\int(2){2}{\spec{2}}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(2){11}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{19}&\int(0){\0}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 78
\orbit{3}{78}{143}
\h{78}&\rat(26/3){8}{\spec{2}}&\int(0){\0}{}&\rat(10/3){2}{}&&\cnt{783}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){6}{\spec{2}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(10/3){4}{\spec{3}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(8/3){8}{\spec{3}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{9}&\rat(7/3){4}{\spec{2}}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(7/3){4}{\spec{3}}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(8/3){2}{\spec{2}}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(7/3){10}{}&\int(0){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 79
\orbit{3}{79}{142}
\h{79}&\int(5){6}{\spec{1}}&\int(7){2}{\spec{2}}&\int(0){\0}{}&&\cnt{839}&\bounds{142}{142}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\rat(3/2){9}{\spec{1}}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(3/2){9}{\spec{2}}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(3/2){3}{}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(3/2){11}{}&\rat(5/2){3}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 80
\orbit{3}{80}{142}
\h{80}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&&\cnt{1143}&\bounds{142}{142}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{288}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(2){11}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 81
\orbit{3}{81}{142}
\h{81}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{983}&\bounds{142}{142}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{7}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(4){6}{\spec{2}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{280}&\bounds{40}{40}{1}{false}&&\cr
\l{7}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(4){9}{}&\int(0){1}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 82
\orbit{3}{82}{141}
\h{82}&\rat(9/4){9}{}&\rat(39/4){1}{\spec{2}}&\int(0){\0}{}&&\cnt{1131}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(3/4){3}{}&\rat(13/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{4}&\rat(1/4){9}{}&\rat(15/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(3/4){11}{}&\rat(13/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\rat(1/4){1}{}&\rat(15/4){1}{}&\int(0){1}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 83
\orbit{3}{83}{141}
\h{83}&\rat(14/3){8}{\spec{2}}&\int(2){\2}{}&\rat(16/3){2}{\spec{1}}&&\cnt{743}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(7/3){4}{}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(5/3){2}{}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(5/3){2}{}&\int(0){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(4/3){10}{}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(2/3){2}{\spec{1}}&\int(1){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(2/3){2}{\spec{2}}&\int(1){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(4/3){1}{}&\int(1){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(2/3){11}{}&\int(1){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 84
\orbit{3}{84}{141}
\h{84}&\rat(5/3){10}{}&\int(3){2}{}&\rat(22/3){1}{}&&\cnt{903}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\rat(4/3){8}{}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(0){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(2/3){10}{}&\int(1){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(1/3){2}{}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(5/6){11}{}&\rat(3/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(5/6){11}{}&\rat(1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{48}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(1/6){1}{}&\rat(3/2){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(-1/6){11}{}&\rat(3/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 85
\orbit{3}{85}{141}
\h{85}&\rat(17/3){10}{\spec{2}}&\int(3){2}{}&\rat(10/3){1}{}&&\cnt{695}&\bounds{141}{141}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(7/3){2}{}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(7/3){2}{}&\int(0){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(4/3){2}{}&\int(1){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(5/6){11}{}&\rat(3/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 86
\orbit{3}{86}{139}
\h{86}&\rat(20/3){8}{\spec{2}}&\int(2){\2}{}&\rat(10/3){2}{}&&\cnt{687}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(7/3){4}{\spec{1}}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(7/3){4}{\spec{2}}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(8/3){2}{}&\int(1){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(8/3){2}{}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(5/3){2}{}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(4/3){10}{\spec{1}}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(4/3){1}{}&\int(1){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\int(0){\0}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 87
\orbit{3}{87}{139}
\h{87}&\rat(20/3){8}{\spec{2}}&\int(4){\4}{}&\rat(4/3){2}{}&&\cnt{687}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){3}{}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){3}{\spec{1}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){3}{\spec{2}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(8/3){2}{}&\int(1){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(8/3){2}{}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(5/3){2}{}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(4/3){1}{}&\int(2){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{\spec{1}}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 88
\orbit{3}{88}{139}
\h{88}&\int(7){6}{\spec{1}}&\int(3){2}{}&\int(2){\2}{}&&\cnt{751}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(3/2){11}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 89
\orbit{3}{89}{139}
\h{89}&\int(4){\4}{}&\int(4){\4}{}&\int(4){\4}{}&&\cnt{687}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(1){11}{}&\int(2){3}{}&\int(1){2}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(1){11}{}&\int(1){3}{}&\int(2){2}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){11}{}&\int(2){3}{}&\int(2){2}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 90
\orbit{3}{90}{139}
\h{90}&\rat(107/12){11}{\spec{1}}&\rat(7/4){3}{}&\rat(4/3){2}{}&&\cnt{911}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(13/4){3}{}&\rat(3/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(9/4){3}{\spec{1}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(9/4){3}{\spec{2}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(19/6){2}{}&\rat(1/2){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{14}&\rat(19/6){2}{}&\rat(-1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(13/6){2}{}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(25/12){1}{}&\rat(5/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 91
\orbit{3}{91}{139}
\h{91}&\int(3){6}{}&\int(5){2}{\spec{1}}&\int(4){\4}{}&&\cnt{735}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){10}{}&\int(2){2}{}&\int(1){1}{}&\ln{2}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(0){10}{}&\int(2){2}{}&\int(2){1}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(1/2){11}{}&\rat(3/2){3}{}&\int(2){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 92
\orbit{3}{92}{139}
\h{92}&\int(4){\4}{}&\int(8){\8}{\spec{1}}&\int(0){\0}{}&&\cnt{895}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(1){9}{\spec{1}}&\int(3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(1){9}{\spec{2}}&\int(3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(1){11}{}&\int(3){3}{}&\int(0){2}{}&\ln{2}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 93
\orbit{3}{93}{139}
\h{93}&\rat(35/12){7}{}&\rat(7/4){3}{}&\rat(22/3){1}{}&&\cnt{915}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(5/3){4}{}&\int(0){\0}{}&\rat(7/3){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\rat(4/3){8}{}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(7/6){10}{}&\rat(1/2){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(5/6){2}{}&\rat(1/2){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{7}&\rat(7/12){11}{}&\rat(7/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(7/12){11}{}&\rat(3/4){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(5/12){1}{}&\rat(5/4){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{10}&\rat(-5/12){11}{}&\rat(7/4){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 94
\orbit{3}{94}{139}
\h{94}&\int(7){6}{\spec{2}}&\int(1){2}{}&\int(4){\4}{}&&\cnt{795}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){8}{\spec{2}}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){8}{\spec{3}}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){4}{\spec{3}}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{9}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(3){10}{}&\int(0){2}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\int(3){10}{}&\int(-1){2}{}&\int(2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\int(1){10}{\spec{2}}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(1){10}{\spec{3}}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(1){2}{\spec{3}}&\int(1){2}{}&\int(2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\rat(3/2){11}{}&\rat(1/2){3}{}&\int(2){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{21}&\int(0){\0}{\spec{2}}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 95
\orbit{3}{95}{139}
\h{95}&\int(5){6}{\spec{1}}&\int(7){2}{\spec{3}}&\int(0){\0}{}&&\cnt{1043}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{245}&\bounds{35}{35}{1}{false}&&\cr
\l{4}&\rat(1/2){9}{\spec{1}}&\rat(7/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(1/2){9}{\spec{2}}&\rat(7/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{7}&\rat(3/2){11}{}&\rat(5/2){3}{}&\int(0){2}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\rat(1/2){1}{}&\rat(7/2){1}{}&\int(0){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 96
\orbit{3}{96}{139}
\h{96}&\int(0){\0}{}&\int(10){\10}{}&\int(2){\2}{}&&\cnt{1195}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(0){10}{}&\int(3){2}{}&\int(1){1}{}&\ln{2}&\cnt{396}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{200}&\bounds{40}{40}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 97
\orbit{3}{97}{139}
\h{97}&\rat(17/3){10}{\spec{2}}&\int(1){2}{}&\rat(16/3){1}{\spec{2}}&&\cnt{735}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(5/3){4}{\spec{1}}&\int(0){\0}{}&\rat(7/3){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(5/3){4}{\spec{2}}&\int(0){\0}{}&\rat(7/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(7/3){2}{}&\int(1){2}{}&\rat(2/3){2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(7/3){2}{}&\int(1){2}{}&\rat(2/3){2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(7/3){2}{}&\int(0){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(5/3){10}{}&\int(0){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(4/3){2}{}&\int(1){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(2/3){10}{}&\int(1){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\rat(7/6){1}{}&\rat(1/2){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 98
\orbit{3}{98}{138}
\h{98}&\rat(33/4){9}{\spec{4}}&\rat(7/4){1}{}&\int(2){\2}{}&&\cnt{1283}&\bounds{138}{138}{1}{false}&&\cr
\l{1}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{231}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(5/2){10}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{462}&\bounds{42}{42}{1}{false}&&\cr
\l{5}&\rat(11/4){11}{}&\rat(5/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(11/4){11}{}&\rat(1/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{210}&\bounds{35}{35}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 99
\orbit{3}{99}{137}
\h{99}&\int(0){\0}{}&\int(12){\12}{\spec{1}}&\int(0){\0}{}&&\cnt{1355}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(0){9}{}&\int(4){1}{}&\int(0){\0}{}&\ln{2}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(0){11}{}&\int(4){3}{}&\int(0){2}{}&\ln{2}&\cnt{324}&\bounds{27}{27}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 100
\orbit{3}{100}{137}
\h{100}&\rat(25/4){9}{\spec{2}}&\rat(23/4){1}{}&\int(0){\0}{}&&\cnt{727}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(5/2){6}{\spec{1}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(5/2){6}{\spec{2}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(11/4){3}{}&\rat(5/4){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(11/4){3}{}&\rat(5/4){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(7/4){3}{\spec{1}}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(7/4){3}{\spec{2}}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(5/2){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(5/4){1}{}&\rat(11/4){1}{}&\int(0){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 101
\orbit{3}{101}{137}
\h{101}&\rat(23/3){10}{\spec{1}}&\int(1){2}{}&\rat(10/3){1}{}&&\cnt{791}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(10/3){8}{\spec{2}}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(8/3){4}{\spec{2}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(7/3){8}{\spec{2}}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(7/3){8}{\spec{3}}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(8/3){10}{}&\int(1){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(8/3){10}{}&\int(0){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{16}&\rat(7/3){2}{\spec{2}}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(7/3){2}{\spec{2}}&\int(0){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(5/3){10}{\spec{2}}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(5/3){10}{\spec{3}}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{20}&\rat(4/3){2}{\spec{2}}&\int(1){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{21}&\rat(11/6){11}{}&\rat(1/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 102
\orbit{3}{102}{137}
\h{102}&\int(7){6}{\spec{1}}&\int(5){2}{\spec{2}}&\int(0){\0}{}&&\cnt{727}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{125}&\bounds{25}{25}{1}{false}&&\cr
\l{4}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(3/2){9}{\spec{1}}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(3/2){9}{\spec{2}}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(3/2){11}{}&\rat(5/2){3}{}&\int(0){2}{}&\ln{2}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 103
\orbit{3}{103}{137}
\h{103}&\int(4){\4}{}&\int(0){\0}{}&\int(8){\8}{\spec{3}}&&\cnt{943}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(1){4}{\spec{1}}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){4}{\spec{2}}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(0){2}{}&\int(2){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(1){10}{}&\int(0){2}{}&\int(3){1}{}&\ln{1}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{12}&\int(1){1}{}&\int(0){1}{}&\int(3){1}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 104
\orbit{3}{104}{137}
\h{104}&\rat(8/3){8}{}&\int(8){\8}{\spec{1}}&\rat(4/3){2}{}&&\cnt{911}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(1){9}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(1){3}{}&\int(3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(4/3){10}{}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(2/3){2}{}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(2/3){11}{}&\int(3){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(1/3){1}{}&\int(3){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(-1/3){11}{}&\int(3){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 105
\orbit{3}{105}{137}
\h{105}&\rat(8/3){8}{}&\int(6){\6}{\spec{1}}&\rat(10/3){2}{}&&\cnt{799}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(4/3){10}{}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(4/3){10}{}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(2/3){2}{}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(1/3){10}{}&\int(2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{10}&\rat(1/3){1}{}&\int(2){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 106
\orbit{3}{106}{137}
\h{106}&\int(8){\8}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{839}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){6}{\spec{3}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\int(3){9}{\spec{2}}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){3}{\spec{2}}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){9}{\spec{2}}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(2){9}{\spec{3}}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){3}{\spec{3}}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(2){11}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 107
\orbit{3}{107}{137}
\h{107}&\rat(20/3){8}{\spec{1}}&\int(2){\2}{}&\rat(10/3){2}{}&&\cnt{743}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(7/3){4}{}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(7/3){10}{}&\int(1){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(7/3){10}{}&\int(0){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(5/3){2}{}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(4/3){10}{\spec{1}}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(4/3){10}{\spec{2}}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{19}&\rat(4/3){1}{}&\int(1){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 108
\orbit{3}{108}{137}
\h{108}&\int(6){\6}{}&\int(6){\6}{}&\int(0){\0}{}&&\cnt{795}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(1){9}{\spec{1}}&\int(3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(1){9}{\spec{2}}&\int(3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{8}&\int(1){11}{}&\int(3){3}{}&\int(0){2}{}&\ln{2}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 109
\orbit{3}{109}{137}
\h{109}&\rat(41/4){9}{\spec{4}}&\rat(7/4){1}{}&\int(0){\0}{}&&\cnt{1019}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{245}&\bounds{35}{35}{1}{false}&&\cr
\l{6}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{7}&\rat(17/4){9}{}&\rat(-1/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\rat(13/4){9}{}&\rat(3/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(11/4){3}{}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(9/4){9}{\spec{1}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(9/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(7/2){10}{}&\rat(1/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 110
\orbit{3}{110}{136}
\h{110}&\rat(11/3){10}{\spec{1}}&\int(7){2}{\spec{1}}&\rat(4/3){1}{}&&\cnt{1291}&\bounds{136}{136}{1}{false}&&\cr
\l{1}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{385}&\bounds{35}{35}{1}{false}&&\cr
\l{2}&\rat(1/2){3}{}&\rat(7/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{231}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(11/6){11}{}&\rat(7/2){3}{}&\rat(-4/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(11/6){11}{}&\rat(3/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\rat(-1/6){11}{}&\rat(7/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 111
\orbit{3}{111}{136}
\h{111}&\rat(9/4){9}{}&\rat(31/4){1}{\spec{2}}&\int(2){\2}{}&&\cnt{1019}&\bounds{136}{136}{1}{false}&&\cr
\l{1}&\rat(3/2){6}{}&\rat(5/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(3/2){10}{}&\rat(5/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(1/2){10}{}&\rat(5/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(1/2){2}{}&\rat(5/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(3/4){11}{}&\rat(9/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(1/4){1}{}&\rat(11/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 112
\orbit{3}{112}{136}
\h{112}&\rat(11/3){10}{\spec{2}}&\int(7){2}{\spec{2}}&\rat(4/3){1}{}&&\cnt{855}&\bounds{136}{136}{1}{false}&&\cr
\l{1}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(5/3){10}{}&\int(2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(4/3){2}{}&\int(2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(2/3){10}{}&\int(2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(7/6){1}{}&\rat(5/2){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{16}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 113
\orbit{3}{113}{135}
\h{113}&\int(6){\6}{}&\int(4){\4}{}&\int(2){\2}{}&&\cnt{695}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(1){11}{}&\int(2){3}{}&\int(1){2}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 114
\orbit{3}{114}{135}
\h{114}&\int(11){6}{\spec{6}}&\int(1){2}{}&\int(0){\0}{}&&\cnt{1151}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{5}&\rat(9/2){9}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{288}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(4){10}{}&\int(0){2}{}&\int(0){1}{}&\ln{1}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\l{9}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 115
\orbit{3}{115}{135}
\h{115}&\int(2){\2}{}&\int(6){\6}{\spec{1}}&\int(4){\4}{}&&\cnt{783}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){10}{}&\int(2){2}{}&\int(1){1}{}&\ln{2}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(0){10}{\spec{1}}&\int(2){2}{}&\int(2){1}{}&\ln{2}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\int(0){10}{\spec{2}}&\int(2){2}{}&\int(2){1}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(1){11}{}&\int(2){3}{}&\int(1){2}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(1){11}{}&\int(1){3}{}&\int(2){2}{}&\ln{2}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){11}{}&\int(2){3}{}&\int(2){2}{}&\ln{2}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 116
\orbit{3}{116}{135}
\h{116}&\rat(14/3){8}{\spec{2}}&\int(4){\4}{}&\rat(10/3){2}{}&&\cnt{695}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(7/3){4}{}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(5/3){2}{}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(4/3){10}{}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\int(2){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(4/3){1}{}&\int(1){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\rat(1/3){1}{}&\int(2){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 117
\orbit{3}{117}{135}
\h{117}&\int(12){\12}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{927}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(4){6}{\spec{3}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){6}{\spec{4}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\int(4){4}{\spec{2}}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\int(4){9}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 118
\orbit{3}{118}{135}
\h{118}&\rat(23/3){10}{\spec{2}}&\int(1){2}{}&\rat(10/3){1}{}&&\cnt{679}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(11/3){4}{}&\int(0){\0}{}&\rat(1/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(8/3){4}{\spec{1}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\rat(8/3){4}{\spec{2}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(7/2){3}{}&\rat(1/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(7/3){2}{}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(7/3){2}{}&\int(0){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(4/3){2}{}&\int(1){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 119
\orbit{3}{119}{135}
\h{119}&\rat(17/3){10}{\spec{2}}&\int(5){2}{\spec{1}}&\rat(4/3){1}{}&&\cnt{735}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(7/3){2}{}&\int(2){2}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(7/3){2}{}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(5/3){10}{}&\int(2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(4/3){2}{}&\int(2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{17}&\rat(2/3){10}{}&\int(2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 120
\orbit{3}{120}{134}
\h{120}&\rat(59/12){7}{\spec{2}}&\rat(23/4){3}{}&\rat(4/3){1}{}&&\cnt{743}&\bounds{134}{134}{1}{false}&&\cr
\l{1}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(5/4){3}{\spec{1}}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(5/4){3}{\spec{2}}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(11/6){2}{}&\rat(3/2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(7/6){10}{}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(17/12){1}{}&\rat(9/4){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(17/12){1}{}&\rat(5/4){1}{\spec{1}}&\rat(4/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(17/12){1}{}&\rat(5/4){1}{\spec{2}}&\rat(4/3){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(7/12){11}{}&\rat(11/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(5/12){1}{}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 121
\orbit{3}{121}{133}
\h{121}&\int(8){\8}{\spec{2}}&\int(0){\0}{}&\int(4){\4}{}&&\cnt{831}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){8}{\spec{2}}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(3){4}{\spec{2}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){8}{\spec{4}}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(2){8}{\spec{5}}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){4}{\spec{4}}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){4}{\spec{5}}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{4}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(3){10}{}&\int(0){2}{}&\int(1){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\int(2){10}{\spec{2}}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{15}&\int(2){2}{\spec{2}}&\int(0){2}{}&\int(2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(2){11}{}&\int(0){3}{}&\int(2){2}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\int(0){\0}{\spec{2}}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 122
\orbit{3}{122}{133}
\h{122}&\rat(17/3){10}{\spec{1}}&\int(1){2}{}&\rat(16/3){1}{\spec{2}}&&\cnt{907}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\rat(5/3){4}{}&\int(0){\0}{}&\rat(7/3){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{3}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(8/3){10}{}&\int(1){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(8/3){10}{}&\int(0){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(8/3){10}{}&\int(-1){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\rat(5/3){10}{}&\int(0){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(4/3){2}{}&\int(1){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{18}&\rat(2/3){10}{\spec{1}}&\int(1){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(2/3){10}{\spec{2}}&\int(1){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(11/6){11}{}&\rat(1/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{21}&\rat(7/6){1}{}&\rat(1/2){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 123
\orbit{3}{123}{133}
\h{123}&\int(0){\0}{}&\int(6){\6}{\spec{1}}&\int(6){\6}{}&&\cnt{1143}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(0){10}{}&\int(2){2}{}&\int(2){1}{}&\ln{2}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(0){11}{}&\int(2){3}{}&\int(2){2}{}&\ln{2}&\cnt{288}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{72}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 124
\orbit{3}{124}{133}
\h{124}&\rat(14/3){8}{\spec{1}}&\int(4){\4}{2}&\rat(10/3){2}{}&&\cnt{919}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(7/3){10}{}&\int(2){2}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(7/3){10}{}&\int(0){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(4/3){10}{\spec{1}}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(4/3){10}{\spec{2}}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(2/3){2}{}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(1/3){10}{}&\int(2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 125
\orbit{3}{125}{133}
\h{125}&\rat(32/3){8}{\spec{3}}&\int(0){\0}{}&\rat(4/3){2}{}&&\cnt{831}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\rat(13/3){4}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(10/3){4}{\spec{1}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(10/3){4}{\spec{2}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(4){3}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(8/3){2}{}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 126
\orbit{3}{126}{133}
\h{126}&\rat(33/4){9}{\spec{2}}&\rat(15/4){1}{}&\int(0){\0}{}&&\cnt{795}&\bounds{133}{133}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(9/2){6}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/2){6}{\spec{1}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\rat(5/2){6}{\spec{1}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(5/2){6}{\spec{2}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(4){4}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(15/4){3}{}&\rat(1/4){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(15/4){3}{}&\rat(1/4){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(11/4){3}{\spec{1}}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{10}&\rat(9/4){9}{\spec{1}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(7/4){3}{\spec{1}}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(7/4){3}{\spec{2}}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(5/2){2}{\spec{1}}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 127
\orbit{3}{127}{132}
\h{127}&\rat(17/3){10}{\spec{1}}&\int(5){2}{\spec{1}}&\rat(4/3){1}{}&&\cnt{907}&\bounds{132}{132}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{3}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(8/3){10}{}&\int(2){2}{}&\rat(-2/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(8/3){10}{}&\int(1){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(8/3){10}{}&\int(0){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(5/3){10}{}&\int(2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(4/3){2}{}&\int(2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{18}&\rat(2/3){10}{\spec{1}}&\int(2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(2/3){10}{\spec{2}}&\int(2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{20}&\rat(11/6){11}{}&\rat(3/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{21}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 128
\orbit{3}{128}{132}
\h{128}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(28/3){2}{\spec{1}}&&\cnt{1243}&\bounds{132}{132}{1}{false}&&\cr
\l{1}&\rat(2/3){8}{}&\int(0){\0}{}&\rat(10/3){2}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(5/6){10}{}&\rat(1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(1/6){2}{}&\rat(1/2){2}{}&\rat(10/3){2}{}&\ln{1}&\cnt{385}&\bounds{35}{35}{1}{false}&&\cr
\l{5}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(11/12){11}{}&\rat(-1/4){3}{}&\rat(10/3){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\rat(1/12){1}{}&\rat(5/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\rat(-1/12){11}{}&\rat(3/4){3}{}&\rat(10/3){2}{}&\ln{1}&\cnt{231}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 129
\orbit{3}{129}{131}
\h{129}&\int(4){\4}{}&\int(6){\6}{\spec{1}}&\int(2){\2}{}&&\cnt{799}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(1){10}{}&\int(2){2}{}&\int(1){1}{}&\ln{2}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(1){11}{}&\int(2){3}{}&\int(1){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 130
\orbit{3}{130}{131}
\h{130}&\int(6){\6}{\spec{1}}&\int(2){\2}{}&\int(4){\4}{}&&\cnt{783}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){2}{}&\int(0){2}{}&\int(2){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(1){2}{}&\int(1){2}{}&\int(2){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(2){11}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{16}&\int(2){11}{}&\int(0){3}{}&\int(2){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\int(1){1}{}&\int(1){1}{}&\int(2){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 131
\orbit{3}{131}{131}
\h{131}&\rat(20/3){8}{\spec{1}}&\int(4){\4}{}&\rat(4/3){2}{}&&\cnt{743}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){9}{\spec{1}}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){9}{\spec{2}}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(7/3){10}{}&\int(1){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{14}&\rat(5/3){2}{}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(5/3){11}{}&\int(2){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(4/3){1}{}&\int(2){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 132
\orbit{3}{132}{131}
\h{132}&\rat(35/12){7}{}&\rat(23/4){3}{}&\rat(10/3){1}{}&&\cnt{747}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(5/4){3}{}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(7/6){10}{}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(5/6){2}{}&\rat(3/2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(7/12){11}{}&\rat(11/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(7/12){11}{}&\rat(7/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(5/12){1}{}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{175}&\bounds{25}{25}{1}{false}&&\cr
\l{11}&\rat(-5/12){11}{}&\rat(11/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 133
\orbit{3}{133}{131}
\h{133}&\int(2){\2}{}&\int(4){\4}{}&\int(6){\6}{}&&\cnt{791}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(1){11}{}&\int(2){3}{}&\int(1){2}{}&\ln{2}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(1){11}{}&\int(1){3}{}&\int(2){2}{}&\ln{2}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(0){11}{}&\int(2){3}{}&\int(2){2}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{54}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 134
\orbit{3}{134}{131}
\h{134}&\rat(35/12){11}{\spec{2}}&\rat(31/4){3}{\spec{1}}&\rat(4/3){2}{}&&\cnt{1015}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(3/2){6}{}&\rat(5/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(5/4){3}{}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(11/6){10}{}&\rat(5/2){2}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(7/6){2}{}&\rat(5/2){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(5/6){10}{}&\rat(5/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(1/6){2}{\spec{1}}&\rat(5/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(1/6){2}{\spec{2}}&\rat(5/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(11/12){11}{}&\rat(11/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(-1/12){11}{}&\rat(11/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 135
\orbit{3}{135}{131}
\h{135}&\rat(14/3){8}{\spec{2}}&\int(4){\4}{2}&\rat(10/3){2}{}&&\cnt{671}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(7/3){4}{}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(5/3){2}{}&\int(2){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(4/3){10}{}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(2/3){2}{\spec{1}}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(2/3){2}{\spec{2}}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(1/3){10}{}&\int(2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(4/3){1}{}&\int(1){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 136
\orbit{3}{136}{130}
\h{136}&\rat(11/3){10}{\spec{2}}&\int(3){2}{}&\rat(16/3){1}{\spec{2}}&&\cnt{743}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(5/3){4}{}&\int(0){\0}{}&\rat(7/3){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(5/3){10}{}&\int(0){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(4/3){2}{}&\int(1){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(2/3){10}{}&\int(1){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(7/6){1}{}&\rat(1/2){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(5/6){11}{}&\rat(3/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{15}&\rat(1/6){1}{}&\rat(3/2){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 137
\orbit{3}{137}{130}
\h{137}&\rat(83/12){7}{\spec{1}}&\rat(15/4){3}{}&\rat(4/3){1}{}&&\cnt{743}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(5/2){6}{\spec{1}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(5/2){6}{\spec{2}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(7/4){9}{\spec{1}}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(7/4){9}{\spec{2}}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(13/6){10}{}&\rat(3/2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(13/6){10}{}&\rat(1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(11/6){2}{}&\rat(3/2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\rat(7/6){10}{\spec{1}}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\rat(7/6){10}{\spec{2}}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(19/12){11}{}&\rat(7/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{22}&\rat(17/12){1}{}&\rat(9/4){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(17/12){1}{}&\rat(5/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{24}&\rat(5/12){1}{}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 138
\orbit{3}{138}{130}
\h{138}&\rat(14/3){8}{\spec{1}}&\int(2){\2}{}&\rat(16/3){2}{\spec{2}}&&\cnt{919}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(4/3){4}{}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(7/3){10}{}&\int(1){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(7/3){10}{}&\int(-1){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(4/3){10}{\spec{1}}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(4/3){10}{\spec{2}}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(1/3){10}{}&\int(1){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{12}&\rat(1/3){1}{}&\int(1){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 139
\orbit{3}{139}{130}
\h{139}&\rat(83/12){11}{\spec{1}}&\rat(15/4){3}{}&\rat(4/3){2}{}&&\cnt{847}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){6}{\spec{1}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(11/4){9}{\spec{1}}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(9/4){3}{\spec{1}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(7/4){9}{\spec{1}}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(13/6){2}{\spec{1}}&\rat(3/2){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(13/6){2}{\spec{1}}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(11/6){10}{\spec{1}}&\rat(3/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(7/6){2}{\spec{1}}&\rat(3/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(25/12){1}{}&\rat(9/4){1}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(25/12){1}{}&\rat(5/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{17}&\rat(11/12){11}{\spec{1}}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 140
\orbit{3}{140}{129}
\h{140}&\rat(17/3){10}{\spec{2}}&\int(5){2}{\spec{2}}&\rat(4/3){1}{}&&\cnt{687}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{}&\rat(3/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{\spec{1}}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(3/2){3}{\spec{2}}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(7/3){2}{}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(7/6){1}{}&\rat(5/2){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 141
\orbit{3}{141}{129}
\h{141}&\rat(33/4){9}{\spec{2}}&\rat(15/4){1}{}&\int(0){\0}{}&&\cnt{783}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(7/2){6}{\spec{2}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(5/2){6}{\spec{3}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(5/2){6}{\spec{4}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(13/4){9}{}&\rat(3/4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(13/4){9}{}&\rat(3/4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(11/4){3}{\spec{2}}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(9/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(9/4){9}{\spec{3}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(7/4){3}{\spec{3}}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(7/4){3}{\spec{4}}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(5/2){10}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{20}&\rat(5/2){2}{\spec{2}}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\rat(7/4){11}{}&\rat(9/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 142
\orbit{3}{142}{129}
\h{142}&\rat(17/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(6){\6}{}&&\cnt{803}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{36}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(3/2){10}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{10}&\rat(5/4){1}{}&\rat(7/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(5/4){1}{}&\rat(3/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\rat(3/4){11}{}&\rat(5/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(1/4){1}{}&\rat(7/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 143
\orbit{3}{143}{129}
\h{143}&\rat(8/3){8}{}&\int(4){\4}{}&\rat(16/3){2}{\spec{1}}&&\cnt{743}&\bounds{129}{129}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(4/3){10}{}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(2/3){2}{}&\int(1){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(2/3){11}{}&\int(1){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(1/3){1}{}&\int(2){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(-1/3){11}{}&\int(2){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 144
\orbit{3}{144}{128}
\h{144}&\rat(11/3){10}{\spec{2}}&\int(5){2}{\spec{1}}&\rat(10/3){1}{}&&\cnt{735}&\bounds{128}{128}{1}{false}&&\cr
\l{1}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(5/3){10}{}&\int(2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(4/3){2}{}&\int(2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(4/3){2}{}&\int(1){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(2/3){10}{}&\int(2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(1/3){2}{\spec{1}}&\int(2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(1/3){2}{\spec{2}}&\int(2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\rat(5/6){11}{}&\rat(3/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 145
\orbit{3}{145}{128}
\h{145}&\rat(107/12){11}{\spec{3}}&\rat(7/4){3}{}&\rat(4/3){2}{}&&\cnt{855}&\bounds{128}{128}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(15/4){9}{}&\rat(1/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(13/4){3}{}&\rat(3/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{14}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(17/6){10}{}&\rat(1/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{16}&\rat(13/6){2}{}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(23/12){11}{}&\rat(7/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(23/12){11}{}&\rat(3/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 146
\orbit{3}{146}{127}
\h{146}&\rat(59/12){7}{\spec{2}}&\rat(15/4){3}{}&\rat(10/3){1}{}&&\cnt{691}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(11/6){2}{}&\rat(3/2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(11/6){2}{}&\rat(1/2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(7/6){10}{}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(5/6){2}{\spec{1}}&\rat(3/2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(5/6){2}{\spec{2}}&\rat(3/2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(17/12){1}{}&\rat(9/4){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(17/12){1}{}&\rat(5/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\rat(7/12){11}{}&\rat(7/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(5/12){1}{}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 147
\orbit{3}{147}{127}
\h{147}&\rat(33/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(2){\2}{}&&\cnt{803}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(7/2){6}{\spec{2}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){8}{\spec{2}}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(3){4}{\spec{3}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(13/4){9}{}&\rat(3/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(11/4){3}{\spec{2}}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(9/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(9/4){9}{\spec{3}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(5/2){10}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{17}&\rat(5/2){2}{\spec{2}}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(7/4){11}{}&\rat(5/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(5/4){1}{\spec{2}}&\rat(7/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 148
\orbit{3}{148}{127}
\h{148}&\int(2){\2}{}&\int(2){\2}{}&\int(8){\8}{\spec{3}}&&\cnt{951}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(1){4}{}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){10}{}&\int(0){2}{}&\int(3){1}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(1){2}{}&\int(1){2}{}&\int(2){2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(0){10}{\spec{1}}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(0){10}{\spec{2}}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(1){11}{}&\int(1){3}{}&\int(2){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(1){1}{}&\int(1){1}{}&\int(2){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(1){1}{}&\int(0){1}{}&\int(3){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){1}{}&\int(1){1}{}&\int(3){1}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 149
\orbit{3}{149}{127}
\h{149}&\rat(41/4){9}{\spec{3}}&\rat(7/4){1}{}&\int(0){\0}{}&&\cnt{839}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(9/2){6}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(7/2){6}{\spec{1}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(7/2){6}{\spec{2}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(4){4}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(15/4){3}{}&\rat(1/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(13/4){9}{}&\rat(3/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(11/4){3}{}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(9/4){9}{\spec{1}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(9/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 150
\orbit{3}{150}{127}
\h{150}&\int(2){\2}{}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&&\cnt{903}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(1){9}{}&\int(3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){10}{}&\int(2){2}{}&\int(1){1}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){11}{}&\int(3){3}{}&\int(0){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(1){11}{}&\int(2){3}{}&\int(1){2}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){11}{}&\int(3){3}{}&\int(1){2}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 151
\orbit{3}{151}{127}
\h{151}&\rat(5/3){10}{}&\int(5){2}{\spec{1}}&\rat(16/3){1}{\spec{2}}&&\cnt{907}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/3){10}{}&\int(2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(5/3){10}{}&\int(0){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(2/3){10}{}&\int(2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(2/3){10}{}&\int(1){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(1/3){2}{}&\int(2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{9}&\rat(-1/3){10}{}&\int(2){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(5/6){11}{}&\rat(3/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\rat(1/6){1}{}&\rat(3/2){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 152
\orbit{3}{152}{127}
\h{152}&\rat(17/4){9}{\spec{2}}&\rat(31/4){1}{\spec{1}}&\int(0){\0}{}&&\cnt{839}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(9/4){9}{}&\rat(7/4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(9/4){9}{}&\rat(7/4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(7/4){3}{}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(3/4){3}{\spec{1}}&\rat(13/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(3/4){3}{\spec{2}}&\rat(13/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(5/4){1}{}&\rat(11/4){1}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(3/4){11}{}&\rat(13/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 153
\orbit{3}{153}{127}
\h{153}&\rat(83/12){11}{\spec{2}}&\rat(15/4){3}{}&\rat(4/3){2}{}&&\cnt{687}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(5/2){6}{\spec{1}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(5/2){6}{\spec{2}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(13/4){3}{}&\rat(3/4){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(13/4){3}{}&\rat(3/4){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(13/6){2}{}&\rat(3/2){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(13/6){2}{}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(11/6){10}{}&\rat(3/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(7/6){2}{}&\rat(3/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{18}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 154
\orbit{3}{154}{127}
\h{154}&\int(3){6}{}&\int(5){2}{\spec{2}}&\int(4){\4}{}&&\cnt{687}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(1/2){11}{}&\rat(5/2){3}{}&\int(1){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(1/2){11}{}&\rat(3/2){3}{}&\int(2){2}{}&\ln{2}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(-1/2){11}{}&\rat(5/2){3}{}&\int(2){2}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 155
\orbit{3}{155}{127}
\h{155}&\int(6){\6}{}&\int(4){\4}{2}&\int(2){\2}{}&&\cnt{671}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{2}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(1){10}{}&\int(2){2}{}&\int(1){1}{}&\ln{2}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 156
\orbit{3}{156}{126}
\h{156}&\rat(59/12){11}{\spec{2}}&\rat(23/4){3}{}&\rat(4/3){2}{}&&\cnt{743}&\bounds{126}{126}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(11/4){9}{}&\rat(5/4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(11/4){9}{}&\rat(5/4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(5/4){3}{\spec{1}}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(5/4){3}{\spec{2}}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(13/6){2}{}&\rat(3/2){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(13/6){2}{}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(11/6){10}{}&\rat(3/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(7/6){2}{}&\rat(3/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{18}&\rat(11/12){11}{}&\rat(11/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(-1/12){11}{}&\rat(11/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 157
\orbit{3}{157}{126}
\h{157}&\int(5){6}{\spec{1}}&\int(5){2}{\spec{1}}&\int(2){\2}{}&&\cnt{735}&\bounds{126}{126}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(1){10}{\spec{1}}&\int(2){2}{}&\int(1){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(1){10}{\spec{2}}&\int(2){2}{}&\int(1){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(1){2}{}&\int(2){2}{}&\int(1){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{14}&\rat(3/2){11}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 158
\orbit{3}{158}{126}
\h{158}&\rat(107/12){7}{\spec{2}}&\rat(7/4){3}{}&\rat(4/3){1}{}&&\cnt{799}&\bounds{126}{126}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(9/2){6}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(7/2){6}{\spec{2}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(11/3){4}{\spec{2}}&\int(0){\0}{}&\rat(1/3){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(8/3){4}{\spec{2}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(8/3){4}{\spec{3}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(13/4){3}{\spec{2}}&\rat(3/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(9/4){3}{\spec{2}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(9/4){3}{\spec{3}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(17/6){2}{\spec{2}}&\rat(1/2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(13/6){10}{}&\rat(1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{18}&\rat(19/12){11}{}&\rat(7/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(17/12){1}{\spec{2}}&\rat(5/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 159
\orbit{3}{159}{125}
\h{159}&\int(8){\8}{\spec{1}}&\int(0){\0}{}&\int(4){\4}{}&&\cnt{1007}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{2}&\cnt{140}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\int(2){11}{}&\int(0){3}{}&\int(2){2}{}&\ln{2}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 160
\orbit{3}{160}{125}
\h{160}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(8){\8}{\spec{2}}&&\cnt{959}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){8}{}&\int(0){\0}{}&\int(3){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(3/2){10}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(1/2){2}{}&\rat(1/2){2}{}&\int(3){2}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\l{7}&\rat(3/4){11}{}&\rat(5/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(3/4){11}{}&\rat(1/4){3}{}&\int(3){2}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(1/4){1}{}&\rat(7/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(-1/4){11}{}&\rat(5/4){3}{}&\int(3){2}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 161
\orbit{3}{161}{125}
\h{161}&\rat(26/3){8}{\spec{3}}&\int(2){\2}{}&\rat(4/3){2}{}&&\cnt{783}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(4){9}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(10/3){10}{}&\int(1){2}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{16}&\rat(7/3){10}{}&\int(1){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(5/3){2}{}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 162
\orbit{3}{162}{125}
\h{162}&\int(11){6}{\spec{4}}&\int(1){2}{}&\int(0){\0}{}&&\cnt{815}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\rat(9/2){9}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 163
\orbit{3}{163}{125}
\h{163}&\rat(20/3){8}{\spec{2}}&\int(0){\0}{}&\rat(16/3){2}{\spec{1}}&&\cnt{719}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(7/3){4}{\spec{1}}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(7/3){4}{\spec{2}}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(8/3){2}{}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(5/3){2}{}&\int(0){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\int(0){\0}{\spec{1}}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 164
\orbit{3}{164}{125}
\h{164}&\rat(20/3){8}{\spec{2}}&\int(2){\2}{}&\rat(10/3){2}{}&&\cnt{919}&\bounds{125}{125}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{3}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(10/3){10}{}&\int(1){2}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(10/3){10}{}&\int(-1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(4/3){10}{\spec{2}}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(0){\0}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 165
\orbit{3}{165}{124}
\h{165}&\rat(17/4){9}{\spec{2}}&\rat(15/4){1}{}&\int(4){\4}{}&&\cnt{687}&\bounds{124}{124}{1}{false}&&\cr
\l{1}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){4}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(7/4){3}{}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(3/2){10}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(3/2){10}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(1/2){10}{}&\rat(3/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(1/2){2}{\spec{1}}&\rat(3/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(1/2){2}{\spec{2}}&\rat(3/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(5/4){1}{}&\rat(7/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(5/4){1}{}&\rat(3/4){1}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(5/4){1}{}&\rat(3/4){1}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\rat(3/4){11}{}&\rat(9/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(3/4){11}{}&\rat(5/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(1/4){1}{}&\rat(7/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{22}&\rat(-1/4){11}{}&\rat(9/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 166
\orbit{3}{166}{124}
\h{166}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(8){\8}{\spec{3}}&&\cnt{959}&\bounds{124}{124}{1}{false}&&\cr
\l{1}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(1){4}{}&\int(0){\0}{}&\int(3){1}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(3/2){10}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(3/2){10}{}&\rat(-1/2){2}{}&\int(3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(1/2){10}{}&\rat(1/2){2}{}&\int(3){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\rat(3/4){11}{}&\rat(5/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(1/4){1}{}&\rat(7/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(1/4){1}{}&\rat(3/4){1}{}&\int(3){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{11}&\rat(-3/4){1}{}&\rat(7/4){1}{}&\int(3){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 167
\orbit{3}{167}{123}
\h{167}&\rat(83/12){7}{\spec{1}}&\rat(7/4){3}{}&\rat(10/3){1}{}&&\cnt{747}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(7/3){8}{\spec{1}}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(7/3){8}{\spec{2}}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(13/6){10}{}&\rat(1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{14}&\rat(11/6){2}{}&\rat(1/2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(19/12){11}{}&\rat(7/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(19/12){11}{}&\rat(3/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(17/12){1}{}&\rat(5/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{18}&\rat(7/12){11}{}&\rat(7/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 168
\orbit{3}{168}{123}
\h{168}&\rat(17/3){10}{\spec{1}}&\int(3){2}{}&\rat(10/3){1}{}&&\cnt{735}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(8/3){10}{}&\int(1){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(8/3){10}{}&\int(0){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(4/3){2}{}&\int(1){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(11/6){11}{}&\rat(3/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(11/6){11}{}&\rat(1/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{48}&\bounds{16}{16}{1}{false}&&\cr
\l{16}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(5/6){11}{}&\rat(3/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 169
\orbit{3}{169}{123}
\h{169}&\rat(9/4){9}{}&\rat(31/4){1}{\spec{1}}&\int(2){\2}{}&&\cnt{851}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\rat(9/4){9}{}&\rat(7/4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(9/4){9}{}&\rat(7/4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(3/4){3}{}&\rat(13/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(3/2){10}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(3/4){11}{}&\rat(13/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(3/4){11}{}&\rat(9/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(1/4){1}{}&\rat(11/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\rat(-1/4){11}{}&\rat(13/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 170
\orbit{3}{170}{123}
\h{170}&\rat(32/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&&\cnt{735}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){6}{\spec{2}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(10/3){4}{\spec{2}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{200}&\bounds{40}{40}{1}{false}&&\cr
\l{7}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(8/3){8}{\spec{3}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(8/3){2}{\spec{2}}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 171
\orbit{3}{171}{123}
\h{171}&\rat(83/12){11}{\spec{1}}&\rat(7/4){3}{}&\rat(10/3){2}{}&&\cnt{851}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(7/3){4}{\spec{1}}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(11/4){9}{\spec{1}}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(9/4){3}{\spec{1}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(13/6){2}{\spec{1}}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{280}&\bounds{35}{35}{1}{false}&&\cr
\l{10}&\rat(11/6){10}{\spec{1}}&\rat(1/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(25/12){1}{}&\rat(5/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(25/12){1}{}&\rat(1/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{13}&\rat(11/12){11}{\spec{1}}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 172
\orbit{3}{172}{123}
\h{172}&\rat(5/3){10}{}&\int(7){2}{\spec{2}}&\rat(10/3){1}{}&&\cnt{847}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(5/3){10}{}&\int(2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(2/3){10}{}&\int(2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(1/3){2}{}&\int(2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(5/6){11}{}&\rat(3/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{48}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(-1/6){11}{}&\rat(5/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 173
\orbit{3}{173}{123}
\h{173}&\int(2){\2}{}&\int(4){\4}{2}&\int(6){\6}{}&&\cnt{767}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){10}{}&\int(2){2}{}&\int(1){1}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(0){10}{\spec{1}}&\int(2){2}{}&\int(2){1}{}&\ln{2}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(0){10}{\spec{2}}&\int(2){2}{}&\int(2){1}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(1){11}{}&\int(1){3}{}&\int(2){2}{}&\ln{2}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 174
\orbit{3}{174}{123}
\h{174}&\rat(11/3){10}{\spec{2}}&\int(3){2}{}&\rat(16/3){1}{\spec{1}}&&\cnt{671}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\rat(4/3){8}{\spec{1}}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(4/3){8}{\spec{2}}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(4/3){2}{}&\int(0){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(1/3){2}{\spec{1}}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(1/3){2}{\spec{2}}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(5/6){11}{}&\rat(1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{72}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\rat(-1/6){11}{}&\rat(3/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 175
\orbit{3}{175}{123}
\h{175}&\rat(33/4){9}{\spec{4}}&\rat(15/4){1}{}&\int(0){\0}{}&&\cnt{1263}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{330}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(5/2){10}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{297}&\bounds{27}{27}{1}{false}&&\cr
\l{5}&\rat(11/4){11}{}&\rat(5/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 176
\orbit{3}{176}{123}
\h{176}&\rat(20/3){8}{\spec{1}}&\int(4){\4}{2}&\rat(4/3){2}{}&&\cnt{719}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){6}{\spec{1}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/3){10}{}&\int(2){2}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(5/3){2}{}&\int(2){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{12}&\rat(4/3){10}{\spec{1}}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(4/3){10}{\spec{2}}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(2/3){2}{\spec{1}}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(2/3){2}{\spec{2}}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{16}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 177
\orbit{3}{177}{122}
\h{177}&\rat(35/12){11}{\spec{2}}&\rat(7/4){3}{}&\rat(22/3){2}{}&&\cnt{907}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(4/3){4}{}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(11/6){10}{}&\rat(1/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(11/6){10}{}&\rat(-1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(7/6){2}{}&\rat(1/2){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{10}&\rat(5/6){10}{}&\rat(1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\rat(13/12){1}{}&\rat(5/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(13/12){1}{}&\rat(1/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{13}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(11/12){11}{}&\rat(3/4){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{15}&\rat(1/12){1}{}&\rat(5/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{16}&\rat(-1/12){11}{}&\rat(7/4){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 178
\orbit{3}{178}{122}
\h{178}&\rat(11/3){10}{\spec{1}}&\int(3){2}{}&\rat(16/3){1}{\spec{1}}&&\cnt{1167}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\rat(4/3){8}{}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{176}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{330}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\rat(1/3){2}{}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(11/6){11}{}&\rat(3/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(11/6){11}{}&\rat(-1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(-1/6){11}{}&\rat(3/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 179
\orbit{3}{179}{122}
\h{179}&\rat(25/4){9}{\spec{2}}&\rat(15/4){1}{}&\int(2){\2}{}&&\cnt{691}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(5/2){6}{\spec{1}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(5/2){6}{\spec{2}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(3){4}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(11/4){3}{}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(7/4){3}{\spec{1}}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(7/4){3}{\spec{2}}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(5/2){2}{}&\rat(3/2){2}{}&\int(0){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(5/2){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(3/2){10}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(5/4){1}{}&\rat(7/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(3/4){11}{}&\rat(9/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 180
\orbit{3}{180}{122}
\h{180}&\rat(14/3){8}{\spec{1}}&\int(0){\0}{}&\rat(22/3){2}{}&&\cnt{879}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(4/3){4}{}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(7/3){10}{}&\int(0){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(4/3){10}{\spec{1}}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(4/3){10}{\spec{2}}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{11}&\rat(5/3){11}{}&\int(0){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 181
\orbit{3}{181}{121}
\h{181}&\rat(17/4){9}{\spec{2}}&\rat(23/4){1}{}&\int(2){\2}{}&&\cnt{747}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(7/4){3}{}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(3/2){10}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(5/4){1}{}&\rat(11/4){1}{}&\int(0){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(5/4){1}{}&\rat(7/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(3/4){11}{}&\rat(9/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\rat(1/4){1}{}&\rat(11/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 182
\orbit{3}{182}{121}
\h{182}&\rat(35/12){7}{}&\rat(15/4){3}{}&\rat(16/3){1}{\spec{2}}&&\cnt{743}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(5/3){4}{}&\int(0){\0}{}&\rat(7/3){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(7/6){10}{}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(7/6){10}{}&\rat(1/2){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(5/6){2}{}&\rat(3/2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(1/6){10}{}&\rat(3/2){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(7/12){11}{}&\rat(7/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{150}&\bounds{25}{25}{1}{false}&&\cr
\l{11}&\rat(5/12){1}{}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\rat(5/12){1}{}&\rat(5/4){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(-7/12){1}{}&\rat(9/4){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 183
\orbit{3}{183}{121}
\h{183}&\rat(59/12){7}{\spec{2}}&\rat(7/4){3}{}&\rat(16/3){1}{\spec{2}}&&\cnt{743}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(5/3){4}{\spec{1}}&\int(0){\0}{}&\rat(7/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(5/3){4}{\spec{2}}&\int(0){\0}{}&\rat(7/3){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(11/6){2}{}&\rat(1/2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{175}&\bounds{25}{25}{1}{false}&&\cr
\l{11}&\rat(7/6){10}{}&\rat(1/2){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{12}&\rat(17/12){1}{}&\rat(5/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(17/12){1}{}&\rat(1/4){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{14}&\rat(7/12){11}{}&\rat(7/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(5/12){1}{}&\rat(5/4){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 184
\orbit{3}{184}{121}
\h{184}&\int(7){6}{\spec{2}}&\int(5){2}{\spec{2}}&\int(0){\0}{}&&\cnt{919}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(5/2){9}{\spec{1}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(5/2){9}{\spec{2}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(3/2){9}{\spec{2}}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{\spec{2}}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(3/2){11}{}&\rat(5/2){3}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 185
\orbit{3}{185}{121}
\h{185}&\rat(25/4){9}{\spec{1}}&\rat(23/4){1}{}&\int(0){\0}{}&&\cnt{907}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(13/4){9}{}&\rat(3/4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(13/4){9}{}&\rat(3/4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(7/4){3}{}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(5/4){9}{\spec{1}}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/4){9}{\spec{2}}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(5/4){9}{\spec{3}}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(1){\2}{\spec{3}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(5/2){10}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(7/4){11}{}&\rat(9/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{19}&\rat(5/4){1}{}&\rat(11/4){1}{}&\int(0){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 186
\orbit{3}{186}{121}
\h{186}&\int(2){\2}{}&\int(0){\0}{}&\int(10){\10}{}&&\cnt{971}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(1){8}{}&\int(0){\0}{}&\int(3){2}{}&\ln{2}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(1){10}{}&\int(0){2}{}&\int(3){1}{}&\ln{2}&\cnt{140}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\int(1){11}{}&\int(0){3}{}&\int(3){2}{}&\ln{2}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 187
\orbit{3}{187}{121}
\h{187}&\rat(83/12){11}{\spec{2}}&\rat(7/4){3}{}&\rat(10/3){2}{}&&\cnt{691}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(7/3){4}{\spec{1}}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(7/3){4}{\spec{2}}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(13/4){3}{}&\rat(3/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(13/6){2}{}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{13}&\rat(11/6){10}{}&\rat(1/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(13/12){1}{}&\rat(5/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 188
\orbit{3}{188}{120}
\h{188}&\rat(9/4){9}{}&\rat(15/4){1}{}&\int(6){\6}{}&&\cnt{795}&\bounds{120}{120}{1}{false}&&\cr
\l{1}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(3/2){10}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(3/2){10}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(1/2){10}{}&\rat(3/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(1/2){2}{}&\rat(3/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(3/4){11}{}&\rat(9/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(3/4){11}{}&\rat(5/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{10}&\rat(1/4){1}{}&\rat(7/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(-1/4){11}{}&\rat(9/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 189
\orbit{3}{189}{120}
\h{189}&\rat(11/12){11}{}&\rat(39/4){3}{\spec{1}}&\rat(4/3){2}{}&&\cnt{1131}&\bounds{120}{120}{1}{false}&&\cr
\l{1}&\rat(3/4){9}{}&\rat(13/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\rat(1/4){3}{}&\rat(15/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(11/12){11}{}&\rat(15/4){3}{}&\rat(-2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(11/12){11}{}&\rat(11/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(1/12){1}{}&\rat(13/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{330}&\bounds{30}{30}{1}{false}&&\cr
\l{8}&\rat(-1/12){11}{}&\rat(15/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{176}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(-1/12){11}{}&\rat(11/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 190
\orbit{3}{190}{119}
\h{190}&\int(4){\4}{}&\int(0){\0}{}&\int(8){\8}{\spec{1}}&&\cnt{759}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){10}{}&\int(0){2}{}&\int(2){1}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 191
\orbit{3}{191}{119}
\h{191}&\int(3){6}{}&\int(9){2}{\spec{2}}&\int(0){\0}{}&&\cnt{623}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 192
\orbit{3}{192}{119}
\h{192}&\int(8){\8}{\spec{2}}&\int(4){\4}{2}&\int(0){\0}{}&&\cnt{815}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){6}{\spec{4}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){6}{\spec{5}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\int(3){9}{\spec{2}}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{224}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(3){3}{\spec{2}}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){10}{\spec{2}}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{10}&\int(2){2}{\spec{2}}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\int(0){\0}{\spec{2}}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 193
\orbit{3}{193}{119}
\h{193}&\int(4){\4}{}&\int(8){\8}{0}&\int(0){\0}{}&&\cnt{759}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{2}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 194
\orbit{3}{194}{119}
\h{194}&\rat(25/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(4){\4}{}&&\cnt{687}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){4}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(2){4}{\spec{1}}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(2){4}{\spec{2}}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(11/4){3}{}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(5/2){2}{}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(5/2){2}{}&\rat(-1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(3/2){10}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(5/4){1}{}&\rat(7/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(5/4){1}{}&\rat(3/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{17}&\rat(3/4){11}{}&\rat(5/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{18}&\rat(1/4){1}{}&\rat(7/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 195
\orbit{3}{195}{119}
\h{195}&\rat(5/3){10}{}&\int(9){2}{\spec{3}}&\rat(4/3){1}{}&&\cnt{971}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(1/2){9}{}&\rat(7/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(1/2){3}{}&\rat(7/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(5/3){10}{}&\int(2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(2/3){10}{}&\int(2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(5/6){11}{}&\rat(7/2){3}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(1/6){1}{}&\rat(7/2){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\rat(-1/6){11}{}&\rat(7/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(-5/6){1}{}&\rat(7/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 196
\orbit{3}{196}{119}
\h{196}&\rat(8/3){8}{}&\int(4){\4}{2}&\rat(16/3){2}{\spec{1}}&&\cnt{719}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(4/3){10}{}&\int(2){2}{}&\rat(2/3){1}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(4/3){10}{}&\int(2){2}{}&\rat(2/3){1}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(2/3){2}{}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(1/3){10}{}&\int(2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(-1/3){2}{}&\int(2){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(2/3){11}{}&\int(1){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 197
\orbit{3}{197}{119}
\h{197}&\rat(14/3){8}{\spec{1}}&\int(6){\6}{\spec{1}}&\rat(4/3){2}{}&&\cnt{783}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(7/3){10}{}&\int(2){2}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(7/3){10}{}&\int(1){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(4/3){10}{\spec{1}}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(4/3){10}{\spec{2}}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(2/3){2}{}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(5/3){11}{}&\int(2){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 198
\orbit{3}{198}{119}
\h{198}&\rat(14/3){8}{\spec{2}}&\int(2){\2}{}&\rat(16/3){2}{\spec{2}}&&\cnt{671}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(4/3){4}{\spec{1}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(4/3){4}{\spec{2}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(5/3){2}{}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(4/3){10}{}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(1/3){10}{}&\int(1){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\int(0){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(1/3){1}{}&\int(1){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 199
\orbit{3}{199}{118}
\h{199}&\rat(107/12){7}{\spec{3}}&\rat(7/4){3}{}&\rat(4/3){1}{}&&\cnt{791}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\rat(13/3){8}{}&\int(0){\0}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\rat(15/4){9}{}&\rat(1/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{9}&\rat(11/4){9}{\spec{1}}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(11/4){9}{\spec{2}}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(19/6){10}{}&\rat(1/2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{15}&\rat(19/6){10}{}&\rat(-1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(13/6){10}{}&\rat(1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(19/12){11}{}&\rat(7/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(17/12){1}{}&\rat(5/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 200
\orbit{3}{200}{118}
\h{200}&\rat(41/4){9}{\spec{5}}&\rat(7/4){1}{}&\int(0){\0}{}&&\cnt{1015}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(13/4){9}{}&\rat(3/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\rat(9/4){9}{\spec{1}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(9/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(7/2){10}{}&\rat(1/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{10}&\rat(11/4){11}{}&\rat(5/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 201
\orbit{3}{201}{118}
\h{201}&\int(0){\0}{}&\int(8){\8}{0}&\int(4){\4}{}&&\cnt{1007}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(0){10}{}&\int(2){2}{}&\int(2){1}{}&\ln{2}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(0){11}{}&\int(2){3}{}&\int(2){2}{}&\ln{2}&\cnt{192}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 202
\orbit{3}{202}{117}
\h{202}&\int(7){6}{\spec{2}}&\int(3){2}{}&\int(2){\2}{}&&\cnt{679}&\bounds{117}{117}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(5/2){9}{\spec{1}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(5/2){9}{\spec{2}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\int(3){10}{}&\int(0){2}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(3/2){11}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\int(0){\0}{\spec{2}}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 203
\orbit{3}{203}{117}
\h{203}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(28/3){2}{\spec{2}}&&\cnt{735}&\bounds{117}{117}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(4/3){4}{}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(4/3){10}{}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 204
\orbit{3}{204}{117}
\h{204}&\rat(5/3){10}{}&\int(1){2}{}&\rat(28/3){1}{\spec{1}}&&\cnt{735}&\bounds{117}{117}{1}{false}&&\cr
\l{1}&\rat(4/3){8}{}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(5/3){10}{}&\int(0){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(2/3){10}{}&\int(1){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(1/3){2}{}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(5/6){11}{}&\rat(1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 205
\orbit{3}{205}{117}
\h{205}&\rat(9/4){9}{}&\rat(23/4){1}{}&\int(4){\4}{}&&\cnt{735}&\bounds{117}{117}{1}{false}&&\cr
\l{1}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(3/2){10}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(3/2){10}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(1/2){10}{}&\rat(3/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(1/2){2}{}&\rat(3/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(3/4){11}{}&\rat(9/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\rat(3/4){11}{}&\rat(5/4){3}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(3/4){11}{}&\rat(5/4){3}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(1/4){1}{}&\rat(11/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(1/4){1}{}&\rat(7/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(-1/4){11}{}&\rat(9/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{15}&\rat(-3/4){1}{}&\rat(11/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 206
\orbit{3}{206}{116}
\h{206}&\rat(59/12){11}{\spec{2}}&\rat(15/4){3}{}&\rat(10/3){2}{}&&\cnt{691}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(7/3){4}{}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(13/6){2}{}&\rat(3/2){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(13/6){2}{}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\rat(11/6){10}{}&\rat(3/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(11/6){10}{}&\rat(1/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(7/6){2}{}&\rat(3/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(5/6){10}{}&\rat(3/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\rat(13/12){1}{}&\rat(5/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{19}&\rat(1/12){1}{}&\rat(9/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 207
\orbit{3}{207}{116}
\h{207}&\rat(83/12){11}{\spec{1}}&\rat(15/4){3}{}&\rat(4/3){2}{}&&\cnt{791}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/2){6}{\spec{2}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(11/4){9}{\spec{2}}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(9/4){3}{\spec{2}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(7/4){9}{\spec{2}}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(7/4){9}{\spec{3}}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\rat(17/6){10}{}&\rat(3/2){2}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(17/6){10}{}&\rat(1/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(13/6){2}{\spec{2}}&\rat(3/2){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(13/6){2}{\spec{2}}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(11/6){10}{\spec{2}}&\rat(3/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\rat(7/6){2}{\spec{2}}&\rat(3/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\rat(23/12){11}{}&\rat(7/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{21}&\rat(23/12){11}{}&\rat(3/4){3}{\spec{1}}&\rat(4/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{22}&\rat(23/12){11}{}&\rat(3/4){3}{\spec{2}}&\rat(4/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{23}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{24}&\rat(11/12){11}{\spec{2}}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 208
\orbit{3}{208}{116}
\h{208}&\rat(35/12){11}{\spec{2}}&\rat(31/4){3}{\spec{2}}&\rat(4/3){2}{}&&\cnt{847}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(5/4){3}{}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\rat(3/4){9}{\spec{1}}&\rat(13/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(3/4){9}{\spec{2}}&\rat(13/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(11/6){10}{}&\rat(3/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(7/6){2}{}&\rat(3/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(13/12){1}{}&\rat(13/4){1}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(11/12){11}{}&\rat(11/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(11/12){11}{}&\rat(7/4){3}{\spec{1}}&\rat(4/3){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(11/12){11}{}&\rat(7/4){3}{\spec{2}}&\rat(4/3){2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(1/12){1}{}&\rat(13/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(-1/12){11}{}&\rat(11/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 209
\orbit{3}{209}{116}
\h{209}&\rat(14/3){8}{\spec{1}}&\int(2){\2}{}&\rat(16/3){2}{\spec{1}}&&\cnt{727}&\bounds{116}{116}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(7/3){10}{}&\int(1){2}{}&\rat(2/3){1}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(7/3){10}{}&\int(1){2}{}&\rat(2/3){1}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(7/3){10}{}&\int(0){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\rat(4/3){10}{\spec{1}}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(4/3){10}{\spec{2}}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(2/3){2}{}&\int(1){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{15}&\rat(5/3){11}{}&\int(0){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(2/3){11}{}&\int(1){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 210
\orbit{3}{210}{115}
\h{210}&\int(10){\10}{}&\int(0){\0}{}&\int(2){\2}{}&&\cnt{655}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(4){6}{\spec{1}}&\int(0){2}{}&\int(0){\0}{}&\ln{2}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{2}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 211
\orbit{3}{211}{115}
\h{211}&\rat(26/3){8}{\spec{2}}&\int(2){\2}{}&\rat(4/3){2}{}&&\cnt{671}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\int(4){6}{\spec{1}}&\int(0){2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(3){6}{\spec{1}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(13/3){4}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(10/3){4}{\spec{1}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(10/3){4}{\spec{2}}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\int(4){3}{}&\int(0){3}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(3){3}{\spec{1}}&\int(1){3}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(8/3){2}{\spec{1}}&\int(1){2}{}&\rat(1/3){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(8/3){2}{\spec{1}}&\int(0){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(5/3){2}{\spec{1}}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 212
\orbit{3}{212}{115}
\h{212}&\int(5){6}{\spec{1}}&\int(5){2}{\spec{2}}&\int(2){\2}{}&&\cnt{687}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(3/2){9}{\spec{1}}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(3/2){9}{\spec{2}}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(3/2){3}{}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(3/2){11}{}&\rat(5/2){3}{}&\int(0){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(3/2){11}{}&\rat(3/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(1/2){11}{}&\rat(5/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(1/2){1}{}&\rat(5/2){1}{}&\int(1){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 213
\orbit{3}{213}{115}
\h{213}&\rat(8/3){8}{}&\int(4){\4}{}&\rat(16/3){2}{\spec{2}}&&\cnt{671}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(4/3){4}{}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(4/3){10}{}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(1/3){10}{}&\int(1){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\rat(1/3){1}{}&\int(1){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(-2/3){1}{}&\int(2){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 214
\orbit{3}{214}{115}
\h{214}&\rat(11/3){10}{\spec{2}}&\int(5){2}{\spec{2}}&\rat(10/3){1}{}&&\cnt{687}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(4/3){2}{}&\int(1){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(7/6){1}{}&\rat(5/2){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(5/6){11}{}&\rat(3/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{14}&\rat(-1/6){11}{}&\rat(5/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 215
\orbit{3}{215}{115}
\h{215}&\rat(11/3){10}{\spec{2}}&\int(7){2}{\spec{3}}&\rat(4/3){1}{}&&\cnt{795}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\rat(1/2){9}{\spec{1}}&\rat(7/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(1/2){9}{\spec{2}}&\rat(7/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(7/6){1}{}&\rat(7/2){1}{}&\rat(-2/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{10}&\rat(1/6){1}{}&\rat(7/2){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\rat(-5/6){1}{}&\rat(7/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 216
\orbit{3}{216}{115}
\h{216}&\int(6){\6}{\spec{1}}&\int(4){\4}{}&\int(2){\2}{}&&\cnt{791}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(1){2}{}&\int(1){2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(2){11}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(2){11}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\int(1){1}{}&\int(2){1}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 217
\orbit{3}{217}{114}
\h{217}&\rat(11/12){11}{}&\rat(31/4){3}{\spec{1}}&\rat(10/3){2}{}&&\cnt{1003}&\bounds{114}{114}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(5/6){10}{}&\rat(5/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(1/6){2}{}&\rat(5/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{275}&\bounds{25}{25}{1}{false}&&\cr
\l{4}&\rat(-1/6){10}{}&\rat(5/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(11/12){11}{}&\rat(11/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(1/12){1}{}&\rat(9/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(-1/12){11}{}&\rat(11/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 218
\orbit{3}{218}{114}
\h{218}&\rat(11/3){10}{\spec{1}}&\int(1){2}{}&\rat(22/3){1}{}&&\cnt{871}&\bounds{114}{114}{1}{false}&&\cr
\l{1}&\rat(4/3){8}{}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(5/3){10}{}&\int(0){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{264}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(1/3){2}{}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(11/6){11}{}&\rat(1/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{8}&\rat(11/6){11}{}&\rat(-1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 219
\orbit{3}{219}{113}
\h{219}&\rat(35/12){11}{\spec{2}}&\rat(23/4){3}{}&\rat(10/3){2}{}&&\cnt{739}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(5/4){3}{}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(11/6){10}{}&\rat(3/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(11/6){10}{}&\rat(1/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(7/6){2}{}&\rat(3/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(5/6){10}{}&\rat(3/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(13/12){1}{}&\rat(5/4){1}{\spec{1}}&\rat(5/3){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(13/12){1}{}&\rat(5/4){1}{\spec{2}}&\rat(5/3){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(11/12){11}{}&\rat(11/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{16}&\rat(1/12){1}{}&\rat(9/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{17}&\rat(-1/12){11}{}&\rat(11/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 220
\orbit{3}{220}{113}
\h{220}&\rat(59/12){7}{\spec{1}}&\rat(7/4){3}{}&\rat(16/3){1}{\spec{1}}&&\cnt{795}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(4/3){8}{\spec{1}}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(4/3){8}{\spec{2}}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(13/6){10}{}&\rat(1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\rat(5/6){2}{}&\rat(1/2){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{8}&\rat(19/12){11}{}&\rat(7/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(19/12){11}{}&\rat(-1/4){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\rat(7/12){11}{}&\rat(3/4){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\rat(-5/12){11}{}&\rat(7/4){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 221
\orbit{3}{221}{113}
\h{221}&\rat(26/3){8}{\spec{3}}&\int(0){\0}{}&\rat(10/3){2}{}&&\cnt{767}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(7/3){4}{}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(4){9}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\rat(7/3){10}{}&\int(0){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 222
\orbit{3}{222}{113}
\h{222}&\rat(14/3){8}{\spec{2}}&\int(6){\6}{}&\rat(4/3){2}{}&&\cnt{679}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(1){9}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(1){3}{\spec{1}}&\int(3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(1){3}{\spec{2}}&\int(3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(5/3){2}{}&\int(1){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(4/3){1}{}&\int(3){1}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(4/3){1}{}&\int(2){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(2/3){11}{}&\int(3){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(1/3){1}{}&\int(3){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(-1/3){11}{}&\int(3){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 223
\orbit{3}{223}{113}
\h{223}&\rat(83/12){11}{\spec{1}}&\rat(7/4){3}{}&\rat(10/3){2}{}&&\cnt{795}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(7/3){4}{\spec{2}}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(11/4){9}{\spec{2}}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\rat(9/4){3}{\spec{2}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{2}}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{3}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(17/6){10}{}&\rat(1/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(17/6){10}{}&\rat(-1/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(13/6){2}{\spec{2}}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(11/6){10}{\spec{2}}&\rat(1/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{15}&\rat(23/12){11}{}&\rat(7/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(23/12){11}{}&\rat(3/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{17}&\rat(13/12){1}{}&\rat(5/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(11/12){11}{\spec{2}}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 224
\orbit{3}{224}{113}
\h{224}&\rat(25/4){9}{\spec{1}}&\rat(15/4){1}{}&\int(2){\2}{}&&\cnt{739}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(13/4){9}{}&\rat(3/4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(13/4){9}{}&\rat(3/4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(7/4){3}{}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(5/2){10}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(5/2){10}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\rat(3/2){10}{\spec{1}}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(3/2){10}{\spec{2}}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(3/2){2}{}&\rat(3/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{20}&\rat(7/4){11}{}&\rat(9/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{21}&\rat(7/4){11}{}&\rat(5/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{22}&\rat(5/4){1}{}&\rat(7/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\rat(3/4){11}{}&\rat(9/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 225
\orbit{3}{225}{113}
\h{225}&\int(2){\2}{}&\int(6){\6}{}&\int(4){\4}{}&&\cnt{795}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(1){9}{}&\int(3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){11}{}&\int(3){3}{}&\int(0){2}{\spec{1}}&\ln{2}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(1){11}{}&\int(3){3}{}&\int(0){2}{\spec{2}}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(1){11}{}&\int(2){3}{}&\int(1){2}{}&\ln{2}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(1){11}{}&\int(1){3}{}&\int(2){2}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(0){11}{}&\int(3){3}{}&\int(1){2}{}&\ln{2}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){11}{}&\int(2){3}{}&\int(2){2}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(-1){11}{}&\int(3){3}{}&\int(2){2}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 226
\orbit{3}{226}{113}
\h{226}&\rat(107/12){7}{\spec{2}}&\rat(7/4){3}{}&\rat(4/3){1}{}&&\cnt{795}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{\spec{1}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\rat(14/3){4}{}&\int(0){\0}{}&\rat(-2/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(11/3){4}{\spec{1}}&\int(0){\0}{}&\rat(1/3){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(8/3){4}{\spec{1}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(17/4){3}{}&\rat(-1/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\rat(13/4){3}{\spec{1}}&\rat(3/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(9/4){3}{\spec{1}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(17/6){2}{\spec{1}}&\rat(1/2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{10}&\rat(17/12){1}{\spec{1}}&\rat(5/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 227
\orbit{3}{227}{112}
\h{227}&\rat(59/12){11}{\spec{2}}&\rat(7/4){3}{}&\rat(16/3){2}{\spec{1}}&&\cnt{743}&\bounds{112}{112}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(7/3){4}{}&\int(0){\0}{}&\rat(5/3){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(5/3){8}{\spec{1}}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(5/3){8}{\spec{2}}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(13/6){2}{}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\rat(13/6){2}{}&\rat(-1/2){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(11/6){10}{}&\rat(1/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{14}&\rat(7/6){2}{}&\rat(1/2){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{15}&\rat(13/12){1}{}&\rat(5/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{16}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(11/12){11}{}&\rat(3/4){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{18}&\rat(-1/12){11}{}&\rat(7/4){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 228
\orbit{3}{228}{112}
\h{228}&\rat(17/4){9}{\spec{1}}&\rat(31/4){1}{\spec{2}}&\int(0){\0}{}&&\cnt{983}&\bounds{112}{112}{1}{false}&&\cr
\l{1}&\rat(3/2){6}{}&\rat(5/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(3/2){10}{}&\rat(5/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{270}&\bounds{27}{27}{1}{false}&&\cr
\l{8}&\rat(7/4){11}{}&\rat(9/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 229
\orbit{3}{229}{112}
\h{229}&\rat(59/12){7}{\spec{1}}&\rat(23/4){3}{}&\rat(4/3){1}{}&&\cnt{735}&\bounds{112}{112}{1}{false}&&\cr
\l{1}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(11/4){9}{}&\rat(5/4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(11/4){9}{}&\rat(5/4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(7/4){9}{\spec{1}}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(7/4){9}{\spec{2}}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(5/4){3}{}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(13/6){10}{}&\rat(3/2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(13/6){10}{}&\rat(1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(7/6){10}{\spec{1}}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(7/6){10}{\spec{2}}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(19/12){11}{}&\rat(11/4){3}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\rat(19/12){11}{}&\rat(7/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{17}&\rat(7/12){11}{}&\rat(11/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(5/12){1}{}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{20}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 230
\orbit{3}{230}{112}
\h{230}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{747}&\bounds{112}{112}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{2}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 231
\orbit{3}{231}{111}
\h{231}&\int(4){\4}{}&\int(6){\6}{}&\int(2){\2}{}&&\cnt{679}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(1){9}{\spec{1}}&\int(3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(1){9}{\spec{2}}&\int(3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(1){11}{}&\int(3){3}{}&\int(0){2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(1){11}{}&\int(2){3}{}&\int(1){2}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){11}{}&\int(3){3}{}&\int(1){2}{}&\ln{2}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 232
\orbit{3}{232}{111}
\h{232}&\int(10){\10}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&&\cnt{747}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{2}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(0){\0}{}&\int(1){\2}{}&\ln{2}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){10}{}&\int(0){2}{}&\int(1){1}{}&\ln{2}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 233
\orbit{3}{233}{111}
\h{233}&\int(0){\0}{}&\int(2){\2}{}&\int(10){\10}{}&&\cnt{971}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(0){10}{}&\int(1){2}{}&\int(3){1}{}&\ln{2}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(0){11}{}&\int(1){3}{}&\int(3){2}{}&\ln{2}&\cnt{192}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{2}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 234
\orbit{3}{234}{111}
\h{234}&\rat(5/3){10}{}&\int(5){2}{\spec{2}}&\rat(16/3){1}{\spec{1}}&&\cnt{919}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\rat(4/3){8}{}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(1/3){2}{}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{5}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(5/6){11}{}&\rat(1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(-1/6){11}{}&\rat(3/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 235
\orbit{3}{235}{111}
\h{235}&\rat(33/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(2){\2}{}&&\cnt{683}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(9/2){6}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/2){6}{\spec{1}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(4){4}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(3){8}{\spec{1}}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(3){4}{\spec{1}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(3){4}{\spec{2}}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(15/4){3}{}&\rat(1/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\rat(11/4){3}{\spec{1}}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(9/4){9}{\spec{1}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(5/2){2}{\spec{1}}&\rat(1/2){2}{}&\int(1){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{13}&\rat(5/4){1}{\spec{1}}&\rat(7/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{18}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 236
\orbit{3}{236}{111}
\h{236}&\rat(107/12){11}{\spec{2}}&\rat(7/4){3}{}&\rat(4/3){2}{}&&\cnt{679}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(9/2){6}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(7/2){6}{\spec{1}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(7/2){6}{\spec{2}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(13/3){4}{}&\int(0){\0}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(11/3){8}{}&\int(0){\0}{}&\rat(1/3){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(10/3){4}{}&\int(0){\0}{}&\rat(2/3){1}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(8/3){8}{\spec{1}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(13/4){3}{}&\rat(3/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(11/4){9}{\spec{1}}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(9/4){3}{\spec{1}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(13/6){2}{\spec{1}}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(11/12){11}{\spec{1}}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 237
\orbit{3}{237}{110}
\h{237}&\rat(83/12){7}{\spec{2}}&\rat(15/4){3}{}&\rat(4/3){1}{}&&\cnt{679}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(5/2){6}{\spec{1}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(11/3){4}{}&\int(0){\0}{}&\rat(1/3){1}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(8/3){4}{\spec{1}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(8/3){4}{\spec{2}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(13/4){3}{}&\rat(3/4){3}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(13/4){3}{}&\rat(3/4){3}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/4){3}{\spec{1}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(9/4){3}{\spec{2}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(7/4){9}{\spec{1}}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\rat(17/6){2}{}&\rat(3/2){2}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(17/6){2}{}&\rat(1/2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(11/6){2}{}&\rat(3/2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{16}&\rat(7/6){10}{\spec{1}}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(17/12){1}{}&\rat(9/4){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(17/12){1}{}&\rat(5/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{19}&\rat(5/12){1}{\spec{1}}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 238
\orbit{3}{238}{110}
\h{238}&\int(6){\6}{\spec{1}}&\int(4){\4}{2}&\int(2){\2}{}&&\cnt{767}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\int(2){2}{}&\int(0){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(1){10}{}&\int(2){2}{}&\int(1){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(1){2}{}&\int(2){2}{}&\int(1){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(2){11}{}&\int(1){3}{}&\int(1){2}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 239
\orbit{3}{239}{109}
\h{239}&\rat(35/12){11}{\spec{2}}&\rat(15/4){3}{}&\rat(16/3){2}{\spec{1}}&&\cnt{735}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(11/6){10}{}&\rat(3/2){2}{}&\rat(2/3){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(11/6){10}{}&\rat(3/2){2}{}&\rat(2/3){1}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(11/6){10}{}&\rat(1/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(7/6){2}{}&\rat(3/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(7/6){2}{}&\rat(1/2){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{12}&\rat(5/6){10}{}&\rat(3/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{13}&\rat(1/6){2}{\spec{1}}&\rat(3/2){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(1/6){2}{\spec{2}}&\rat(3/2){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(13/12){1}{}&\rat(5/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{18}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{19}&\rat(11/12){11}{}&\rat(3/4){3}{\spec{1}}&\rat(7/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{20}&\rat(11/12){11}{}&\rat(3/4){3}{\spec{2}}&\rat(7/3){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{21}&\rat(1/12){1}{}&\rat(9/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{22}&\rat(-1/12){11}{}&\rat(7/4){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{25}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{26}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 240
\orbit{3}{240}{109}
\h{240}&\rat(14/3){8}{\spec{1}}&\int(4){\4}{}&\rat(10/3){2}{}&&\cnt{679}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(7/3){10}{}&\int(1){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(7/3){10}{}&\int(0){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(4/3){10}{\spec{1}}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(4/3){10}{\spec{2}}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(5/3){11}{}&\int(2){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{12}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(1/3){1}{}&\int(2){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 241
\orbit{3}{241}{109}
\h{241}&\rat(17/4){9}{\spec{1}}&\rat(15/4){1}{}&\int(4){\4}{}&&\cnt{795}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(5/2){10}{}&\rat(3/2){2}{}&\int(0){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(5/2){10}{}&\rat(3/2){2}{}&\int(0){1}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/2){10}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(5/2){10}{}&\rat(-1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(3/2){10}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(3/2){10}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(1/2){10}{}&\rat(3/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(1/2){2}{}&\rat(3/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(7/4){11}{}&\rat(9/4){3}{}&\int(0){2}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(7/4){11}{}&\rat(9/4){3}{}&\int(0){2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(7/4){11}{}&\rat(5/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{16}&\rat(7/4){11}{}&\rat(1/4){3}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(7/4){11}{}&\rat(1/4){3}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{18}&\rat(3/4){11}{}&\rat(9/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\rat(3/4){11}{}&\rat(5/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{20}&\rat(1/4){1}{}&\rat(7/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{21}&\rat(-1/4){11}{}&\rat(9/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{22}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{23}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 242
\orbit{3}{242}{109}
\h{242}&\rat(59/12){11}{\spec{1}}&\rat(23/4){3}{}&\rat(4/3){2}{}&&\cnt{907}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{2}&\rat(5/4){3}{}&\rat(11/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(11/6){10}{}&\rat(3/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(7/6){2}{}&\rat(3/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(23/12){11}{}&\rat(11/4){3}{}&\rat(-2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\rat(23/12){11}{}&\rat(7/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(23/12){11}{}&\rat(3/4){3}{\spec{1}}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\rat(23/12){11}{}&\rat(3/4){3}{\spec{2}}&\rat(4/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(-1/12){11}{}&\rat(11/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 243
\orbit{3}{243}{108}
\h{243}&\rat(25/4){9}{\spec{1}}&\rat(7/4){1}{}&\int(4){\4}{}&&\cnt{735}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){8}{\spec{1}}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){8}{\spec{2}}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){4}{}&\int(0){\0}{}&\int(2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(13/4){9}{}&\rat(3/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(5/2){10}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{14}&\rat(5/2){10}{}&\rat(-1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(3/2){10}{\spec{1}}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(3/2){10}{\spec{2}}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{17}&\rat(3/2){2}{}&\rat(1/2){2}{}&\int(2){2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{18}&\rat(7/4){11}{}&\rat(5/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{19}&\rat(7/4){11}{}&\rat(1/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{20}&\rat(5/4){1}{}&\rat(7/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{21}&\rat(5/4){1}{}&\rat(3/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{22}&\rat(3/4){11}{}&\rat(5/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{23}&\rat(1/4){1}{}&\rat(7/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{24}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 244
\orbit{3}{244}{108}
\h{244}&\int(2){\2}{}&\int(10){\10}{\spec{1}}&\int(0){\0}{}&&\cnt{983}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\int(1){9}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(0){3}{\spec{1}}&\int(4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(0){3}{\spec{2}}&\int(4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){1}{}&\int(3){1}{}&\int(0){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(0){11}{}&\int(4){3}{}&\int(0){2}{}&\ln{1}&\cnt{270}&\bounds{27}{27}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 245
\orbit{3}{245}{108}
\h{245}&\rat(59/12){7}{\spec{1}}&\rat(15/4){3}{}&\rat(10/3){1}{}&&\cnt{683}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(7/4){9}{\spec{1}}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(7/4){9}{\spec{2}}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(13/6){10}{}&\rat(3/2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(13/6){10}{}&\rat(1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(7/6){10}{\spec{1}}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(7/6){10}{\spec{2}}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(5/6){2}{}&\rat(3/2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(19/12){11}{}&\rat(7/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(19/12){11}{}&\rat(3/4){3}{\spec{1}}&\rat(5/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{16}&\rat(19/12){11}{}&\rat(3/4){3}{\spec{2}}&\rat(5/3){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(7/12){11}{}&\rat(7/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{18}&\rat(5/12){1}{}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 246
\orbit{3}{246}{108}
\h{246}&\rat(5/3){10}{}&\int(7){2}{\spec{1}}&\rat(10/3){1}{}&&\cnt{919}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(1/2){3}{}&\rat(7/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{3}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(5/6){11}{}&\rat(7/2){3}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(5/6){11}{}&\rat(3/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{350}&\bounds{35}{35}{1}{false}&&\cr
\l{7}&\rat(-1/6){11}{}&\rat(7/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 247
\orbit{3}{247}{107}
\h{247}&\int(0){\0}{}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&&\cnt{879}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\int(0){10}{}&\int(2){2}{}&\int(2){1}{}&\ln{2}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(0){11}{}&\int(3){3}{}&\int(1){2}{}&\ln{2}&\cnt{192}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(0){11}{}&\int(2){3}{}&\int(2){2}{}&\ln{2}&\cnt{96}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 248
\orbit{3}{248}{107}
\h{248}&\int(2){\2}{}&\int(10){\10}{\spec{2}}&\int(0){\0}{}&&\cnt{859}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\int(1){9}{}&\int(3){1}{}&\int(0){\0}{}&\ln{2}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(1){11}{}&\int(3){3}{}&\int(0){2}{}&\ln{2}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 249
\orbit{3}{249}{107}
\h{249}&\rat(59/12){7}{\spec{1}}&\rat(7/4){3}{}&\rat(16/3){1}{\spec{2}}&&\cnt{735}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/3){8}{}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(5/3){4}{}&\int(0){\0}{}&\rat(7/3){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(13/6){10}{}&\rat(1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{10}&\rat(13/6){10}{}&\rat(-1/2){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(7/6){10}{\spec{1}}&\rat(1/2){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(7/6){10}{\spec{2}}&\rat(1/2){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{13}&\rat(19/12){11}{}&\rat(7/4){3}{}&\rat(2/3){2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(19/12){11}{}&\rat(7/4){3}{}&\rat(2/3){2}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(19/12){11}{}&\rat(3/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\rat(7/12){11}{}&\rat(7/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{17}&\rat(5/12){1}{}&\rat(5/4){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 250
\orbit{3}{250}{107}
\h{250}&\rat(35/12){7}{}&\rat(15/4){3}{}&\rat(16/3){1}{\spec{1}}&&\cnt{671}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(4/3){8}{}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(7/6){10}{}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(5/6){2}{}&\rat(1/2){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(-1/6){2}{}&\rat(3/2){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(7/12){11}{}&\rat(3/4){3}{\spec{1}}&\rat(8/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(7/12){11}{}&\rat(3/4){3}{\spec{2}}&\rat(8/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(5/12){1}{}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(-5/12){11}{}&\rat(7/4){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 251
\orbit{3}{251}{107}
\h{251}&\rat(11/3){10}{\spec{1}}&\int(5){2}{\spec{2}}&\rat(10/3){1}{}&&\cnt{919}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{275}&\bounds{25}{25}{1}{false}&&\cr
\l{5}&\rat(11/6){11}{}&\rat(5/2){3}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(11/6){11}{}&\rat(3/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(11/6){11}{}&\rat(1/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(-1/6){11}{}&\rat(5/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 252
\orbit{3}{252}{107}
\h{252}&\rat(59/12){7}{\spec{2}}&\rat(7/4){3}{}&\rat(16/3){1}{\spec{1}}&&\cnt{671}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(8/3){4}{}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\rat(4/3){8}{}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(11/6){2}{}&\rat(-1/2){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(5/6){2}{\spec{1}}&\rat(1/2){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(5/6){2}{\spec{2}}&\rat(1/2){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(17/12){1}{}&\rat(5/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(7/12){11}{}&\rat(3/4){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(-5/12){11}{}&\rat(7/4){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 253
\orbit{3}{253}{107}
\h{253}&\rat(11/12){11}{}&\rat(23/4){3}{}&\rat(16/3){2}{\spec{1}}&&\cnt{907}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/6){10}{}&\rat(3/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(1/6){2}{}&\rat(3/2){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(11/12){11}{}&\rat(11/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(11/12){11}{}&\rat(3/4){3}{\spec{1}}&\rat(7/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(11/12){11}{}&\rat(3/4){3}{\spec{2}}&\rat(7/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(1/12){1}{}&\rat(9/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{275}&\bounds{25}{25}{1}{false}&&\cr
\l{10}&\rat(-1/12){11}{}&\rat(11/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(-1/12){11}{}&\rat(7/4){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 254
\orbit{3}{254}{106}
\h{254}&\rat(8/3){8}{}&\int(6){\6}{}&\rat(10/3){2}{}&&\cnt{679}&\bounds{106}{106}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(1){9}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){3}{}&\int(3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(4/3){10}{}&\int(1){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(2/3){11}{}&\int(3){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(1/3){1}{}&\int(3){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(1/3){1}{}&\int(2){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(-1/3){11}{}&\int(3){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\rat(-2/3){1}{}&\int(3){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 255
\orbit{3}{255}{106}
\h{255}&\rat(59/12){11}{\spec{1}}&\rat(7/4){3}{}&\rat(16/3){2}{\spec{1}}&&\cnt{907}&\bounds{106}{106}{1}{false}&&\cr
\l{1}&\rat(5/3){8}{}&\int(0){\0}{}&\rat(7/3){2}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(11/6){10}{}&\rat(1/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{350}&\bounds{35}{35}{1}{false}&&\cr
\l{8}&\rat(7/6){2}{}&\rat(1/2){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{70}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\rat(23/12){11}{}&\rat(7/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(23/12){11}{}&\rat(3/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(23/12){11}{}&\rat(-1/4){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{12}&\rat(13/12){1}{}&\rat(5/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(-1/12){11}{}&\rat(7/4){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 256
\orbit{3}{256}{105}
\h{256}&\rat(5/3){10}{}&\int(5){2}{\spec{2}}&\rat(16/3){1}{\spec{2}}&&\cnt{727}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(0){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(2/3){10}{}&\int(1){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(5/6){11}{}&\rat(3/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(1/6){1}{}&\rat(3/2){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(-1/6){11}{}&\rat(5/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(-5/6){1}{}&\rat(5/2){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 257
\orbit{3}{257}{105}
\h{257}&\rat(14/3){8}{\spec{1}}&\int(6){\6}{}&\rat(4/3){2}{}&&\cnt{795}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(1){9}{\spec{1}}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(1){9}{\spec{2}}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){3}{}&\int(3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(7/3){10}{}&\int(1){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\rat(5/3){11}{}&\int(3){3}{}&\rat(-2/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(5/3){11}{}&\int(2){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(2/3){11}{}&\int(3){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(1/3){1}{}&\int(3){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(-1/3){11}{}&\int(3){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 258
\orbit{3}{258}{105}
\h{258}&\rat(59/12){11}{\spec{2}}&\rat(7/4){3}{}&\rat(16/3){2}{\spec{2}}&&\cnt{671}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(4/3){4}{\spec{1}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(4/3){4}{\spec{2}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(9/4){3}{}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(13/6){2}{}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(11/6){10}{}&\rat(-1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\rat(5/6){10}{}&\rat(1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{11}&\rat(13/12){1}{}&\rat(1/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{12}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\rat(1/12){1}{}&\rat(5/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 259
\orbit{3}{259}{105}
\h{259}&\rat(11/12){11}{}&\rat(15/4){3}{}&\rat(22/3){2}{}&&\cnt{891}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(5/6){10}{}&\rat(3/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(5/6){10}{}&\rat(1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(1/6){2}{}&\rat(3/2){2}{}&\rat(7/3){2}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(-1/6){10}{}&\rat(3/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(11/12){11}{}&\rat(3/4){3}{\spec{1}}&\rat(7/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(11/12){11}{}&\rat(3/4){3}{\spec{2}}&\rat(7/3){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(1/12){1}{}&\rat(9/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(1/12){1}{}&\rat(5/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(-1/12){11}{}&\rat(7/4){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(-11/12){1}{}&\rat(9/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 260
\orbit{3}{260}{105}
\h{260}&\rat(83/12){7}{\spec{2}}&\rat(7/4){3}{}&\rat(10/3){1}{}&&\cnt{683}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(7/2){6}{}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(11/3){4}{}&\int(0){\0}{}&\rat(1/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(8/3){4}{\spec{1}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(8/3){4}{\spec{2}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(7/3){8}{\spec{1}}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\rat(13/4){3}{}&\rat(3/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\rat(9/4){3}{\spec{1}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/4){3}{\spec{2}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(17/6){2}{}&\rat(1/2){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(17/6){2}{}&\rat(-1/2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(11/6){2}{}&\rat(1/2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\rat(17/12){1}{}&\rat(5/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(7/12){11}{\spec{1}}&\rat(7/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 261
\orbit{3}{261}{105}
\h{261}&\rat(35/12){11}{\spec{2}}&\rat(15/4){3}{}&\rat(16/3){2}{\spec{2}}&&\cnt{795}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(4/3){4}{}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(11/6){10}{}&\rat(3/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\rat(11/6){10}{}&\rat(-1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(7/6){2}{}&\rat(3/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(5/6){10}{}&\rat(1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(-1/6){10}{\spec{1}}&\rat(3/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(-1/6){10}{\spec{2}}&\rat(3/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(13/12){1}{}&\rat(1/4){1}{\spec{1}}&\rat(8/3){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\rat(13/12){1}{}&\rat(1/4){1}{\spec{2}}&\rat(8/3){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\rat(1/12){1}{}&\rat(5/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{16}&\rat(-11/12){1}{}&\rat(9/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{18}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 262
\orbit{3}{262}{104}
\h{262}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{883}&\bounds{104}{104}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{2}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){11}{}&\int(2){3}{}&\int(0){2}{}&\ln{2}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 263
\orbit{3}{263}{103}
\h{263}&\rat(11/12){11}{}&\rat(31/4){3}{\spec{2}}&\rat(10/3){2}{}&&\cnt{835}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\rat(3/4){9}{}&\rat(13/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(5/6){10}{}&\rat(3/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(11/12){11}{}&\rat(11/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(11/12){11}{}&\rat(7/4){3}{\spec{1}}&\rat(4/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(11/12){11}{}&\rat(7/4){3}{\spec{2}}&\rat(4/3){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(1/12){1}{}&\rat(13/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(1/12){1}{}&\rat(9/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(-1/12){11}{}&\rat(11/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(-11/12){1}{}&\rat(13/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 264
\orbit{3}{264}{103}
\h{264}&\int(0){\0}{}&\int(4){\4}{}&\int(8){\8}{\spec{3}}&&\cnt{935}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(0){10}{}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{264}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(0){11}{}&\int(2){3}{}&\int(2){2}{}&\ln{1}&\cnt{240}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(0){1}{}&\int(2){1}{}&\int(2){1}{}&\ln{1}&\cnt{48}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(0){1}{}&\int(1){1}{}&\int(3){1}{}&\ln{1}&\cnt{192}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 265
\orbit{3}{265}{103}
\h{265}&\rat(20/3){8}{\spec{1}}&\int(0){\0}{}&\rat(16/3){2}{\spec{2}}&&\cnt{703}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\rat(4/3){4}{\spec{1}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(4/3){4}{\spec{2}}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\rat(4/3){10}{\spec{1}}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(4/3){10}{\spec{2}}&\int(0){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{9}&\rat(4/3){1}{}&\int(0){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 266
\orbit{3}{266}{103}
\h{266}&\rat(83/12){7}{\spec{2}}&\rat(15/4){3}{}&\rat(4/3){1}{}&&\cnt{795}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(5/2){6}{\spec{2}}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(15/4){9}{}&\rat(1/4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(15/4){9}{}&\rat(1/4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\rat(7/4){9}{\spec{2}}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(19/6){10}{}&\rat(3/2){2}{}&\rat(-2/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\rat(19/6){10}{}&\rat(1/2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(19/6){10}{}&\rat(-1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(13/6){10}{}&\rat(3/2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(13/6){10}{}&\rat(1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(7/6){10}{\spec{2}}&\rat(3/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(19/12){11}{}&\rat(7/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{16}&\rat(5/12){1}{\spec{2}}&\rat(9/4){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 267
\orbit{3}{267}{103}
\h{267}&\int(3){6}{}&\int(7){2}{\spec{1}}&\int(2){\2}{}&&\cnt{671}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\rat(1/2){3}{}&\rat(7/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(1/2){11}{}&\rat(7/2){3}{}&\int(0){2}{}&\ln{1}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(1/2){1}{}&\rat(5/2){1}{}&\int(1){1}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{6}&\rat(-1/2){11}{}&\rat(7/2){3}{}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 268
\orbit{3}{268}{103}
\h{268}&\rat(9/4){9}{}&\rat(39/4){1}{\spec{1}}&\int(0){\0}{}&&\cnt{791}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\rat(3/2){6}{}&\rat(5/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(9/4){9}{}&\rat(7/4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(9/4){9}{}&\rat(7/4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(3/4){3}{}&\rat(13/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(3/2){10}{}&\rat(5/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\rat(3/4){11}{}&\rat(13/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 269
\orbit{3}{269}{102}
\h{269}&\rat(8/3){8}{}&\int(8){\8}{0}&\rat(4/3){2}{}&&\cnt{511}&\bounds{102}{102}{1}{false}&&\cr
\l{1}&\int(2){6}{}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(4/3){10}{}&\int(2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\rat(2/3){2}{}&\int(2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(2/3){11}{}&\int(2){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 270
\orbit{3}{270}{101}
\h{270}&\rat(17/3){10}{\spec{1}}&\int(5){2}{\spec{2}}&\rat(4/3){1}{}&&\cnt{727}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){9}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(3/2){9}{\spec{1}}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(3/2){9}{\spec{2}}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\rat(5/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(8/3){10}{}&\int(1){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(8/3){10}{}&\int(0){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\rat(11/6){11}{}&\rat(5/2){3}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(11/6){11}{}&\rat(3/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{15}&\rat(7/6){1}{}&\rat(5/2){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{16}&\rat(7/6){1}{}&\rat(3/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{18}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{19}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 271
\orbit{3}{271}{101}
\h{271}&\rat(29/3){10}{\spec{2}}&\int(1){2}{}&\rat(4/3){1}{}&&\cnt{623}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){6}{\spec{3}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(10/3){8}{\spec{2}}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(8/3){4}{\spec{3}}&\int(0){\0}{}&\rat(4/3){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(8/3){10}{}&\int(1){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\rat(8/3){10}{}&\int(0){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\rat(7/3){2}{\spec{2}}&\int(1){2}{}&\rat(2/3){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{15}&\rat(5/3){10}{\spec{2}}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(5/3){10}{\spec{3}}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{17}&\rat(13/6){1}{}&\rat(1/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 272
\orbit{3}{272}{100}
\h{272}&\rat(33/4){9}{\spec{3}}&\rat(7/4){1}{}&\int(2){\2}{}&&\cnt{779}&\bounds{100}{100}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(3){8}{}&\int(0){\0}{}&\int(1){2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\rat(13/4){9}{}&\rat(3/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(7/2){10}{}&\rat(1/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(7/2){10}{}&\rat(-1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(7/4){11}{}&\rat(5/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(5/4){1}{}&\rat(7/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 273
\orbit{3}{273}{100}
\h{273}&\rat(17/4){9}{\spec{1}}&\rat(7/4){1}{}&\int(6){\6}{}&&\cnt{779}&\bounds{100}{100}{1}{false}&&\cr
\l{1}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{90}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(5/2){10}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(5/2){10}{}&\rat(-1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(3/2){10}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{210}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(7/4){11}{}&\rat(5/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(7/4){11}{}&\rat(1/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{11}&\rat(3/4){11}{}&\rat(5/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(1/4){1}{}&\rat(7/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{30}&\bounds{3}{3}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 274
\orbit{3}{274}{99}
\h{274}&\rat(41/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(0){\0}{}&&\cnt{679}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(7/2){6}{\spec{2}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(13/4){9}{}&\rat(3/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\rat(11/4){3}{\spec{2}}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\rat(9/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/4){9}{\spec{3}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{13}&\rat(9/4){1}{}&\rat(7/4){1}{}&\int(0){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 275
\orbit{3}{275}{99}
\h{275}&\int(7){6}{\spec{2}}&\int(5){2}{\spec{1}}&\int(0){\0}{}&&\cnt{703}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(3){6}{\spec{2}}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){6}{\spec{2}}&\int(2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(7/2){9}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(5/2){9}{\spec{1}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(5/2){9}{\spec{2}}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{3}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{4}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(2){10}{}&\int(2){2}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{13}&\int(0){\0}{\spec{2}}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 276
\orbit{3}{276}{99}
\h{276}&\rat(41/4){9}{\spec{2}}&\rat(7/4){1}{}&\int(0){\0}{}&&\cnt{647}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\rat(9/2){6}{}&\rat(-1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(7/2){6}{\spec{1}}&\rat(1/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\int(4){4}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(15/4){3}{}&\rat(1/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{6}&\rat(11/4){3}{\spec{1}}&\rat(5/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(9/4){9}{\spec{1}}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 277
\orbit{3}{277}{99}
\h{277}&\rat(17/3){10}{\spec{1}}&\int(1){2}{}&\rat(16/3){1}{\spec{1}}&&\cnt{703}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(4/3){8}{\spec{1}}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(4/3){8}{\spec{2}}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(8/3){10}{}&\int(0){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\rat(4/3){2}{}&\int(0){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(1/3){2}{\spec{1}}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(1/3){2}{\spec{2}}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(11/6){11}{}&\rat(-1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(5/6){11}{}&\rat(1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 278
\orbit{3}{278}{99}
\h{278}&\int(0){\0}{}&\int(4){\4}{}&\int(8){\8}{\spec{1}}&&\cnt{883}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(0){11}{}&\int(2){3}{}&\int(2){2}{}&\ln{2}&\cnt{288}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 279
\orbit{3}{279}{98}
\h{279}&\rat(59/12){11}{\spec{1}}&\rat(15/4){3}{}&\rat(10/3){2}{}&&\cnt{723}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\rat(7/4){9}{}&\rat(9/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\rat(11/6){10}{}&\rat(3/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(11/6){10}{}&\rat(1/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(7/6){2}{}&\rat(3/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{50}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\rat(5/6){10}{}&\rat(3/2){2}{}&\rat(5/3){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(23/12){11}{}&\rat(7/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(23/12){11}{}&\rat(3/4){3}{\spec{1}}&\rat(4/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{13}&\rat(23/12){11}{}&\rat(3/4){3}{\spec{2}}&\rat(4/3){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(13/12){1}{}&\rat(9/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\rat(13/12){1}{}&\rat(5/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{16}&\rat(1/12){1}{}&\rat(9/4){1}{}&\rat(5/3){1}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 280
\orbit{3}{280}{98}
\h{280}&\int(0){\0}{}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&&\cnt{859}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(0){11}{}&\int(3){3}{}&\int(1){2}{}&\ln{2}&\cnt{288}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 281
\orbit{3}{281}{98}
\h{281}&\int(0){\0}{}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&&\cnt{983}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\int(0){3}{}&\int(4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(0){11}{}&\int(4){3}{}&\int(0){2}{}&\ln{1}&\cnt{180}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(0){1}{}&\int(3){1}{}&\int(1){1}{}&\ln{1}&\cnt{432}&\bounds{36}{36}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 282
\orbit{3}{282}{97}
\h{282}&\rat(17/4){9}{\spec{1}}&\rat(23/4){1}{}&\int(2){\2}{}&&\cnt{723}&\bounds{97}{97}{1}{false}&&\cr
\l{1}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(5/2){10}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(5/2){10}{}&\rat(1/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(3/2){10}{}&\rat(3/2){2}{}&\int(1){1}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/4){11}{}&\rat(9/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{11}&\rat(7/4){11}{}&\rat(5/4){3}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(7/4){11}{}&\rat(5/4){3}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(3/4){11}{}&\rat(9/4){3}{}&\int(1){2}{}&\ln{1}&\cnt{30}&\bounds{5}{5}{1}{false}&&\cr
\l{14}&\rat(1/4){1}{}&\rat(11/4){1}{}&\int(1){1}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{15}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 283
\orbit{3}{283}{97}
\h{283}&\rat(11/3){10}{\spec{1}}&\int(7){2}{\spec{2}}&\rat(4/3){1}{}&&\cnt{823}&\bounds{97}{97}{1}{false}&&\cr
\l{1}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{176}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(11/6){11}{}&\rat(5/2){3}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(11/6){11}{}&\rat(3/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 284
\orbit{3}{284}{95}
\h{284}&\rat(33/4){9}{\spec{3}}&\rat(15/4){1}{}&\int(0){\0}{}&&\cnt{759}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(5/2){6}{}&\rat(3/2){2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\rat(13/4){9}{}&\rat(3/4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(13/4){9}{}&\rat(3/4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(7/4){3}{}&\rat(9/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/2){10}{}&\rat(1/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(7/4){11}{}&\rat(9/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 285
\orbit{3}{285}{95}
\h{285}&\int(9){6}{\spec{4}}&\int(1){2}{}&\int(2){\2}{}&&\cnt{647}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){8}{}&\int(0){\0}{}&\int(0){2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(9/2){9}{}&\rat(-1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(3){10}{}&\int(1){2}{}&\int(0){1}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(3){10}{}&\int(0){2}{}&\int(1){1}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 286
\orbit{3}{286}{95}
\h{286}&\rat(11/3){10}{\spec{1}}&\int(5){2}{\spec{1}}&\rat(10/3){1}{}&&\cnt{703}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(5/3){10}{}&\int(2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(1/3){2}{}&\int(2){2}{}&\rat(5/3){2}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(11/6){11}{}&\rat(3/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\rat(11/6){11}{}&\rat(1/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 287
\orbit{3}{287}{94}
\h{287}&\rat(5/3){10}{}&\int(9){2}{\spec{2}}&\rat(4/3){1}{}&&\cnt{623}&\bounds{94}{94}{1}{false}&&\cr
\l{1}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(5/3){10}{}&\int(2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(2/3){10}{}&\int(2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 288
\orbit{3}{288}{93}
\h{288}&\rat(17/4){9}{\spec{1}}&\rat(31/4){1}{\spec{1}}&\int(0){\0}{}&&\cnt{815}&\bounds{93}{93}{1}{false}&&\cr
\l{1}&\rat(9/4){9}{}&\rat(7/4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(9/4){9}{}&\rat(7/4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(5/4){9}{}&\rat(11/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(3/4){3}{}&\rat(13/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/2){10}{}&\rat(3/2){2}{}&\int(0){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(7/4){11}{}&\rat(9/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\rat(3/4){11}{}&\rat(13/4){3}{}&\int(0){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 289
\orbit{3}{289}{93}
\h{289}&\rat(11/3){10}{\spec{1}}&\int(3){2}{}&\rat(16/3){1}{\spec{2}}&&\cnt{711}&\bounds{93}{93}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(5/3){10}{}&\int(0){2}{}&\rat(7/3){1}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(11/6){11}{}&\rat(3/2){3}{}&\rat(2/3){2}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(11/6){11}{}&\rat(3/2){3}{}&\rat(2/3){2}{\spec{2}}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(11/6){11}{}&\rat(1/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(1/6){1}{}&\rat(3/2){1}{}&\rat(7/3){1}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 290
\orbit{3}{290}{91}
\h{290}&\int(3){6}{}&\int(1){2}{}&\int(8){\8}{\spec{1}}&&\cnt{511}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(4){\2}{}&\ln{2}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{90}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 291
\orbit{3}{291}{91}
\h{291}&\int(0){\0}{}&\int(4){\4}{2}&\int(8){\8}{\spec{3}}&&\cnt{911}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(0){10}{}&\int(2){2}{}&\int(2){1}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(0){2}{}&\int(2){2}{}&\int(2){2}{}&\ln{1}&\cnt{330}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\int(0){1}{}&\int(1){1}{}&\int(3){1}{}&\ln{1}&\cnt{384}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 292
\orbit{3}{292}{91}
\h{292}&\int(6){\6}{\spec{1}}&\int(6){\6}{}&\int(0){\0}{}&&\cnt{783}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){9}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){9}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){3}{}&\int(3){3}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\int(2){11}{}&\int(2){3}{}&\int(0){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{10}&\int(1){1}{}&\int(3){1}{}&\int(0){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 293
\orbit{3}{293}{91}
\h{293}&\int(5){6}{\spec{1}}&\int(7){2}{\spec{1}}&\int(0){\0}{}&&\cnt{647}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(3){6}{}&\int(1){2}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(3/2){9}{\spec{1}}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(3/2){9}{\spec{2}}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\rat(1/2){3}{}&\rat(7/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{6}&\rat(1/2){11}{}&\rat(7/2){3}{}&\int(0){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 294
\orbit{3}{294}{91}
\h{294}&\int(2){\2}{}&\int(2){\2}{}&\int(8){\8}{\spec{1}}&&\cnt{635}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(1){10}{}&\int(1){2}{}&\int(2){1}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(1){11}{}&\int(1){3}{}&\int(2){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 295
\orbit{3}{295}{90}
\h{295}&\int(12){\12}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{639}&\bounds{90}{90}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{216}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 296
\orbit{3}{296}{90}
\h{296}&\int(2){\2}{}&\int(8){\8}{0}&\int(2){\2}{}&&\cnt{635}&\bounds{90}{90}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(1){10}{}&\int(2){2}{}&\int(1){1}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(1){11}{}&\int(2){3}{}&\int(1){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 297
\orbit{3}{297}{89}
\h{297}&\int(0){\0}{}&\int(6){\6}{}&\int(6){\6}{}&&\cnt{783}&\bounds{89}{89}{1}{false}&&\cr
\l{1}&\int(0){11}{}&\int(3){3}{}&\int(1){2}{}&\ln{2}&\cnt{72}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(0){11}{}&\int(2){3}{}&\int(2){2}{}&\ln{2}&\cnt{216}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{2}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 298
\orbit{3}{298}{89}
\h{298}&\rat(11/12){11}{}&\rat(39/4){3}{\spec{2}}&\rat(4/3){2}{}&&\cnt{791}&\bounds{89}{89}{1}{false}&&\cr
\l{1}&\rat(3/4){9}{}&\rat(13/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{110}&\bounds{11}{11}{1}{false}&&\cr
\l{4}&\rat(5/6){10}{}&\rat(5/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(1/6){2}{}&\rat(5/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(11/12){11}{}&\rat(11/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(11/12){11}{}&\rat(7/4){3}{\spec{1}}&\rat(4/3){2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\rat(11/12){11}{}&\rat(7/4){3}{\spec{2}}&\rat(4/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(1/12){1}{}&\rat(13/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(-1/12){11}{}&\rat(11/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 299
\orbit{3}{299}{88}
\h{299}&\rat(83/12){7}{\spec{2}}&\rat(7/4){3}{}&\rat(10/3){1}{}&&\cnt{667}&\bounds{88}{88}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(10/3){8}{}&\int(0){\0}{}&\rat(2/3){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(7/3){8}{\spec{2}}&\int(0){\0}{}&\rat(5/3){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(15/4){9}{}&\rat(1/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(11/4){9}{}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(19/6){10}{}&\rat(1/2){2}{}&\rat(1/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(19/6){10}{}&\rat(-1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\rat(13/6){10}{}&\rat(1/2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(19/12){11}{}&\rat(7/4){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(19/12){11}{}&\rat(3/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\rat(7/12){11}{\spec{2}}&\rat(7/4){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 300
\orbit{3}{300}{88}
\h{300}&\int(0){\0}{}&\int(12){\12}{2}&\int(0){\0}{}&&\cnt{687}&\bounds{88}{88}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{396}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{216}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 301
\orbit{3}{301}{88}
\h{301}&\rat(11/3){10}{\spec{2}}&\int(7){2}{\spec{1}}&\rat(4/3){1}{}&&\cnt{663}&\bounds{88}{88}{1}{false}&&\cr
\l{1}&\rat(3/2){9}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(1/2){3}{\spec{1}}&\rat(7/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(1/2){3}{\spec{2}}&\rat(7/2){3}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(7/6){1}{}&\rat(5/2){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\rat(5/6){11}{}&\rat(7/2){3}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(1/6){1}{}&\rat(5/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\rat(-1/6){11}{}&\rat(7/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 302
\orbit{3}{302}{87}
\h{302}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{635}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{2}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){10}{}&\int(1){2}{}&\int(1){1}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){11}{}&\int(1){3}{}&\int(1){2}{}&\ln{2}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 303
\orbit{3}{303}{87}
\h{303}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(28/3){2}{\spec{2}}&&\cnt{735}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{110}&\bounds{11}{11}{1}{false}&&\cr
\l{3}&\rat(5/6){10}{}&\rat(1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{154}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(11/12){11}{}&\rat(3/4){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(1/12){1}{}&\rat(5/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{154}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\rat(-1/12){11}{}&\rat(7/4){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 304
\orbit{3}{304}{87}
\h{304}&\rat(20/3){8}{\spec{2}}&\int(0){\0}{}&\rat(16/3){2}{\spec{1}}&&\cnt{687}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{3}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{\spec{1}}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{\spec{2}}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(5/3){11}{}&\int(0){3}{}&\rat(7/3){2}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{\spec{2}}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 305
\orbit{3}{305}{86}
\h{305}&\rat(59/12){11}{\spec{1}}&\rat(7/4){3}{}&\rat(16/3){2}{\spec{2}}&&\cnt{703}&\bounds{86}{86}{1}{false}&&\cr
\l{1}&\rat(4/3){4}{}&\int(0){\0}{}&\rat(8/3){1}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(11/6){10}{}&\rat(-1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{70}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(5/6){10}{}&\rat(1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(23/12){11}{}&\rat(3/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\rat(13/12){1}{}&\rat(1/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\rat(1/12){1}{}&\rat(5/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{70}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 306
\orbit{3}{306}{83}
\h{306}&\rat(20/3){8}{\spec{2}}&\int(4){\4}{}&\rat(4/3){2}{}&&\cnt{655}&\bounds{83}{83}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(3){9}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\rat(10/3){10}{}&\int(1){2}{}&\rat(-1/3){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(10/3){10}{}&\int(0){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(5/3){11}{}&\int(2){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(5/3){11}{}&\int(1){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 307
\orbit{3}{307}{83}
\h{307}&\rat(5/3){10}{}&\int(7){2}{\spec{3}}&\rat(10/3){1}{}&&\cnt{655}&\bounds{83}{83}{1}{false}&&\cr
\l{1}&\rat(1/2){9}{}&\rat(7/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(5/6){11}{}&\rat(5/2){3}{}&\rat(2/3){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(1/6){1}{}&\rat(7/2){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(-1/6){11}{}&\rat(5/2){3}{}&\rat(5/3){2}{}&\ln{1}&\cnt{140}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\rat(-5/6){1}{}&\rat(7/2){1}{}&\rat(4/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 308
\orbit{3}{308}{83}
\h{308}&\rat(11/12){11}{}&\rat(23/4){3}{}&\rat(16/3){2}{\spec{2}}&&\cnt{703}&\bounds{83}{83}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/6){10}{}&\rat(1/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(-1/6){10}{}&\rat(3/2){2}{}&\rat(8/3){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(11/12){11}{}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(1/12){1}{}&\rat(5/4){1}{\spec{1}}&\rat(8/3){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(1/12){1}{}&\rat(5/4){1}{\spec{2}}&\rat(8/3){1}{}&\ln{1}&\cnt{22}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(-1/12){11}{}&\rat(11/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\rat(-11/12){1}{}&\rat(9/4){1}{}&\rat(8/3){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 309
\orbit{3}{309}{83}
\h{309}&\rat(5/3){10}{}&\int(5){2}{\spec{1}}&\rat(16/3){1}{\spec{1}}&&\cnt{703}&\bounds{83}{83}{1}{false}&&\cr
\l{1}&\rat(4/3){8}{}&\int(0){\0}{}&\rat(8/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(2/3){10}{}&\int(2){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(1/3){2}{}&\int(1){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\rat(-2/3){2}{}&\int(2){2}{}&\rat(8/3){2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/6){11}{}&\rat(1/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(-1/6){11}{}&\rat(3/2){3}{}&\rat(8/3){2}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 310
\orbit{3}{310}{79}
\h{310}&\int(0){\0}{}&\int(0){\0}{}&\int(12){\12}{\spec{2}}&&\cnt{663}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{396}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 311
\orbit{3}{311}{78}
\h{311}&\int(0){\0}{}&\int(12){\12}{}&\int(0){\0}{}&&\cnt{651}&\bounds{78}{78}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{396}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{216}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 312
\orbit{3}{312}{77}
\h{312}&\rat(107/12){11}{\spec{2}}&\rat(7/4){3}{}&\rat(4/3){2}{}&&\cnt{567}&\bounds{77}{77}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\rat(8/3){8}{\spec{2}}&\int(0){\0}{}&\rat(4/3){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(11/4){9}{\spec{2}}&\rat(5/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(9/4){3}{\spec{2}}&\rat(7/4){3}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(17/6){10}{}&\rat(1/2){2}{}&\rat(2/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\rat(13/6){2}{\spec{2}}&\rat(1/2){2}{}&\rat(4/3){2}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\rat(25/12){1}{}&\rat(5/4){1}{}&\rat(2/3){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{12}&\rat(23/12){11}{}&\rat(7/4){3}{}&\rat(1/3){2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\rat(23/12){11}{}&\rat(3/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\rat(11/12){11}{\spec{2}}&\rat(7/4){3}{}&\rat(4/3){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 313
\orbit{3}{313}{74}
\h{313}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(8){\8}{\spec{1}}&&\cnt{511}&\bounds{74}{74}{1}{false}&&\cr
\l{1}&\int(2){8}{}&\int(0){\0}{}&\int(2){2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(9/4){9}{}&\rat(7/4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(3/2){10}{}&\rat(1/2){2}{}&\int(2){1}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(3/4){11}{}&\rat(5/4){3}{}&\int(2){2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\rat(1/4){1}{}&\rat(7/4){1}{}&\int(2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[11] + D[7] + E[6]
% Class 314
\orbit{3}{314}{65}
\h{314}&\rat(11/3){10}{\spec{1}}&\int(7){2}{\spec{3}}&\rat(4/3){1}{}&&\cnt{631}&\bounds{65}{65}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{231}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(5/3){10}{}&\int(1){2}{}&\rat(4/3){1}{}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(11/6){11}{}&\rat(5/2){3}{}&\rat(-1/3){2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\rat(1/6){1}{}&\rat(7/2){1}{}&\rat(1/3){1}{}&\ln{1}&\cnt{176}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_A15_D9.tex <==
% -*- TeX -*-
% Niemeier lattice A15_D9
% 101 classes
\newcs{max-A15_D9}{178}%
\newcs{count-A15_D9}{101}%
\newcs{counts-A15_D9}{\DO{1}{178}\DO{2}{163}\DO{3}{159}\DO{4}{155}\DO{5}{151}\DO{6}{147}\DO{7}{143}\DO{8}{139}\DO{9}{135}\DO{10}{135}\DO{11}{135}\DO{12}{131}\DO{13}{131}\DO{14}{127}\DO{15}{127}\DO{16}{127}\DO{17}{127}\DO{18}{126}\DO{19}{123}\DO{20}{123}\DO{21}{123}\DO{22}{123}\DO{23}{122}\DO{24}{121}\DO{25}{121}\DO{26}{119}\DO{27}{119}\DO{28}{119}\DO{29}{119}\DO{30}{118}\DO{31}{115}\DO{32}{115}\DO{33}{114}\DO{34}{113}\DO{35}{112}\DO{36}{111}\DO{37}{111}\DO{38}{111}\DO{39}{111}\DO{40}{110}\DO{41}{108}\DO{42}{107}\DO{43}{107}\DO{44}{106}\DO{45}{106}\DO{46}{105}\DO{47}{103}\DO{48}{103}\DO{49}{103}\DO{50}{102}\DO{51}{102}\DO{52}{101}\DO{53}{99}\DO{54}{99}\DO{55}{97}\DO{56}{96}\DO{57}{96}\DO{58}{95}\DO{59}{95}\DO{60}{95}\DO{61}{94}\DO{62}{94}\DO{63}{94}\DO{64}{93}\DO{65}{93}\DO{66}{92}\DO{67}{91}\DO{68}{91}\DO{69}{90}\DO{70}{90}\DO{71}{90}\DO{72}{89}\DO{73}{89}\DO{74}{87}\DO{75}{87}\DO{76}{87}\DO{77}{87}\DO{78}{87}\DO{79}{87}\DO{80}{86}\DO{81}{85}\DO{82}{85}\DO{83}{84}\DO{84}{84}\DO{85}{83}\DO{86}{81}\DO{87}{80}\DO{88}{79}\DO{89}{79}\DO{90}{79}\DO{91}{79}\DO{92}{75}\DO{93}{74}\DO{94}{74}\DO{95}{71}\DO{96}{71}\DO{97}{63}\DO{98}{62}\DO{99}{60}\DO{100}{58}\DO{101}{55}}%
\orbits
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 1
\orbit{2}{1}{178}
\h{1}&\int(12){\12}{\spec{4}}&\int(0){\0}{}&&\cnt{1459}&\bounds{178}{178}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{810}&\bounds{90}{90}{1}{false}&&\cr
\l{5}&\int(4){4}{}&\int(0){2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){14}{}&\int(0){3}{}&\ln{1}&\cnt{256}&\bounds{39}{39}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 2
\orbit{2}{2}{163}
\h{2}&\int(12){8}{\spec{6}}&\int(0){\0}{}&&\cnt{1755}&\bounds{163}{163}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{396}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{864}&\bounds{72}{72}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 3
\orbit{2}{3}{159}
\h{3}&\int(10){8}{\spec{5}}&\int(2){\2}{}&&\cnt{1215}&\bounds{159}{159}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{3}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{280}&\bounds{28}{28}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){14}{}&\int(1){3}{}&\ln{1}&\cnt{320}&\bounds{60}{60}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 4
\orbit{2}{4}{155}
\h{4}&\int(3){12}{}&\int(9){2}{\spec{2}}&&\cnt{1659}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(1){12}{}&\int(3){2}{}&\ln{1}&\cnt{396}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(1){4}{}&\int(3){2}{}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{768}&\bounds{64}{64}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 5
\orbit{2}{5}{151}
\h{5}&\int(11){12}{\spec{1}}&\int(1){2}{}&&\cnt{1039}&\bounds{151}{151}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\int(4){4}{}&\int(0){2}{}&\ln{1}&\cnt{336}&\bounds{42}{42}{1}{false}&&\cr
\l{6}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(3){4}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\int(3){4}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{10}&\rat(7/2){2}{}&\rat(1/2){1}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 6
\orbit{2}{6}{147}
\h{6}&\int(12){\12}{}&\int(0){\0}{}&&\cnt{1011}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{4}&\int(4){12}{}&\int(0){2}{}&\ln{2}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 7
\orbit{2}{7}{143}
\h{7}&\int(12){8}{\spec{4}}&\int(0){\0}{}&&\cnt{987}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(4){12}{}&\int(0){2}{}&\ln{2}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 8
\orbit{2}{8}{139}
\h{8}&\int(4){8}{}&\int(8){\8}{\spec{1}}&&\cnt{895}&\bounds{139}{139}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){12}{}&\int(2){2}{}&\ln{2}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(1){14}{}&\int(3){3}{}&\ln{2}&\cnt{224}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 9
\orbit{2}{9}{135}
\h{9}&\int(9){12}{\spec{1}}&\int(3){2}{}&&\cnt{999}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(3){4}{}&\int(1){2}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(5/2){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{288}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 10
\orbit{2}{10}{135}
\h{10}&\int(11){12}{\spec{5}}&\int(1){2}{}&&\cnt{1151}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{192}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(3){12}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{192}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\rat(7/2){14}{}&\rat(1/2){3}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 11
\orbit{2}{11}{135}
\h{11}&\int(8){\8}{}&\int(4){\4}{}&&\cnt{671}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){12}{}&\int(0){2}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){12}{}&\int(1){2}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(2){14}{}&\int(2){3}{}&\ln{2}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 12
\orbit{2}{12}{131}
\h{12}&\int(12){8}{\spec{8}}&\int(0){\0}{}&&\cnt{1231}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){12}{\spec{1}}&\int(0){2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){12}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{594}&\bounds{54}{54}{1}{false}&&\cr
\l{6}&\int(4){14}{}&\int(0){3}{}&\ln{1}&\cnt{256}&\bounds{39}{39}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 13
\orbit{2}{13}{131}
\h{13}&\rat(39/4){10}{\spec{1}}&\rat(9/4){1}{}&&\cnt{1115}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\rat(7/2){4}{}&\rat(1/2){2}{}&\ln{1}&\cnt{315}&\bounds{35}{35}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{288}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\rat(11/4){2}{}&\rat(5/4){1}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\l{6}&\rat(7/4){2}{}&\rat(9/4){1}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 14
\orbit{2}{14}{127}
\h{14}&\int(12){\12}{\spec{3}}&\int(0){\0}{}&&\cnt{911}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(4){12}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{378}&\bounds{42}{42}{1}{false}&&\cr
\l{7}&\int(4){4}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 15
\orbit{2}{15}{127}
\h{15}&\int(8){8}{\spec{2}}&\int(4){\4}{2}&&\cnt{1011}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){12}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){12}{\spec{3}}&\int(2){2}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){12}{\spec{4}}&\int(2){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(2){4}{\spec{4}}&\int(2){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{320}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\int(3){14}{}&\int(1){3}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(0){\0}{\spec{2}}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 16
\orbit{2}{16}{127}
\h{16}&\rat(39/4){10}{\spec{5}}&\rat(9/4){1}{}&&\cnt{1323}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\rat(9/2){12}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/2){12}{}&\rat(1/2){2}{}&\ln{1}&\cnt{324}&\bounds{27}{27}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{432}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\rat(13/4){14}{}&\rat(3/4){3}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{6}&\rat(9/4){14}{}&\rat(7/4){3}{}&\ln{1}&\cnt{108}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 17
\orbit{2}{17}{127}
\h{17}&\int(11){12}{\spec{4}}&\int(1){2}{}&&\cnt{987}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{7}&\int(5){12}{}&\int(-1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{320}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\int(3){12}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\int(3){12}{\spec{3}}&\int(1){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(3){4}{}&\int(1){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{13}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{14}&\rat(7/2){14}{}&\rat(1/2){3}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 18
\orbit{2}{18}{126}
\h{18}&\rat(15/4){10}{}&\rat(33/4){1}{\spec{2}}&&\cnt{1111}&\bounds{126}{126}{1}{false}&&\cr
\l{1}&\rat(3/2){12}{}&\rat(5/2){2}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\rat(3/2){4}{}&\rat(5/2){2}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{480}&\bounds{48}{48}{1}{false}&&\cr
\l{4}&\rat(5/4){14}{}&\rat(11/4){3}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(3/4){2}{}&\rat(13/4){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 19
\orbit{2}{19}{123}
\h{19}&\int(11){12}{\spec{3}}&\int(1){2}{}&&\cnt{815}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(4){4}{}&\int(0){2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\int(3){12}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(3){4}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(3){4}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 20
\orbit{2}{20}{123}
\h{20}&\int(6){\6}{}&\int(6){\6}{\spec{1}}&&\cnt{767}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){12}{}&\int(1){2}{}&\ln{2}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){12}{\spec{1}}&\int(2){2}{}&\ln{2}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(2){12}{\spec{2}}&\int(2){2}{}&\ln{2}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{108}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){14}{}&\int(2){3}{}&\ln{2}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 21
\orbit{2}{21}{123}
\h{21}&\int(9){12}{\spec{2}}&\int(3){2}{}&&\cnt{775}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){12}{\spec{3}}&\int(1){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(3){4}{\spec{3}}&\int(1){2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\rat(5/2){14}{}&\rat(3/2){3}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{13}&\rat(5/2){2}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 22
\orbit{2}{22}{123}
\h{22}&\int(8){8}{\spec{1}}&\int(4){\4}{}&&\cnt{727}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(3){12}{}&\int(1){2}{}&\ln{2}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{2}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){14}{}&\int(2){3}{}&\ln{2}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 23
\orbit{2}{23}{122}
\h{23}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&&\cnt{879}&\bounds{122}{122}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(4){12}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\int(4){4}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(3){12}{\spec{3}}&\int(1){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){4}{\spec{3}}&\int(1){2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(3){14}{}&\int(1){3}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 24
\orbit{2}{24}{121}
\h{24}&\int(9){12}{\spec{4}}&\int(3){2}{}&&\cnt{1415}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{273}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{504}&\bounds{36}{36}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(7/2){14}{}&\rat(1/2){3}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\rat(5/2){14}{}&\rat(3/2){3}{}&\ln{1}&\cnt{448}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 25
\orbit{2}{25}{121}
\h{25}&\int(9){12}{\spec{2}}&\int(3){2}{}&&\cnt{663}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(4){4}{}&\int(0){2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){12}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{6}&\int(3){4}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(3){4}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(5/2){2}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 26
\orbit{2}{26}{119}
\h{26}&\int(8){\8}{}&\int(4){\4}{2}&&\cnt{763}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){12}{}&\int(0){2}{}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){12}{\spec{1}}&\int(2){2}{}&\ln{2}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(2){12}{\spec{3}}&\int(2){2}{}&\ln{2}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 27
\orbit{2}{27}{119}
\h{27}&\int(12){8}{\spec{7}}&\int(0){\0}{}&&\cnt{927}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{360}&\bounds{40}{40}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 28
\orbit{2}{28}{119}
\h{28}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&&\cnt{951}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{42}{42}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{2}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{7}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(4){12}{\spec{2}}&\int(0){2}{}&\ln{2}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 29
\orbit{2}{29}{119}
\h{29}&\int(8){\8}{\spec{1}}&\int(4){\4}{2}&&\cnt{1471}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(2){12}{}&\int(2){2}{}&\ln{2}&\cnt{364}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{2}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 30
\orbit{2}{30}{118}
\h{30}&\rat(15/4){10}{}&\rat(33/4){1}{\spec{1}}&&\cnt{831}&\bounds{118}{118}{1}{false}&&\cr
\l{1}&\rat(5/2){12}{}&\rat(3/2){2}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{180}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\rat(5/4){14}{}&\rat(11/4){3}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{4}&\rat(3/4){2}{}&\rat(13/4){1}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\rat(1/4){14}{}&\rat(15/4){3}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 31
\orbit{2}{31}{115}
\h{31}&\int(11){12}{\spec{2}}&\int(1){2}{}&&\cnt{763}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(5){4}{}&\int(-1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){4}{}&\int(0){2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(3){12}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\int(3){4}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){4}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 32
\orbit{2}{32}{115}
\h{32}&\int(10){\10}{}&\int(2){\2}{}&&\cnt{655}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(4){12}{}&\int(0){2}{}&\ln{2}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(3){12}{}&\int(1){2}{}&\ln{2}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 33
\orbit{2}{33}{114}
\h{33}&\int(0){\0}{}&\int(12){\12}{\spec{2}}&&\cnt{1299}&\bounds{114}{114}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{240}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(0){14}{}&\int(4){3}{}&\ln{2}&\cnt{480}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{72}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{5}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 34
\orbit{2}{34}{113}
\h{34}&\int(10){8}{\spec{3}}&\int(2){\2}{}&&\cnt{767}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(3){12}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(3){4}{}&\int(1){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(3){14}{}&\int(1){3}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 35
\orbit{2}{35}{112}
\h{35}&\int(5){12}{\spec{2}}&\int(7){2}{\spec{1}}&&\cnt{831}&\bounds{112}{112}{1}{false}&&\cr
\l{1}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){12}{}&\int(2){2}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(2){2}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{30}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{150}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(3/2){14}{}&\rat(5/2){3}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 36
\orbit{2}{36}{111}
\h{36}&\int(8){\8}{\spec{2}}&\int(4){\4}{}&&\cnt{823}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(3){4}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(3){14}{}&\int(1){3}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){14}{\spec{2}}&\int(2){3}{}&\ln{1}&\cnt{176}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){2}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 37
\orbit{2}{37}{111}
\h{37}&\int(2){\2}{}&\int(10){\10}{}&&\cnt{1387}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(1){12}{}&\int(3){2}{}&\ln{2}&\cnt{364}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{196}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 38
\orbit{2}{38}{111}
\h{38}&\rat(39/4){14}{\spec{1}}&\rat(9/4){3}{}&&\cnt{943}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(7/2){12}{}&\rat(1/2){2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(7/2){4}{}&\rat(1/2){2}{}&\ln{1}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(13/4){2}{}&\rat(3/4){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(9/4){2}{}&\rat(7/4){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(7/4){14}{}&\rat(9/4){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 39
\orbit{2}{39}{111}
\h{39}&\int(7){12}{\spec{2}}&\int(5){2}{\spec{2}}&&\cnt{671}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){12}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{75}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(3){4}{}&\int(1){2}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(5/2){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(3/2){14}{\spec{1}}&\rat(5/2){3}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){\0}{\spec{1}}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 40
\orbit{2}{40}{110}
\h{40}&\int(6){8}{\spec{1}}&\int(6){\6}{\spec{1}}&&\cnt{767}&\bounds{110}{110}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(2){12}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){12}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(2){4}{}&\int(2){2}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){14}{}&\int(2){3}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 41
\orbit{2}{41}{108}
\h{41}&\int(7){12}{\spec{1}}&\int(5){2}{\spec{1}}&&\cnt{875}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){12}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){12}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(2){12}{\spec{3}}&\int(2){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){4}{}&\int(2){2}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{154}&\bounds{14}{14}{1}{false}&&\cr
\l{12}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(1){\2}{\spec{3}}&\int(3){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(5/2){14}{}&\rat(3/2){3}{}&\ln{1}&\cnt{192}&\bounds{36}{36}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 42
\orbit{2}{42}{107}
\h{42}&\int(8){8}{\spec{2}}&\int(4){\4}{}&&\cnt{655}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){12}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(3){14}{}&\int(1){3}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){14}{}&\int(2){3}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{9}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 43
\orbit{2}{43}{107}
\h{43}&\int(4){\4}{}&\int(8){\8}{\spec{1}}&&\cnt{879}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){12}{}&\int(2){2}{}&\ln{2}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{96}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){14}{}&\int(2){3}{}&\ln{2}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(1){14}{}&\int(3){3}{}&\ln{2}&\cnt{192}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{48}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 44
\orbit{2}{44}{106}
\h{44}&\int(3){12}{}&\int(9){2}{\spec{1}}&&\cnt{1011}&\bounds{106}{106}{1}{false}&&\cr
\l{1}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(3/2){14}{}&\rat(5/2){3}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\rat(1/2){2}{}&\rat(7/2){1}{}&\ln{1}&\cnt{594}&\bounds{54}{54}{1}{false}&&\cr
\l{4}&\rat(-1/2){14}{}&\rat(9/2){3}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 45
\orbit{2}{45}{106}
\h{45}&\int(10){8}{\spec{4}}&\int(2){\2}{}&&\cnt{887}&\bounds{106}{106}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(5){12}{}&\int(-1){2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){12}{\spec{1}}&\int(0){2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){12}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{154}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(3){14}{}&\int(1){3}{}&\ln{1}&\cnt{192}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 46
\orbit{2}{46}{105}
\h{46}&\rat(15/4){14}{\spec{2}}&\rat(33/4){3}{\spec{1}}&&\cnt{1099}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(3/2){12}{\spec{1}}&\rat(5/2){2}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\rat(3/2){12}{\spec{2}}&\rat(5/2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(3/2){4}{}&\rat(5/2){2}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{96}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{288}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\rat(7/4){14}{}&\rat(9/4){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\rat(5/4){2}{}&\rat(11/4){1}{}&\ln{1}&\cnt{96}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(3/4){14}{}&\rat(13/4){3}{}&\ln{1}&\cnt{36}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 47
\orbit{2}{47}{103}
\h{47}&\int(3){12}{}&\int(9){2}{\spec{4}}&&\cnt{935}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){12}{}&\int(2){2}{}&\ln{1}&\cnt{48}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{240}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(3/2){14}{}&\rat(5/2){3}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\rat(1/2){14}{}&\rat(7/2){3}{}&\ln{1}&\cnt{192}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\rat(1/2){2}{}&\rat(7/2){1}{}&\ln{1}&\cnt{264}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 48
\orbit{2}{48}{103}
\h{48}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&&\cnt{1111}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){12}{}&\int(2){2}{}&\ln{1}&\cnt{286}&\bounds{26}{26}{1}{false}&&\cr
\l{3}&\int(2){4}{}&\int(2){2}{}&\ln{1}&\cnt{78}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{156}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{52}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){14}{}&\int(2){3}{}&\ln{1}&\cnt{416}&\bounds{32}{32}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(2){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 49
\orbit{2}{49}{103}
\h{49}&\rat(23/4){10}{\spec{2}}&\rat(25/4){1}{}&&\cnt{723}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){12}{}&\rat(3/2){2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\rat(5/2){4}{}&\rat(3/2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\rat(7/4){2}{}&\rat(9/4){1}{}&\ln{1}&\cnt{168}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\rat(5/4){14}{}&\rat(11/4){3}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{9}&\rat(3/4){2}{\spec{1}}&\rat(13/4){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(3/4){2}{\spec{2}}&\rat(13/4){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 50
\orbit{2}{50}{102}
\h{50}&\rat(39/4){14}{\spec{4}}&\rat(9/4){3}{}&&\cnt{987}&\bounds{102}{102}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(7/2){12}{}&\rat(1/2){2}{}&\ln{1}&\cnt{594}&\bounds{54}{54}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(15/4){14}{}&\rat(1/4){3}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{6}&\rat(9/4){2}{}&\rat(7/4){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(7/4){14}{}&\rat(9/4){3}{}&\ln{1}&\cnt{24}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 51
\orbit{2}{51}{102}
\h{51}&\rat(39/4){14}{\spec{3}}&\rat(9/4){3}{}&&\cnt{831}&\bounds{102}{102}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(9/2){12}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(7/2){12}{}&\rat(1/2){2}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\rat(7/2){4}{}&\rat(1/2){2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\rat(11/4){14}{}&\rat(5/4){3}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(9/4){2}{}&\rat(7/4){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(7/4){14}{\spec{1}}&\rat(9/4){3}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\rat(7/4){14}{\spec{2}}&\rat(9/4){3}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 52
\orbit{2}{52}{101}
\h{52}&\int(7){12}{\spec{2}}&\int(5){2}{\spec{1}}&&\cnt{703}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){12}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(3){4}{}&\int(1){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){12}{}&\int(2){2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(2){4}{\spec{1}}&\int(2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(2){4}{\spec{2}}&\int(2){2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(5/2){2}{}&\rat(3/2){1}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(0){\0}{\spec{1}}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 53
\orbit{2}{53}{99}
\h{53}&\int(9){12}{\spec{3}}&\int(3){2}{}&&\cnt{743}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{144}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){12}{\spec{1}}&\int(1){2}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{72}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(7/2){14}{}&\rat(1/2){3}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{11}&\rat(5/2){14}{}&\rat(3/2){3}{}&\ln{1}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 54
\orbit{2}{54}{99}
\h{54}&\int(8){8}{\spec{1}}&\int(4){\4}{2}&&\cnt{687}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){12}{\spec{1}}&\int(2){2}{}&\ln{2}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(2){12}{\spec{2}}&\int(2){2}{}&\ln{2}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{2}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 55
\orbit{2}{55}{97}
\h{55}&\int(12){8}{\spec{5}}&\int(0){\0}{}&&\cnt{783}&\bounds{97}{97}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(4){12}{\spec{1}}&\int(0){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{7}&\int(4){12}{\spec{2}}&\int(0){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 56
\orbit{2}{56}{96}
\h{56}&\rat(39/4){14}{\spec{5}}&\rat(9/4){3}{}&&\cnt{1263}&\bounds{96}{96}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{504}&\bounds{36}{36}{1}{false}&&\cr
\l{4}&\rat(11/4){14}{}&\rat(5/4){3}{}&\ln{1}&\cnt{504}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\rat(7/4){14}{}&\rat(9/4){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 57
\orbit{2}{57}{96}
\h{57}&\rat(39/4){10}{\spec{2}}&\rat(9/4){1}{}&&\cnt{779}&\bounds{96}{96}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(7/2){12}{}&\rat(1/2){2}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(7/2){4}{\spec{3}}&\rat(1/2){2}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(11/4){2}{\spec{2}}&\rat(5/4){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{10}&\rat(9/4){14}{}&\rat(7/4){3}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(7/4){2}{\spec{2}}&\rat(9/4){1}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 58
\orbit{2}{58}{95}
\h{58}&\int(7){12}{\spec{2}}&\int(5){2}{\spec{2}}&&\cnt{1135}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{455}&\bounds{35}{35}{1}{false}&&\cr
\l{3}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{280}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(7/2){14}{}&\rat(1/2){3}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\rat(3/2){14}{\spec{2}}&\rat(5/2){3}{}&\ln{1}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 59
\orbit{2}{59}{95}
\h{59}&\int(6){8}{\spec{1}}&\int(6){\6}{}&&\cnt{663}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(2){14}{}&\int(2){3}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(1){14}{\spec{1}}&\int(3){3}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(1){14}{\spec{2}}&\int(3){3}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 60
\orbit{2}{60}{95}
\h{60}&\rat(7/4){14}{}&\rat(41/4){3}{\spec{1}}&&\cnt{1099}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{168}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(7/4){14}{}&\rat(9/4){3}{\spec{1}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/4){14}{}&\rat(9/4){3}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(3/4){14}{}&\rat(13/4){3}{}&\ln{1}&\cnt{280}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(1/4){2}{}&\rat(15/4){1}{}&\ln{1}&\cnt{455}&\bounds{35}{35}{1}{false}&&\cr
\l{6}&\rat(-1/4){14}{}&\rat(17/4){3}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 61
\orbit{2}{61}{94}
\h{61}&\int(3){12}{}&\int(9){2}{\spec{3}}&&\cnt{591}&\bounds{94}{94}{1}{false}&&\cr
\l{1}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){12}{}&\int(2){2}{}&\ln{1}&\cnt{96}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{96}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\rat(3/2){14}{}&\rat(5/2){3}{}&\ln{1}&\cnt{192}&\bounds{48}{48}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 62
\orbit{2}{62}{94}
\h{62}&\rat(31/4){10}{\spec{2}}&\rat(17/4){1}{}&&\cnt{663}&\bounds{94}{94}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(7/2){4}{}&\rat(1/2){2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\rat(5/2){12}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\rat(5/2){4}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(5/2){4}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\rat(11/4){2}{}&\rat(5/4){1}{\spec{1}}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(11/4){2}{}&\rat(5/4){1}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(7/4){2}{}&\rat(9/4){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(5/4){14}{\spec{1}}&\rat(11/4){3}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 63
\orbit{2}{63}{94}
\h{63}&\int(4){\4}{}&\int(8){\8}{0}&&\cnt{727}&\bounds{94}{94}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){12}{}&\int(2){2}{}&\ln{2}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){14}{}&\int(2){3}{}&\ln{2}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 64
\orbit{2}{64}{93}
\h{64}&\int(6){\6}{}&\int(6){\6}{}&&\cnt{663}&\bounds{93}{93}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){12}{}&\int(1){2}{}&\ln{2}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{4}&\int(2){14}{}&\int(2){3}{}&\ln{2}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(1){14}{}&\int(3){3}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 65
\orbit{2}{65}{93}
\h{65}&\int(7){12}{\spec{1}}&\int(5){2}{\spec{2}}&&\cnt{711}&\bounds{93}{93}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\rat(5/2){14}{}&\rat(3/2){3}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(3/2){14}{\spec{1}}&\rat(5/2){3}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(3/2){14}{\spec{2}}&\rat(5/2){3}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 66
\orbit{2}{66}{92}
\h{66}&\rat(31/4){14}{\spec{1}}&\rat(17/4){3}{}&&\cnt{875}&\bounds{92}{92}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(7/2){12}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/2){12}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(5/2){4}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(9/4){2}{\spec{1}}&\rat(7/4){1}{}&\ln{1}&\cnt{308}&\bounds{28}{28}{1}{false}&&\cr
\l{9}&\rat(7/4){14}{\spec{1}}&\rat(9/4){3}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(5/4){2}{\spec{1}}&\rat(11/4){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 67
\orbit{2}{67}{91}
\h{67}&\rat(39/4){14}{\spec{2}}&\rat(9/4){3}{}&&\cnt{663}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(4){8}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\rat(9/2){4}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(7/2){12}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\rat(7/2){4}{}&\rat(1/2){2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\rat(9/4){2}{\spec{1}}&\rat(7/4){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\rat(7/4){14}{\spec{1}}&\rat(9/4){3}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 68
\orbit{2}{68}{91}
\h{68}&\rat(31/4){10}{\spec{1}}&\rat(17/4){1}{}&&\cnt{719}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(7/2){12}{}&\rat(1/2){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(5/2){12}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\rat(5/2){12}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(5/2){4}{}&\rat(3/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\rat(9/4){14}{}&\rat(7/4){3}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{12}&\rat(7/4){2}{}&\rat(9/4){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\rat(5/4){14}{\spec{1}}&\rat(11/4){3}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{14}&\rat(5/4){14}{\spec{2}}&\rat(11/4){3}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 69
\orbit{2}{69}{90}
\h{69}&\rat(23/4){14}{\spec{2}}&\rat(25/4){3}{}&&\cnt{719}&\bounds{90}{90}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(7/2){12}{}&\rat(1/2){2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/2){12}{}&\rat(3/2){2}{}&\ln{1}&\cnt{80}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(5/2){4}{}&\rat(3/2){2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\rat(9/4){2}{}&\rat(7/4){1}{\spec{1}}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\rat(9/4){2}{}&\rat(7/4){1}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(7/4){14}{}&\rat(9/4){3}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{11}&\rat(5/4){2}{}&\rat(11/4){1}{}&\ln{1}&\cnt{140}&\bounds{14}{14}{1}{false}&&\cr
\l{12}&\rat(3/4){14}{}&\rat(13/4){3}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 70
\orbit{2}{70}{90}
\h{70}&\rat(31/4){14}{\spec{2}}&\rat(17/4){3}{}&&\cnt{667}&\bounds{90}{90}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\rat(7/2){12}{}&\rat(1/2){2}{}&\ln{1}&\cnt{40}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(7/2){4}{}&\rat(1/2){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(5/2){12}{}&\rat(3/2){2}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(5/2){4}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(5/2){4}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{15}{15}{1}{false}&&\cr
\l{9}&\rat(9/4){2}{}&\rat(7/4){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(7/4){14}{}&\rat(9/4){3}{}&\ln{1}&\cnt{80}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\rat(5/4){2}{}&\rat(11/4){1}{}&\ln{1}&\cnt{24}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 71
\orbit{2}{71}{90}
\h{71}&\int(8){\8}{\spec{2}}&\int(4){\4}{2}&&\cnt{783}&\bounds{90}{90}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){12}{\spec{4}}&\int(2){2}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(2){12}{\spec{5}}&\int(2){2}{}&\ln{1}&\cnt{33}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){4}{\spec{4}}&\int(2){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){4}{\spec{5}}&\int(2){2}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\ln{1}&\cnt{176}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(3){14}{}&\int(1){3}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(0){\0}{\spec{2}}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 72
\orbit{2}{72}{89}
\h{72}&\int(2){\2}{}&\int(10){\10}{\spec{2}}&&\cnt{967}&\bounds{89}{89}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{84}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){14}{}&\int(3){3}{}&\ln{2}&\cnt{168}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(0){14}{\spec{1}}&\int(4){3}{}&\ln{2}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\int(0){14}{\spec{2}}&\int(4){3}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 73
\orbit{2}{73}{89}
\h{73}&\rat(15/4){14}{\spec{2}}&\rat(33/4){3}{\spec{2}}&&\cnt{819}&\bounds{89}{89}{1}{false}&&\cr
\l{1}&\rat(5/2){12}{}&\rat(3/2){2}{}&\ln{1}&\cnt{36}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{54}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{108}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(7/4){14}{}&\rat(9/4){3}{\spec{1}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(7/4){14}{}&\rat(9/4){3}{\spec{2}}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(5/4){2}{}&\rat(11/4){1}{}&\ln{1}&\cnt{180}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\rat(3/4){14}{}&\rat(13/4){3}{}&\ln{1}&\cnt{216}&\bounds{18}{18}{1}{false}&&\cr
\l{9}&\rat(1/4){2}{\spec{1}}&\rat(15/4){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(1/4){2}{\spec{2}}&\rat(15/4){1}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 74
\orbit{2}{74}{87}
\h{74}&\int(4){8}{}&\int(8){\8}{}&&\cnt{647}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){14}{}&\int(3){3}{}&\ln{2}&\cnt{224}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\int(0){14}{}&\int(4){3}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 75
\orbit{2}{75}{87}
\h{75}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&&\cnt{715}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){12}{}&\int(1){2}{}&\ln{2}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{2}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(3){14}{}&\int(1){3}{}&\ln{2}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 76
\orbit{2}{76}{87}
\h{76}&\rat(23/4){10}{\spec{1}}&\rat(25/4){1}{}&&\cnt{707}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\rat(7/2){12}{}&\rat(1/2){2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(5/2){12}{\spec{1}}&\rat(3/2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/2){12}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{154}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(9/4){14}{}&\rat(7/4){3}{\spec{1}}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{8}&\rat(9/4){14}{}&\rat(7/4){3}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(5/4){14}{\spec{1}}&\rat(11/4){3}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\rat(5/4){14}{\spec{2}}&\rat(11/4){3}{}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\rat(3/4){2}{}&\rat(13/4){1}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 77
\orbit{2}{77}{87}
\h{77}&\int(5){12}{\spec{1}}&\int(7){2}{\spec{1}}&&\cnt{799}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{39}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){12}{}&\int(2){2}{}&\ln{1}&\cnt{156}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{39}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{130}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{78}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(5/2){14}{}&\rat(3/2){3}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\rat(3/2){14}{\spec{1}}&\rat(5/2){3}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(3/2){14}{\spec{2}}&\rat(5/2){3}{}&\ln{1}&\cnt{208}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 78
\orbit{2}{78}{87}
\h{78}&\int(12){\12}{\spec{5}}&\int(0){\0}{}&&\cnt{831}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{396}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{432}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 79
\orbit{2}{79}{87}
\h{79}&\int(4){\4}{}&\int(8){\8}{}&&\cnt{763}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(2){14}{}&\int(2){3}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(1){14}{}&\int(3){3}{}&\ln{2}&\cnt{192}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(0){14}{\spec{1}}&\int(4){3}{}&\ln{2}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(0){14}{\spec{2}}&\int(4){3}{}&\ln{2}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 80
\orbit{2}{80}{86}
\h{80}&\int(4){8}{}&\int(8){\8}{0}&&\cnt{479}&\bounds{86}{86}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){12}{}&\int(2){2}{}&\ln{2}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 81
\orbit{2}{81}{85}
\h{81}&\int(11){12}{\spec{2}}&\int(1){2}{}&&\cnt{703}&\bounds{85}{85}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(4){12}{}&\int(0){2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(3){12}{\spec{3}}&\int(1){2}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(3){4}{\spec{3}}&\int(1){2}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{9}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 82
\orbit{2}{82}{85}
\h{82}&\int(0){\0}{}&\int(12){\12}{2}&&\cnt{903}&\bounds{85}{85}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{720}&\bounds{48}{48}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{180}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 83
\orbit{2}{83}{84}
\h{83}&\rat(39/4){10}{\spec{3}}&\rat(9/4){1}{}&&\cnt{763}&\bounds{84}{84}{1}{false}&&\cr
\l{1}&\int(4){8}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(9/2){12}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\rat(7/2){12}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(7/2){12}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{270}&\bounds{27}{27}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\rat(13/4){14}{}&\rat(3/4){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{10}&\rat(9/4){14}{}&\rat(7/4){3}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\rat(7/4){2}{}&\rat(9/4){1}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 84
\orbit{2}{84}{84}
\h{84}&\rat(31/4){14}{\spec{1}}&\rat(17/4){3}{}&&\cnt{763}&\bounds{84}{84}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{44}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(7/2){12}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\rat(5/2){12}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(5/2){12}{\spec{3}}&\rat(3/2){2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(5/2){4}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{2}}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{12}&\rat(11/4){14}{}&\rat(5/4){3}{\spec{1}}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\rat(11/4){14}{}&\rat(5/4){3}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\rat(9/4){2}{\spec{2}}&\rat(7/4){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{15}&\rat(7/4){14}{\spec{2}}&\rat(9/4){3}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\rat(7/4){14}{\spec{3}}&\rat(9/4){3}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{17}&\rat(5/4){2}{\spec{2}}&\rat(11/4){1}{}&\ln{1}&\cnt{22}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 85
\orbit{2}{85}{83}
\h{85}&\int(5){12}{\spec{2}}&\int(7){2}{\spec{2}}&&\cnt{655}&\bounds{83}{83}{1}{false}&&\cr
\l{1}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{35}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\rat(3/2){14}{}&\rat(5/2){3}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(3/2){2}{}&\rat(5/2){1}{}&\ln{1}&\cnt{140}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\rat(1/2){14}{}&\rat(7/2){3}{}&\ln{1}&\cnt{100}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(1/2){2}{\spec{1}}&\rat(7/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\rat(1/2){2}{\spec{2}}&\rat(7/2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 86
\orbit{2}{86}{81}
\h{86}&\rat(31/4){10}{\spec{2}}&\rat(17/4){1}{}&&\cnt{763}&\bounds{81}{81}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\rat(9/2){12}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/2){12}{}&\rat(1/2){2}{}&\ln{1}&\cnt{192}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(5/2){12}{\spec{2}}&\rat(3/2){2}{}&\ln{1}&\cnt{24}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(5/2){12}{\spec{3}}&\rat(3/2){2}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{192}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(13/4){14}{}&\rat(3/4){3}{\spec{1}}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\rat(13/4){14}{}&\rat(3/4){3}{\spec{2}}&\ln{1}&\cnt{8}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\rat(9/4){14}{}&\rat(7/4){3}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\rat(5/4){14}{\spec{2}}&\rat(11/4){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\rat(5/4){14}{\spec{3}}&\rat(11/4){3}{}&\ln{1}&\cnt{24}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 87
\orbit{2}{87}{80}
\h{87}&\rat(7/4){14}{}&\rat(41/4){3}{\spec{2}}&&\cnt{871}&\bounds{80}{80}{1}{false}&&\cr
\l{1}&\rat(3/2){12}{}&\rat(5/2){2}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{196}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(7/4){14}{}&\rat(9/4){3}{\spec{1}}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\rat(7/4){14}{}&\rat(9/4){3}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(3/4){14}{}&\rat(13/4){3}{}&\ln{1}&\cnt{196}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\rat(1/4){2}{}&\rat(15/4){1}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{42}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 88
\orbit{2}{88}{79}
\h{88}&\int(0){\0}{}&\int(12){\12}{\spec{1}}&&\cnt{1031}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(0){2}{}&\int(4){1}{}&\ln{1}&\cnt{960}&\bounds{64}{64}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 89
\orbit{2}{89}{79}
\h{89}&\rat(15/4){14}{\spec{1}}&\rat(33/4){3}{\spec{1}}&&\cnt{1051}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\rat(3/2){12}{}&\rat(5/2){2}{}&\ln{1}&\cnt{455}&\bounds{35}{35}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{120}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(7/4){14}{}&\rat(9/4){3}{}&\ln{1}&\cnt{420}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 90
\orbit{2}{90}{79}
\h{90}&\rat(23/4){14}{\spec{1}}&\rat(25/4){3}{}&&\cnt{875}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){12}{}&\rat(3/2){2}{}&\ln{1}&\cnt{156}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{3}}&\int(3){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(11/4){14}{}&\rat(5/4){3}{\spec{1}}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{11}&\rat(11/4){14}{}&\rat(5/4){3}{\spec{2}}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{12}&\rat(7/4){14}{}&\rat(9/4){3}{}&\ln{1}&\cnt{273}&\bounds{21}{21}{1}{false}&&\cr
\l{13}&\rat(5/4){2}{}&\rat(11/4){1}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{14}&\rat(3/4){14}{\spec{1}}&\rat(13/4){3}{}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{15}&\rat(3/4){14}{\spec{2}}&\rat(13/4){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 91
\orbit{2}{91}{79}
\h{91}&\int(5){12}{\spec{1}}&\int(7){2}{\spec{2}}&&\cnt{887}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{273}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\rat(5/2){14}{}&\rat(3/2){3}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(3/2){14}{\spec{1}}&\rat(5/2){3}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\rat(3/2){14}{\spec{2}}&\rat(5/2){3}{}&\ln{1}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\rat(1/2){14}{}&\rat(7/2){3}{}&\ln{1}&\cnt{52}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(1/2){2}{}&\rat(7/2){1}{}&\ln{1}&\cnt{156}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 92
\orbit{2}{92}{75}
\h{92}&\int(0){\0}{}&\int(12){\12}{}&&\cnt{843}&\bounds{75}{75}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{720}&\bounds{48}{48}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 93
\orbit{2}{93}{74}
\h{93}&\rat(39/4){10}{\spec{2}}&\rat(9/4){1}{}&&\cnt{651}&\bounds{74}{74}{1}{false}&&\cr
\l{1}&\int(4){8}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(9/2){4}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(7/2){4}{\spec{1}}&\rat(1/2){2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\rat(7/2){4}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\rat(11/4){2}{\spec{1}}&\rat(5/4){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(7/4){2}{\spec{1}}&\rat(9/4){1}{}&\ln{1}&\cnt{12}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 94
\orbit{2}{94}{74}
\h{94}&\int(2){\2}{}&\int(10){\10}{\spec{1}}&&\cnt{827}&\bounds{74}{74}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{56}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\int(1){14}{}&\int(3){3}{}&\ln{2}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 95
\orbit{2}{95}{71}
\h{95}&\int(6){\6}{\spec{1}}&\int(6){\6}{}&&\cnt{743}&\bounds{71}{71}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{195}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(2){14}{}&\int(2){3}{}&\ln{1}&\cnt{312}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(1){14}{}&\int(3){3}{}&\ln{1}&\cnt{8}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(3){1}{}&\ln{1}&\cnt{104}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 96
\orbit{2}{96}{71}
\h{96}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&&\cnt{851}&\bounds{71}{71}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{2}&\cnt{84}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(2){14}{}&\int(2){3}{}&\ln{2}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 97
\orbit{2}{97}{63}
\h{97}&\rat(39/4){10}{\spec{4}}&\rat(9/4){1}{}&&\cnt{603}&\bounds{63}{63}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{234}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\rat(9/2){12}{}&\rat(-1/2){2}{}&\ln{1}&\cnt{117}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\rat(13/4){14}{}&\rat(3/4){3}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 98
\orbit{2}{98}{62}
\h{98}&\int(3){12}{}&\int(9){2}{\spec{5}}&&\cnt{615}&\bounds{62}{62}{1}{false}&&\cr
\l{1}&\int(3){12}{}&\int(1){2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(1/2){14}{}&\rat(7/2){3}{}&\ln{1}&\cnt{432}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\rat(-1/2){2}{}&\rat(9/2){1}{}&\ln{1}&\cnt{48}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 99
\orbit{2}{99}{60}
\h{99}&\rat(39/4){14}{\spec{2}}&\rat(9/4){3}{}&&\cnt{591}&\bounds{60}{60}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(7/2){12}{\spec{2}}&\rat(1/2){2}{}&\ln{1}&\cnt{108}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(11/4){14}{}&\rat(5/4){3}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\rat(9/4){2}{\spec{2}}&\rat(7/4){1}{}&\ln{1}&\cnt{108}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\rat(7/4){14}{\spec{2}}&\rat(9/4){3}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(7/4){14}{\spec{3}}&\rat(9/4){3}{}&\ln{1}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 100
\orbit{2}{100}{58}
\h{100}&\rat(15/4){14}{\spec{1}}&\rat(33/4){3}{\spec{2}}&&\cnt{771}&\bounds{58}{58}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{270}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\rat(7/4){14}{}&\rat(9/4){3}{\spec{1}}&\ln{1}&\cnt{300}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\rat(7/4){14}{}&\rat(9/4){3}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\rat(1/4){2}{}&\rat(15/4){1}{}&\ln{1}&\cnt{105}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[15] + D[9]
% Class 101
\orbit{2}{101}{55}
\h{101}&\int(7){12}{\spec{2}}&\int(5){2}{\spec{1}}&&\cnt{639}&\bounds{55}{55}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(3){12}{\spec{2}}&\int(1){2}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{392}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\rat(7/2){14}{}&\rat(1/2){3}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(0){\0}{\spec{2}}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_A17_E7.tex <==
% -*- TeX -*-
% Niemeier lattice A17_E7
% 67 classes
\newcs{max-A17_E7}{147}%
\newcs{count-A17_E7}{67}%
\newcs{counts-A17_E7}{\DO{1}{147}\DO{2}{134}\DO{3}{127}\DO{4}{123}\DO{5}{123}\DO{6}{123}\DO{7}{115}\DO{8}{113}\DO{9}{112}\DO{10}{109}\DO{11}{107}\DO{12}{107}\DO{13}{107}\DO{14}{106}\DO{15}{105}\DO{16}{105}\DO{17}{103}\DO{18}{103}\DO{19}{101}\DO{20}{100}\DO{21}{99}\DO{22}{99}\DO{23}{98}\DO{24}{97}\DO{25}{95}\DO{26}{95}\DO{27}{95}\DO{28}{94}\DO{29}{93}\DO{30}{93}\DO{31}{93}\DO{32}{91}\DO{33}{91}\DO{34}{89}\DO{35}{89}\DO{36}{87}\DO{37}{87}\DO{38}{87}\DO{39}{87}\DO{40}{86}\DO{41}{85}\DO{42}{85}\DO{43}{83}\DO{44}{83}\DO{45}{83}\DO{46}{81}\DO{47}{79}\DO{48}{79}\DO{49}{79}\DO{50}{79}\DO{51}{75}\DO{52}{73}\DO{53}{72}\DO{54}{71}\DO{55}{71}\DO{56}{71}\DO{57}{71}\DO{58}{71}\DO{59}{69}\DO{60}{66}\DO{61}{63}\DO{62}{63}\DO{63}{62}\DO{64}{61}\DO{65}{61}\DO{66}{57}\DO{67}{47}}%
\orbits
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 1
\orbit{2}{1}{147}
\h{1}&\int(12){\12}{}&\int(0){\0}{}&&\cnt{747}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 2
\orbit{2}{2}{134}
\h{2}&\int(10){12}{\spec{1}}&\int(2){\2}{}&&\cnt{1103}&\bounds{134}{134}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){1}{}&\ln{1}&\cnt{432}&\bounds{48}{48}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 3
\orbit{2}{3}{127}
\h{3}&\int(12){\12}{\spec{4}}&\int(0){\0}{}&&\cnt{1443}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){15}{}&\int(0){1}{}&\ln{1}&\cnt{672}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 4
\orbit{2}{4}{123}
\h{4}&\int(0){\0}{}&\int(12){\12}{\spec{2}}&&\cnt{1979}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(0){15}{}&\int(4){1}{}&\ln{2}&\cnt{816}&\bounds{48}{48}{1}{false}&&\cr
\l{2}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{306}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 5
\orbit{2}{5}{123}
\h{5}&\rat(21/2){9}{\spec{5}}&\rat(3/2){1}{}&&\cnt{1263}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{165}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{330}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\rat(7/2){15}{}&\rat(1/2){1}{}&\ln{1}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\l{4}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{297}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 6
\orbit{2}{6}{123}
\h{6}&\rat(9/2){9}{}&\rat(15/2){1}{}&&\cnt{939}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\rat(3/2){15}{}&\rat(5/2){1}{}&\ln{2}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 7
\orbit{2}{7}{115}
\h{7}&\int(12){12}{\spec{3}}&\int(0){\0}{}&&\cnt{791}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{245}&\bounds{35}{35}{1}{false}&&\cr
\l{3}&\int(4){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\int(4){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\int(4){3}{}&\int(0){1}{}&\ln{1}&\cnt{56}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 8
\orbit{2}{8}{113}
\h{8}&\int(12){12}{\spec{1}}&\int(0){\0}{}&&\cnt{1127}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{315}&\bounds{35}{35}{1}{false}&&\cr
\l{3}&\int(4){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\l{6}&\int(4){3}{}&\int(0){1}{}&\ln{1}&\cnt{392}&\bounds{28}{28}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 9
\orbit{2}{9}{112}
\h{9}&\rat(21/2){15}{\spec{1}}&\rat(3/2){1}{}&&\cnt{983}&\bounds{112}{112}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(7/2){3}{}&\rat(1/2){1}{}&\ln{1}&\cnt{270}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 10
\orbit{2}{10}{109}
\h{10}&\int(10){12}{\spec{5}}&\int(2){\2}{}&&\cnt{1415}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{273}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(4){15}{}&\int(0){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){15}{}&\int(1){1}{}&\ln{1}&\cnt{504}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{448}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 11
\orbit{2}{11}{107}
\h{11}&\int(12){12}{\spec{4}}&\int(0){\0}{}&&\cnt{971}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\int(4){12}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){6}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{10}&\int(4){15}{}&\int(0){1}{}&\ln{1}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 12
\orbit{2}{12}{107}
\h{12}&\int(12){12}{\spec{2}}&\int(0){\0}{}&&\cnt{995}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(4){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(4){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{240}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(4){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\int(4){3}{}&\int(0){1}{}&\ln{1}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 13
\orbit{2}{13}{107}
\h{13}&\int(10){\10}{}&\int(2){\2}{}&&\cnt{655}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{2}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(3){15}{}&\int(1){1}{}&\ln{2}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{25}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 14
\orbit{2}{14}{106}
\h{14}&\int(10){12}{\spec{2}}&\int(2){\2}{}&&\cnt{767}&\bounds{106}{106}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(4){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(3){15}{}&\int(1){1}{}&\ln{1}&\cnt{180}&\bounds{30}{30}{1}{false}&&\cr
\l{8}&\int(3){3}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 15
\orbit{2}{15}{105}
\h{15}&\int(12){\12}{\spec{3}}&\int(0){\0}{}&&\cnt{903}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(4){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){6}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\int(4){15}{}&\int(0){1}{}&\ln{1}&\cnt{168}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 16
\orbit{2}{16}{105}
\h{16}&\rat(17/2){15}{\spec{1}}&\rat(7/2){1}{}&&\cnt{923}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\rat(3/2){1}{}&\ln{1}&\cnt{462}&\bounds{42}{42}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{84}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 17
\orbit{2}{17}{103}
\h{17}&\int(12){12}{\spec{6}}&\int(0){\0}{}&&\cnt{1135}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{264}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{264}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(4){15}{}&\int(0){1}{}&\ln{1}&\cnt{336}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 18
\orbit{2}{18}{103}
\h{18}&\int(12){12}{\spec{2}}&\int(0){\0}{}&&\cnt{799}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(4){6}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{42}{42}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 19
\orbit{2}{19}{101}
\h{19}&\rat(17/2){9}{\spec{1}}&\rat(7/2){1}{}&&\cnt{715}&\bounds{101}{101}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{2}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{2}&\cnt{56}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 20
\orbit{2}{20}{100}
\h{20}&\int(6){12}{\spec{2}}&\int(6){\6}{\spec{1}}&&\cnt{767}&\bounds{100}{100}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){15}{}&\int(2){1}{}&\ln{1}&\cnt{210}&\bounds{35}{35}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(2){1}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{140}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 21
\orbit{2}{21}{99}
\h{21}&\int(12){12}{\spec{7}}&\int(0){\0}{}&&\cnt{1415}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{455}&\bounds{35}{35}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){15}{}&\int(0){1}{}&\ln{1}&\cnt{840}&\bounds{56}{56}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 22
\orbit{2}{22}{99}
\h{22}&\rat(21/2){15}{\spec{2}}&\rat(3/2){1}{}&&\cnt{647}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(4){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(4){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\rat(7/2){3}{}&\rat(1/2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\rat(5/2){15}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 23
\orbit{2}{23}{98}
\h{23}&\int(4){12}{}&\int(8){\8}{\spec{2}}&&\cnt{983}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){15}{}&\int(2){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(1){15}{}&\int(3){1}{}&\ln{1}&\cnt{180}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(1){3}{}&\int(3){1}{}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{432}&\bounds{36}{36}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 24
\orbit{2}{24}{97}
\h{24}&\int(10){12}{\spec{4}}&\int(2){\2}{}&&\cnt{1367}&\bounds{97}{97}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{455}&\bounds{35}{35}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{315}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(5){15}{}&\int(-1){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){15}{}&\int(1){1}{}&\ln{1}&\cnt{540}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 25
\orbit{2}{25}{95}
\h{25}&\rat(21/2){9}{\spec{3}}&\rat(3/2){1}{}&&\cnt{759}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(4){6}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\rat(7/2){15}{}&\rat(1/2){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(5/2){15}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\rat(5/2){15}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 26
\orbit{2}{26}{95}
\h{26}&\int(8){\8}{}&\int(4){\4}{}&&\cnt{655}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{2}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(3){15}{}&\int(1){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){15}{}&\int(2){1}{}&\ln{2}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 27
\orbit{2}{27}{95}
\h{27}&\rat(5/2){15}{}&\rat(19/2){1}{\spec{2}}&&\cnt{1307}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(3/2){15}{}&\rat(5/2){1}{}&\ln{1}&\cnt{45}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(1/2){15}{}&\rat(7/2){1}{}&\ln{1}&\cnt{315}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\rat(1/2){3}{}&\rat(7/2){1}{}&\ln{1}&\cnt{455}&\bounds{35}{35}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{450}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 28
\orbit{2}{28}{94}
\h{28}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&&\cnt{871}&\bounds{94}{94}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{165}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(4){6}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\ln{1}&\cnt{88}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(4){15}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(3){15}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{264}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(3){3}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 29
\orbit{2}{29}{93}
\h{29}&\int(8){12}{\spec{2}}&\int(4){\4}{}&&\cnt{655}&\bounds{93}{93}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(1){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){15}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){3}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){3}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(0){\0}{\spec{1}}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 30
\orbit{2}{30}{93}
\h{30}&\rat(21/2){15}{\spec{5}}&\rat(3/2){1}{}&&\cnt{1303}&\bounds{93}{93}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\rat(7/2){15}{}&\rat(1/2){1}{}&\ln{1}&\cnt{405}&\bounds{27}{27}{1}{false}&&\cr
\l{4}&\rat(5/2){15}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{105}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(5/2){15}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{405}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 31
\orbit{2}{31}{93}
\h{31}&\rat(21/2){15}{\spec{3}}&\rat(3/2){1}{}&&\cnt{815}&\bounds{93}{93}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){6}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\rat(7/2){15}{}&\rat(1/2){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(7/2){3}{}&\rat(1/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\rat(5/2){15}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{4}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(5/2){15}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{40}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(5/2){3}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{3}{3}{1}{false}&&\cr
\l{12}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 32
\orbit{2}{32}{91}
\h{32}&\rat(17/2){15}{\spec{4}}&\rat(7/2){1}{}&&\cnt{1547}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{1}&\cnt{952}&\bounds{56}{56}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{595}&\bounds{35}{35}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 33
\orbit{2}{33}{91}
\h{33}&\int(10){12}{\spec{2}}&\int(2){\2}{}&&\cnt{647}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){6}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(4){6}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(4){3}{}&\int(0){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){3}{\spec{1}}&\int(1){1}{}&\ln{1}&\cnt{216}&\bounds{36}{36}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 34
\orbit{2}{34}{89}
\h{34}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&&\cnt{935}&\bounds{89}{89}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{3}}&\int(0){\0}{}&\ln{2}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{2}&\cnt{48}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{2}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{7}}&\int(0){\0}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(4){15}{}&\int(0){1}{}&\ln{2}&\cnt{56}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 35
\orbit{2}{35}{89}
\h{35}&\rat(17/2){15}{\spec{2}}&\rat(7/2){1}{}&&\cnt{659}&\bounds{89}{89}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){6}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\rat(7/2){3}{}&\rat(1/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(5/2){15}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{126}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 36
\orbit{2}{36}{87}
\h{36}&\int(4){\4}{}&\int(8){\8}{\spec{2}}&&\cnt{967}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){15}{}&\int(2){1}{}&\ln{2}&\cnt{84}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(1){15}{\spec{1}}&\int(3){1}{}&\ln{2}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(1){15}{\spec{2}}&\int(3){1}{}&\ln{2}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{168}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 37
\orbit{2}{37}{87}
\h{37}&\rat(9/2){15}{\spec{2}}&\rat(15/2){1}{}&&\cnt{923}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\rat(3/2){15}{}&\rat(5/2){1}{}&\ln{1}&\cnt{234}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\rat(5/2){1}{}&\ln{1}&\cnt{234}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{65}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{260}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 38
\orbit{2}{38}{87}
\h{38}&\int(6){12}{\spec{1}}&\int(6){\6}{\spec{2}}&&\cnt{995}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){15}{}&\int(1){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(1){15}{\spec{1}}&\int(3){1}{}&\ln{1}&\cnt{78}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(1){15}{\spec{2}}&\int(3){1}{}&\ln{1}&\cnt{78}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){3}{}&\int(3){1}{}&\ln{1}&\cnt{286}&\bounds{26}{26}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{351}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 39
\orbit{2}{39}{87}
\h{39}&\int(12){\12}{\spec{5}}&\int(0){\0}{}&&\cnt{927}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{546}&\bounds{42}{42}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{378}&\bounds{42}{42}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 40
\orbit{2}{40}{86}
\h{40}&\rat(13/2){9}{\spec{1}}&\rat(11/2){1}{}&&\cnt{703}&\bounds{86}{86}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\rat(3/2){15}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\rat(3/2){15}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{70}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{}&\rat(5/2){1}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{70}&\bounds{7}{7}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 41
\orbit{2}{41}{85}
\h{41}&\rat(21/2){15}{\spec{4}}&\rat(3/2){1}{}&&\cnt{971}&\bounds{85}{85}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{286}&\bounds{26}{26}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{26}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{52}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{78}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\rat(9/2){15}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(7/2){15}{}&\rat(1/2){1}{}&\ln{1}&\cnt{351}&\bounds{27}{27}{1}{false}&&\cr
\l{8}&\rat(5/2){15}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{26}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(5/2){15}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\rat(5/2){3}{}&\rat(3/2){1}{}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 42
\orbit{2}{42}{85}
\h{42}&\int(6){\6}{}&\int(6){\6}{\spec{1}}&&\cnt{759}&\bounds{85}{85}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){15}{}&\int(1){1}{}&\ln{2}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(2){15}{}&\int(2){1}{}&\ln{2}&\cnt{216}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{135}&\bounds{27}{27}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{72}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 43
\orbit{2}{43}{83}
\h{43}&\int(2){\2}{}&\int(10){\10}{}&&\cnt{1035}&\bounds{83}{83}{1}{false}&&\cr
\l{1}&\int(1){15}{}&\int(3){1}{}&\ln{2}&\cnt{240}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{2}&\cnt{128}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{240}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 44
\orbit{2}{44}{83}
\h{44}&\rat(13/2){15}{\spec{2}}&\rat(11/2){1}{}&&\cnt{703}&\bounds{83}{83}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{11}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\rat(3/2){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\rat(3/2){15}{}&\rat(5/2){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\rat(3/2){3}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(3/2){3}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{22}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 45
\orbit{2}{45}{83}
\h{45}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&&\cnt{1095}&\bounds{83}{83}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){15}{}&\int(2){1}{}&\ln{1}&\cnt{630}&\bounds{42}{42}{1}{false}&&\cr
\l{3}&\int(2){3}{}&\int(2){1}{}&\ln{1}&\cnt{90}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{225}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{60}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 46
\orbit{2}{46}{81}
\h{46}&\int(6){\6}{}&\int(6){\6}{\spec{2}}&&\cnt{747}&\bounds{81}{81}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){15}{}&\int(1){1}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(1){15}{\spec{1}}&\int(3){1}{}&\ln{2}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(1){15}{\spec{2}}&\int(3){1}{}&\ln{2}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 47
\orbit{2}{47}{79}
\h{47}&\rat(17/2){15}{\spec{2}}&\rat(7/2){1}{}&&\cnt{755}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\rat(7/2){15}{}&\rat(1/2){1}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(5/2){15}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(5/2){15}{\spec{3}}&\rat(3/2){1}{}&\ln{1}&\cnt{252}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{84}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{84}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 48
\orbit{2}{48}{79}
\h{48}&\int(8){12}{\spec{1}}&\int(4){\4}{}&&\cnt{703}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\int(3){15}{}&\int(1){1}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(2){15}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{20}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){15}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(2){3}{}&\int(2){1}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 49
\orbit{2}{49}{79}
\h{49}&\int(10){12}{\spec{3}}&\int(2){\2}{}&&\cnt{743}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{6}{6}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{66}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(4){15}{}&\int(0){1}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(3){15}{\spec{1}}&\int(1){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(3){15}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{144}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{24}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 50
\orbit{2}{50}{79}
\h{50}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&&\cnt{1083}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{240}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(2){15}{}&\int(2){1}{}&\ln{2}&\cnt{240}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{2}&\cnt{160}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 51
\orbit{2}{51}{75}
\h{51}&\rat(21/2){9}{\spec{4}}&\rat(3/2){1}{}&&\cnt{747}&\bounds{75}{75}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{198}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\rat(9/2){15}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(7/2){15}{}&\rat(1/2){1}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\rat(5/2){15}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{9}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(5/2){15}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 52
\orbit{2}{52}{73}
\h{52}&\int(8){\8}{\spec{2}}&\int(4){\4}{}&&\cnt{799}&\bounds{73}{73}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{39}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{39}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){15}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{208}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(3){3}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){15}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{156}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){15}{\spec{3}}&\int(2){1}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){3}{\spec{3}}&\int(2){1}{}&\ln{1}&\cnt{78}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{4}}&\int(2){\2}{}&\ln{1}&\cnt{130}&\bounds{10}{10}{1}{false}&&\cr
\l{11}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 53
\orbit{2}{53}{72}
\h{53}&\rat(17/2){9}{\spec{2}}&\rat(7/2){1}{}&&\cnt{643}&\bounds{72}{72}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{110}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{55}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\rat(7/2){15}{}&\rat(1/2){1}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\rat(5/2){15}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(5/2){15}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{77}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{154}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 54
\orbit{2}{54}{71}
\h{54}&\rat(13/2){15}{\spec{1}}&\rat(11/2){1}{}&&\cnt{859}&\bounds{71}{71}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(7/2){15}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/2){15}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{1}&\cnt{280}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\rat(3/2){15}{\spec{1}}&\rat(5/2){1}{}&\ln{1}&\cnt{14}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\rat(3/2){15}{\spec{2}}&\rat(5/2){1}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\rat(3/2){15}{\spec{3}}&\rat(5/2){1}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(3/2){3}{}&\rat(5/2){1}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\l{13}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{14}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{28}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(1){\2}{\spec{3}}&\int(3){\2}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 55
\orbit{2}{55}{71}
\h{55}&\int(4){12}{}&\int(8){\8}{\spec{1}}&&\cnt{463}&\bounds{71}{71}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){15}{}&\int(2){1}{}&\ln{1}&\cnt{240}&\bounds{40}{40}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 56
\orbit{2}{56}{71}
\h{56}&\int(8){12}{\spec{2}}&\int(4){\4}{}&&\cnt{871}&\bounds{71}{71}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(4){15}{}&\int(0){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){15}{\spec{1}}&\int(1){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(3){15}{\spec{2}}&\int(1){1}{}&\ln{1}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){15}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{112}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{280}&\bounds{20}{20}{1}{false}&&\cr
\l{8}&\int(0){\0}{\spec{2}}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 57
\orbit{2}{57}{71}
\h{57}&\int(0){\0}{}&\int(12){\12}{\spec{1}}&&\cnt{963}&\bounds{71}{71}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{918}&\bounds{54}{54}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 58
\orbit{2}{58}{71}
\h{58}&\int(4){\4}{}&\int(8){\8}{\spec{1}}&&\cnt{711}&\bounds{71}{71}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){15}{}&\int(2){1}{}&\ln{2}&\cnt{168}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 59
\orbit{2}{59}{69}
\h{59}&\int(6){12}{\spec{1}}&\int(6){\6}{\spec{1}}&&\cnt{743}&\bounds{69}{69}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){15}{}&\int(1){1}{}&\ln{1}&\cnt{72}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(2){15}{\spec{1}}&\int(2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(2){15}{\spec{2}}&\int(2){1}{}&\ln{1}&\cnt{312}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{195}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{104}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{8}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 60
\orbit{2}{60}{66}
\h{60}&\int(6){12}{\spec{2}}&\int(6){\6}{\spec{2}}&&\cnt{623}&\bounds{66}{66}{1}{false}&&\cr
\l{1}&\int(4){12}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){15}{}&\int(3){1}{}&\ln{1}&\cnt{210}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(1){3}{\spec{1}}&\int(3){1}{}&\ln{1}&\cnt{70}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(1){3}{\spec{2}}&\int(3){1}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 61
\orbit{2}{61}{63}
\h{61}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&&\cnt{699}&\bounds{63}{63}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{2}&\cnt{14}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(3){15}{}&\int(1){1}{}&\ln{2}&\cnt{168}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{2}&\cnt{14}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 62
\orbit{2}{62}{63}
\h{62}&\rat(5/2){15}{}&\rat(19/2){1}{\spec{1}}&&\cnt{799}&\bounds{63}{63}{1}{false}&&\cr
\l{1}&\rat(5/2){15}{}&\rat(3/2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){15}{}&\rat(3/2){1}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(3/2){15}{}&\rat(5/2){1}{}&\ln{1}&\cnt{270}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{270}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{210}&\bounds{15}{15}{1}{false}&&\cr
\l{6}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 63
\orbit{2}{63}{62}
\h{63}&\rat(21/2){15}{\spec{2}}&\rat(3/2){1}{}&&\cnt{631}&\bounds{62}{62}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{78}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{39}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{156}&\bounds{13}{13}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\rat(7/2){15}{}&\rat(1/2){1}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\rat(5/2){15}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\rat(5/2){15}{\spec{3}}&\rat(3/2){1}{}&\ln{1}&\cnt{39}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(5/2){3}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{78}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 64
\orbit{2}{64}{61}
\h{64}&\int(12){12}{\spec{5}}&\int(0){\0}{}&&\cnt{743}&\bounds{61}{61}{1}{false}&&\cr
\l{1}&\int(4){12}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{286}&\bounds{26}{26}{1}{false}&&\cr
\l{2}&\int(4){12}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{39}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{234}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\int(4){15}{}&\int(0){1}{}&\ln{1}&\cnt{168}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 65
\orbit{2}{65}{61}
\h{65}&\rat(9/2){15}{\spec{1}}&\rat(15/2){1}{}&&\cnt{875}&\bounds{61}{61}{1}{false}&&\cr
\l{1}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{1}&\cnt{160}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(3/2){15}{}&\rat(5/2){1}{}&\ln{1}&\cnt{360}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{240}&\bounds{15}{15}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{80}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 66
\orbit{2}{66}{57}
\h{66}&\rat(17/2){15}{\spec{3}}&\rat(7/2){1}{}&&\cnt{707}&\bounds{57}{57}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(7/2){15}{}&\rat(1/2){1}{}&\ln{1}&\cnt{315}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\rat(5/2){15}{}&\rat(3/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{210}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[17] + E[7]
% Class 67
\orbit{2}{67}{47}
\h{67}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{2}}&&\cnt{687}&\bounds{47}{47}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){15}{}&\int(3){1}{}&\ln{1}&\cnt{30}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(1){3}{}&\int(3){1}{}&\ln{1}&\cnt{210}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{405}&\bounds{27}{27}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_A24.tex <==
% -*- TeX -*-
% Niemeier lattice A24
% 19 classes
\newcs{max-A24}{121}%
\newcs{count-A24}{19}%
\newcs{counts-A24}{\DO{1}{121}\DO{2}{91}\DO{3}{84}\DO{4}{84}\DO{5}{79}\DO{6}{79}\DO{7}{76}\DO{8}{75}\DO{9}{70}\DO{10}{66}\DO{11}{63}\DO{12}{61}\DO{13}{58}\DO{14}{57}\DO{15}{57}\DO{16}{55}\DO{17}{52}\DO{18}{44}\DO{19}{31}}%
\orbits
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 1
\orbit{1}{1}{121}
\h{1}&\int(12){15}{\spec{1}}&&\cnt{1287}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){5}{}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\ln{1}&\cnt{792}&\bounds{66}{66}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 2
\orbit{1}{2}{91}
\h{2}&\int(12){15}{\spec{5}}&&\cnt{1547}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(4){20}{}&\ln{1}&\cnt{595}&\bounds{35}{35}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\ln{1}&\cnt{952}&\bounds{56}{56}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 3
\orbit{1}{3}{84}
\h{3}&\int(12){20}{\spec{6}}&&\cnt{1527}&\bounds{84}{84}{1}{false}&&\cr
\l{1}&\int(4){20}{\spec{1}}&\ln{1}&\cnt{570}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(4){20}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{380}&\bounds{20}{20}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{570}&\bounds{30}{30}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 4
\orbit{1}{4}{84}
\h{4}&\int(12){20}{\spec{7}}&&\cnt{1771}&\bounds{84}{84}{1}{false}&&\cr
\l{1}&\int(4){20}{}&\ln{1}&\cnt{1771}&\bounds{84}{84}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 5
\orbit{1}{5}{79}
\h{5}&\int(12){\12}{\spec{4}}&&\cnt{1387}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(4){20}{}&\ln{1}&\cnt{969}&\bounds{57}{57}{1}{false}&&\cr
\l{2}&\int(4){5}{}&\ln{1}&\cnt{19}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{228}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{171}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 6
\orbit{1}{6}{79}
\h{6}&\int(12){20}{\spec{1}}&&\cnt{1051}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(4){20}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(4){5}{}&\ln{1}&\cnt{455}&\bounds{35}{35}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{120}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{420}&\bounds{28}{28}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 7
\orbit{1}{7}{76}
\h{7}&\int(12){15}{\spec{2}}&&\cnt{727}&\bounds{76}{76}{1}{false}&&\cr
\l{1}&\int(4){20}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(4){5}{\spec{3}}&\ln{1}&\cnt{220}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{12}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{240}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 8
\orbit{1}{8}{75}
\h{8}&\int(12){\12}{}&&\cnt{615}&\bounds{75}{75}{1}{false}&&\cr
\l{1}&\int(4){20}{}&\ln{2}&\cnt{195}&\bounds{15}{15}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 9
\orbit{1}{9}{70}
\h{9}&\int(12){20}{\spec{2}}&&\cnt{615}&\bounds{70}{70}{1}{false}&&\cr
\l{1}&\int(4){20}{\spec{1}}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\int(4){5}{\spec{1}}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){5}{\spec{2}}&\ln{1}&\cnt{264}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 10
\orbit{1}{10}{66}
\h{10}&\int(12){\12}{\spec{5}}&&\cnt{1263}&\bounds{66}{66}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{1260}&\bounds{63}{63}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 11
\orbit{1}{11}{63}
\h{11}&\int(12){15}{\spec{2}}&&\cnt{603}&\bounds{63}{63}{1}{false}&&\cr
\l{1}&\int(4){5}{\spec{1}}&\ln{1}&\cnt{117}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\int(4){5}{\spec{2}}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{234}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 12
\orbit{1}{12}{61}
\h{12}&\int(12){\12}{\spec{3}}&&\cnt{875}&\bounds{61}{61}{1}{false}&&\cr
\l{1}&\int(4){20}{\spec{2}}&\ln{1}&\cnt{360}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(4){20}{\spec{3}}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){5}{\spec{3}}&\ln{1}&\cnt{80}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{5}}&\ln{1}&\cnt{160}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{6}}&\ln{1}&\cnt{240}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 13
\orbit{1}{13}{58}
\h{13}&\int(12){20}{\spec{3}}&&\cnt{771}&\bounds{58}{58}{1}{false}&&\cr
\l{1}&\int(4){20}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){20}{\spec{2}}&\ln{1}&\cnt{300}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(4){5}{}&\ln{1}&\cnt{105}&\bounds{7}{7}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{45}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{270}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 14
\orbit{1}{14}{57}
\h{14}&\int(12){20}{\spec{4}}&&\cnt{915}&\bounds{57}{57}{1}{false}&&\cr
\l{1}&\int(4){20}{\spec{1}}&\ln{1}&\cnt{36}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){20}{\spec{2}}&\ln{1}&\cnt{459}&\bounds{27}{27}{1}{false}&&\cr
\l{3}&\int(4){20}{\spec{3}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{36}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{216}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(4){\4}{\spec{5}}&\ln{1}&\cnt{153}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 15
\orbit{1}{15}{57}
\h{15}&\int(12){15}{\spec{3}}&&\cnt{707}&\bounds{57}{57}{1}{false}&&\cr
\l{1}&\int(4){20}{\spec{1}}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){20}{\spec{2}}&\ln{1}&\cnt{315}&\bounds{21}{21}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{210}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{105}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 16
\orbit{1}{16}{55}
\h{16}&\int(12){15}{\spec{4}}&&\cnt{939}&\bounds{55}{55}{1}{false}&&\cr
\l{1}&\int(4){20}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){20}{\spec{2}}&\ln{1}&\cnt{324}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\int(4){20}{\spec{3}}&\ln{1}&\cnt{153}&\bounds{9}{9}{1}{false}&&\cr
\l{4}&\int(4){\4}{}&\ln{1}&\cnt{459}&\bounds{27}{27}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 17
\orbit{1}{17}{52}
\h{17}&\int(12){\12}{\spec{2}}&&\cnt{879}&\bounds{52}{52}{1}{false}&&\cr
\l{1}&\int(4){20}{\spec{2}}&\ln{2}&\cnt{171}&\bounds{9}{9}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\ln{2}&\cnt{76}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\ln{2}&\cnt{19}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{5}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{6}}&\ln{2}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{7}}&\ln{1}&\cnt{342}&\bounds{19}{19}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 18
\orbit{1}{18}{44}
\h{18}&\int(12){20}{\spec{2}}&&\cnt{687}&\bounds{44}{44}{1}{false}&&\cr
\l{1}&\int(4){20}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){20}{\spec{3}}&\ln{1}&\cnt{180}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{180}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{306}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{20}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice A[24]
% Class 19
\orbit{1}{19}{31}
\h{19}&\int(12){20}{\spec{5}}&&\cnt{651}&\bounds{31}{31}{1}{false}&&\cr
\l{1}&\int(4){20}{}&\ln{1}&\cnt{21}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\ln{1}&\cnt{630}&\bounds{30}{30}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_D10_2E7.tex <==
% -*- TeX -*-
% Niemeier lattice D10_2E7
% 82 classes
\newcs{max-D10_2E7}{195}%
\newcs{count-D10_2E7}{82}%
\newcs{counts-D10_2E7}{\DO{1}{195}\DO{2}{195}\DO{3}{194}\DO{4}{164}\DO{5}{158}\DO{6}{155}\DO{7}{155}\DO{8}{155}\DO{9}{149}\DO{10}{147}\DO{11}{147}\DO{12}{146}\DO{13}{143}\DO{14}{143}\DO{15}{137}\DO{16}{135}\DO{17}{135}\DO{18}{131}\DO{19}{131}\DO{20}{131}\DO{21}{131}\DO{22}{131}\DO{23}{131}\DO{24}{131}\DO{25}{131}\DO{26}{130}\DO{27}{130}\DO{28}{127}\DO{29}{123}\DO{30}{123}\DO{31}{121}\DO{32}{119}\DO{33}{119}\DO{34}{119}\DO{35}{119}\DO{36}{119}\DO{37}{119}\DO{38}{119}\DO{39}{119}\DO{40}{117}\DO{41}{115}\DO{42}{115}\DO{43}{115}\DO{44}{115}\DO{45}{115}\DO{46}{113}\DO{47}{111}\DO{48}{111}\DO{49}{111}\DO{50}{109}\DO{51}{108}\DO{52}{107}\DO{53}{105}\DO{54}{104}\DO{55}{103}\DO{56}{102}\DO{57}{99}\DO{58}{99}\DO{59}{99}\DO{60}{99}\DO{61}{98}\DO{62}{95}\DO{63}{95}\DO{64}{95}\DO{65}{94}\DO{66}{93}\DO{67}{91}\DO{68}{91}\DO{69}{91}\DO{70}{91}\DO{71}{90}\DO{72}{90}\DO{73}{87}\DO{74}{87}\DO{75}{83}\DO{76}{80}\DO{77}{79}\DO{78}{79}\DO{79}{75}\DO{80}{67}\DO{81}{66}\DO{82}{56}}%
\orbits
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 1
\orbit{3}{1}{195}
\h{1}&\int(9){2}{\spec{1}}&\rat(3/2){1}{}&\rat(3/2){1}{}&&\cnt{1755}&\bounds{195}{195}{1}{false}&&\cr
\l{1}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{486}&\bounds{54}{54}{1}{false}&&\cr
\l{2}&\int(3){2}{}&\rat(3/2){1}{}&\rat(-1/2){1}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){2}{}&\rat(1/2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{729}&\bounds{81}{81}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 2
\orbit{3}{2}{195}
\h{2}&\int(0){\0}{}&\int(6){\6}{\spec{2}}&\int(6){\6}{\spec{2}}&&\cnt{1863}&\bounds{195}{195}{1}{false}&&\cr
\l{1}&\int(0){2}{}&\int(3){1}{}&\int(1){1}{}&\ln{2}&\cnt{540}&\bounds{54}{54}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{729}&\bounds{81}{81}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 3
\orbit{3}{3}{194}
\h{3}&\int(0){\0}{}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&&\cnt{1979}&\bounds{194}{194}{1}{false}&&\cr
\l{1}&\int(0){1}{}&\int(4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{512}&\bounds{71}{71}{1}{false}&&\cr
\l{2}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(0){2}{}&\int(4){1}{}&\int(0){1}{}&\ln{1}&\cnt{1120}&\bounds{80}{80}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 4
\orbit{3}{4}{164}
\h{4}&\int(4){\4}{2}&\int(6){\6}{\spec{2}}&\int(2){\2}{}&&\cnt{1367}&\bounds{164}{164}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){1}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{39}{39}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{486}&\bounds{54}{54}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(3){1}{}&\int(-1){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\int(1){1}{}&\int(1){1}{}&\ln{1}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\l{7}&\int(0){2}{}&\int(3){1}{}&\int(1){1}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 5
\orbit{3}{5}{158}
\h{5}&\int(1){2}{}&\rat(19/2){1}{\spec{2}}&\rat(3/2){1}{}&&\cnt{1307}&\bounds{158}{158}{1}{false}&&\cr
\l{1}&\rat(1/2){1}{}&\rat(7/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{39}{39}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(1){2}{}&\rat(7/2){1}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\rat(5/2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(0){2}{}&\rat(7/2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{486}&\bounds{54}{54}{1}{false}&&\cr
\l{7}&\int(0){2}{}&\rat(5/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(-1){2}{}&\rat(7/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 6
\orbit{3}{6}{155}
\h{6}&\int(4){\4}{}&\int(8){\8}{\spec{2}}&\int(0){\0}{}&&\cnt{959}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\int(1){1}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{6}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(3){1}{}&\int(0){1}{}&\ln{1}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 7
\orbit{3}{7}{155}
\h{7}&\int(4){\4}{2}&\int(8){\8}{\spec{1}}&\int(0){\0}{}&&\cnt{1579}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{576}&\bounds{64}{64}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){2}{}&\int(2){1}{}&\int(0){1}{}&\ln{1}&\cnt{672}&\bounds{48}{48}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 8
\orbit{3}{8}{155}
\h{8}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{1483}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(4){\2}{\spec{1}}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(4){\2}{\spec{1}}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(3){\2}{\spec{1}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{512}&\bounds{64}{64}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(3){2}{}&\int(1){1}{}&\int(0){1}{}&\ln{1}&\cnt{672}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 9
\orbit{3}{9}{149}
\h{9}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&&\cnt{1095}&\bounds{149}{149}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{384}&\bounds{64}{64}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(2){1}{}&\int(0){1}{}&\ln{1}&\cnt{336}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 10
\orbit{3}{10}{147}
\h{10}&\int(0){\0}{}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{1}}&&\cnt{1095}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(0){2}{}&\int(2){1}{}&\int(2){1}{}&\ln{1}&\cnt{720}&\bounds{72}{72}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{2}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 11
\orbit{3}{11}{147}
\h{11}&\int(2){\2}{}&\int(10){\10}{}&\int(0){\0}{}&&\cnt{1035}&\bounds{147}{147}{1}{false}&&\cr
\l{1}&\int(1){1}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(3){1}{}&\int(0){1}{}&\ln{1}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 12
\orbit{3}{12}{146}
\h{12}&\int(8){\8}{0}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{1083}&\bounds{146}{146}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{48}{48}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{320}&\bounds{40}{40}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(2){1}{}&\int(0){1}{}&\ln{1}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 13
\orbit{3}{13}{143}
\h{13}&\int(2){\2}{}&\int(8){\8}{\spec{2}}&\int(2){\2}{}&&\cnt{975}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(1){1}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\int(3){1}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(2){1}{}&\int(1){1}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(0){2}{}&\int(3){1}{}&\int(1){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 14
\orbit{3}{14}{143}
\h{14}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{879}&\bounds{143}{143}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){2}{}&\int(1){1}{}&\int(1){1}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 15
\orbit{3}{15}{137}
\h{15}&\int(10){\10}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&&\cnt{1367}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(5){3}{}&\int(0){\0}{}&\int(-1){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){1}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{560}&\bounds{40}{40}{1}{false}&&\cr
\l{4}&\int(3){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{540}&\bounds{60}{60}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 16
\orbit{3}{16}{135}
\h{16}&\int(3){2}{}&\rat(15/2){1}{}&\rat(3/2){1}{}&&\cnt{927}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\rat(3/2){1}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\rat(5/2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(0){2}{}&\rat(5/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 17
\orbit{3}{17}{135}
\h{17}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{847}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\int(2){1}{}&\int(0){1}{}&\ln{1}&\cnt{112}&\bounds{8}{8}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 18
\orbit{3}{18}{131}
\h{18}&\int(0){\0}{}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&&\cnt{1083}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(0){2}{}&\int(2){1}{}&\int(2){1}{}&\ln{1}&\cnt{480}&\bounds{48}{48}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{\spec{1}}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{\spec{2}}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{320}&\bounds{40}{40}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 19
\orbit{3}{19}{131}
\h{19}&\int(0){\0}{}&\int(10){\10}{}&\int(2){\2}{}&&\cnt{1035}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{2}&\int(0){2}{}&\int(3){1}{}&\int(1){1}{}&\ln{1}&\cnt{480}&\bounds{48}{48}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 20
\orbit{3}{20}{131}
\h{20}&\rat(17/2){3}{\spec{1}}&\int(2){\2}{}&\rat(3/2){1}{}&&\cnt{1151}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{288}&\bounds{32}{32}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\rat(5/2){2}{}&\int(1){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{324}&\bounds{36}{36}{1}{false}&&\cr
\l{9}&\rat(5/2){2}{}&\int(0){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 21
\orbit{3}{21}{131}
\h{21}&\int(4){\4}{}&\int(8){\8}{\spec{1}}&\int(0){\0}{}&&\cnt{835}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{384}&\bounds{64}{64}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 22
\orbit{3}{22}{131}
\h{22}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(19/2){1}{\spec{2}}&&\cnt{1307}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{3}&\rat(1/2){3}{}&\int(0){\0}{}&\rat(7/2){1}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{450}&\bounds{50}{50}{1}{false}&&\cr
\l{5}&\rat(1/2){2}{}&\int(0){1}{}&\rat(7/2){1}{}&\ln{1}&\cnt{560}&\bounds{40}{40}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 23
\orbit{3}{23}{131}
\h{23}&\int(4){\4}{}&\int(6){\6}{\spec{1}}&\int(2){\2}{}&&\cnt{767}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\int(2){1}{}&\int(1){1}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 24
\orbit{3}{24}{131}
\h{24}&\int(6){\6}{}&\int(6){\6}{\spec{1}}&\int(0){\0}{}&&\cnt{735}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{225}&\bounds{45}{45}{1}{false}&&\cr
\l{5}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 25
\orbit{3}{25}{131}
\h{25}&\int(10){\10}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{959}&\bounds{131}{131}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(4){3}{\spec{1}}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(4){1}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(3){1}{\spec{1}}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 26
\orbit{3}{26}{130}
\h{26}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{811}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{384}&\bounds{64}{64}{1}{false}&&\cr
\l{6}&\int(4){\2}{\spec{2}}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(4){\2}{\spec{2}}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\int(3){\2}{\spec{2}}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 27
\orbit{3}{27}{130}
\h{27}&\int(12){\12}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1283}&\bounds{130}{130}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{6}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(4){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{448}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 28
\orbit{3}{28}{127}
\h{28}&\int(1){2}{}&\rat(15/2){1}{}&\rat(7/2){1}{}&&\cnt{911}&\bounds{127}{127}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\int(1){2}{}&\rat(5/2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(0){2}{}&\rat(5/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{378}&\bounds{42}{42}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{175}&\bounds{35}{35}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 29
\orbit{3}{29}{123}
\h{29}&\int(12){\12}{}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{939}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{378}&\bounds{42}{42}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 30
\orbit{3}{30}{123}
\h{30}&\int(6){\6}{}&\int(6){\6}{\spec{2}}&\int(0){\0}{}&&\cnt{1119}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(1){1}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\int(3){1}{}&\int(0){1}{}&\ln{1}&\cnt{336}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 31
\orbit{3}{31}{121}
\h{31}&\int(12){\12}{2}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1011}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{378}&\bounds{42}{42}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 32
\orbit{3}{32}{119}
\h{32}&\int(8){\8}{}&\int(4){\4}{}&\int(0){\0}{}&&\cnt{871}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{1}&\cnt{112}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(4){1}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{280}&\bounds{40}{40}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 33
\orbit{3}{33}{119}
\h{33}&\int(9){2}{\spec{3}}&\rat(3/2){1}{}&\rat(3/2){1}{}&&\cnt{927}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{2}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{7}&\int(2){2}{}&\rat(3/2){1}{}&\rat(1/2){1}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 34
\orbit{3}{34}{119}
\h{34}&\int(0){\0}{}&\int(8){\8}{\spec{2}}&\int(4){\4}{}&&\cnt{943}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(0){2}{}&\int(3){1}{}&\int(1){1}{}&\ln{1}&\cnt{320}&\bounds{32}{32}{1}{false}&&\cr
\l{2}&\int(0){2}{}&\int(2){1}{}&\int(2){1}{}&\ln{1}&\cnt{240}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 35
\orbit{3}{35}{119}
\h{35}&\int(4){\4}{2}&\int(4){\4}{}&\int(4){\4}{}&&\cnt{871}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{3}&\int(2){2}{}&\int(2){1}{}&\int(0){1}{}&\ln{2}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){2}{}&\int(1){1}{}&\int(1){1}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(0){2}{}&\int(2){1}{}&\int(2){1}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 36
\orbit{3}{36}{119}
\h{36}&\int(0){\0}{}&\int(12){\12}{\spec{1}}&\int(0){\0}{}&&\cnt{963}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{540}&\bounds{60}{60}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{378}&\bounds{42}{42}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 37
\orbit{3}{37}{119}
\h{37}&\rat(21/2){3}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&&\cnt{1083}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{18}{18}{1}{false}&&\cr
\l{3}&\rat(9/2){3}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){1}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{336}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{24}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 38
\orbit{3}{38}{119}
\h{38}&\int(4){\4}{}&\int(4){\4}{}&\int(4){\4}{}&&\cnt{655}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){3}{}&\int(0){\0}{}&\int(2){1}{}&\ln{2}&\cnt{64}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\int(2){1}{}&\int(1){1}{}&\ln{2}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(0){2}{}&\int(2){1}{}&\int(2){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 39
\orbit{3}{39}{119}
\h{39}&\int(7){2}{\spec{1}}&\rat(7/2){1}{}&\rat(3/2){1}{}&&\cnt{815}&\bounds{119}{119}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{32}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\rat(5/2){1}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{224}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\rat(3/2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\rat(1/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 40
\orbit{3}{40}{117}
\h{40}&\int(2){\2}{}&\int(6){\6}{\spec{2}}&\int(4){\4}{}&&\cnt{871}&\bounds{117}{117}{1}{false}&&\cr
\l{1}&\int(1){1}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\int(3){1}{}&\int(0){1}{}&\ln{1}&\cnt{40}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\int(1){1}{}&\int(2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(0){2}{}&\int(3){1}{}&\int(1){1}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(-1){2}{}&\int(3){1}{}&\int(2){1}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 41
\orbit{3}{41}{115}
\h{41}&\int(5){2}{\spec{2}}&\rat(11/2){1}{}&\rat(3/2){1}{}&&\cnt{703}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\rat(5/2){1}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{32}{32}{1}{false}&&\cr
\l{4}&\rat(3/2){1}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{80}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\rat(5/2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{8}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{50}&\bounds{10}{10}{1}{false}&&\cr
\l{9}&\int(0){2}{}&\rat(5/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 42
\orbit{3}{42}{115}
\h{42}&\int(1){2}{}&\rat(11/2){1}{}&\rat(11/2){1}{}&&\cnt{859}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(1){2}{}&\rat(5/2){1}{}&\rat(1/2){1}{\spec{1}}&\ln{2}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){2}{}&\rat(5/2){1}{}&\rat(1/2){1}{\spec{2}}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{100}&\bounds{20}{20}{1}{false}&&\cr
\l{5}&\int(0){2}{}&\rat(5/2){1}{}&\rat(3/2){1}{}&\ln{2}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\int(-1){2}{}&\rat(5/2){1}{}&\rat(5/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\ln{2}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\ln{2}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 43
\orbit{3}{43}{115}
\h{43}&\rat(17/2){3}{\spec{2}}&\int(0){\0}{}&\rat(7/2){1}{}&&\cnt{791}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(4){1}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\rat(5/2){3}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{245}&\bounds{35}{35}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{105}&\bounds{21}{21}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 44
\orbit{3}{44}{115}
\h{44}&\rat(13/2){3}{}&\int(0){\0}{}&\rat(11/2){1}{}&&\cnt{859}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{\spec{2}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{280}&\bounds{40}{40}{1}{false}&&\cr
\l{5}&\rat(3/2){3}{\spec{1}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\rat(3/2){3}{\spec{2}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{1}}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{\spec{2}}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{10}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{11}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(3/2){2}{}&\int(0){1}{}&\rat(5/2){1}{}&\ln{1}&\cnt{112}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 45
\orbit{3}{45}{115}
\h{45}&\int(5){2}{\spec{1}}&\rat(11/2){1}{}&\rat(3/2){1}{}&&\cnt{859}&\bounds{115}{115}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(3/2){1}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(2){2}{}&\rat(5/2){1}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\rat(3/2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\rat(1/2){1}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{12}&\int(2){2}{}&\rat(1/2){1}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(1){2}{}&\rat(5/2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{14}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{15}&\int(0){2}{}&\rat(5/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{16}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{17}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 46
\orbit{3}{46}{113}
\h{46}&\rat(17/2){3}{\spec{1}}&\int(0){\0}{}&\rat(7/2){1}{}&&\cnt{1127}&\bounds{113}{113}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{252}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{315}&\bounds{35}{35}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\rat(5/2){2}{}&\int(0){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{392}&\bounds{28}{28}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 47
\orbit{3}{47}{111}
\h{47}&\int(6){\6}{\spec{1}}&\int(4){\4}{}&\int(2){\2}{}&&\cnt{751}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{140}&\bounds{20}{20}{1}{false}&&\cr
\l{9}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{10}&\int(2){2}{}&\int(2){1}{}&\int(0){1}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{11}&\int(2){2}{}&\int(1){1}{}&\int(1){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{12}&\int(1){2}{}&\int(2){1}{}&\int(1){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 48
\orbit{3}{48}{111}
\h{48}&\int(6){\6}{}&\int(4){\4}{}&\int(2){\2}{}&&\cnt{655}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(3){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\int(2){1}{}&\int(1){1}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 49
\orbit{3}{49}{111}
\h{49}&\int(2){\2}{}&\int(6){\6}{\spec{1}}&\int(4){\4}{}&&\cnt{751}&\bounds{111}{111}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\int(2){1}{}&\int(1){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\int(1){1}{}&\int(2){1}{}&\ln{1}&\cnt{48}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\int(0){2}{}&\int(2){1}{}&\int(2){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{150}&\bounds{30}{30}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 50
\orbit{3}{50}{109}
\h{50}&\rat(17/2){3}{\spec{2}}&\int(2){\2}{}&\rat(3/2){1}{}&&\cnt{815}&\bounds{109}{109}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{3}&\int(4){1}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\rat(5/2){3}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{81}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\int(1){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{36}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 51
\orbit{3}{51}{108}
\h{51}&\rat(5/2){3}{}&\int(8){\8}{\spec{2}}&\rat(3/2){1}{}&&\cnt{983}&\bounds{108}{108}{1}{false}&&\cr
\l{1}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(1){1}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\rat(1/2){2}{}&\int(3){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{270}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\rat(1/2){2}{}&\int(2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(-1/2){2}{}&\int(3){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 52
\orbit{3}{52}{107}
\h{52}&\rat(5/2){3}{}&\int(2){\2}{}&\rat(15/2){1}{}&&\cnt{935}&\bounds{107}{107}{1}{false}&&\cr
\l{1}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{225}&\bounds{25}{25}{1}{false}&&\cr
\l{4}&\rat(1/2){2}{}&\int(1){1}{}&\rat(5/2){1}{}&\ln{1}&\cnt{360}&\bounds{36}{36}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 53
\orbit{3}{53}{105}
\h{53}&\rat(9/2){3}{}&\int(0){\0}{}&\rat(15/2){1}{}&&\cnt{903}&\bounds{105}{105}{1}{false}&&\cr
\l{1}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{2}&\rat(3/2){3}{\spec{1}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{252}&\bounds{36}{36}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{\spec{2}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\int(0){1}{}&\rat(5/2){1}{}&\ln{1}&\cnt{168}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 54
\orbit{3}{54}{104}
\h{54}&\rat(21/2){3}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&&\cnt{911}&\bounds{104}{104}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(4){1}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{56}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\rat(5/2){3}{\spec{1}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{6}&\rat(5/2){3}{\spec{2}}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\int(4){\2}{}&\int(0){\0}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{9}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\rat(5/2){2}{}&\int(0){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{56}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 55
\orbit{3}{55}{103}
\h{55}&\int(3){2}{}&\rat(11/2){1}{}&\rat(7/2){1}{}&&\cnt{703}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\rat(3/2){1}{}&\rat(5/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\rat(5/2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{63}&\bounds{9}{9}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{7}&\int(0){2}{}&\rat(5/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{98}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 56
\orbit{3}{56}{102}
\h{56}&\int(4){\4}{2}&\int(8){\8}{\spec{2}}&\int(0){\0}{}&&\cnt{911}&\bounds{102}{102}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){1}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{39}{39}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(2){1}{}&\int(0){1}{}&\ln{1}&\cnt{336}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 57
\orbit{3}{57}{99}
\h{57}&\rat(13/2){3}{}&\int(2){\2}{}&\rat(7/2){1}{}&&\cnt{711}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{21}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{96}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{7}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\int(1){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 58
\orbit{3}{58}{99}
\h{58}&\int(4){\4}{}&\int(6){\6}{\spec{2}}&\int(2){\2}{}&&\cnt{623}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){1}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{6}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\int(3){1}{}&\int(0){1}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(0){2}{}&\int(3){1}{}&\int(1){1}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 59
\orbit{3}{59}{99}
\h{59}&\int(2){\2}{}&\int(8){\8}{\spec{1}}&\int(2){\2}{}&&\cnt{587}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\int(2){1}{}&\int(1){1}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 60
\orbit{3}{60}{99}
\h{60}&\int(5){2}{\spec{1}}&\rat(7/2){1}{}&\rat(7/2){1}{}&&\cnt{687}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(2){2}{}&\rat(3/2){1}{}&\rat(1/2){1}{}&\ln{2}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 61
\orbit{3}{61}{98}
\h{61}&\int(8){\8}{0}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{587}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(1){1}{}&\int(1){1}{}&\ln{1}&\cnt{288}&\bounds{48}{48}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 62
\orbit{3}{62}{95}
\h{62}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&&\cnt{1079}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\int(0){\0}{}&\ln{2}&\cnt{56}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(4){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{448}&\bounds{32}{32}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 63
\orbit{3}{63}{95}
\h{63}&\int(4){\4}{2}&\int(6){\6}{\spec{1}}&\int(2){\2}{}&&\cnt{719}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(2){2}{}&\int(2){1}{}&\int(0){1}{}&\ln{1}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(2){2}{}&\int(1){1}{}&\int(1){1}{}&\ln{1}&\cnt{144}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 64
\orbit{3}{64}{95}
\h{64}&\int(5){2}{\spec{2}}&\rat(7/2){1}{}&\rat(7/2){1}{}&&\cnt{663}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{5}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{2}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{245}&\bounds{35}{35}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 65
\orbit{3}{65}{94}
\h{65}&\int(1){2}{}&\rat(19/2){1}{\spec{1}}&\rat(3/2){1}{}&&\cnt{799}&\bounds{94}{94}{1}{false}&&\cr
\l{1}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(1){2}{}&\rat(5/2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{4}&\int(1){2}{}&\rat(3/2){1}{\spec{1}}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\rat(3/2){1}{\spec{2}}&\rat(3/2){1}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(0){2}{}&\rat(5/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 66
\orbit{3}{66}{93}
\h{66}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(19/2){1}{\spec{1}}&&\cnt{799}&\bounds{93}{93}{1}{false}&&\cr
\l{1}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{\spec{2}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\int(0){\2}{}&\int(0){\0}{}&\int(4){\2}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{6}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{30}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 67
\orbit{3}{67}{91}
\h{67}&\rat(5/2){3}{}&\int(6){\6}{\spec{1}}&\rat(7/2){1}{}&&\cnt{767}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{6}{6}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(1/2){2}{}&\int(2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{420}&\bounds{42}{42}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{105}&\bounds{15}{15}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 68
\orbit{3}{68}{91}
\h{68}&\rat(9/2){3}{}&\int(2){\2}{}&\rat(11/2){1}{}&&\cnt{703}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{\spec{1}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(3/2){3}{\spec{2}}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{144}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{1}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(1){\2}{\spec{2}}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{9}&\rat(3/2){2}{}&\int(1){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{120}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\int(0){1}{}&\rat(5/2){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\rat(1/2){2}{}&\int(1){1}{}&\rat(5/2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{12}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{14}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 69
\orbit{3}{69}{91}
\h{69}&\int(7){2}{\spec{2}}&\rat(7/2){1}{}&\rat(3/2){1}{}&&\cnt{647}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{35}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\rat(7/2){1}{}&\rat(1/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\rat(5/2){1}{}&\rat(3/2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{196}&\bounds{28}{28}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{147}&\bounds{21}{21}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{49}&\bounds{7}{7}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 70
\orbit{3}{70}{91}
\h{70}&\rat(13/2){3}{}&\int(4){\4}{}&\rat(3/2){1}{}&&\cnt{703}&\bounds{91}{91}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{2}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{16}{16}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(2){1}{\spec{1}}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{112}&\bounds{16}{16}{1}{false}&&\cr
\l{6}&\int(2){1}{\spec{2}}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{8}&\int(3){\2}{}&\int(0){\0}{}&\int(1){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{9}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\rat(3/2){2}{}&\int(2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{11}&\rat(3/2){2}{}&\int(1){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{12}&\rat(1/2){2}{}&\int(2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{13}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 71
\orbit{3}{71}{90}
\h{71}&\rat(9/2){3}{}&\int(6){\6}{\spec{2}}&\rat(3/2){1}{}&&\cnt{747}&\bounds{90}{90}{1}{false}&&\cr
\l{1}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){1}{\spec{1}}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\int(1){1}{\spec{2}}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{6}&\rat(3/2){2}{}&\int(3){1}{}&\rat(-1/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\int(1){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{8}&\rat(1/2){2}{}&\int(3){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{9}&\rat(-1/2){2}{}&\int(3){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 72
\orbit{3}{72}{90}
\h{72}&\int(9){2}{\spec{4}}&\rat(3/2){1}{}&\rat(3/2){1}{}&&\cnt{747}&\bounds{90}{90}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{126}&\bounds{21}{21}{1}{false}&&\cr
\l{2}&\rat(9/2){3}{}&\int(0){\0}{}&\rat(-1/2){1}{}&\ln{2}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\rat(7/2){3}{}&\int(0){\0}{}&\rat(1/2){1}{}&\ln{2}&\cnt{243}&\bounds{27}{27}{1}{false}&&\cr
\l{4}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{2}&\cnt{36}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 73
\orbit{3}{73}{87}
\h{73}&\int(8){\8}{}&\int(2){\2}{}&\int(2){\2}{}&&\cnt{639}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{2}&\int(4){3}{}&\int(0){\0}{}&\int(0){1}{}&\ln{2}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{3}&\int(3){3}{}&\int(0){\0}{}&\int(1){1}{}&\ln{2}&\cnt{192}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{28}&\bounds{4}{4}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 74
\orbit{3}{74}{87}
\h{74}&\rat(9/2){3}{}&\int(6){\6}{\spec{1}}&\rat(3/2){1}{}&&\cnt{759}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{9}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{216}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{135}&\bounds{15}{15}{1}{false}&&\cr
\l{5}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\int(2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{162}&\bounds{18}{18}{1}{false}&&\cr
\l{8}&\rat(3/2){2}{}&\int(1){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{12}&\bounds{2}{2}{1}{false}&&\cr
\l{9}&\rat(1/2){2}{}&\int(2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 75
\orbit{3}{75}{83}
\h{75}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{2}}&\int(0){\0}{}&&\cnt{687}&\bounds{83}{83}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{14}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(1){1}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{378}&\bounds{42}{42}{1}{false}&&\cr
\l{6}&\int(1){2}{}&\int(3){1}{}&\int(0){1}{}&\ln{1}&\cnt{112}&\bounds{8}{8}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 76
\orbit{3}{76}{80}
\h{76}&\int(9){2}{\spec{2}}&\rat(3/2){1}{}&\rat(3/2){1}{}&&\cnt{575}&\bounds{80}{80}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{2}&\cnt{64}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(4){\2}{}&\int(0){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\int(0){\0}{}&\ln{2}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{6}&\int(2){2}{}&\rat(3/2){1}{}&\rat(1/2){1}{}&\ln{2}&\cnt{54}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\int(1){2}{}&\rat(3/2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 77
\orbit{3}{77}{79}
\h{77}&\rat(9/2){3}{}&\int(4){\4}{}&\rat(7/2){1}{}&&\cnt{655}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(3){1}{}&\int(1){1}{}&\int(0){\0}{}&\ln{1}&\cnt{16}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{72}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{5}&\int(2){\2}{}&\int(0){\0}{}&\int(2){\2}{}&\ln{1}&\cnt{63}&\bounds{7}{7}{1}{false}&&\cr
\l{6}&\rat(3/2){2}{}&\int(2){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{42}&\bounds{6}{6}{1}{false}&&\cr
\l{7}&\rat(3/2){2}{}&\int(1){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{112}&\bounds{14}{14}{1}{false}&&\cr
\l{8}&\rat(1/2){2}{}&\int(2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{70}&\bounds{10}{10}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 78
\orbit{3}{78}{79}
\h{78}&\rat(5/2){3}{}&\int(4){\4}{}&\rat(11/2){1}{}&&\cnt{703}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\rat(3/2){3}{}&\int(0){\0}{}&\rat(5/2){1}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{4}&\int(1){\2}{}&\int(0){\0}{}&\int(3){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\l{5}&\rat(1/2){2}{}&\int(2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{200}&\bounds{20}{20}{1}{false}&&\cr
\l{6}&\rat(1/2){2}{}&\int(1){1}{}&\rat(5/2){1}{}&\ln{1}&\cnt{160}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\rat(-1/2){2}{}&\int(2){1}{}&\rat(5/2){1}{}&\ln{1}&\cnt{20}&\bounds{2}{2}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{9}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{160}&\bounds{20}{20}{1}{false}&&\cr
\l{10}&\int(0){\0}{}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{11}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{10}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 79
\orbit{3}{79}{75}
\h{79}&\int(0){\0}{}&\int(6){\6}{\spec{1}}&\int(6){\6}{\spec{2}}&&\cnt{687}&\bounds{75}{75}{1}{false}&&\cr
\l{1}&\int(0){2}{}&\int(1){1}{}&\int(3){1}{}&\ln{1}&\cnt{240}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 80
\orbit{3}{80}{67}
\h{80}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&\int(0){\0}{}&&\cnt{575}&\bounds{67}{67}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{2}&\int(4){1}{}&\int(0){1}{}&\int(0){\0}{}&\ln{1}&\cnt{320}&\bounds{32}{32}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 81
\orbit{3}{81}{66}
\h{81}&\rat(5/2){3}{}&\int(6){\6}{\spec{2}}&\rat(7/2){1}{}&&\cnt{623}&\bounds{66}{66}{1}{false}&&\cr
\l{1}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{7}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){1}{}&\int(3){1}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{13}{13}{1}{false}&&\cr
\l{3}&\rat(1/2){2}{}&\int(3){1}{}&\rat(1/2){1}{}&\ln{1}&\cnt{210}&\bounds{21}{21}{1}{false}&&\cr
\l{4}&\rat(-1/2){2}{}&\int(3){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{70}&\bounds{7}{7}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{189}&\bounds{21}{21}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[10] + 2*E[7]
% Class 82
\orbit{3}{82}{56}
\h{82}&\rat(5/2){3}{}&\int(8){\8}{\spec{1}}&\rat(3/2){1}{}&&\cnt{463}&\bounds{56}{56}{1}{false}&&\cr
\l{1}&\rat(5/2){3}{}&\int(0){\0}{}&\rat(3/2){1}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){1}{}&\int(2){1}{}&\int(0){\0}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(4){\2}{}&\int(0){\0}{}&\ln{1}&\cnt{90}&\bounds{10}{10}{1}{false}&&\cr
\l{4}&\rat(1/2){2}{}&\int(2){1}{}&\rat(3/2){1}{}&\ln{1}&\cnt{120}&\bounds{12}{12}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{72}&\bounds{9}{9}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_D16_E8.tex <==
% -*- TeX -*-
% Niemeier lattice D16_E8
% 28 classes
\newcs{max-D16_E8}{155}%
\newcs{count-D16_E8}{28}%
\newcs{counts-D16_E8}{\DO{1}{155}\DO{2}{155}\DO{3}{137}\DO{4}{135}\DO{5}{123}\DO{6}{121}\DO{7}{120}\DO{8}{103}\DO{9}{103}\DO{10}{102}\DO{11}{99}\DO{12}{99}\DO{13}{99}\DO{14}{98}\DO{15}{95}\DO{16}{87}\DO{17}{87}\DO{18}{85}\DO{19}{79}\DO{20}{75}\DO{21}{71}\DO{22}{67}\DO{23}{67}\DO{24}{66}\DO{25}{61}\DO{26}{51}\DO{27}{47}\DO{28}{31}}%
\orbits
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 1
\orbit{2}{1}{155}
\h{1}&\int(4){\4}{2}&\int(8){\8}{\spec{2}}&&\cnt{2227}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1680}&\bounds{112}{112}{1}{false}&&\cr
\l{3}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{420}&\bounds{28}{28}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 2
\orbit{2}{2}{155}
\h{2}&\int(10){\10}{\spec{1}}&\int(2){\2}{}&&\cnt{2059}&\bounds{155}{155}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{364}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{1568}&\bounds{112}{112}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 3
\orbit{2}{3}{137}
\h{3}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&&\cnt{1187}&\bounds{137}{137}{1}{false}&&\cr
\l{1}&\int(4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{512}&\bounds{71}{71}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{240}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{180}&\bounds{20}{20}{1}{false}&&\cr
\l{7}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{240}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 4
\orbit{2}{4}{135}
\h{4}&\int(12){\12}{\spec{3}}&\int(0){\0}{}&&\cnt{975}&\bounds{135}{135}{1}{false}&&\cr
\l{1}&\int(4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{512}&\bounds{64}{64}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{392}&\bounds{56}{56}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 5
\orbit{2}{5}{123}
\h{5}&\int(12){\12}{\spec{1}}&\int(0){\0}{}&&\cnt{1515}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{792}&\bounds{72}{72}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{720}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 6
\orbit{2}{6}{121}
\h{6}&\int(12){\12}{2}&\int(0){\0}{}&&\cnt{1659}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{936}&\bounds{72}{72}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{720}&\bounds{48}{48}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 7
\orbit{2}{7}{120}
\h{7}&\int(0){\0}{}&\int(12){\12}{}&&\cnt{1563}&\bounds{120}{120}{1}{false}&&\cr
\l{1}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{1440}&\bounds{96}{96}{1}{false}&&\cr
\l{2}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{120}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{3}&\bounds{0}{0}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 8
\orbit{2}{8}{103}
\h{8}&\int(4){\4}{}&\int(8){\8}{\spec{1}}&&\cnt{1007}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{168}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{768}&\bounds{64}{64}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 9
\orbit{2}{9}{103}
\h{9}&\int(12){\12}{\spec{2}}&\int(0){\0}{}&&\cnt{1023}&\bounds{103}{103}{1}{false}&&\cr
\l{1}&\int(4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{528}&\bounds{48}{48}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{5}}&\int(0){\0}{}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 10
\orbit{2}{10}{102}
\h{10}&\int(10){\10}{\spec{3}}&\int(2){\2}{}&&\cnt{911}&\bounds{102}{102}{1}{false}&&\cr
\l{1}&\int(4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{256}&\bounds{39}{39}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{270}&\bounds{30}{30}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{336}&\bounds{24}{24}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{18}&\bounds{2}{2}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 11
\orbit{2}{11}{99}
\h{11}&\int(2){\2}{}&\int(10){\10}{}&&\cnt{1163}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(2){\2}{}&\int(2){\2}{\spec{1}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{\spec{2}}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{672}&\bounds{48}{48}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{5}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{364}&\bounds{28}{28}{1}{false}&&\cr
\l{6}&\int(0){\0}{}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{32}&\bounds{4}{4}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{60}&\bounds{12}{12}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 12
\orbit{2}{12}{99}
\h{12}&\int(12){1}{\spec{2}}&\int(0){\0}{}&&\cnt{987}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\l{2}&\int(4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{396}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 13
\orbit{2}{13}{99}
\h{13}&\int(10){1}{\spec{2}}&\int(2){\2}{}&&\cnt{1415}&\bounds{99}{99}{1}{false}&&\cr
\l{1}&\int(4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{105}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{455}&\bounds{35}{35}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{840}&\bounds{56}{56}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{15}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 14
\orbit{2}{14}{98}
\h{14}&\int(8){\8}{0}&\int(4){\4}{}&&\cnt{1235}&\bounds{98}{98}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{364}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{784}&\bounds{56}{56}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 15
\orbit{2}{15}{95}
\h{15}&\int(8){\8}{}&\int(4){\4}{}&&\cnt{591}&\bounds{95}{95}{1}{false}&&\cr
\l{1}&\int(4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{128}&\bounds{24}{24}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{392}&\bounds{56}{56}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 16
\orbit{2}{16}{87}
\h{16}&\int(8){\8}{\spec{1}}&\int(4){\4}{}&&\cnt{783}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{132}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{256}&\bounds{32}{32}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{84}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{308}&\bounds{28}{28}{1}{false}&&\cr
\l{7}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 17
\orbit{2}{17}{87}
\h{17}&\int(12){1}{\spec{1}}&\int(0){\0}{}&&\cnt{1151}&\bounds{87}{87}{1}{false}&&\cr
\l{1}&\int(4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{364}&\bounds{28}{28}{1}{false}&&\cr
\l{2}&\int(4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{182}&\bounds{14}{14}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{364}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{240}&\bounds{16}{16}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 18
\orbit{2}{18}{85}
\h{18}&\int(6){\6}{\spec{1}}&\int(6){\6}{}&&\cnt{999}&\bounds{85}{85}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{26}&\bounds{2}{2}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{108}&\bounds{12}{12}{1}{false}&&\cr
\l{4}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\l{5}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{702}&\bounds{54}{54}{1}{false}&&\cr
\l{6}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{4}&\bounds{2}{2}{1}{false}&&\cr
\l{7}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{104}&\bounds{8}{8}{1}{false}&&\cr
\l{8}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 19
\orbit{2}{19}{79}
\h{19}&\int(4){1}{}&\int(8){\8}{\spec{1}}&&\cnt{1031}&\bounds{79}{79}{1}{false}&&\cr
\l{1}&\int(4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{960}&\bounds{64}{64}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 20
\orbit{2}{20}{75}
\h{20}&\int(6){\6}{}&\int(6){\6}{}&&\cnt{687}&\bounds{75}{75}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{405}&\bounds{45}{45}{1}{false}&&\cr
\l{3}&\int(1){\2}{}&\int(3){\2}{}&\ln{1}&\cnt{240}&\bounds{24}{24}{1}{false}&&\cr
\l{4}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 21
\orbit{2}{21}{71}
\h{21}&\int(4){\4}{2}&\int(8){\8}{\spec{1}}&&\cnt{911}&\bounds{71}{71}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{840}&\bounds{56}{56}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 22
\orbit{2}{22}{67}
\h{22}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&&\cnt{575}&\bounds{67}{67}{1}{false}&&\cr
\l{1}&\int(4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{320}&\bounds{32}{32}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{4}}&\int(0){\0}{}&\ln{1}&\cnt{210}&\bounds{30}{30}{1}{false}&&\cr
\l{3}&\int(2){\2}{\spec{3}}&\int(2){\2}{}&\ln{1}&\cnt{45}&\bounds{5}{5}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 23
\orbit{2}{23}{67}
\h{23}&\int(4){\4}{}&\int(8){\8}{\spec{2}}&&\cnt{739}&\bounds{67}{67}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{336}&\bounds{24}{24}{1}{false}&&\cr
\l{3}&\int(0){\2}{\spec{1}}&\int(4){\2}{}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(0){\2}{\spec{2}}&\int(4){\2}{}&\ln{1}&\cnt{264}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 24
\orbit{2}{24}{66}
\h{24}&\int(10){\10}{\spec{2}}&\int(2){\2}{}&&\cnt{715}&\bounds{66}{66}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{2}&\bounds{2}{2}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{48}&\bounds{4}{4}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\int(0){\0}{}&\ln{1}&\cnt{264}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(4){\2}{}&\int(0){\2}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\l{6}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{224}&\bounds{16}{16}{1}{false}&&\cr
\l{7}&\int(2){\2}{\spec{1}}&\int(2){\2}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{8}&\int(2){\2}{\spec{2}}&\int(2){\2}{}&\ln{1}&\cnt{48}&\bounds{4}{4}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 25
\orbit{2}{25}{61}
\h{25}&\int(10){1}{\spec{1}}&\int(2){\2}{}&&\cnt{743}&\bounds{61}{61}{1}{false}&&\cr
\l{1}&\int(4){1}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{286}&\bounds{26}{26}{1}{false}&&\cr
\l{2}&\int(4){1}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{1}}&\int(0){\0}{}&\ln{1}&\cnt{13}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{2}}&\int(0){\0}{}&\ln{1}&\cnt{234}&\bounds{18}{18}{1}{false}&&\cr
\l{5}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{168}&\bounds{12}{12}{1}{false}&&\cr
\l{6}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{39}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 26
\orbit{2}{26}{51}
\h{26}&\int(8){1}{}&\int(4){\4}{}&&\cnt{639}&\bounds{51}{51}{1}{false}&&\cr
\l{1}&\int(4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{2}&\int(4){\4}{}&\int(0){\0}{}&\ln{1}&\cnt{91}&\bounds{7}{7}{1}{false}&&\cr
\l{3}&\int(3){\2}{}&\int(1){\2}{}&\ln{1}&\cnt{64}&\bounds{8}{8}{1}{false}&&\cr
\l{4}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{392}&\bounds{28}{28}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 27
\orbit{2}{27}{47}
\h{27}&\int(6){1}{}&\int(6){\6}{}&&\cnt{687}&\bounds{47}{47}{1}{false}&&\cr
\l{1}&\int(4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{15}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(2){\2}{}&\int(2){\2}{}&\ln{1}&\cnt{405}&\bounds{27}{27}{1}{false}&&\cr
\l{3}&\int(1){\2}{\spec{1}}&\int(3){\2}{}&\ln{1}&\cnt{30}&\bounds{2}{2}{1}{false}&&\cr
\l{4}&\int(1){\2}{\spec{2}}&\int(3){\2}{}&\ln{1}&\cnt{210}&\bounds{14}{14}{1}{false}&&\cr
\l{5}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{27}&\bounds{3}{3}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[16] + E[8]
% Class 28
\orbit{2}{28}{31}
\h{28}&\int(4){1}{}&\int(8){\8}{\spec{2}}&&\cnt{367}&\bounds{31}{31}{1}{false}&&\cr
\l{1}&\int(4){1}{}&\int(0){\0}{}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(0){\2}{}&\int(4){\2}{}&\ln{1}&\cnt{240}&\bounds{16}{16}{1}{false}&&\cr
\l{3}&\int(0){\0}{}&\int(4){\4}{}&\ln{1}&\cnt{126}&\bounds{14}{14}{1}{false}&&\cr
\endorbit
\endorbits
\endinput


==> 3/3_D24.tex <==
% -*- TeX -*-
% Niemeier lattice D24
% 7 classes
\newcs{max-D24}{123}%
\newcs{count-D24}{7}%
\newcs{counts-D24}{\DO{1}{123}\DO{2}{121}\DO{3}{84}\DO{4}{71}\DO{5}{66}\DO{6}{55}\DO{7}{31}}%
\orbits
% -*- TeX -*-
% Niemeier lattice D[24]
% Class 1
\orbit{1}{1}{123}
\h{1}&\int(12){\12}{\spec{1}}&&\cnt{2283}&\bounds{123}{123}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{3}&\bounds{3}{3}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{2280}&\bounds{120}{120}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[24]
% Class 2
\orbit{1}{2}{121}
\h{2}&\int(12){\12}{2}&&\cnt{2523}&\bounds{121}{121}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\ln{1}&\cnt{2520}&\bounds{120}{120}{1}{false}&&\cr
\l{2}&\int(4){\4}{2}&\ln{1}&\cnt{3}&\bounds{1}{1}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[24]
% Class 3
\orbit{1}{3}{84}
\h{3}&\int(12){1}{\spec{2}}&&\cnt{1771}&\bounds{84}{84}{1}{false}&&\cr
\l{1}&\int(4){\4}{}&\ln{1}&\cnt{1771}&\bounds{84}{84}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[24]
% Class 4
\orbit{1}{4}{71}
\h{4}&\int(12){\12}{\spec{3}}&&\cnt{911}&\bounds{71}{71}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{70}&\bounds{14}{14}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{840}&\bounds{56}{56}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[24]
% Class 5
\orbit{1}{5}{66}
\h{5}&\int(12){\12}{\spec{2}}&&\cnt{1059}&\bounds{66}{66}{1}{false}&&\cr
\l{1}&\int(4){\4}{2}&\ln{1}&\cnt{2}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{12}&\bounds{4}{4}{1}{false}&&\cr
\l{3}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{1}&\bounds{1}{1}{1}{false}&&\cr
\l{4}&\int(4){\4}{\spec{3}}&\ln{1}&\cnt{432}&\bounds{24}{24}{1}{false}&&\cr
\l{5}&\int(4){\4}{\spec{4}}&\ln{1}&\cnt{612}&\bounds{36}{36}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[24]
% Class 6
\orbit{1}{6}{55}
\h{6}&\int(12){\12}{\spec{2}}&&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{5}}&\ln{1}&\cnt{495}&\bounds{55}{55}{1}{false}&&\cr
\endorbit
% -*- TeX -*-
% Niemeier lattice D[24]
% Class 7
\orbit{1}{7}{31}
\h{7}&\int(12){1}{\spec{1}}&&\cnt{651}&\bounds{31}{31}{1}{false}&&\cr
\l{1}&\int(4){\4}{\spec{1}}&\ln{1}&\cnt{21}&\bounds{1}{1}{1}{false}&&\cr
\l{2}&\int(4){\4}{\spec{2}}&\ln{1}&\cnt{630}&\bounds{30}{30}{1}{false}&&\cr
\endorbit
\endorbits
\endinput

